Model Sketching: Centering Concepts in Early-Stage Machine Learning Model Design

Machine learning practitioners often end up tunneling on low-level technical details like model architectures and performance metrics. Could early model development instead focus on high-level questions of which factors a model ought to pay attention to? Inspired by the practice of sketching in design, which distills ideas to their minimal representation, we introduce model sketching: a technical framework for iteratively and rapidly authoring functional approximations of a machine learning model's decision-making logic. Model sketching refocuses practitioner attention on composing high-level, human-understandable concepts that the model is expected to reason over (e.g., profanity, racism, or sarcasm in a content moderation task) using zero-shot concept instantiation. In an evaluation with 17 ML practitioners, model sketching reframed thinking from implementation to higher-level exploration, prompted iteration on a broader range of model designs, and helped identify gaps in the problem formulation$\unicode{x2014}$all in a fraction of the time ordinarily required to build a model.

==> sections/old_versions/1_intro_v1.tex <==
% [Machine learning development is unwieldy/slow/inflexible; tunneling/fixation is bad]
Though widely leveraged in today’s technologies, machine learning (ML) models are surprisingly unwieldy to develop and iterate upon. Because there are so many interconnected steps that go into model development—from mathematical formulation to dataset annotation to feature engineering—and because all of these steps must be fully implemented to produce a functional system, it takes a significant investment of time and effort to implement and deploy a new machine learning model. Thus, there is a great deal of inertia in model development: it is difficult to edit or rethink the design of a model, so ML developers cannot broadly explore the design space of task formulation or model design. Rather, they are incentivized to rely upon existing models or tools and are thus much more likely to fixate on a certain task formulation early on in the development process. Tunneling  approaches that dive quickly into implementation may work sufficiently well for tasks that can be clearly defined and have a single solution. However, as we know in HCI, such tunneling is disastrous for ill-defined domains where practitioners must grapple with the tradeoffs of multiple viable solutions, and most human-facing deployments of machine learning fall in this category.

% [ML needs a sketching practice; why sketching is beneficial; most importantly, it focuses attention]
Machine learning lacks a sketching practice and is in dire need of one. Sketching is a powerful technique that designers use to combat against the trap of tunneling; sketches allow them to rapidly and broadly explore a design space in the early stages of the design process. Much of the value of a sketch derives from its ability to distill an idea to its minimal representation—to focus attention on the most important aspects of a design direction. In doing so, sketches act as valuable cognitive tools for practitioners themselves to understand nascent designs, and as boundary objects for users and stakeholders that facilitate early communication of ideas. Unfortunately, almost everything about modern ML development runs counter to the key characteristics of a sketching practice. Sketches are meant to be quick, expressive, and have minimal detail. Today’s most advanced and expressive models are generally slow and detail-laden: end-to-end blackbox models that take years or months to develop and require large amounts of human labor and compute. Meanwhile, current modeling approaches that are quick and lightweight are generally lacking in expressivity: pretrained models with minimal levers or simple models that learn from labeled data (an indirect means of communicating modeling goals that may be brittle to revisions in task formulation or deployment setting).

% [We think sketching in ML should be about concepts; this is especially important in human-facing, subjective tasks where we need a great deal of expressivity and control]
Sketches force practitioners to direct their attention to the most critical axes of their designs, and we hold that in an ML task, the most important parts to get right ought to be the concepts with which the model will reason to make decisions. Much of the conceptually difficult work of a modeling task is translating from a high-level decisionmaking goal or concept (which is often vague and underspecified) to a crisp and refined decisionmaking logic that aligns with a practitioner’s goals and end users’ needs. What do we really mean when we classify a comment as profane or political? What factors make a film or novel worth recommending to a user? Prior work on concept evolution has demonstrated that, even in seemingly objective tasks like classifying whether an image contains a cat, nuances and subjectivities arise that must be clarified (i.e., should we include a cartoon cat? should we include a lion?). However, getting these concepts right is especially important in subjective tasks where the general population is likely to disagree. In these kinds of tasks, it is critical to ensure that we achieve a strong grasp of our subjective understanding of a concept before we go and build a model around it, and we must have the expressivity and control to translate this subjective understanding to a technical system. 

% [We introduce model sketching]
We present model sketching, a technical approach that allows ML practitioners to create expressive, sketch-like versions of models. Our approach foregrounds concepts as the core building blocks of an ML-authoring design language. Instead of working at the level of hyperparameters and mathematical operators, users producing model sketches work at the level of concepts (e.g., profanity, racism, politics, and hate speech in a content moderation context) to author models that instantiate their vision. With this approach, users can iteratively define and refine what they really mean when, for example, they term a comment as high-quality, entertaining, or toxic. A benefit of this shift to concepts as first-class citizens is that we can leverage recent developments in zero-shot learning to map from raw data fields (i.e., the text of a post or an image of an art piece) to a concept score (i.e., a racism score or a realism score) with zero training time. We term these helper models that map from data fields to concept scores concept models. By iteratively specifying a small set of underlying concept models and determining how they will be aggregated into a sketch model, users can author and instantiate a series of sketch models in real time to explore different modeling approaches. Not only are these sketch models expressive and quick to author, but they are also working models that can take in unseen data and produce user-facing outputs. [To add: something about how many other model dev decisions fall out from decisions around the concepts (ex: data fields, the kinds of data needed, how the model scores will be used in an interface]] [To add: mention how we anticipate model sketches getting translated to full models]

% [Recap of our evaluation; imagined for now] 
In an evaluation with 15 ML practitioners, we found that model sketching enabled users to take drastically different cognitive approaches to model development. Users took on average [5-10] minutes to author a model sketch, and they were able to create [4-5] different sketches for a given task within a one-hour session. With this dramatically reduced authoring speed and a concept-oriented entrypoint, we observed that users spent most of their time refining their concept and were able to explore on average [2-3] alternative formulations of the same task. In contrast, using traditional ML approaches, users typically did not spend any time refining their concept and did not explore any alternative task formulations. Models authored using our model sketching approach also aligned better with users’ views; in performance evaluations on a held-out test set, model sketch candidates achieved [X%] higher F1 scores and [X%] lower MAE. Finally, participants felt that model sketching enabled them to more broadly explore the design space and indicated higher levels of expressivity and control with the model sketching approach.

% [What else you can do with model sketches; ceiling]
To further explore the possibilities of our sketch-based approach, we provide 5 case studies to illustrate the wide range of tasks that model sketching can support. [TODO: feed ranking, travel planning, resume screening, political alignment research, reviewer bias audit, creative inspiration generator]

% [Why our brand of sketching addresses common pain points/problems in ML]
Over-reliance on technical tools and approaches early on in the ML development process is the status quo today, but this pulls practitioners into the technical minutiae and away from important high-level, definitional questions and ethical implications of their model candidates. Today, many of AI’s most pressing challenges, such as algorithmic bias and model failure under distribution shift, are unfortunate byproducts of model development methods that do not sufficiently explore the solution space to arrive at robust and diverse solutions. As with traditional sketching, much of the value of model sketching comes from the novel work practices that arise from radically shifting the speed, cost, and focus of model development. By drastically reducing the ML development cycle, model sketches allow ML practitioners to develop many sketches that they can evaluate, compare, and share for feedback. Rapid iteration allows practitioners to more quickly identify and address gaps in their modeling approach such as data fields that would be necessary to understand a certain concept, classes of examples that are not represented, and additional user feedback that would be needed to refine a given concept. With our approach, ML practitioners can better anticipate model failures and reason over the high-level value trade-offs embedded in their models. We view model sketching as an important step that moves beyond the mode of fixing individual models and towards one of helping ML practitioners to become better model designers from the start.



==> sections/old_versions/1_intro_v2.tex <==
% V2 9/3/22

% [Machine learning development is unwieldy/slow/inflexible; tunneling/fixation is bad]
Though widely leveraged in today’s technologies, machine learning (ML) models are surprisingly unwieldy to develop and iterate upon. Because there are so many interconnected steps that go into model development—from mathematical formulation to dataset annotation to feature engineering—and because all of these steps must be fully implemented to produce a functional system, it takes a significant investment of time and effort to implement and deploy a new machine learning model~\MSLcite{}. 

Worse, this significant inertia encourages ML practitioners to take a primarily \textit{technical}, \textit{implementation-focused} approach to model development. 
Given long development cycles, model developers tend to fixate on low-level implementation details and co-opt familiar modeling approaches for new problems even when they may be sub-optimal~\cite{jun_hypothesisFormalization}.
% For example, when designing an ML model to screen job applicant resumes, developers are more likely to dive into questions around the number of dimensions in a text embedding rather than interrogating whether candidates of different demographic groups write resumes in similar ways. 
For example, when designing an ML model to screen job applicant resumes, developers are more likely to dive into questions around which parsing algorithm would most accurately process resume text or which text embedding method would most faithfully capture semantics rather deliberating over whether the inclusion of university names will codify bias in favor of well-known institutions. If they've previously found success on article topic classification using a deep learning framework that takes text embeddings as input, they're likely to port over that same technical approach to this new context.
% Model development tools place a similar focus on technical minutiae and only further pull ML practitioners into the weeds of implementation~\MSLcite{}.

This status quo is concerning because in human-facing deployments of machine learning, one of the most challenging and critical pieces to get right is the translation from a vague, high-level decison-making goal to a refined, quantifiable decision-making policy. While company leadership may set an initial goal of identifying promising, qualified candidates with a resume-screening model, ML teams must turn this idea into a particular instantiation of what it means to be promising or qualified and how a resume might be used to ascertain these qualities. The more value-laden and ethically-dubious a problem area, the more ML practitioners need to take care during the model design process to get this translation right. A primary focus on technical implementation promotes a tunneling mindset that fixates on a single task formulation (i.e., identify candidates most similar to the highest-performing employees) and runs with it---exactly the opposite of what we must do when the task formulation itself is contested and when we must grapple with the ethical tradeoffs of multiple viable approaches (i.e., what about highlighting candidates who achieved the most given the opportunities available to them, or surfacing candidates who balanced academic endeavors with extracurricular pursuits in line with the company's mission?)~\MSLcite{}.
But without the right training or tools to navigate these ill-defined problem spaces, we cannot expect ML practitioners to think and act otherwise.


% Thus, there is a great deal of inertia in model development: it is difficult to edit or rethink the design of a model, so ML developers cannot broadly explore the design space of task formulation or model design. Rather, they are incentivized to rely upon existing models or tools and are thus much more likely to fixate on a certain task formulation early on in the development process. Tunneling  approaches that dive quickly into implementation may work sufficiently well for tasks that can be clearly defined and have a single solution. However, as we know in HCI, such tunneling is disastrous for ill-defined domains where practitioners must grapple with the tradeoffs of multiple viable solutions, and most human-facing deployments of machine learning fall in this category.

% [ML needs a sketching practice; why sketching is beneficial; most importantly, it focuses attention]
% msl: think about how to strengthen/motivate connection between ML development and product/interaction design
% Machine learning lacks a sketching practice and is in dire need of one. 
To refocus their attention away from implementation-oriented questions of \textit{how to execute} on an idea and equip them to confront design-oriented questions of \textit{which ideas to pursue} in the first place, ML practitioners are in need of a \textit{sketching practice}. Sketching is a powerful technique that designers use to combat against the trap of tunneling; sketches allow them to rapidly and broadly explore a design space in the early stages of the design process~\MSLcite{}. Much of the value of a sketch derives from its ability to distill an idea to its minimal representation—to focus attention on the most important aspects of a design direction. In doing so, sketches act as valuable cognitive tools for practitioners themselves to understand nascent designs, and as boundary objects that facilitate communication between users and stakeholders~\MSLcite{}. 

Unfortunately, almost everything about modern ML development runs counter to the key characteristics of a sketching practice. Sketches are meant to be quick, expressive, and have minimal detail~\cite{buxton2010sketching}. However, today’s most advanced and expressive models are generally slow and detail-laden: end-to-end blackbox models that take years or months to develop and require large amounts of human labor and compute~\MSLcite{}. 
% The extreme cost of retraining has even inspired lines of work to allow for model editing, which ... TODO: decide if that's relevant/necessary here
Current modeling approaches that are quick and lightweight are generally lacking in expressivity. Simple example- or demonstration-based tools (e.g., Apple's Create ML or Google's Teachable Machine~\MSLcite{}) only allow users to indirectly express their modeling goals via data, which may be brittle and may lead to unexpected outcomes if the model's learnings from the data differ from what the user hoped.
Emerging tools like prompt-based model authoring with large language models (LLMs) are quick and expressive~\MSLcite{ GPT-3, CLIP}, but still tend to lead practitioners towards overly-detailed implementation rabbitholes (i.e., prompt hacking) unless designers provide significant scaffolds and abstractions~\cite{wu_AI_chains}.
Today's tools do not yet allow ML practitioners to successfully engage in sketching as a tool for thinking.
% In short, the existing tools at the disposal of ML practitioners are 
% if sketching is meant to be a tool for thinking, then today's tools 
% In their current form, all of these tools are insufficient vehicles to aid 
% ML practitioners to engage in sketching as a tool for thinking.
% Sketching is a tool for thinking, and in their current form, all of the above tools

% [We think sketching in ML should be about concepts; this is especially important in human-facing, subjective tasks where we need a great deal of expressivity and control]
% Sketches force practitioners to direct their attention to the most critical axes of their designs, and we hold that in an ML task, the most important parts to get right ought to be the concepts with which the model will reason to make decisions. Much of the conceptually difficult work of a modeling task is translating from a high-level decisionmaking goal or concept (which is often vague and underspecified) to a crisp and refined decisionmaking logic that aligns with a practitioner’s goals and end users’ needs. What do we really mean when we classify a comment as profane or political? What factors make a film or novel worth recommending to a user? Prior work on concept evolution has demonstrated that, even in seemingly objective tasks like classifying whether an image contains a cat, nuances and subjectivities arise that must be clarified (i.e., should we include a cartoon cat? should we include a lion?)~\cite{kulesza_conceptEvolution, chang_revolt}. However, getting these concepts right is especially important in subjective tasks where the general population is likely to disagree. In these kinds of tasks, it is critical to ensure that we achieve a strong grasp of our subjective understanding of a concept before we go and build a model around it, and we must have the expressivity and control to translate this subjective understanding to a technical system. 

% [We introduce model sketching]
To address this gap, we introduce \textit{model sketching}, a technical approach that allows ML practitioners to create expressive, sketch-like versions of models.
Our insight is that model developers currently lack sufficient \textit{intermediate representations} as they translate from high-level, underspecified modeling goals to concrete implementations. Because of this missing middle-ground, they jump directly from vague goals to hyperspecific instantiations (fretting over model architecture, objective functions, hyperparameters, and training infrastructure) and bypass the valuable task of deliberating over diverse ways to interpret and codify a modeling goal.

Our model sketching approach leverages \textit{concepts}---human-understandable ideas or factors that are relevant to a decision-making task---as a cognitive intermediary between an overall modeling task and its detailed implementation.
For example, concepts in a resume-screening task could range from concrete factors like ``high grades'' or ``leadership experience'' to more abstract ideas like ``creativity'' or ``independence.''
Prior work on concept evolution in data labeling demonstrated that many decision-making goals are malleable and subjective, but these goals can be clarified through an iterative process of concept elicitation and refinement~\cite{kulesza_conceptEvolution, chang_revolt}.
The introduction of concepts as a layer of abstraction above technical implementation in model authoring allows us to negotiate the tradeoff between the goals of expressivity, speed, and minimal detail while maintaining user understanding, which is critical if model sketching is to serve as a tool for thinking.
Leveraging recent developments in zero-shot learning using pre-trained models like GPT-3 and CLIP, our method allows users to turn concept ideas into functioning models in real time. With our \texttt{ModelSketchBook} tool loaded in a computational notebook environment, users can specify a concept like ``friendly'' or ``profanity'' and provide several image or text examples. In moments, they receive scores that roughly capture how friendly each example is or how likely it is to include profanity. After iteratively exploring various potentially-relevant concepts, they can combine sets of concepts into a holistic model, which we term a \textit{sketch model}. By interactively authoring concepts, incorporating them into sketches, and inspecting resultant modeling outcomes, users can flexibly explore different modeling approaches and their ramifications.

% Our approach foregrounds concepts as the core building blocks of an ML-authoring design language. Instead of working at the level of hyperparameters and mathematical operators, users producing model sketches work at the level of concepts (e.g., profanity, racism, politics, and hate speech in a content moderation context) to author models that instantiate their vision. With this approach, users can iteratively define and refine what they really mean when, for example, they term a comment as high-quality, entertaining, or toxic. A benefit of this shift to concepts as first-class citizens is that we can leverage recent developments in zero-shot learning to map from raw data fields (i.e., the text of a post or an image of an art piece) to a concept score (i.e., a racism score or a realism score) with zero training time. We term these helper models that map from data fields to concept scores concept models. By iteratively specifying a small set of underlying concept models and determining how they will be aggregated into a sketch model, users can author and instantiate a series of sketch models in real time to explore different modeling approaches. Not only are these sketch models expressive and quick to author, but they are also working models that can take in unseen data and produce user-facing outputs. [To add: something about how many other model dev decisions fall out from decisions around the concepts (ex: data fields, the kinds of data needed, how the model scores will be used in an interface]] [To add: mention how we anticipate model sketches getting translated to full models]

% [Recap of our evaluation; imagined for now] 
In an evaluation with \MSLtempValue{20} ML practitioners, we found that model sketching successfully enabled users to shift from a technical, implementation-focused mindset to a higher-level, design-oriented one. 
Using a Colab notebook~\MSLcite{ Colab} with our \texttt{ModelSketchBook} tool enabled, participants were tasked with authoring sketch models that would determine whether internet memes sourced from the Hateful Memes Challenge~\cite{kiela_hatefulMemes} should be removed from a social platform. This task is challenging even for state-of-the-art models due to the subjectivity of humor and content moderation decisions, the complexity of dealing with multiple modalities (image and text), and the fact that the semantics of a meme frequently depend on the interaction between image, text, and external context (e.g., global events, the poster's identity, the community in which a meme is posted).
% Change from technical to conceptual (modeling plan, concept evol)
\MSLtempValue{All} participants initially focused on technical details (e.g., model types like convolutional neural networks and transformers; performance metrics like F1 and AUC) when proposing a modeling plan for this task before we introduced model sketching. However, after learning about model sketching and using our \texttt{ModelSketchBook} tool, \MSLtempValue{the majority} of participants shifted to describe their approach in terms of higher-level design and problem formulation decisions.
The model sketching approach enabled users to iteratively explore and experiment with concepts that might address gaps exposed by their early sketch models: \MSLtempValue{all} participants branched out beyond the initial set of concepts that they brainstormed before using our \texttt{ModelSketchBook} tool, eventually covering concepts ranging from ``racism'' and ``islamophobia'' to ``sarcasm,'' ``irony,'' and ``controversial.''
% Noticing modeling gaps; what kinds of concepts they should consider
With this new expressive, lightweight interaction mode, participants were able to turn their attention beyond modeling to identify gaps in the dataset, scoring scheme, labeling method, and task formulation; users noted factors such as seemingly inconsistent labels, class imbalance, lack of representation of certain types of harm, and subtleties of interaction between text and image semantics.
% Time required but maintaining satisfaction
While participants initially estimated that it would take from days to months to produce a model for this task, after using our tool for an average of \MSLtempValue{20-30} minutes, \MSLtempValue{the majority} of participants were somewhat satisfied, satisfied, or very satisfied with the models they'd created.
% To potentially add: performance metrics on participant test sets; user expressivity and control


% [What else you can do with model sketches; ceiling]
To further demonstrate the flexibility of our model sketching approach, we provide case studies to illustrate the broad range of tasks that model sketching can support. Using our \texttt{ModelSketchBook} tool, we authored 1)~an Amazon product re-ranking model, 2)~a political candidate alignment research tool, 3)~a creative inspiration generator, 4)~a reviewer bias auditing tool for restaurant reviews, and 5)~a travel planning tool. Model sketching can be applied to a variety of common machine learning task formulations from simple classification and regression tasks to ranking, recommendation, clustering, search, and decision-making.

% Implications/takeaways
In a space dominated by high-fidelity technical implementation and engineering effort, we recommend moving in a direction of low-fidelity, flexible, quick, and expressive explorations with model sketching. Today, many of the most pressing challenges in artificial intelligence (AI), such as algorithmic bias and model failure under distribution shift~\MSLcite{}, are unfortunate byproducts of model development methods that do not sufficiently explore the solution space to arrive at robust and diverse solutions. As with traditional sketching, much of the value of model sketching comes from the alternate \textit{cognitive frame} that arises from radically shifting the focus and speed of iteration. By drastically minimizing the ML development cycle, model sketches allow ML practitioners to develop many sketches that they can evaluate, compare, and share for feedback. Rapid iteration allows practitioners to more quickly identify and address gaps in their modeling approach such as data fields that would be necessary to understand a certain concept, classes of examples that are not sufficiently represented, and additional user feedback needed to refine a given concept. With our approach, ML practitioners can better anticipate model failures and reason over the high-level value tradeoffs embedded in their models. We view model sketching as an important step that moves beyond the mode of retroactively fixing broken models and towards one of helping ML practitioners to become better model designers from the start.

% Contributions
% Model sketching approach
% ModelSketchBook API
% Evaluation of MSB on hateful memes task and case studies of other applications
To summarize, this paper makes the following contributions:
\begin{itemize}
    \item \textbf{A model sketching approach}. We introduce a concept-based approach supported by zero-shot models that enables users to author sketch-like versions of machine learning models.
    \item \textbf{The {ModelSketchBook} tool}. We instantiate our idea of model sketching in an open-source Python package that allows users to interactively author concepts and sketch models in a computational notebook.
    \item \textbf{An evaluation of model sketching with ML practitioners}. We perform a user evaluation with \MSLtempValue{20} machine learning practitioners who use our \texttt{ModelSketchBook} tool to author models for a challenging hateful meme detection task. We find that ML practitioners are successfully able to scope out from technical implementation details to higher-level decision-making logic. This cognitive shift helps ML practitioners to more broadly explore the model design space and to quickly discover gaps in the dataset, labeling method, and problem formulation.
    % \item \textbf{Model sketching case studies}. We demonstrate [x] additional case studies that leverage \texttt{ModelSketchBook} to perform tasks ranging from feed ranking to creative inspiration to bias auditing.
\end{itemize}

% [Why our brand of sketching addresses common pain points/problems in ML]
% Over-reliance on technical tools and approaches early on in the ML development process is the status quo today, but this pulls practitioners into the technical minutiae and away from important high-level, definitional questions and ethical implications of their model candidates. Today, many of AI’s most pressing challenges, such as algorithmic bias and model failure under distribution shift, are unfortunate byproducts of model development methods that do not sufficiently explore the solution space to arrive at robust and diverse solutions. As with traditional sketching, much of the value of model sketching comes from the novel work practices that arise from radically shifting the speed, cost, and focus of model development. By drastically reducing the ML development cycle, model sketches allow ML practitioners to develop many sketches that they can evaluate, compare, and share for feedback. Rapid iteration allows practitioners to more quickly identify and address gaps in their modeling approach such as data fields that would be necessary to understand a certain concept, classes of examples that are not represented, and additional user feedback that would be needed to refine a given concept. With our approach, ML practitioners can better anticipate model failures and reason over the high-level value trade-offs embedded in their models. We view model sketching as an important step that moves beyond the mode of fixing individual models and towards one of helping ML practitioners to become better model designers from the start.



==> sections/old_versions/1_intro_v3.tex <==
% V3 9/7/22

% [Machine learning development is unwieldy/slow/inflexible; tunneling/fixation is bad]
% Though widely leveraged in today’s technologies, machine learning (ML) models are surprisingly unwieldy to develop and iterate upon. Because there are so many interconnected steps that go into model development—from mathematical formulation to dataset annotation to feature engineering—and because all of these steps must be fully implemented to produce a functional system, it takes a significant investment of time and effort to implement and deploy a new machine learning model~\MSLcite{}. 

\msb{I think this first sentence is too ``apple pie'' in that it is unobjectionable but also uninteresting --- sort of like when papers recapitulate Weiser's ubicomp vision. I'd cut it and start with the more trenchant observation about focusing on low level implementation details. You can bring up the ``ML impacts us'' rationale later in a less important space.}
Machine learning has permeated much of our daily life and now plays a defining role in numerous high-stakes domains ranging from employment and healthcare to content moderation and communication, all of which have considerable implications on our online and offline well-being~\MSLcite{}.
However, when ML practitioners develop machine learning models, they are not primarily thinking about these kinds of high-level, human implications \msb{it's not clear that model sketching directly points people at high-level human implications --- more at high level modeling decisions. We should be careful to set out the problem that we solve most directly}---instead, they tend to focus on low-level implementation details~\cite{jun_hypothesisFormalization}. For example, when designing a model to detect hateful posts that should be removed from a platform, their first questions are rarely about what kind of language ought to be classified as hateful, but instead are questions like: What model architecture should they use? Should they leverage a convolutional neural network or transformer model? What performance metric should they benchmark on?

% Worse, this significant inertia encourages ML practitioners to take a primarily \textit{technical}, \textit{implementation-focused} approach to model development. 
% Given long development cycles, model developers tend to fixate on low-level implementation details and co-opt familiar modeling approaches for new problems even when they may be sub-optimal~\cite{jun_hypothesisFormalization}.
% For example, when designing an ML model to screen job applicant resumes, developers are more likely to dive into questions around which parsing algorithm would most accurately process resume text or which text embedding method would most faithfully capture semantics rather deliberating over whether the inclusion of university names will codify bias in favor of well-known institutions. If they've previously found success on article topic classification using a deep learning framework that takes text embeddings as input, they're likely to port over that same technical approach to this new context.

\msb{This paragraph takes a largely normative approach to the dangers of technical focus. While I agree with the critique, I worry that it's not a strong enough argument on its own to convince ML practitioners to adopt model sketching, and so it undersells the contribution. It comes across a bit like we want people to take vitamins more. But given that you also got some very positive feedback from the practitioners in your study, I would encourage you to pop up a level and reflect on what led to that positive feedback, then lob a higher level critique that implies BOTH the normative critique and the ``wow I like this better!'' perspective. For example is there evidence that people want to think about the higher level stuff, but focus on the details because that's the only approach they have in front of them? Or maybe that this technical focus encodes implicit values into the models, e.g., what kinds of comments ``count'' as toxic, that the developer didn't intend and later surface as bugs and embarrassing errors? Or maybe your users were excited because it let them communicate their high level intent, which hasn't been possible before?}
This status quo is concerning because in human-facing deployments of machine learning, one of the most challenging and critical pieces to get right is the translation from a vague, high-level decision-making goal (e.g., ``detect hateful posts'') to one of many possible technical implementations \msb{the phrase technical implementations is confusing here, since the previous paragraph sets me up to equate technical implementations = low level questions. Is that what was intended? Or do you mean many possible instantiations, policy decisions, design decisions, or some other phrase?} that would instantiate this vision. 
% While company leadership may set an initial goal of identifying promising, qualified candidates with a resume-screening model, ML teams must turn this idea into a particular instantiation of what it means to be promising or qualified and how a resume might be used to ascertain these qualities. 
The more value-laden and ethically-dubious a problem area, the more ML practitioners need to take care during the model design process to get this translation right \msb{good place to add cites}. 
A default focus on technical implementation promotes a tunneling mindset that fixates on a single task formulation (e.g., detect posts that are most similar to posts those that were previously removed from the platform) and runs with it---exactly the opposite of what we must do when the task formulation itself is contested and when we must grapple with the ethical tradeoffs of multiple viable approaches (e.g., flag posts if this specific community's members would likely want it removed, or flag posts related to user-specified topics)~\MSLcite{}.
But without the right training or tools to navigate these ill-defined problem spaces, we cannot expect ML practitioners to think and act otherwise.



% [ML needs a sketching practice; why sketching is beneficial; most importantly, it focuses attention]
% msl: think about how to strengthen/motivate connection between ML development and product/interaction design
% Machine learning lacks a sketching practice and is in dire need of one. 
\msb{Same comment as on the last paragraph diffuses here as well --- we're being very normative here. Which isn't wrong, but I have a hunch that just like sketching and prototyping allow us to examine the normative elements of our interaction designs, they're also more fluid and enjoyable approaches to design that allow me to iterate faster.}
To refocus their attention away from implementation-oriented questions of \textit{how to execute} a solution and equip them to confront design-oriented questions of \textit{which kinds of solutions to pursue} in the first place, ML practitioners are in need of a \textit{sketching practice}. Sketching is a powerful technique that designers use to combat against the trap of tunneling; sketches allow them to rapidly and broadly explore a design space in the early stages of the design process~\cite{buxton2010sketching,landay_interactiveSketching}. Much of the value of a sketch derives from its ability to distill an idea to its minimal representation \msb{great phrase, love it}—to focus attention on the most important aspects of a design direction. In doing so, sketches act as valuable cognitive tools for practitioners themselves to understand nascent designs~\MSLcite{}. However, today's tools do not yet allow ML practitioners to successfully engage in sketching as a tool for thinking, especially in the early phases of model development. \msb{I think this set of critiques would be stronger if you took requirements for sketches from prior work, and showed how existing tools failed those, rather than coming up with our own shortcomings. e.g., FamousAuthorX says that sketches should be (1) rapid, (2) expressive, and (3) ... State of the art models fail rapid because they take forever to train, low-code options fail expressivity, etc. Pick criteria that best highlight what your model sketches do but prior work hasn't. UPDATE: I now see, having read your System section, that you've done this down there. I suggest using those same criteria up here.} State-of-the-art models generally lack interpretability and take significant time and effort to develop; low-code or no-code ML toolkits like scikit-learn, Apple's Create ML, or Google's Teachable Machine~\cite{scikit_learn} are example-based and thus have limited expressivity; and emerging prompt-based model authoring techniques~\cite{GPT-3} are quick and expressive, but are still too detailed and tend to pull practitioners toward implementation rabbitholes like prompt hacking \msb{I'm not sure what we mean by too detailed here. GPT-3 prompts are typically just a few sentences.}.

% Unfortunately, almost everything about modern ML development runs counter to the key characteristics of a sketching practice. Sketches are meant to be quick, expressive, and have minimal detail~\cite{buxton2010sketching}. However, today’s most advanced and expressive models are generally slow and detail-laden: end-to-end blackbox models that take years or months to develop and require large amounts of human labor and compute~\MSLcite{}. 
% Current modeling approaches that are quick and lightweight are generally lacking in expressivity. Simple example- or demonstration-based tools (e.g., Apple's Create ML or Google's Teachable Machine~\MSLcite{}) only allow users to indirectly express their modeling goals via data, which may be brittle and may lead to unexpected outcomes if the model's learnings from the data differ from what the user hoped.
% Emerging tools like prompt-based model authoring with large language models (LLMs) are quick and expressive~\cite{GPT-3}, but still tend to lead practitioners towards overly-detailed implementation rabbitholes (i.e., prompt hacking) unless designers provide significant scaffolds and abstractions~\cite{wu_AI_chains}.
% Today's tools do not yet allow ML practitioners to successfully engage in sketching as a tool for thinking.

% [We introduce model sketching]
\msb{This paragraph almost makes it feel too easy. I wonder if it might come across as more of a new idea if we start at a higher level. e.g., what we want to enable is people to specify the concepts that the model learn to reason over: not that hateful content is the following examples, but that hateful content should mostly be paying attention to racism, profanity, and sexism. (you might look up the defn of hate speech to make sure that's not missing anything major, like violence.) And that they should be able to see how a model using those concepts behaves, then add new concepts, like violence, or refine existing concepts. And that this focused the developer on what intermediate ideas the model should be capturing.}
To address this gap, we introduce \textit{model sketching}, a technical framework that allows ML practitioners to create expressive, sketch-like versions of models in the early stages of model development.
\msb{Since I think your big idea is model sketching, I think it's confusing to then say that your insight is something else. Perhaps change this to just jump to we pursue intermediate representations}
Our insight is that model developers currently lack sufficient intermediate representations as they translate from high-level, underspecified modeling goals to concrete implementations.
% Because of this missing middle-ground, they jump directly from vague goals to hyperspecific instantiations (fretting over model architecture, objective functions, hyperparameters, and training infrastructure) and bypass the valuable task of deliberating over diverse ways to interpret and codify a modeling goal.
Thus, our model sketching framework leverages \textit{concepts}---human-understandable ideas or factors that are relevant to a decision-making task---as a cognitive intermediary between an overall modeling task and its detailed implementation.
For example, concepts in a hateful post detection task could range from concrete factors such as ``profanity,'' ``violence,'' and ``sexism'' to more abstract factors such as ``sarcasm,'' ``humor,'' and ``controversial.''
\msb{I agree with this sentence, but it feels like it's hanging out in the middle of this paragraph with only weak connections to the logic that precedes it or follows it}Prior work on concept evolution in data labeling demonstrated that many decision-making goals are malleable and subjective, but these goals can be clarified through an iterative process of concept elicitation and refinement~\cite{kulesza_conceptEvolution, chang_revolt}.
% The introduction of concepts as a layer of abstraction above technical implementation in model authoring allows us to negotiate the tradeoff between the goals of expressivity, speed, and minimal detail while maintaining user understanding, which is critical if model sketching is to serve as a tool for thinking.
We instantiate our model sketching framework in a tool called \texttt{ModelSketchBook}, which leverages recent developments in zero-shot learning with pretrained models like GPT-3 and CLIP to allow users to turn concept ideas into functioning models in real time \msb{I think a reader might get confused here, since the paper has previously used ``model'' to refer to the end to end model, and now it's referring to an internal black box inside that model. I suggest }. With the tool loaded in a computational notebook environment, users can specify a concept like ``sexist'' or ``profanity'' \msb{the inconsistency in part of speech between concepts throughout this intro is confusing. Can we normalize them? e.g., ``sexism'' and ``profanity'' vs. ``sexist'' and ``profane'', and similarly above} \msl{ah yeah, I purposely used different parts of speech to show that we're not limited to just nouns or just adjectives, etc., but maybe that's too jarring} and provide several image or text examples. ModelSketchBook draws on pretrained models to roughly score each input on how sexist each example might be or how likely it is to include profanity. After iteratively exploring various potentially-relevant concepts, users combine sets of concepts together into a holistic model, which we term a \textit{sketch model}. By interactively authoring concepts, incorporating them into sketches, and inspecting resultant modeling outcomes, users can flexibly explore different modeling approaches and their ramifications.


% [Recap of our evaluation; imagined for now] 
In an evaluation with \MSLtempValue{20} ML \msb{the first time you use ML in the paper, it should be written out ``machine learning (ML)''} practitioners, we found that model sketching successfully enabled users to shift from a technical, implementation-focused mindset to a higher-level, design-oriented one. 
Using a Colab notebook~\cite{colab} with our \texttt{ModelSketchBook} tool enabled, participants were tasked with authoring sketch models that would determine whether internet memes sourced from the Hateful Memes Challenge~\cite{kiela_hatefulMemes} should be removed from a social media platform. 
% This task is challenging even for state-of-the-art models due to the subjectivity of humor and content moderation decisions, the complexity of dealing with multiple modalities (image and text), and the fact that the semantics of a meme frequently depend on the interaction between image, text, and external context (e.g., global events, the poster's identity, the community in which a meme is posted).
We selected this task because it sets a high bar for technical difficulty (involving interacting text and image modalities, a challenge even for state-of-the-art models), involves subjective judgement (providing sufficient interpretive flexibility to create a broad model design space), and involves ethical tradeoffs (requiring a consideration of multiple competing viewpoints).
% Change from technical to conceptual (modeling plan, concept evol)
Before being introduced to ModelSketchBook, \MSLtempValue{every} participant initially focused on technical details (e.g., model types like convolutional neural networks and transformers; performance metrics like F1 and AUC) when proposing a modeling plan for this task. However, after learning about model sketching and using our \texttt{ModelSketchBook} tool, \MSLtempValue{the majority} of participants shifted to describe their approach in terms of higher-level design and problem formulation decisions.
The model sketching framework enabled users to iteratively explore and experiment with concepts that might address gaps exposed by their early sketch models: \MSLtempValue{all} participants branched out beyond the initial set of concepts that they brainstormed before using our \texttt{ModelSketchBook} tool, eventually covering concepts ranging from ``racism'' and ``islamophobia'' to ``sarcasm,'' ``irony,'' and ``controversial'' that would have not arisen if the model were developed with traditional methods.
% Noticing modeling gaps; what kinds of concepts they should consider
With this new expressive, lightweight interaction mode, participants were able to turn their attention beyond modeling to identify gaps in the dataset, scoring scheme, labeling method, and task formulation; users noted factors such as seemingly inconsistent labels, class imbalance, lack of representation of certain types of harm, and subtleties of interaction between text and image semantics.
% Time required but maintaining satisfaction
While participants initially estimated that it would take from days to months to produce a model for this task, after using our tool for 20-30 minutes, \MSLtempValue{the majority} of participants were somewhat satisfied, satisfied, or very satisfied with the models they created. We further demonstrate the flexibility of our model sketching framework with case studies ranging from political candidate research to creative inspiration to reviewer bias auditing. 
% Using our \texttt{ModelSketchBook} tool, we authored 1)~an Amazon product re-ranking model, 2)~a political candidate alignment research tool, 3)~a creative inspiration generator, 4)~a reviewer bias auditing tool for restaurant reviews, and 5)~a travel planning tool. Model sketching can be applied to a variety of common machine learning task formulations from simple classification and regression tasks to ranking, recommendation, clustering, search, and decision-making.

% Implications/takeaways
In a space dominated by high-fidelity technical implementation and engineering effort, we argue for low-fidelity, quick, and expressive explorations with model sketching. \msb{As I read this, it makes me think of the long history in EUP and PBD for AI systems that we are building on. I think it would be best to nod to that history here and cite them.} Today, many of the most pressing challenges in artificial intelligence (AI), such as algorithmic bias and model failure under distribution shift~\MSLcite{}, are consequences of model development methods that do not sufficiently explore the solution space to arrive at robust and diverse solutions. As with traditional sketching, much of the value of model sketching comes from the alternate \textit{cognitive frame} that arises from radically shifting the focus and speed of iteration. By drastically minimizing the ML development cycle, model sketching allows ML practitioners to develop many models that they can evaluate, compare, and share for feedback. %Rapid iteration allows practitioners to more quickly identify and address gaps in their modeling approach such as data fields that would be necessary to understand a certain concept, classes of examples that are not sufficiently represented, and additional user feedback needed to refine a given concept. With our framework, ML practitioners can better anticipate model failures and reason over the high-level value tradeoffs embedded in their models. 
We view model sketching as an important step that moves beyond the mode of retroactively fixing broken models and towards one of helping ML practitioners to become better model designers from the start. \msb{This last sentence feels like a big leap to me: how do we go from a person articulating concepts to deployed models not being racist? I think it would help if the paragraph laid out how we envision model sketches informing eventual production models, which presumably won't have these concepts baked in in the same way.}

% Contributions
% Model sketching approach
% ModelSketchBook API
% Evaluation of MSB on hateful memes task and case studies of other applications
To summarize, this paper makes the following contributions:
\begin{itemize}
    \item \textbf{Model sketching}. We introduce a concept-based approach that enables users to author sketch-like versions of machine learning models.
    \item \textbf{The {ModelSketchBook} tool}. We instantiate our idea of model sketching as combinations of zero-shot concept models in an open-source Python package that allows users to interactively author concepts and sketch models in a computational notebook.
    \item \textbf{An evaluation of model sketching with ML practitioners}. We perform a user evaluation with \MSLtempValue{20} machine learning practitioners who use our \texttt{ModelSketchBook} tool to author models for a challenging hateful meme detection task. We find that ML practitioners are successfully able to scope out from technical implementation details to higher-level decision-making logic. This cognitive shift helps ML practitioners to more broadly explore the model design space and to quickly discover gaps in the dataset, labeling method, and problem formulation.
\end{itemize}



==> sections/old_versions/1_intro_v4.tex <==
% v4 9/12/22 (post-MSB comments)

% \msb{I think this first sentence is too ``apple pie'' in that it is unobjectionable but also uninteresting --- sort of like when papers recapitulate Weiser's ubicomp vision. I'd cut it and start with the more trenchant observation about focusing on low level implementation details. You can bring up the ``ML impacts us'' rationale later in a less important space.}
% Machine learning has permeated much of our daily life and now plays a defining role in numerous high-stakes domains ranging from employment and healthcare to content moderation and communication, all of which have considerable implications on our online and offline well-being.
% When practitioners develop machine learning (ML) models today, there is a gap between the kinds of tasks that they \textit{want} to spend time on and the kinds of tasks that actually end up occupying their time. 
As much as they may want to think creatively about high-level modeling decisions and the human-facing implications of their models, ML practitioners often are pulled into more formulaic tasks that have them focusing on low-level implementation details~\cite{jun_hypothesisFormalization}. 
% \msb{it's not clear that model sketching directly points people at high-level human implications --- more at high level modeling decisions. We should be careful to set out the problem that we solve most directly}
For example, when designing a model to detect hateful image posts that should be removed from a platform, the questions they tackle are less often about what kind of language ought to be classified as hateful, but instead are questions like: What model architecture should they use? Should they leverage a convolutional neural network or transformer model? What performance metric should they benchmark on?


% \msb{This paragraph takes a largely normative approach to the dangers of technical focus. While I agree with the critique, I worry that it's not a strong enough argument on its own to convince ML practitioners to adopt model sketching, and so it undersells the contribution. It comes across a bit like we want people to take vitamins more. But given that you also got some very positive feedback from the practitioners in your study, I would encourage you to pop up a level and reflect on what led to that positive feedback, then lob a higher level critique that implies BOTH the normative critique and the ``wow I like this better!'' perspective. For example is there evidence that people want to think about the higher level stuff, but focus on the details because that's the only approach they have in front of them? Or maybe that this technical focus encodes implicit values into the models, e.g., what kinds of comments ``count'' as toxic, that the developer didn't intend and later surface as bugs and embarrassing errors? Or maybe your users were excited because it let them communicate their high level intent, which hasn't been possible before?}
This status quo is concerning because in human-facing deployments of machine learning, one of the most challenging and critical pieces to get right is the translation from a vague, high-level decision-making goal (e.g., ``detect hateful posts'') to one of many possible instantiations of this vision~\cite{passi_barocas_problemFormulationFairness, jacobs_wallach_measurementAndFairness}. 
% \msb{the phrase technical implementations is confusing here, since the previous paragraph sets me up to equate technical implementations = low level questions. Is that what was intended? Or do you mean many possible instantiations, policy decisions, design decisions, or some other phrase?}
The more value-laden and ethically-dubious a problem area, the more ML practitioners need to take care during the model design process to get this translation right, but work along these lines tends to get buried and de-emphasized~\cite{zhang_howDoDataScienceWorkersCollaborate}. 
% \msb{good place to add cites}
Current tools frame model development primarily around technical implementation, which promotes a tunneling mindset that assumes that we can fixate on a single task formulation (e.g., detect posts that are most similar to posts those that were previously removed from the platform) and run with it~\cite{passi_jackson_dataVision, jun_hypothesisFormalization}. This is exactly the opposite of what ML practitioners need to spend time on when the task formulation itself is contested and when they must grapple with the ethical tradeoffs of multiple viable approaches (e.g., flag posts if this specific community's members would likely want it removed, or flag posts related to user-specified topics).
But without the right tools to navigate these ill-defined problem spaces, it remains difficult for ML practitioners to work on these high-level tasks, or their attempts to do so remain invisible and unnoticed.

% [ML needs a sketching practice; why sketching is beneficial; most importantly, it focuses attention]
% msl: think about how to strengthen/motivate connection between ML development and product/interaction design
% Machine learning lacks a sketching practice and is in dire need of one. 
% \msb{Same comment as on the last paragraph diffuses here as well --- we're being very normative here. Which isn't wrong, but I have a hunch that just like sketching and prototyping allow us to examine the normative elements of our interaction designs, they're also more fluid and enjoyable approaches to design that allow me to iterate faster.}
To help them to spend less time on implementation-oriented questions of \textit{how to execute} a solution and engage them in more creative, design-oriented questions of \textit{which kinds of solutions to pursue} in the first place, ML practitioners are in need of a \textit{sketching practice}. Sketching is a powerful technique that designers use to combat against the trap of tunneling; sketches allow them to rapidly and broadly explore a design space in the early stages of the design process~\cite{buxton2010sketching,landay_interactiveSketching}. Much of the value of a sketch derives from its ability to distill an idea to its minimal representation---to focus attention on the most important aspects of a design direction. 
% \msb{great phrase, love it}
In doing so, sketches act as valuable cognitive tools for practitioners themselves to understand nascent designs~\cite{fallman_designOrientedHCI}. However, today's tools do not yet allow ML practitioners to successfully engage in sketching as a tool for thinking, especially in the early phases of model development. 
% \msb{I think this set of critiques would be stronger if you took requirements for sketches from prior work, and showed how existing tools failed those, rather than coming up with our own shortcomings. e.g., FamousAuthorX says that sketches should be (1) rapid, (2) expressive, and (3) ... State of the art models fail rapid because they take forever to train, low-code options fail expressivity, etc. Pick criteria that best highlight what your model sketches do but prior work hasn't. UPDATE: I now see, having read your System section, that you've done this down there. I suggest using those same criteria up here.} 
Sketches are meant to be expressive, quick, and minimal in detail~\cite{buxton2010sketching}.
However, state-of-the-art models generally lack interpretability and take significant time and effort to develop, and low-code or no-code ML toolkits like scikit-learn, Apple's Create ML, or Google's Teachable Machine~\cite{scikit_learn} are example-based and thus have limited expressivity. Emerging prompt-based model authoring techniques~\cite{GPT-3} are quick and expressive and get closest to this vision of sketching, but require additional scaffolding to shift away from the details of individual prompts and towards higher-level model designs~\cite{wu_AI_chains}.
% \msl{<-- need to better clarify what's missing with AI Chains line of work}
% \msb{I'm not sure what we mean by too detailed here. GPT-3 prompts are typically just a few sentences.}



% \msb{This paragraph almost makes it feel too easy. I wonder if it might come across as more of a new idea if we start at a higher level. e.g., what we want to enable is people to specify the concepts that the model learn to reason over: not that hateful content is the following examples, but that hateful content should mostly be paying attention to racism, profanity, and sexism. (you might look up the defn of hate speech to make sure that's not missing anything major, like violence.) And that they should be able to see how a model using those concepts behaves, then add new concepts, like violence, or refine existing concepts. And that this focused the developer on what intermediate ideas the model should be capturing.}

% New paragraph leading in to model sketching
When embarking on building a new ML system, we need early signals on \textit{how we should approach} our modeling task. Taking a black-box or example-driven approach doesn't teach us much along these lines: what we want to ask with our early experiments are not narrow questions like ``how would our model perform if we define hateful content as <these 20 data examples>,'' but instead broader questions like ``what would it look like for a model to pay attention to factors like violence, racism, sexism, and profanity to determine what content is hateful?'' \msb{That sentence was when it finally clicked for me! Can we move it up top somehow?} Answers to questions of the latter form help us to make downstream decisions about what conceptual directions seem promising, what additional information we need to gather, and how we might divide up the modeling task among team members---all decisions that are currently very difficult to make in the early development phases.
% What we want is a tool that might enable us to more directly express and manipulate the concepts that a model should learn to reason over: to not just declare that hateful posts are these 20 data examples, but to determine what is a hateful posts, we want to be attuned to factors like violence, racism, sexism, and profanity.

% [We introduce model sketching]
To help answer these sorts of questions, we introduce \textit{model sketching}, a technical framework that allows ML practitioners to create expressive, sketch-like versions of models in the early stages of model development.
% \msb{Since I think your big idea is model sketching, I think it's confusing to then say that your insight is something else. Perhaps change this to just jump to we pursue intermediate representations}
Model developers currently lack sufficient intermediate representations as they translate from high-level, underspecified modeling goals to concrete implementations.
% Because of this missing middle-ground, they jump directly from vague goals to hyperspecific instantiations (fretting over model architecture, objective functions, hyperparameters, and training infrastructure) and bypass the valuable task of deliberating over diverse ways to interpret and codify a modeling goal.
Thus, our model sketching framework leverages \textit{concepts}---human-understandable ideas or factors that are relevant to a decision-making task---as a cognitive intermediary between an overall modeling task and its detailed implementation.
For example, concepts in a hateful post detection task could range from concrete factors such as ``profanity,'' ``violence,'' and ``sexism'' to more abstract factors such as ``sarcasm'' and ``humor.''
% \msb{I agree with this sentence, but it feels like it's hanging out in the middle of this paragraph with only weak connections to the logic that precedes it or follows it}
% Prior work on concept evolution in data labeling demonstrated that many decision-making goals are malleable and subjective, but these goals can be clarified through an iterative process of concept elicitation and refinement~\cite{kulesza_conceptEvolution, chang_revolt}.
% The introduction of concepts as a layer of abstraction above technical implementation in model authoring allows us to negotiate the tradeoff between the goals of expressivity, speed, and minimal detail while maintaining user understanding, which is critical if model sketching is to serve as a tool for thinking.
We instantiate our model sketching framework in a tool called {ModelSketchBook}, which leverages recent developments in zero-shot learning with pretrained models like GPT-3 and CLIP to allow users to turn concept ideas into functioning building blocks in real time.
% \msb{I think a reader might get confused here, since the paper has previously used ``model'' to refer to the end to end model, and now it's referring to an internal black box inside that model. I suggest }. 
With the tool loaded in a computational notebook environment, users can specify a concept like ``sexism'' or ``profanity'' and provide several image or text examples. ModelSketchBook draws on pretrained models to roughly score each input on how sexist it might be or how likely it is to include profanity. 
% \msb{the inconsistency in part of speech between concepts throughout this intro is confusing. Can we normalize them? e.g., ``sexism'' and ``profanity'' vs. ``sexist'' and ``profane'', and similarly above} \msl{ah yeah, I purposely used different parts of speech to show that we're not limited to just nouns or just adjectives, etc., but maybe that's too jarring}
After iteratively exploring various potentially-relevant concepts, users combine sets of concepts together into a holistic model, which we term a \textit{sketch model}. By interactively authoring concepts, incorporating them into sketch models, and inspecting resultant modeling outcomes, users can flexibly explore different modeling approaches and their ramifications.


In an evaluation with 17 ML practitioners, we found that model sketching successfully enabled users to shift from a technical, implementation-focused mindset to a higher-level, design-oriented one. 
Using a Colab notebook~\cite{colab} with our {ModelSketchBook} tool enabled, participants were tasked with authoring sketch models that would determine whether internet memes sourced from the Hateful Memes Challenge~\cite{kiela_hatefulMemes} should be removed from a social media platform. 
% This task is challenging even for state-of-the-art models due to the subjectivity of humor and content moderation decisions, the complexity of dealing with multiple modalities (image and text), and the fact that the semantics of a meme frequently depend on the interaction between image, text, and external context (e.g., global events, the poster's identity, the community in which a meme is posted).
We selected this task because it sets a high bar for technical difficulty (involving interacting text and image modalities, a challenge even for state-of-the-art models), involves subjective judgement (providing sufficient interpretive flexibility to create a broad model design space), and involves ethical tradeoffs (requiring a consideration of multiple competing viewpoints).
% Change from technical to conceptual (modeling plan, concept evol)
Before being introduced to ModelSketchBook, participants initially focused on technical details (e.g., model types like convolutional neural networks and transformers; performance metrics like F1 and AUC) when proposing a modeling plan for this task. However, after learning about model sketching and using our {ModelSketchBook} tool, participants shifted to describe their approach in terms of higher-level design and problem formulation decisions.
The model sketching framework enabled users to iteratively explore and experiment with concepts that might address gaps exposed by their early sketch models: all participants branched out beyond the initial set of concepts that they brainstormed before using our {ModelSketchBook} tool, eventually covering concepts ranging from ``racism'' and ``islamophobia'' to ``sarcasm,'' ``irony,'' and ``controversial'' that would have not arisen if the model were developed with traditional methods.
% Noticing modeling gaps; what kinds of concepts they should consider
With this new expressive, lightweight interaction mode, participants were able to turn their attention beyond modeling to identify gaps in the dataset, scoring scheme, labeling method, and task formulation; users noted factors such as seemingly inconsistent labels, class imbalance, lack of representation of certain types of harm, and subtleties of interaction between text and image semantics.
% Time required but maintaining satisfaction
While participants initially estimated that it would take from days to months to produce a model for this task, after using our tool for 20-30 minutes, the vast majority of participants (14 of 17) were somewhat satisfied, satisfied, or very satisfied with the models they created. We further demonstrate the flexibility of our model sketching framework with case studies ranging from political candidate research to creative inspiration to reviewer bias auditing. 

% Implications/takeaways
In a space dominated by high-fidelity technical implementation and engineering effort, we argue for low-fidelity, quick, and expressive explorations with model sketching. 
% \msb{As I read this, it makes me think of the long history in EUP and PBD for AI systems that we are building on. I think it would be best to nod to that history here and cite them.} 
Just as work in end-user programming and programming by demonstration for AI systems has long worked towards enabling users to focus on \textit{what} the system should do rather than \textit{how}, we seek to enable model authors to focus on \textit{what} their models should reason over rather than dive too early into \textit{how} their models are implemented~\msl{cite EUP and PBD work}.
Today, many of the most pressing challenges in artificial intelligence (AI), such as algorithmic bias and model failure under distribution shift~\cite{buolamwini2018genderShades, koenecke2020ASR, wilds2021}, are consequences of model development methods that do not sufficiently explore the solution space to arrive at robust and diverse solutions. As with traditional sketching, much of the value of model sketching comes from the alternate cognitive frame that arises from radically shifting the focus and speed of iteration. 
% By drastically minimizing the ML development cycle, model sketching allows ML practitioners to develop many models that they can evaluate, compare, and share for feedback. 
Instead of waiting weeks or months until a model is implemented before evaluating in the real world and discovering that a model has learned racial biases from historical data, we hope that ML practitioners can, in the course of a few days, instantiate multiple high-level model ideas and test them with users. Then, if they discover that their modeling approach is prone to racial bias in several ways, they can experiment with rounds of sketch models that might counter this bias. Only after this valuable early-stage iteration will they move on to implement full production models. Their sketches, refined through trial and error, will now serve as a roadmap: outlining details ranging from the task formulation to the sub-models that they will need to build to the data they will require. 
We view model sketching as an important step that moves beyond the mode of retroactively fixing broken models and towards one of helping ML practitioners to become better model designers from the start. 
% \msb{This last sentence feels like a big leap to me: how do we go from a person articulating concepts to deployed models not being racist? I think it would help if the paragraph laid out how we envision model sketches informing eventual production models, which presumably won't have these concepts baked in in the same way.}

% Contributions
% Model sketching approach
% ModelSketchBook API
% Evaluation of MSB on hateful memes task and case studies of other applications
To summarize, this paper makes the following contributions:
\begin{itemize}
    \item \textbf{Model sketching}. We introduce a concept-based approach that enables users to author sketch-like versions of machine learning models.
    \item \textbf{The {ModelSketchBook} tool}. We instantiate our idea of model sketching by aggregating zero-shot models that capture human-understandable concepts, and we release an open-source Python package that allows users to interactively author concepts and sketch models in a computational notebook.
    \item \textbf{An evaluation of model sketching with ML practitioners}. We perform a user evaluation with 17 machine learning practitioners who use our {ModelSketchBook} tool to author models for a challenging hateful meme detection task. We find that ML practitioners are successfully able to scope out from technical implementation details to higher-level decision-making logic. This cognitive shift helps ML practitioners to more broadly explore the model design space and to quickly discover gaps in the dataset, labeling method, and problem formulation.
\end{itemize}


% Kittens
% Just as work in end-user programming and programming by demonstration for AI systems has long worked towards creating flexible user-understandable entrypoints for complex technical systems, we seek to provide a simplified but expressive entrypoint to model authoring that allows users to show the model

==> sections/old_versions/1_intro_v5.1.tex <==
% v5.1 9/15/22 (ML edits after MSB refinement)

% msl edit
Imagine that you are a machine learning practitioner tasked with creating a model to flag hateful image memes on a social media site. Once you dive into building and iterating on your model, the questions you are tackling quickly become ones like, ``How would a transformer model perform if we train on these examples and use these hyperparameters?'' Once you're in this mode, it is challenging to escape. How could we have helped your early model development work to instead stay focused on questions like, ``What factors---such as violence, racism, sexism, and profanity---should our model pay attention to when determining what content is hateful?'' Could machine learning tools help to center early efforts not on \textit{how to execute a solution}, but on \textit{what kinds of solutions to pursue} in the first place?

% msb inverting a bit
% Imagine that you are a machine learning practitioner tasked with creating a model to flag hateful image memes on a social media site. You may quickly get dragged into implementation questions such as, ``How would a transformer model perform if we train on these examples and use these hyperparameters?'' Once you're in this mode, it is challenging to escape. Could we help your early model development work to instead stay focused on questions like, ``What factors, such as violence, racism, sexism, and profanity, should our model pay attention to when determining what content is hateful?'' Could machine learning tools help to center early development not on \textit{how to execute}, but on \textit{what kinds of solutions to pursue} in the first place?

% \msl{new (after feedback from Mitchell and Lindsay):}\\
%Imagine that you are a machine learning practitioner tasked with creating a model to flag hateful image memes on a social media site. You may initially start with questions like, ``What factors should our model pay attention to, such as violence, racism, sexism, and profanity, when determining what content is hateful?'' But once you start diving into implementing and iterating on your model, your questions quickly become ones like, ``How would a transformer model perform if we train on these examples and use these hyperparameters?'' Once you're in this mode, it is challenging to return to those initial high-level questions or revisit early decisions you made on this problem formulation. Could machine learning development focus not on \textit{how to execute}, but on \textit{what kinds of solutions to pursue} in the first place?


% \msl{old:}\\
% Imagine that you are a machine learning practitioner tasked with creating a model to flag hateful image memes on a social media site. Instead of beginning with questions like ``how would a transformer model perform if we train on these examples and use these hyperparameters?'', what if your early model development began with questions like ``what factors should our model pay attention to, like violence, racism, sexism, and profanity, when determining what content is hateful?'' 
% Could machine learning development begin not with \textit{how to execute}, but with \textit{what kinds of solutions to pursue} in the first place?
% msl: decide whether to weave in parts of blurbs like this:
% When embarking on building a new machine learning (ML) system, we need early signals on \textit{how we should approach} our modeling task. ML practitioners may initially set out to find these answers---but often without realizing it, they're pulled into a cascade of low-level technical decisions that provide little signal on whether the high-level modeling approach will succeed.
% What we want to ask with our early experiments are not narrow questions like ``how would our model perform if we define hateful content as <these few hundred data examples> and use <this model architecture>,'' but instead broader questions like ``what would it look like for a model to pay attention to factors like violence, racism, sexism, and profanity to determine what content is hateful?'' 
% Answers to questions of the latter form help us to make informed downstream decisions about what conceptual directions seem promising, what additional information we need to gather, and how we might divide up the modeling task among team members---all decisions that are currently very difficult to make in the early development phases.

Current tools and approaches in machine learning (ML) promote a tunneling mindset that focuses attention on technical implementation~\cite{jun_hypothesisFormalization}. 
% These tools pull us into a cascade of low-level tasks---gathering a dataset, extracting features, identifying pretrained feature embeddings, planning out data and feature pipelines, considering tradeoffs in model architectures, and deciding on a performance metric---all to arrive at a first version of a model. 
These tools pull us into a cascade of low-level tasks---gathering a dataset, extracting features, planning out data pipelines, considering tradeoffs in model architectures, deciding on a performance metric---all to arrive at a first version of a model. 
Such tunneling is dangerous because it locks us into a single problem formulation, %(e.g., detecting posts in the dataset we have at hand), 
which often persists even as we iterate~\cite{passi_barocas_problemFormulationFairness}. 
In contrast, it is the problem formulation itself that is the most important to iterate on early in the process, when high-level, underspecified decision-making goals such as ``detect hateful posts'' are translated into one of many concrete problem definitions~\cite{passi_barocas_problemFormulationFairness, jacobs_wallach_measurementAndFairness, passi_jackson_dataVision}. 
The more value-laden and ethically challenging a problem area, the more ML practitioners need to take care during the model design process to get this translation right. Unfortunately, this translation work tends to get buried and de-emphasized~\cite{zhang_howDoDataScienceWorkersCollaborate}.

% Fluid exploration of high-level possibilities is the purpose of a \textit{sketching practice}. 
% While technical tools pull us into low-level implementation, 
To counter similar technical tunneling in their work, designers have long adopted a \textit{sketching practice} that purposefully foregrounds fluid exploration of high-level design possibilities.
Buxton defines sketching as any design process whose output is quick, plentiful, ambiguous, and minimal in detail~\cite{buxton2010sketching}.
Sketches distill an idea to its minimal representation, focusing attention on the most important aspects of a design direction. In doing so, sketches act as valuable cognitive tools for practitioners themselves to understand nascent designs~\cite{fallman_designOrientedHCI}. However, today's tools do not yet allow ML practitioners to successfully engage in sketching as a tool for thinking, especially in the early phases of model development. 
State-of-the-art models are not quick, requiring significant time and effort to develop; low-code or no-code ML toolkits like scikit-learn, Apple's Create ML, and Google's Teachable Machine~\cite{scikit_learn, create_ml,teachable_machine} are example-based and thus have limited expressivity; prompt-based model authoring techniques such as GPT-3~\cite{GPT-3} tend to fixate on individual prompt details rather than higher-level value tradeoffs in model design.
% are often black boxes with respect to the value tradeoffs encoded in the model.
% \msb{see if you agree with the GPT-3 critique I changed it to. basically arguing that you can't easily tell GPT-3 what to pay attention to with respect to, say, toxicity}.

In this paper, we introduce \textit{model sketching}, a technical framework that allows ML practitioners to create expressive, sketch-like versions of machine learning models.
We take the position that a minimal representation for ML sketches should focus on \textit{concepts}---the human-understandable ideas or factors that are relevant to a decision-making task---as a cognitive intermediary between an overall modeling task and its detailed implementation.
For example, concepts in a hateful image meme detection task could range from concrete factors such as ``profanity,'' ``violence,'' and ``sexism'' to more abstract factors such as ``sarcasm'' and ``humor.''
We instantiate our framework in a tool called \textit{ModelSketchBook}, which leverages recent developments in zero-shot learning with pretrained models like GPT-3 and CLIP~\cite{GPT-3, CLIP} to allow users to turn open-ended concept descriptions into functioning building blocks.
With our tool loaded in a computational notebook environment, users can specify a concept like ``sexism'' or ``profanity'' and provide several image or text examples. 
ModelSketchBook draws on pretrained models to score each input on how sexist it might be or how likely it is to include profanity, and then the user combines sets of concepts together to train a holistic \textit{sketch model}. 
By interactively authoring concepts, incorporating them into sketch models, and inspecting resultant modeling outcomes, users can flexibly explore different modeling approaches and their ramifications.

\begin{figure}[!tb]
  \includegraphics[width=0.89\textwidth]{figures/case_studies_v1c.pdf}
  \caption{
    Model sketching case studies: (1)~Travel Planning, a personalized recommendation task, (2)~Creative Inspiration, an unsupervised clustering task, (3)~Political Candidate Research, a personalized search task, and (4)~Restaurant Reviews, a reviewer bias auditing task.
  }
  \label{fig:case_studies}
\end{figure}

We illustrate the generalizability of our model sketching framework through demonstration case studies and a field evaluation. We provide case studies ranging from political candidate research to creative inspiration to reviewer bias auditing~(\autoref{fig:case_studies}).
Then, in a field evaluation, we asked 17 ML practitioners to author sketches that would determine whether internet memes sourced from the Hateful Memes Challenge~\cite{kiela_hatefulMemes} should be removed from a social media site. This task sets a high bar for technical difficulty (involving interacting text and image modalities), involves subjective judgement (providing sufficient interpretive flexibility to create a broad model design space), and involves ethical tradeoffs (requiring a consideration of multiple competing viewpoints).

Model sketching successfully enabled participants to shift from a technical mindset to a higher-level, design-oriented mindset that reasoned about the concepts that the model should and should not capture.
% Change from technical to conceptual (modeling plan, concept evol)
Before being introduced to model sketching, participants initially focused on technical details (e.g., model types like convolutional neural networks and transformers; performance metrics like F1 and AUC) when proposing a modeling plan for this task. After using ModelSketchBook, participants shifted to describe their approach in terms of higher-level design and problem formulation decisions.
Participants iteratively experimented with concepts to address gaps exposed by their early sketch models: all participants branched out beyond their initial set of concepts, eventually covering concepts ranging from ``racism'' and ``Islamophobia'' to ``sarcasm,'' ``irony,'' and ``controversial'', that would have not arisen if the model were developed with traditional methods.
% Noticing modeling gaps; what kinds of concepts they should consider
With this expressive, lightweight interaction mode, participants turned their attention beyond modeling and identified gaps in the dataset, labeling method, and problem formulation; they noted factors such as inconsistent labels, class imbalance, lack of representation of certain types of harm, and subtleties of interaction between text and image semantics.
% Time required but maintaining satisfaction
While participants initially estimated that it would take from days to months to produce a model for this task, after using our tool for 20-30 minutes, the vast majority of participants (14 of 17) were satisfied with the models they created. 
% \msb{I collapsed the categories}

%Today, many of the most pressing challenges in artificial intelligence (AI), such as algorithmic bias and model failure under distribution shift~\cite{buolamwini2018genderShades, koenecke2020ASR, wilds2021}, are consequences of model development methods that do not sufficiently explore the solution space to arrive at robust and diverse solutions. 
%As with traditional sketching, much of the value of model sketching comes from the alternate cognitive frame that arises from shifting the focus and speed of iteration. 
We view model sketching as an important step that moves beyond the mode of retroactively fixing broken models and towards one of helping ML practitioners to become better model designers from the start.
% Contributions
To summarize, this paper makes the following contributions:
\begin{itemize}
    \item \textbf{Model sketching}. We introduce a concept-based technical framework that enables users to author sketch versions of machine learning models.
    \item \textbf{The ModelSketchBook tool}. We instantiate our framework of model sketching by aggregating zero-shot models that capture human-understandable concepts, and we release an open-source Python package that allows users to interactively author concepts and sketch models in a computational notebook.
    \item \textbf{An evaluation of model sketching with ML practitioners}. We perform a user evaluation with 17 machine learning practitioners who use our tool to author models for a challenging hateful meme detection task. We find that ML practitioners are successfully able to scope out from technical implementation details to higher-level decision-making logic. This cognitive shift helps ML practitioners to more broadly explore the model design space and to quickly discover gaps in the dataset, labeling method, and problem formulation.
\end{itemize}

% \msb{original:}

% % Grounded lead-in vignette
% Imagine that you are a machine learning practitioner tasked with removing hateful image memes from a social media site. Your first steps would likely be to gather a dataset, decide what features to extract, plan out data and feature pipelines, and think about what model architectures would allow you to detect signs of hate originating from both images and text. Each of these decisions pull you further into technical details---should you use a convolutional neural network or a transformer model? What performance metric should you benchmark on? Which embedding method should you use to encode text? Before you know it, you're deep in the code testing out a messy assortment of data pipelines and model versions.


% % Scoping up to what model development should look like
% When embarking on building a new machine learning (ML) system, we need early signals on \textit{how we should approach} our modeling task. ML practitioners may initially set out to find these answers---but often without realizing it, they're pulled into a cascade of low-level technical decisions that provide little signal on whether the high-level modeling approach will succeed.
% What we want to ask with our early experiments are not narrow questions like ``how would our model perform if we define hateful content as <these few hundred data examples> and use <this model architecture>,'' but instead broader questions like ``what would it look like for a model to pay attention to factors like violence, racism, sexism, and profanity to determine what content is hateful?'' 
% Answers to questions of the latter form help us to make informed downstream decisions about what conceptual directions seem promising, what additional information we need to gather, and how we might divide up the modeling task among team members---all decisions that are currently very difficult to make in the early development phases.


% % Tunneling is a problem; focuses us on technical details
% The problem is that current tools and approaches in ML frame model development primarily around technical implementation, which promotes a tunneling mindset. Tunneling is dangerous because it assumes that we can fixate on a single problem formulation (e.g., detect posts that are most similar to posts those that were previously removed from the platform) and run with it~\cite{passi_jackson_dataVision, jun_hypothesisFormalization}. This is exactly the opposite of what ML practitioners need to spend time on when the problem formulation itself is contested and when they must grapple with the ethical tradeoffs of multiple viable approaches (e.g., flag posts if this specific community's members would likely want it removed, or flag posts related to user-specified topics).
% In human-facing deployments of machine learning, one of the most challenging and critical pieces to get right is this translation from a vague, high-level decision-making goal (e.g., ``detect hateful posts'') to one of many possible instantiations of this vision~\cite{passi_barocas_problemFormulationFairness, jacobs_wallach_measurementAndFairness}. 
% The more value-laden and ethically-dubious a problem area, the more ML practitioners need to take care during the model design process to get this translation right, but work along these lines tends to get buried and de-emphasized~\cite{zhang_howDoDataScienceWorkersCollaborate}.
% Without the right tools to navigate these ill-defined problem spaces, it remains difficult for ML practitioners to work on these high-level tasks, or their attempts to do so remain invisible and unnoticed.
% % msl: potentially add something about there being lots of high-level recommendations, but these are hard to put into practice


% % Need for a sketching practice; what sketches are
% To help them to spend less time on implementation-oriented questions of \textit{how to execute} a solution and engage them in more creative, design-oriented questions of \textit{what kinds of solutions to pursue} in the first place, ML practitioners are in need of a \textit{sketching practice}. Sketching is a powerful technique that designers use to combat against the trap of tunneling; the term applies to any design process whose output is quick, disposable, ambiguous, and minimal in detail~\cite{buxton2010sketching}. Similar to prototypes, but better targeted towards the early stages of the design process, sketches allow designers to rapidly and broadly explore a design space by raising questions rather than proposing solutions~\cite{buxton2010sketching,landay_interactiveSketching}. Much of the value of a sketch derives from its ability to distill an idea to its minimal representation---to focus attention on the most important aspects of a design direction. In doing so, sketches act as valuable cognitive tools for practitioners themselves to understand nascent designs~\cite{fallman_designOrientedHCI}. However, today's tools do not yet allow ML practitioners to successfully engage in sketching as a tool for thinking, especially in the early phases of model development. 
% Sketches are meant to be expressive, quick, and minimal in detail~\cite{buxton2010sketching}.
% % Current ML tools fail sketching criteria
% However, state-of-the-art models generally lack interpretability and take significant time and effort to develop, and low-code or no-code ML toolkits like scikit-learn, Apple's Create ML, or Google's Teachable Machine~\cite{scikit_learn} are example-based and thus have limited expressivity. Emerging prompt-based model authoring techniques~\cite{GPT-3} are quick and expressive and get closest to this vision of sketching, but require additional scaffolding to shift away from the details of individual prompts and towards higher-level model designs~\cite{wu_AI_chains}.


% % Introduce model sketching
% To help answer these sorts of questions, we introduce \textit{model sketching}, a technical framework that allows ML practitioners to create expressive, sketch-like versions of models in the early stages of model development. Model developers currently lack sufficient intermediate representations as they translate from high-level, underspecified modeling goals to concrete implementations.
% Thus, our model sketching framework leverages \textit{concepts}---human-understandable ideas or factors that are relevant to a decision-making task---as a cognitive intermediary between an overall modeling task and its detailed implementation.
% For example, concepts in a hateful image meme detection task could range from concrete factors such as ``profanity,'' ``violence,'' and ``sexism'' to more abstract factors such as ``sarcasm'' and ``humor.''
% We instantiate our model sketching framework in a tool called {ModelSketchBook}, which leverages recent developments in zero-shot learning with pretrained models like GPT-3 and CLIP to allow users to turn concept ideas into functioning building blocks in real time.
% With the tool loaded in a computational notebook environment, users can specify a concept like ``sexism'' or ``profanity'' and provide several image or text examples. ModelSketchBook draws on pretrained models to roughly score each input on how sexist it might be or how likely it is to include profanity. After iteratively exploring various potentially-relevant concepts, users combine sets of concepts together into a holistic model, which we term a \textit{sketch model}. By interactively authoring concepts, incorporating them into sketch models, and inspecting resultant modeling outcomes, users can flexibly explore different modeling approaches and their ramifications.


% % Evaluation
% In an evaluation with 17 ML practitioners, we found that model sketching successfully enabled users to shift from a technical, implementation-focused mindset to a higher-level, design-oriented one. 
% Using a Colab notebook~\cite{colab} with our {ModelSketchBook} tool enabled, participants were tasked with authoring sketch models that would determine whether internet memes sourced from the Hateful Memes Challenge~\cite{kiela_hatefulMemes} should be removed from a social media site. We selected this task because it sets a high bar for technical difficulty (involving interacting text and image modalities, a challenge even for state-of-the-art models), involves subjective judgement (providing sufficient interpretive flexibility to create a broad model design space), and involves ethical tradeoffs (requiring a consideration of multiple competing viewpoints).
% % Change from technical to conceptual (modeling plan, concept evol)
% Before being introduced to ModelSketchBook, participants initially focused on technical details (e.g., model types like convolutional neural networks and transformers; performance metrics like F1 and AUC) when proposing a modeling plan for this task. However, after learning about model sketching and using our {ModelSketchBook} tool, participants shifted to describe their approach in terms of higher-level design and problem formulation decisions.
% The model sketching framework enabled users to iteratively explore and experiment with concepts that might address gaps exposed by their early sketch models: all participants branched out beyond the initial set of concepts that they brainstormed before using our {ModelSketchBook} tool, eventually covering concepts ranging from ``racism'' and ``islamophobia'' to ``sarcasm,'' ``irony,'' and ``controversial'' that would have not arisen if the model were developed with traditional methods.
% % Noticing modeling gaps; what kinds of concepts they should consider
% With this new expressive, lightweight interaction mode, participants were able to turn their attention beyond modeling to identify gaps in the dataset, scoring scheme, labeling method, and task formulation; users noted factors such as seemingly inconsistent labels, class imbalance, lack of representation of certain types of harm, and subtleties of interaction between text and image semantics.
% % Time required but maintaining satisfaction
% While participants initially estimated that it would take from days to months to produce a model for this task, after using our tool for 20-30 minutes, the vast majority of participants (14 of 17) were somewhat satisfied, satisfied, or very satisfied with the models they created. We further demonstrate the flexibility of our model sketching framework with case studies ranging from political candidate research to creative inspiration to reviewer bias auditing. 

% % Implications/takeaways
% In a space dominated by high-fidelity technical implementation and engineering effort, we argue for low-fidelity, quick, and expressive explorations with model sketching. 
% % \msb{As I read this, it makes me think of the long history in EUP and PBD for AI systems that we are building on. I think it would be best to nod to that history here and cite them.} 
% Just as work in end-user programming and programming by demonstration for AI systems has long worked towards enabling users to focus on \textit{what} the system should do rather than \textit{how}~\cite{eager_progByExample, watchWhatIDo_PBD}, we seek to enable model authors to focus on \textit{what} their models should reason over rather than dive too early into \textit{how} their models are implemented.
% Today, many of the most pressing challenges in artificial intelligence (AI), such as algorithmic bias and model failure under distribution shift~\cite{buolamwini2018genderShades, koenecke2020ASR, wilds2021}, are consequences of model development methods that do not sufficiently explore the solution space to arrive at robust and diverse solutions. As with traditional sketching, much of the value of model sketching comes from the alternate cognitive frame that arises from radically shifting the focus and speed of iteration. 
% Instead of waiting weeks or months until a model is implemented before evaluating in the real world and discovering that a model has learned racial biases from historical data, we hope that ML practitioners can, in the course of a few days, instantiate multiple high-level model ideas and test them with users. Then, if they discover that their modeling approach is prone to racial bias in several ways, they can experiment with rounds of sketch models that might counter this bias. Only after this valuable early-stage iteration will they move on to implement full production models. Their sketches, refined through trial and error, will now serve as a roadmap: outlining details ranging from the task formulation to the sub-models that they will need to build to the data they will require. 
% We view model sketching as an important step that moves beyond the mode of retroactively fixing broken models and towards one of helping ML practitioners to become better model designers from the start. 


% % Contributions
% To summarize, this paper makes the following contributions:
% \begin{itemize}
%     \item \textbf{Model sketching}. We introduce a concept-based approach that enables users to author sketch-like versions of machine learning models.
%     \item \textbf{The {ModelSketchBook} tool}. We instantiate our idea of model sketching by aggregating zero-shot models that capture human-understandable concepts, and we release an open-source Python package that allows users to interactively author concepts and sketch models in a computational notebook.
%     \item \textbf{An evaluation of model sketching with ML practitioners}. We perform a user evaluation with 17 machine learning practitioners who use our {ModelSketchBook} tool to author models for a challenging hateful meme detection task. We find that ML practitioners are successfully able to scope out from technical implementation details to higher-level decision-making logic. This cognitive shift helps ML practitioners to more broadly explore the model design space and to quickly discover gaps in the dataset, labeling method, and problem formulation.
% \end{itemize}


==> sections/old_versions/1_intro_v5.tex <==
% v5 9/14/22 rework

\msb{MSB refinement}
Imagine that you are a machine learning practitioner tasked with creating a model to flag hateful image memes on a social media site. Instead of early model development beginning with ``how would a transformer model perform if we train on these examples?'', what if your model development began with questions like ``what factors should our model pay attention to, like violence, racism, sexism, and profanity, when determining what content is hateful?'' Could machine learning development begin not with \textit{how to execute}, but with the \textit{what kinds of solutions to pursue} in the first place?

Current tools and approaches in machine learning (ML) promote a tunneling mindset that focuses attention on technical implementation. 
These tools focus our attention on gathering a dataset, extracting features, identifying pretrained feature embeddings, planning out data and feature pipelines, considering tradeoffs in model architectures, and deciding on a performance metric---all to arrive at a first version of a model. 
Such tunneling is dangerous because it hardens us into a single problem formulation (e.g., detecting posts in the dataset we have at hand), which often persists even as we iterate~\cite{passi_jackson_dataVision, jun_hypothesisFormalization}. 
In contrast, it is the problem formulation itself that is the most important to iterate on early in the process, when high-level decision-making goals such as ``detect hateful posts'' become translated into concrete problem definitions~\cite{passi_barocas_problemFormulationFairness, jacobs_wallach_measurementAndFairness}. 
The more value-laden and ethically challenging a problem area, the more ML practitioners need to take care during the model design process to get this translation right. Unfortunately, this translation work tends to get buried and de-emphasized~\cite{zhang_howDoDataScienceWorkersCollaborate}.

Fluid exploration of high-level possibilities is the purpose of a \textit{sketching practice}. Buxton defines sketching as any design process whose output is quick, disposable, ambiguous, and minimal in detail~\cite{buxton2010sketching}.
Much of the value of a sketch derives from its ability to distill an idea to its minimal representation---to focus attention on the most important aspects of a design direction. In doing so, sketches act as valuable cognitive tools for practitioners themselves to understand nascent designs~\cite{fallman_designOrientedHCI}. However, today's tools do not yet allow ML practitioners to successfully engage in sketching as a tool for thinking, especially in the early phases of model development. 
State-of-the-art models are not quick, requiring significant time and effort to develop; low-code or no-code ML toolkits like scikit-learn, Apple's Create ML, and Google's Teachable Machine~\cite{scikit_learn} are example-based and thus have limited expressivity; prompt-based model authoring techniques such as GPT-3~\cite{GPT-3} are often black boxes with respect to the value tradeoffs encoded in the model~\cite{wu_AI_chains} \msb{see if you agree with the GPT-3 critique I changed it to. basically arguing that you can't easily tell GPT-3 what to pay attention to with respect to, say, toxicity}.

In this paper, we introduce \textit{model sketching}, a technical framework that allows ML practitioners to create expressive, sketch-like versions of machine learning models.
We take the position that the proper minimal representation for ML sketches should focus on the \textit{concepts}---the human-understandable ideas or factors that are relevant to a decision-making task---as a cognitive intermediary between an overall modeling task and its detailed implementation.
For example, concepts in a hateful image meme detection task could range from concrete factors such as ``profanity,'' ``violence,'' and ``sexism'' to more abstract factors such as ``sarcasm'' and ``humor.''
Our framework leverages recent developments in zero-shot learning with pretrained models like GPT-3 and CLIP to allow users to turn open-ended concept descriptions into functioning building blocks.
With the tool loaded in a computational notebook environment, users can specify a concept like ``sexism'' or ``profanity'' and provide several image or text examples. 
The framework draws on pretrained models to roughly score each input on how sexist it might be or how likely it is to include profanity, then the user combines sets of concepts together into a holistic \textit{sketch model}. 
By interactively authoring concepts, incorporating them into sketch models, and inspecting resultant modeling outcomes, users can flexibly explore different modeling approaches and their ramifications.

In an evaluation with 17 ML practitioners, we found that model sketching successfully enabled users to shift from a technical mindset to a mindset reasoning about the concepts that the model should and should not capture.
Using a Colab notebook~\cite{colab} with our model sketching framework, participants were tasked with authoring sketch models that would determine whether internet memes sourced from the Hateful Memes Challenge~\cite{kiela_hatefulMemes} should be removed from a social media site. We selected this task because it sets a high bar for technical difficulty (involving interacting text and image modalities, a challenge even for state-of-the-art models), involves subjective judgement (providing sufficient interpretive flexibility to create a broad model design space), and involves ethical tradeoffs (requiring a consideration of multiple competing viewpoints).
% Change from technical to conceptual (modeling plan, concept evol)
Before being introduced to model sketching, participants initially focused on technical details (e.g., model types like convolutional neural networks and transformers; performance metrics like F1 and AUC) when proposing a modeling plan for this task. However, after using our model sketching framework, participants shifted to describe their approach in terms of higher-level design and problem formulation decisions.
Participants iteratively experimented with concepts that might address gaps exposed by their early sketch models: all participants branched out beyond their initial set of concepts, eventually covering concepts ranging from ``racism'' and ``islamophobia'' to ``sarcasm,'' ``irony,'' and ``controversial'' that would have not arisen if the model were developed with traditional methods.
% Noticing modeling gaps; what kinds of concepts they should consider
With this new expressive, lightweight interaction mode, participants turned their attention beyond modeling to identifying gaps in the dataset, scoring scheme, labeling method, and task formulation; they noted factors such as seemingly inconsistent labels, class imbalance, lack of representation of certain types of harm, and subtleties of interaction between text and image semantics.
% Time required but maintaining satisfaction
While participants initially estimated that it would take from days to months to produce a model for this task, after using our tool for 20-30 minutes, the vast majority of participants (14 of 17) were satisfied \msb{I collapsed the categories} with the models they created. 

We further demonstrate the flexibility of our model sketching framework with case studies ranging from political candidate research to creative inspiration to reviewer bias auditing. 
Today, many of the most pressing challenges in artificial intelligence (AI), such as algorithmic bias and model failure under distribution shift~\cite{buolamwini2018genderShades, koenecke2020ASR, wilds2021}, are consequences of model development methods that do not sufficiently explore the solution space to arrive at robust and diverse solutions. As with traditional sketching, much of the value of model sketching comes from the alternate cognitive frame that arises from shifting the focus and speed of iteration. 
We view model sketching as an important step that moves beyond the mode of retroactively fixing broken models and towards one of helping ML practitioners to become better model designers from the start.

% Contributions
To summarize, this paper makes the following contributions:
\begin{itemize}
    \item \textbf{Model sketching}. We introduce a concept-based approach that enables users to author sketch-like versions of machine learning models.
    \item \textbf{Python-based model sketching framework}. We instantiate our idea of model sketching by aggregating zero-shot models that capture human-understandable concepts, and we release an open-source Python package that allows users to interactively author concepts and sketch models in a computational notebook.
    \item \textbf{An evaluation of model sketching with ML practitioners}. We perform a user evaluation with 17 machine learning practitioners who use our Python framework to author models for a challenging hateful meme detection task. We find that ML practitioners are successfully able to scope out from technical implementation details to higher-level decision-making logic. This cognitive shift helps ML practitioners to more broadly explore the model design space and to quickly discover gaps in the dataset, labeling method, and problem formulation.
\end{itemize}

% \msb{original:}

% % Grounded lead-in vignette
% Imagine that you are a machine learning practitioner tasked with removing hateful image memes from a social media site. Your first steps would likely be to gather a dataset, decide what features to extract, plan out data and feature pipelines, and think about what model architectures would allow you to detect signs of hate originating from both images and text. Each of these decisions pull you further into technical details---should you use a convolutional neural network or a transformer model? What performance metric should you benchmark on? Which embedding method should you use to encode text? Before you know it, you're deep in the code testing out a messy assortment of data pipelines and model versions.


% % Scoping up to what model development should look like
% When embarking on building a new machine learning (ML) system, we need early signals on \textit{how we should approach} our modeling task. ML practitioners may initially set out to find these answers---but often without realizing it, they're pulled into a cascade of low-level technical decisions that provide little signal on whether the high-level modeling approach will succeed.
% What we want to ask with our early experiments are not narrow questions like ``how would our model perform if we define hateful content as <these few hundred data examples> and use <this model architecture>,'' but instead broader questions like ``what would it look like for a model to pay attention to factors like violence, racism, sexism, and profanity to determine what content is hateful?'' 
% Answers to questions of the latter form help us to make informed downstream decisions about what conceptual directions seem promising, what additional information we need to gather, and how we might divide up the modeling task among team members---all decisions that are currently very difficult to make in the early development phases.


% % Tunneling is a problem; focuses us on technical details
% The problem is that current tools and approaches in ML frame model development primarily around technical implementation, which promotes a tunneling mindset. Tunneling is dangerous because it assumes that we can fixate on a single problem formulation (e.g., detect posts that are most similar to posts those that were previously removed from the platform) and run with it~\cite{passi_jackson_dataVision, jun_hypothesisFormalization}. This is exactly the opposite of what ML practitioners need to spend time on when the problem formulation itself is contested and when they must grapple with the ethical tradeoffs of multiple viable approaches (e.g., flag posts if this specific community's members would likely want it removed, or flag posts related to user-specified topics).
% In human-facing deployments of machine learning, one of the most challenging and critical pieces to get right is this translation from a vague, high-level decision-making goal (e.g., ``detect hateful posts'') to one of many possible instantiations of this vision~\cite{passi_barocas_problemFormulationFairness, jacobs_wallach_measurementAndFairness}. 
% The more value-laden and ethically-dubious a problem area, the more ML practitioners need to take care during the model design process to get this translation right, but work along these lines tends to get buried and de-emphasized~\cite{zhang_howDoDataScienceWorkersCollaborate}.
% Without the right tools to navigate these ill-defined problem spaces, it remains difficult for ML practitioners to work on these high-level tasks, or their attempts to do so remain invisible and unnoticed.
% % msl: potentially add something about there being lots of high-level recommendations, but these are hard to put into practice


% % Need for a sketching practice; what sketches are
% To help them to spend less time on implementation-oriented questions of \textit{how to execute} a solution and engage them in more creative, design-oriented questions of \textit{what kinds of solutions to pursue} in the first place, ML practitioners are in need of a \textit{sketching practice}. Sketching is a powerful technique that designers use to combat against the trap of tunneling; the term applies to any design process whose output is quick, disposable, ambiguous, and minimal in detail~\cite{buxton2010sketching}. Similar to prototypes, but better targeted towards the early stages of the design process, sketches allow designers to rapidly and broadly explore a design space by raising questions rather than proposing solutions~\cite{buxton2010sketching,landay_interactiveSketching}. Much of the value of a sketch derives from its ability to distill an idea to its minimal representation---to focus attention on the most important aspects of a design direction. In doing so, sketches act as valuable cognitive tools for practitioners themselves to understand nascent designs~\cite{fallman_designOrientedHCI}. However, today's tools do not yet allow ML practitioners to successfully engage in sketching as a tool for thinking, especially in the early phases of model development. 
% Sketches are meant to be expressive, quick, and minimal in detail~\cite{buxton2010sketching}.
% % Current ML tools fail sketching criteria
% However, state-of-the-art models generally lack interpretability and take significant time and effort to develop, and low-code or no-code ML toolkits like scikit-learn, Apple's Create ML, or Google's Teachable Machine~\cite{scikit_learn} are example-based and thus have limited expressivity. Emerging prompt-based model authoring techniques~\cite{GPT-3} are quick and expressive and get closest to this vision of sketching, but require additional scaffolding to shift away from the details of individual prompts and towards higher-level model designs~\cite{wu_AI_chains}.


% % Introduce model sketching
% To help answer these sorts of questions, we introduce \textit{model sketching}, a technical framework that allows ML practitioners to create expressive, sketch-like versions of models in the early stages of model development. Model developers currently lack sufficient intermediate representations as they translate from high-level, underspecified modeling goals to concrete implementations.
% Thus, our model sketching framework leverages \textit{concepts}---human-understandable ideas or factors that are relevant to a decision-making task---as a cognitive intermediary between an overall modeling task and its detailed implementation.
% For example, concepts in a hateful image meme detection task could range from concrete factors such as ``profanity,'' ``violence,'' and ``sexism'' to more abstract factors such as ``sarcasm'' and ``humor.''
% We instantiate our model sketching framework in a tool called {ModelSketchBook}, which leverages recent developments in zero-shot learning with pretrained models like GPT-3 and CLIP to allow users to turn concept ideas into functioning building blocks in real time.
% With the tool loaded in a computational notebook environment, users can specify a concept like ``sexism'' or ``profanity'' and provide several image or text examples. ModelSketchBook draws on pretrained models to roughly score each input on how sexist it might be or how likely it is to include profanity. After iteratively exploring various potentially-relevant concepts, users combine sets of concepts together into a holistic model, which we term a \textit{sketch model}. By interactively authoring concepts, incorporating them into sketch models, and inspecting resultant modeling outcomes, users can flexibly explore different modeling approaches and their ramifications.


% % Evaluation
% In an evaluation with 17 ML practitioners, we found that model sketching successfully enabled users to shift from a technical, implementation-focused mindset to a higher-level, design-oriented one. 
% Using a Colab notebook~\cite{colab} with our {ModelSketchBook} tool enabled, participants were tasked with authoring sketch models that would determine whether internet memes sourced from the Hateful Memes Challenge~\cite{kiela_hatefulMemes} should be removed from a social media site. We selected this task because it sets a high bar for technical difficulty (involving interacting text and image modalities, a challenge even for state-of-the-art models), involves subjective judgement (providing sufficient interpretive flexibility to create a broad model design space), and involves ethical tradeoffs (requiring a consideration of multiple competing viewpoints).
% % Change from technical to conceptual (modeling plan, concept evol)
% Before being introduced to ModelSketchBook, participants initially focused on technical details (e.g., model types like convolutional neural networks and transformers; performance metrics like F1 and AUC) when proposing a modeling plan for this task. However, after learning about model sketching and using our {ModelSketchBook} tool, participants shifted to describe their approach in terms of higher-level design and problem formulation decisions.
% The model sketching framework enabled users to iteratively explore and experiment with concepts that might address gaps exposed by their early sketch models: all participants branched out beyond the initial set of concepts that they brainstormed before using our {ModelSketchBook} tool, eventually covering concepts ranging from ``racism'' and ``islamophobia'' to ``sarcasm,'' ``irony,'' and ``controversial'' that would have not arisen if the model were developed with traditional methods.
% % Noticing modeling gaps; what kinds of concepts they should consider
% With this new expressive, lightweight interaction mode, participants were able to turn their attention beyond modeling to identify gaps in the dataset, scoring scheme, labeling method, and task formulation; users noted factors such as seemingly inconsistent labels, class imbalance, lack of representation of certain types of harm, and subtleties of interaction between text and image semantics.
% % Time required but maintaining satisfaction
% While participants initially estimated that it would take from days to months to produce a model for this task, after using our tool for 20-30 minutes, the vast majority of participants (14 of 17) were somewhat satisfied, satisfied, or very satisfied with the models they created. We further demonstrate the flexibility of our model sketching framework with case studies ranging from political candidate research to creative inspiration to reviewer bias auditing. 

% % Implications/takeaways
% In a space dominated by high-fidelity technical implementation and engineering effort, we argue for low-fidelity, quick, and expressive explorations with model sketching. 
% % \msb{As I read this, it makes me think of the long history in EUP and PBD for AI systems that we are building on. I think it would be best to nod to that history here and cite them.} 
% Just as work in end-user programming and programming by demonstration for AI systems has long worked towards enabling users to focus on \textit{what} the system should do rather than \textit{how}~\cite{eager_progByExample, watchWhatIDo_PBD}, we seek to enable model authors to focus on \textit{what} their models should reason over rather than dive too early into \textit{how} their models are implemented.
% Today, many of the most pressing challenges in artificial intelligence (AI), such as algorithmic bias and model failure under distribution shift~\cite{buolamwini2018genderShades, koenecke2020ASR, wilds2021}, are consequences of model development methods that do not sufficiently explore the solution space to arrive at robust and diverse solutions. As with traditional sketching, much of the value of model sketching comes from the alternate cognitive frame that arises from radically shifting the focus and speed of iteration. 
% Instead of waiting weeks or months until a model is implemented before evaluating in the real world and discovering that a model has learned racial biases from historical data, we hope that ML practitioners can, in the course of a few days, instantiate multiple high-level model ideas and test them with users. Then, if they discover that their modeling approach is prone to racial bias in several ways, they can experiment with rounds of sketch models that might counter this bias. Only after this valuable early-stage iteration will they move on to implement full production models. Their sketches, refined through trial and error, will now serve as a roadmap: outlining details ranging from the task formulation to the sub-models that they will need to build to the data they will require. 
% We view model sketching as an important step that moves beyond the mode of retroactively fixing broken models and towards one of helping ML practitioners to become better model designers from the start. 


% % Contributions
% To summarize, this paper makes the following contributions:
% \begin{itemize}
%     \item \textbf{Model sketching}. We introduce a concept-based approach that enables users to author sketch-like versions of machine learning models.
%     \item \textbf{The {ModelSketchBook} tool}. We instantiate our idea of model sketching by aggregating zero-shot models that capture human-understandable concepts, and we release an open-source Python package that allows users to interactively author concepts and sketch models in a computational notebook.
%     \item \textbf{An evaluation of model sketching with ML practitioners}. We perform a user evaluation with 17 machine learning practitioners who use our {ModelSketchBook} tool to author models for a challenging hateful meme detection task. We find that ML practitioners are successfully able to scope out from technical implementation details to higher-level decision-making logic. This cognitive shift helps ML practitioners to more broadly explore the model design space and to quickly discover gaps in the dataset, labeling method, and problem formulation.
% \end{itemize}


==> sections/old_versions/1_intro_v6.tex <==
% v6 12/10/22
Imagine that you are a machine learning practitioner tasked with creating a model to flag hateful image memes on a social media site. Once you dive into building and iterating on your model, the questions you are tackling quickly become ones like, ``How would a transformer model perform if we train on these examples and use these hyperparameters?'' Once you're in this mode, it is challenging to escape. How could we have helped your early model development work to instead stay focused on questions like, ``What factors---such as violence, racism, sexism, and profanity---should our model pay attention to when determining what content is hateful?'' Could machine learning tools help to center early efforts not on \textit{how to execute a solution}, but on \textit{what kinds of solutions to pursue} in the first place?

Current tools and approaches in machine learning (ML) promote a tunneling mindset that focuses attention on technical implementation~\cite{jun_hypothesisFormalization}. 
These tools pull us into a cascade of low-level tasks---gathering a dataset, extracting features, planning out data pipelines, considering tradeoffs in model architectures, deciding on a performance metric---all to arrive at a first version of a model. 
Such tunneling is dangerous because it locks us into a single problem formulation, %(e.g., detecting posts in the dataset we have at hand), 
which often persists even as we iterate~\cite{passi_barocas_problemFormulationFairness}. 
In contrast, it is the problem formulation itself that is the most important to iterate on early in the process, when high-level, underspecified decision-making goals such as ``detect hateful posts'' are translated into one of many concrete problem definitions~\cite{passi_barocas_problemFormulationFairness, jacobs_wallach_measurementAndFairness, passi_jackson_dataVision}. 
The more value-laden and ethically challenging a problem area, the more ML practitioners need to take care during the model design process to get this translation right. Unfortunately, this translation work tends to get buried and de-emphasized~\cite{zhang_howDoDataScienceWorkersCollaborate}.

To counter similar technical tunneling in their work, designers have long adopted a \textit{sketching practice} that purposefully foregrounds fluid exploration of high-level design possibilities.
Buxton defines sketching as any design process whose output is quick, plentiful, ambiguous, and minimal in detail~\cite{buxton2010sketching}.
Sketches distill an idea to its minimal representation, focusing attention on the most important aspects of a design direction. In doing so, sketches act as valuable cognitive tools for practitioners themselves to understand nascent designs~\cite{fallman_designOrientedHCI}. 
\rev{What is the right minimal representation for ML model development?
Interactive machine learning approaches (like Wekinator, Apple's Create ML, and Google's Teachable Machine~\cite{wekinator, create_ml, teachable_machine}) and prompt-based approaches (like GPT-3~\cite{GPT-3, wu_AI_chains} and Stable Diffusion~\cite{Rombach_2022_CVPR}) allow for rapid model development, but they are centered around inputs and outputs, largely abstracting away the decision-making logic in between.
For problem formulation tasks, it's precisely that \textit{decision-making logic} that we need to directly iterate on: what are the factors that our model should consider to make its decision?
% Work in interactive machine teaching turns its attention towards the decisionmaking logic of the model, but is targeted more towards scenarios where model developers are executing on their vision in high-fidelity rather than exploring approaches in low-fidelity.
Today's tools do not yet allow ML practitioners to sketch a model's decision-making logic to rapidly answer these kinds of critical model design questions.}
% State-of-the-art models are not quick, requiring significant time and effort to develop. 
% \rev{Interactive machine learning approaches instantiated in toolkits like Wekinator, Apple's Create ML, and Google's Teachable Machine~\cite{wekinator, create_ml, teachable_machine} are quick, but are example-based and thus have limited expressivity. Methods that emphasize greater expressivity beyond examples, like interactive machine teaching and prompt-based model authoring techniques such as GPT-3~\cite{GPT-3}, tend to include rich detail that can run counter to the pared-down representations required by sketching.
% }

In this paper, we introduce \textit{model sketching}, a technical framework that allows ML practitioners to create expressive, sketch-like versions of machine learning models.
% We take the position that a minimal representation for ML sketches should focus on \textit{concepts}---the human-understandable ideas or factors that are relevant to a decision-making task---as a cognitive intermediary between an overall modeling task and its detailed implementation.
\rev{To allow for direct iteration on a model's core logic, we use \textit{concepts}---the human-understandable ideas or factors that are relevant to a decision-making task---as the minimal representation for ML sketches.}
For example, concepts in a hateful image meme detection task could range from concrete factors such as ``profanity,'' ``violence,'' and ``sexism'' to more abstract factors such as ``sarcasm'' and ``humor.''
% \rev{While prior work has explored concept-oriented abstractions in ML, a key difference in our approach is that we enable users to instantiate arbitrary novel concepts in a matter of seconds, unlocking interactions where users can directly sketch model logic rather than model inputs.}
% \msl{cite concept bottleneck work, their IMT work}
% \msl{
% Centering on these concepts as a method of rapidly iterating on model logic
% zero-shot concepts allow us to rapidly construct and iterate on model logic
% doing both rapid iteration and centering about concepts
% concepts can be authored rapidly and interactively in a way that focuses us on decisionmaking logic
% }
\rev{While prior work has explored concept-oriented abstractions in ML~\cite{koh2020ConceptBottleneck, kim2018TCAV, ramos2020IMT, ng_IMTknowledgeDecomp}, a key difference in our approach is that we not only center concepts, but we also enable rapid instantiation and iteration of arbitrary concepts by leveraging zero-shot methods. This combination of concepts and flexible, rapid authoring unlocks new interactions where users can directly sketch model logic.}
\rev{We implement our model sketching framework in a Python package called \textit{ModelSketchBook}}, which leverages recent developments in zero-shot learning with pretrained models like GPT-3 and CLIP~\cite{GPT-3, CLIP} to allow users to turn open-ended concept descriptions into functioning building blocks.
With our tool loaded in a computational notebook environment, users can specify a concept like ``sexism'' or ``profanity'' and provide several image or text examples. 
ModelSketchBook draws on pretrained models to score each input on how sexist it might be or how likely it is to include profanity, and then the user combines sets of concepts together to train a holistic \textit{sketch model}. 
By interactively authoring concepts, incorporating them into sketch models, and inspecting resultant modeling outcomes, users can flexibly explore different modeling approaches and their ramifications.

\begin{figure*}[!tb]
  \includegraphics[width=0.89\textwidth]{figures/case_studies_v1c.pdf}
  \caption{
    Model sketching case studies: (1)~Travel Planning, a personalized recommendation task, (2)~Creative Inspiration, an unsupervised clustering task, (3)~Political Candidate Research, a personalized search task, and (4)~Restaurant Reviews, a reviewer bias auditing task.
  }
  \label{fig:case_studies}
\end{figure*}

We illustrate the generalizability of our model sketching framework through demonstration case studies and a field evaluation. We provide case studies ranging from political candidate research to creative inspiration to reviewer bias auditing~(\autoref{fig:case_studies}).
Then, in a field evaluation, we asked 17 ML practitioners to author sketches that would determine whether internet memes sourced from the Hateful Memes Challenge~\cite{kiela_hatefulMemes} should be removed from a social media site. This task sets a high bar for technical difficulty (involving interacting text and image modalities), involves subjective judgement (providing sufficient interpretive flexibility to create a broad model design space), and involves ethical tradeoffs (requiring a consideration of multiple competing viewpoints).

Model sketching successfully enabled participants to shift from a technical mindset to a higher-level, design-oriented mindset that reasoned about the concepts that the model should and should not capture.
% Change from technical to conceptual (modeling plan, concept evol)
Before being introduced to model sketching, participants initially focused on technical details (e.g., model types like convolutional neural networks and transformers; performance metrics like F1 and AUC) when proposing a modeling plan for this task. After using ModelSketchBook, participants shifted to describe their approach in terms of higher-level design and problem formulation decisions.
Participants iteratively experimented with concepts to address gaps exposed by their early sketch models: all participants branched out beyond their initial set of concepts, eventually covering concepts ranging from ``racism'' and ``Islamophobia'' to ``sarcasm,'' ``irony,'' and ``controversial'', that would have not arisen if the model were developed with traditional methods.
% Noticing modeling gaps; what kinds of concepts they should consider
With this expressive, lightweight interaction mode, participants turned their attention beyond modeling and identified gaps in the dataset, labeling method, and problem formulation; they noted factors such as inconsistent labels, class imbalance, lack of representation of certain types of harm, and subtleties of interaction between text and image semantics.
% Time required but maintaining satisfaction
While participants initially estimated that it would take from days to months to produce a model for this task, after using our tool for 20-30 minutes, the vast majority of participants (14 of 17) were satisfied with the models they created. 
% \msb{I collapsed the categories}

%Today, many of the most pressing challenges in artificial intelligence (AI), such as algorithmic bias and model failure under distribution shift~\cite{buolamwini2018genderShades, koenecke2020ASR, wilds2021}, are consequences of model development methods that do not sufficiently explore the solution space to arrive at robust and diverse solutions. 
%As with traditional sketching, much of the value of model sketching comes from the alternate cognitive frame that arises from shifting the focus and speed of iteration. 
We view model sketching as an important step that moves beyond the mode of retroactively fixing broken models and towards one of helping ML practitioners to become better model designers from the start.
% Contributions
To summarize, this paper makes the following contributions:
\begin{itemize}
    \item \textbf{Model sketching}. 
    % We introduce a concept-based technical framework that enables users to author sketch versions of machine learning models.
    \rev{We introduce a framework for authoring zero-shot concept building blocks that can be flexibly aggregated into composite models, allowing machine learning practitioners to rapidly iterate over concepts to sketch a model's decision-making logic.}
    \item \textbf{The ModelSketchBook tool}. 
    % We instantiate our framework of model sketching by aggregating zero-shot models that capture human-understandable concepts, and we release an open-source Python package that allows users to interactively author concepts and sketch models in a computational notebook.
    \rev{We instantiate our model sketching framework by introducing an open-source Python package that allows users to interactively author concepts and sketch models in computational notebooks.}
    \item \textbf{An evaluation of model sketching with ML practitioners}. We perform a field evaluation with 17 machine learning practitioners who use our tool to author models for a challenging hateful meme detection task. We find that ML practitioners are successfully able to scope out from technical implementation details to higher-level decision-making logic. This cognitive shift helps ML practitioners to more broadly explore the model design space and to quickly discover gaps in the dataset, labeling method, and problem formulation.
\end{itemize}

% Kittens

% \rev{
% In early-stage model development, we primarily need to sketch the \textit{model's decisionmaking strategy}, not the end outcomes of the model. 
% \msl{(in progress)}
% Existing tools have supported speed and minimal detail: work in interactive machine learning has improved model development speed by focusing on inputs and outputs and abstracting away the decisionmaking logic in between~\cite{wekinator, create_ml, teachable_machine}. 
% However, for problem formulation tasks, it's precisely that decisionmaking logic that we need to directly iterate on: how do we map from inputs to outputs? how do we turn examples into quantitative representations? what are the factors that our model should consider to make its decision? 
% Given that sketches are more about the means than the end, it matters \textit{what} we are sketching, not just that we are creating models rapidly and with reduced effort.

% What's missing is the minimal representation. 
% What's missing is \textit{what} we're representing in a minimal way. For problem formulation tasks, it's precisely the decisionmaking logic that we must directly iterate on: how do we map from inputs to outputs? how do we turn examples into quantitative representations? what are the factors that our model should consider to make its decision? While inputs and outputs may change, they change as a result of decisions about the decisionmaking logic. 
% }
% Building on interactive machine learning that rethought the speed and interactivity of ML development and interactive machine teaching that enhances the expressivity of model developers, 
% tend to fixate on individual prompt details rather than higher-level value tradeoffs in model design.
% are often black boxes with respect to the value tradeoffs encoded in the model.
% \msb{see if you agree with the GPT-3 critique I changed it to. basically arguing that you can't easily tell GPT-3 what to pay attention to with respect to, say, toxicity}.


==> sections/old_versions/2_related_work_temp_IML_IMT_drafts.tex <==
\rev{\subsection{Early-stage machine learning model design \msl{v3 (old)}}}
\rev{Work in interactive machine learning (IML) has long been interested in how we might engage humans in the machine learning development process.  In reaction to the slow and effortful process of building models, classic work in IML demonstrated that by enabling users to interactively train and refine ML models, 
users can more rapidly develop models and keep them aligned with their goals~\cite{fails_olsen_IML,amershi_powerToThePeople}.
In most IML systems, interactions take the form of labeled examples and demonstrations. For example, in CueFlik, users could author rules (nearest-neighbor classifiers for concepts like ``scenic'') by providing sets of positive and negative image examples~\cite{cueflik}, and in Wekinator, users can demonstrate pairs of input gestures and outputs to guide the system to learn a mapping between the two~\cite{wekinator}.

Building on IML, work on interactive machine teaching (IMT) emphasizes the metaphor of \textit{teaching} to focus on the human's role as a teacher rather than just a label-provider~\cite{ramos2020IMT, simard2017IMT}. Through this metaphor, IMT highlights new challenges like the need for richer teaching strategies beyond data labeling.
% and the need to support teachers who are domain experts, but not ML experts.
% Work in this vein has explored how people might express their knowledge to a model
A wizard-of-oz study along this vein explored how users might teach knowledge to a model, and this work found that users decomposed knowledge in terms of concepts, relationships between concepts, and rules that combine and apply these concepts~\cite{ng_IMTknowledgeDecomp}. However, without actually instantiating and evaluating their concepts, users struggled to form a mental model of how the ML model works, which made it especially difficult for them to know how to articulate subtle, abstract forms of knowledge. \msl{May trim down these first two paragraphs a bit.}

\begin{table*}[!tb]
  \centering
  \footnotesize
    \rev{
    \begin{tabular}{p{0.2\textwidth}p{0.07\textwidth} p{0.25\textwidth} p{0.25\textwidth} p{0.1\textwidth}}
    \toprule
    \textbf{Paradigm} & \textbf{Emphasis} & \textbf{Paradigm shift} & \textbf{Strategy to improve ML models} & \textbf{Descriptor}\\
    \midrule
    {Interactive Machine Learning} &
    {\textit{interactive}} &
    {ML models don't need to exist in a vacuum---through human \textit{interaction} and feedback}, we can achieve user alignment and rapid model authoring&
    {Better feedback loops}&
    {Quick}\\
    \midrule
    {Interactive Machine Teaching} &
    {\textit{teaching}} &
    {ML isn't just about learning---we need to focus on \textit{teaching}: \textit{who} is developing ML models and \textit{how} they're sharing their knowledge} &
    {Better teaching}&
    {Expressive}\\
    \midrule
    {Model Sketching} &
    {\textit{sketching}} &
    {ML models don't need to be high-fidelity---in fact, \textit{low-fidelity}, \textit{transient} models are better at helping us to explore the multiverse of model designs} &
    {Better design space exploration}&
    {Minimal detail, Quick, Expressive}\\
    \bottomrule
    \end{tabular}
    }
    \caption{
    \rev{A brief summary of key ideas put forward by Interactive Machine Learning and Interactive Machine Teaching, alongside that of Model Sketching. The three paradigms are complementary, but they each emphasize different perspectives and recommend different strategies.}
    }
    \label{table:related_work_comparison}
\end{table*}

Our work on model sketching shares many of the same motivations that underlie IML and IMT; with IML, we share an interest in enabling rapid iteration on ML models through human interaction, and with IMT, we share the goal of enriching users' abilities to share their knowledge with a model. However, IML and IMT would suggest \textit{different} solutions to the problem of early-stage machine learning model design. 
Interactive machine learning would likely recommend a \textit{faster} mode of model development to enable more feedback loops.
Meanwhile, interactive machine teaching would likely suggest a more \textit{expressive} model development method to faithfully capture the ideas in an expert's mind. While these are both reasonable approaches, our work posits that they are necessary but not sufficient to tackle early-phase model development challenges.

To illustrate where the existing paradigms start to fall short, let us take the example of prompt-based model authoring (or \textit{prompting}), which might seem like an ideal method to achieve both the speed and expressivity that IML and IMT would recommend. There are two key problems with prompting that limit its efficacy for early-stage model development. First, its \textit{internal decisionmaking logic} is not interpretable or iterable. While this internal logic may not matter in settings where the model builder is executing on a clear vision and primarily concerned with instantiating their model, this decisionmaking strategy is the core piece to that a user must iterate on when exploring the model design space. Second, the insights we gather from prompting do not lend themselves to \textit{transferable insights} for a future production-ready model. Unless we want our final model to be implemented with prompt-based models, our early prototyping will not meaningfully inform our full-scale model implementation. 

These two problems point to a missing piece when we enter the domain of early model development: the need for a \textit{minimal representation} that will allow us to explore the model design space and yield transferable insights that will persist beyond our initial prototypes. Our choice of \textit{sketching} as a metaphor emphasizes that models do not need to be high-fidelity, and that low-fidelity models that distill ideas to a minimal-detail representation can help us to tackle nebulous modeling tasks where we are not executing a vision, but exploring what that vision ought to be~(Table \ref{table:related_work_comparison}). Sketches are especially critical for early phases of model development when these questions are unanswered, and for subjective or ethically-challenging problem spaces where there may be multiple valid approaches to explore.

This shift in emphasis drives several critical design constraints that do not always apply to IML and IMT systems more broadly:
\subsubsection*{What representation?}
\msl{Reduce repetition from two paragraphs up:}
First, the primary purpose of a sketch is not to achieve an end, but to explore the means to that end. The end-product of the sketching process is insight on the \textit{strategy} that the sketch took. This means that we need to both understand and primarily focus our iteration on the decision-making strategy itself (the factors that the model is reasoning over). Second, since sketches are meant to be transient artifacts, we need the strategies we uncover to be \textit{transferable} to the production models we will eventually build. Both of these factors motivated our choice of concept-based models rather than opaque, black-box techniques.

\subsubsection*{How do we instantiate that representation?}
Sketches are meant to explore a broad design space of models. To the extent possible, we wanted users to be able to instantiate whichever concepts they imagine might be helpful for their modeling task, so we could not restrict our users to sets of predefined features or static dictionaries.
However, an added challenge of sketching is that there is a steep cost associated with diverting the user's attention to different tasks (e.g., switching to label examples, develop a feature pipeline, or train a new helper model). Each of these tasks costs the user additional time and effort, pulls them away from the sketching mindset, and puts them at risk of falling back into technical tunneling. In order to instantiate concepts, we could not afford to have the user switch over to example-based or demonstration-based approaches if they would pull the user out of their focused state. In the subjective and ethically-challenging domains we care about, concepts are complex and nuanced, so example-based approaches indeed require a substantial amount of user attention. Thus, we avoided example-based approaches for concept instantiation to streamline the user's attention to concept creation, iteration, and aggregation. Instead, we turned to zero-shot modeling approaches to instantiate concepts flexibly, but rapidly. 

\msl{TODO: add wrap-up sentences}
% \msl{TODO: add things related to how IML/IMT executes rather than explores, and IML/IMT tends to assume one form of knowledge rather than multiple}

% Early-stage concerns; Other tools and how they relate to sketching goals
\msl{If there's room, add back some of the previous version of the section (covering other existing tools and sketching ideas in ML)}
}

\rev{\subsection{Early-stage machine learning model design \msl{v2 (old)}}}
\rev{Work in interactive machine learning (IML) has long been interested in how we might engage humans in the machine learning development process.  In reaction to the slow and effortful process of building models, classic work in IML demonstrated that by enabling users to interactively train and refine ML models, 
users can more rapidly develop models and keep them aligned with their goals~\cite{fails_olsen_IML,amershi_powerToThePeople}.
In most IML systems, interactions take the form of labeled examples and demonstrations. For example, in CueFlik, users could author rules (nearest-neighbor classifiers for concepts like ``scenic'') by providing sets of positive and negative image examples~\cite{cueflik}, and in Wekinator, users can demonstrate pairs of input gestures and outputs to guide the system to learn a mapping between the two~\cite{wekinator}.

Building on IML, work on interactive machine teaching (IMT) emphasizes the metaphor of \textit{teaching} to focus on the human's role as a teacher rather than just a label-provider~\cite{ramos2020IMT, simard2017IMT}. Through this metaphor, IMT highlights new challenges like the need for richer teaching strategies beyond data labeling.
% and the need to support teachers who are domain experts, but not ML experts.
% Work in this vein has explored how people might express their knowledge to a model
A wizard-of-oz study along this vein explored how users might teach knowledge to a model, and this work found that users decomposed knowledge in terms of concepts, relationships between concepts, and rules that combine and apply these concepts~\cite{ng_IMTknowledgeDecomp}. However, without actually instantiating and evaluating their concepts, users struggled to form a mental model of how the ML model works, which made it especially difficult for them to know how to articulate subtle, abstract forms of knowledge.

Our work on model sketching shares many of the same motivations that underlie IML and IMT; with IML, we share an interest in enabling rapid iteration on ML models through human interaction, and with IMT, we share the goal of enriching users' abilities to share their knowledge with a model. However, our choice of \textit{sketching} as a metaphor emphasizes that models do not need to be high-fidelity, and that low-fidelity models that distill ideas to their \textit{minimal representation} can help us to tackle nebulous modeling tasks where we are not executing a vision, but exploring what that vision ought to be. Sketches are especially critical for early phases of model development when these questions are unanswered and for subjective or ethically-challenging problem spaces where there may be multiple valid approaches to explore and trade off.

\msl{Need to improve this paragraph}
This emphasis drives several critical design constraints that do not always apply to IML and IMT systems more broadly.
First, the primary purpose of a sketch is not to achieve an end, but to explore the means to that end. The end-product of the sketching process is insight on the \textit{strategy} that the sketch took. This means that we need to both understand and primarily focus our iteration on the decision-making strategy itself (the factors that the model is reasoning over). Second, since sketches are meant to be transient artifacts, we need the strategies we uncover to be \textit{transferable} to the production models we will eventually build. Both of these factors motivate our choice of concept-based models rather than opaque, black-box techniques. \msl{TODO: something explaining why we must instantiate concepts?}
Third, in sketching, there is a steep cost associated with diverting the user's attention to different tasks (e.g., switching to label examples, develop a feature pipeline, or train a new helper model). Each of these tasks costs the user additional time and effort, pulls them away from the sketching mindset, and puts them at risk of falling back into technical tunneling. Thus, in order to instantiate concepts, we can't afford to have the user switch over to example-based or demonstration-based approaches. We must streamline the user's attention to concept creation, iteration, and aggregation.
Fourth, sketches are meant to explore a broad design space of models. Thus, it is not reasonable to restrict our users to sets of pre-defined features and dictionaries. To the extent possible, we want users to be able to instantiate whatever concepts they imagine might be helpful for their modeling task.
\msl{TODO: add things related to how IML/IMT executes rather than explores, and IML/IMT tends to assume one form of knowledge rather than multiple}

% Early-stage concerns; Other tools and how they relate to sketching goals
\msl{Add back section covering existing tools and sketching ideas in ML}

% Scratch notes
% Why concepts? -> the end-product of a sketch is the insights on the decision-making approach
% We must both expose the internals of its decision-making strategy and allow users to \textit{iterate primarily on that strategy} in their different sketches.
% Since sketching is a temporary representation to learn about ML approaches for production models (exploration rather than execution), it requires us to primarily understand and iterate on the factors that the model is reasoning over. We need to iterate over the concepts, so we need to instantiate them interactively
% Why not example-based?
% In sketching, there is an even heightened cost of switching between representations and tasks. We can't afford to use example-based approaches to instantiate concepts
% Why not pre-defined?
% In sketching, we need to be able to explore a broad space. We don't want to be restricted to pre-defined features or dictionaries
}

\rev{
\subsection{Early-stage machine learning model design \msl{v1 (old)}}
Our work builds on the foundation set by interactive machine learning (IML) and interactive machine teaching (IMT), which established some of the key paradigms for how we might incorporate rich human insight into the model authoring process. 
Each of these bodies of work not only introduced new methods and techniques for reorienting the design of ML models around human expertise, but also introduced valuable metaphors to guide ML practitioners' approach to the modeling process.

% IML - emphasis on iteratively improving the system with human interaction
Interactive machine learning placed much of the ideological emphasis on the idea of \textit{interactivity}, which had been previously under-explored as a strategy to both improve ML models and achieve greater user alignment \msl{TODO: cite IML work like Crayons, CueFlik, Wekinator}. Given that ``machine learning'' had been the primary mode of operation prior to IML, the emphasis here was on ``interactive'': this work demonstrated that bringing humans directly into the loop through interactive processes could address many of the challenges in building machine learning models \msl{such as [...]}.

% IMT - emphasis on the expert who is teaching the system
Building on IML, interactive machine teaching provided a powerful new metaphor---one that focuses on the human expert who is \textit{teaching} the system. This change in metaphor was significant because in shifting attention to the role of the teacher, it highlighted new challenges such as the need for richer teaching strategies beyond data labeling and the need to support teachers who are domain experts, but not necessarily ML experts \msl{TODO: cite IMT work}.

% Model sketching - emphasis on the purpose of a model to aid problem formulation and design space exploration
With our model sketching work, we hope to provide another metaphor for approaching the task of machine learning. We use the metaphor of \textit{sketching} to shift attention to the \textit{purpose} of a model as a cognitive aid for approaching the challenging tasks of problem formulation and design space exploration. 
% \msl{potentially cut: Traditional pencil sketching was not a novel approach (its mechanics are largely the same as drawing, writing, or drafting); its value came from the particular opinionated \textit{approach} it took to drawing: one that focused on exploring, proposing, and riffing on ambiguous early ideas. However, any change in metaphor means a change in goals and thus a change in design requirements. While traditional sketching used many of the same tools as formal drawing and drafting, since its goal was to explore different ideas, it needed to be quick, so it intentionally took on conventions of low-fidelity with rough lines and minimal shading.}
While our approach necessarily builds on the foundation set by IML and IMT, it has different goals that imply different core \textit{representations}. 
Work in IML and IMT has used varied representations: most commonly example-based labels and demonstrations, but also spanning to richer features and concepts. However, with sketching, there is a steep cost associated with each diversion to a different task or representation. Any task that costs the user additional time, focus, or technical effort (e.g., switching to label examples, developing a feature pipeline, or training a new helper model) pulls the user away from the sketching mindset and puts them at risk of falling back into technical tunneling. 
% There is cost in switching to labeling examples or authoring a helper model: in time, attention/focus, and technical effort
% All of those factors pull someone away from a sketching mindset and risk them falling into technical tunneling

Thus, model sketching requires that we simplify to \textit{one} core representation that the user can specify, instantiate, and iterate on throughout. We chose to focus on the concept level because it strikes a balance between expressivity and modularity \msl{cite other good properties from prior work}. Previous work involving concept-based representations has relied on examples, predefined features, or user-defined features to train concept models \msl{[cite]}. However, given the strict design constraints of the sketching task, we unfortunately could not use these methods for concept instantiation. Our approach needed to both support novel concepts and avoid costly context-switching tasks like labeling or feature engineering---all within the tight time and data limits that sketching also imposes. We address this challenge with zero-shot models authored with natural language, allowing users to interactively instantiate concepts without breaking out of their sketching practice.
% we needed for users to be able to interactively instantiate novel concepts without context-switching to tasks like labeling or feature pipelining, a task that was previously not possible given the small amounts of data and time that sketching also requires.
% A key challenge prior to this work was that users could not interactively specify and instantiate novel concepts with small amounts of data and time. 
% This real-time concept instantiation is critical to avoid derailment (e.g., to labels, features, and helper models) and preserve the sketching interaction. 
% Thus, a major component of our work focuses on how we could support real-time concept instantiation without pulling the user away to distracting side-tasks.

% \msl{older version:}
% Given that sketching emphasizes distilling design ideas to their minimal form, model sketching requires a pared-down, but expressive design language. Thus, in contrast to the varied representations leveraged in IML and IMT---which typically tend towards example-based demonstration, but also span to richer features and concepts---model sketching requires us to simplify to one core expressive representation that we can specify, instantiate, and iterate upon. We chose to focus on concepts because they strike a balance between expressivity and modularity: concepts map well to human understanding of decision tasks and model behavior, but they are also modular enough to flexibly combine in remix in different ways. However, a key challenge prior to this work was that users could not interactively specify and instantiate novel concepts with small amounts of data and time. This real-time instantiation is critical because, in order to maintain a sketch-like interaction, user iteration needs to be solely focused on the concept level, without needing to derail to side-tasks like labeling examples for a new concept or creating a helper model from scratch.
}

==> sections/old_versions/2_related_work_v1.tex <==
\msl{TODO: Note that this section will probably be the roughest of this draft and hasn't undergone iteration. Feel free to devote less attention here; mostly wanted to lay out the main bodies of work that I want to cover! I need to bring this section more in resonance with the arguments in the rest of the paper}

We survey work from HCI on sketching, prototyping, and the work practices of ML practitioners, all of which motivates our model sketching approach.


% We survey work from HCI on sketching, prototyping, and the work practices of ML practitioners as well as work from the ML and algorithmic fairness communities on incorporating values in machine learning modeling, all of which motivates our model sketching approach.

% Potential sections:
% \begin{itemize}
%     \item Sketching/prototyping research (in design/HCI)
%     \item Interactive machine learning
%     \item Algorithmic fairness; ML ethics; incorporating values in ML
%     \item Data scientists' and ML practitioners' work practices
%     \item Large language models; prompting
% \end{itemize}

\subsection{Sketching and prototyping in design}
% Importance of sketching; what value it provides
The field of HCI has long upheld the practice of sketching as a valuable tool for thought. A sketch is similar to a prototype in that both are instantiations of a design concept, but a sketch serves a different purpose: to explore and raise questions about design approaches rather than to propose answers or solutions~\cite{buxton2010sketching}. Thus, sketches are suitable for the early ideation stages of a design process while prototypes are intended for the later stages. While the exact nature of a sketch (beyond its purpose) can be difficult to pin down, Buxton characterizes sketches as quick and plentiful with ambiguity and minimal detail.

Sketches are powerful tools because they allow a practitioner to quickly explore and test high-level ideas. While sketches may seem rudimentary, it is because they are so disposable and easy to generate that they allow for designers to more broadly explore a design space and prune unpromising design directions before they become ossified. In fact, overly detailed prototyping approaches detract from this valuable cognitive work~\cite{landay_interactiveSketching}. 
% More than just unlocking quick iteration, sketches are a valuable cognitive tool for practitioners themselves to understand their nascent designs before communicating about them with others.
Lower-fidelity prototyping enables practitioners to more readily create parallel prototypes that simultaneously explore design paths, an approach that combats harmful design fixation and leads to more diverse, higher-quality designs~\cite{dow_parallelPrototyping}. 

A key trait of a successful early-phase sketching or prototyping tool is that it refocuses cognitive processes, empowering the practitioner to engage in ``design thinking rather than implementation tinkering''~\cite{hartmann_dTools}.
Work on prototyping has highlighted that early artifacts can serve different purposes: to clarify the role of a technology, experiment with its implementation, or convey its look and feel~\cite{houde_whatDoPrototypesPrototype}. While we aim to primarily engage ML practitioners in high-level thinking during model sketching, we seek to provide a pathway from sketch models to full-scale models, just as prior work has enabled seamless transformations from rough interface design sketches to operational, look-and-feel interfaces~\cite{landay_interactiveSketching}. Thus, we situate our model sketches between a role and implementation prototype, as we seek to emulate the behavior of a full machine learning model in a real-world decision-making setting while roughly capturing its implementation via constituent concepts.

\subsection{The cognitive focus of ML practitioners}
% What we mean by ML practitioner; Typical workflow and challenges of data science workers; Current tools they use
\msl{Need to clarify the intent of this section} In our work, we use the terms ML practitioner and model developer interchangeably to refer to users who identify as performing work that primarily deals with authoring, designing, developing, and iterating on machine learning models. ML practitioners often occupy industry roles with the title of data scientist, research scientist, or AI developer \msl{TODO: clarify what roles we think fit}.  
% Cover main challenges that data science workers encounter. What they spend their time on. What tools they typically use.
Prior research has investigated how data scientists navigate tensions between the rational and subjective aspects of their work and have documented major challenges that they encounter in their work~\cite{passi_trustInDataScience, muller_HowDataScienceWorkersWorkWithData}. Some major challenges arise around how data scientists collaborate with various stakeholders across disciplines and organizations~\cite{zhang_howDoDataScienceWorkersCollaborate}.

% Hypothesis formalization; why it's bad that the focus is more on the technical
A current problem with the data science workflow is that much of the translational work that ML practitioners perform to bridge between high-level goals and low-level implementations (i.e., via feature extraction and feature engineering) is invisible~\cite{zhang_howDoDataScienceWorkersCollaborate}. Thus, current processes lose important knowledge about the nature and meaning of features and the assumptions and reasoning that underlie modeling decisions, which is especially problematic if ML practitioners need to revisit those decisions to counter harmful model behavior.
Similarly, in the domain of statistical model authoring, recent research has documented that model developers focus their attention on technical, implementation-oriented aspects of the modeling process rather than high-level conceptual hypotheses, and software tools exacerbate the problem~\cite{jun_hypothesisFormalization}. This research has directly called for high-level libraries to ``[express] conceptual hypotheses to bootstrap model implementations'' and bidirectional conceptual modeling to ``[co-author] conceptual models and model implementations''. Our work directly seeks to carry out this vision in the domain of ML model development by allowing ML practitioners to instantiate models using concept-based abstractions and to bridge between that abstraction level to a functional model implementation.

% TODO: cite Software Engineering for ML paper on nine-stage workflow for ML

\subsection{Sketching and machine learning}
While the value of sketching is broadly acknowledged in HCI and design, sketching is a relatively foreign concept in machine learning. Recent lines of research have called for a greater acknowledgement of ML as a design material and has explored the experiences of UX designers for ML products and services, especially noting the ways in which AI presents unique difficulties for designers~\cite{yang_investigatingHowExperiencedUXDesigners, yang_reexaminingWhetherWhy}. Research in this vein has explored how we might bring sketch-like practices into the design of ML-powered experiences to address these challenges~\cite{yang_sketchingNLP}. 
% Data iteration: Chameleon paper?

However, HCI researchers have not yet explored how we might further expand the reach of sketching practices to the design of machine learning models themselves in terms of their core structure, values, and decision-making logic.
Classic work on interactive machine learning (IML) has explored how we might enable users to author ML models in drastically different manner where the user could coach and refine their model in real time~\cite{fails_olsen_IML}. The focus of work in IML tends to be on speed and iteration of model development in service of rapid error correction, so IML techniques tend to abstract away features and delegate those sensemaking responsibilities to the algorithm~\MSLcite{ other IML work}. Thus, IML approaches are not quite like the sketches that we seek that would aid ML practitioners in thinking about and designing their model's decisionmaking policy.
% Recent work on LLMs and HCI; using prompts to author classifiers and perform other zero-shot tasks
% AI Chains work; comparison with their prototyping approach
Recent work has explored how we might leverage advances in Large Language Models (LLMs) to allow for rapid model authoring via flexible natural language prompts~\cite{wu_AI_chains, jiang_PromptMaker}
We are excited by this line of work because it unlocks a method for users to take a more active, hands-on role in model design while maintaining a lightweight interaction mode. In our work, we seek to take these LLM-based prototyping methods further in the direction of a sketching practice. We further pare down the design language of prompt-based model authoring to center design decisions around the abstraction of concepts, which helps practitioners to focus on the core high-level aspects of their model rather than getting bogged down with implementation tweaks and execution details.

% \subsection{Incorporating human values in machine learning}
% TODO: potentially add this section
% Related thread of work on how to better incorporate values into ML



==> sections/old_versions/2_related_work_v2.tex <==
\msl{TODO: Note that this section will probably be the roughest of this draft and hasn't undergone iteration. Feel free to devote less attention here; mostly wanted to lay out the main bodies of work that I want to cover! I need to bring this section more in resonance with the arguments in the rest of the paper}

We survey research on sketching, prototyping, and the work practices of machine learning practitioners, all of which motivates our model sketching approach.

\subsection{Sketching and prototyping in design}
% Importance of sketching; what value it provides
The fields of design and HCI have long upheld the practice of sketching as a valuable tool for thought~\cite{fallman_designOrientedHCI}. A sketch is similar to a prototype in that both are instantiations of a design concept, but a sketch serves a different purpose: to explore and raise questions about design approaches rather than to propose answers or solutions~\cite{buxton2010sketching}. Thus, sketches are suitable for the early ideation stages of a design process while prototypes are intended for the later stages. While the exact nature of a sketch (beyond its purpose) can be difficult to pin down, Buxton characterizes sketches as quick, plentiful, ambiguous, and minimal in detail~\cite{buxton2010sketching}.

Sketches are powerful tools because they allow a practitioner to quickly explore and test high-level ideas. While sketches may seem rudimentary, it is because they are so disposable and easy to generate that they allow for designers to more broadly explore a design space and prune unpromising design directions before they become ossified. In fact, overly detailed prototyping approaches detract from this valuable cognitive work~\cite{landay_interactiveSketching}. 
Lower-fidelity prototyping enables practitioners to more readily create parallel prototypes that simultaneously explore design paths, an approach that combats harmful design fixation and leads to more diverse, higher-quality designs~\cite{dow_parallelPrototyping}. 
% gould_lewis_designingForUsability

A key trait of a successful early-phase sketching or prototyping tool is that it refocuses cognitive processes, empowering the practitioner to engage in ``design thinking rather than implementation tinkering''~\cite{hartmann_dTools}.
Work on prototyping has highlighted that early artifacts can serve different purposes: to clarify the role of a technology, experiment with its implementation, or convey its look and feel~\cite{houde_whatDoPrototypesPrototype}. While we aim to primarily engage ML practitioners in high-level thinking during model sketching, we seek to provide a pathway from sketch models to full-scale models, just as prior work has enabled seamless transformations from rough interface design sketches to operational, look-and-feel interfaces~\cite{landay_interactiveSketching}. Thus, we situate our model sketches between a role and implementation prototype, as we seek to emulate the behavior of a full machine learning model in a real-world decision-making setting while roughly capturing its implementation via constituent concepts.

\subsection{The cognitive focus of ML practitioners}
% TODO: revised flow
% Who we consider ML practitioners
% The typical work practices of ML practitioners; where their focus lies (more on low-level than on high-level)
% The challenges that ML practitioners face re: algorithmic bias/fairness; problems with the status quo (decisionmaking is buried, not well documented; hard to revisit technical decisions made upstream, not enough iteration re: human values and problem formulation)

% What we mean by ML practitioner; Typical workflow and challenges of data science workers; Current tools they use
\msl{Need to clarify the intent of this section} In our work, we use the terms ML practitioner and model developer interchangeably to refer to users who identify as performing work that primarily deals with authoring, designing, developing, and iterating on machine learning models. ML practitioners often occupy industry roles with the title of data scientist, research scientist, or AI developer \msl{TODO: clarify what roles we think fit}.  
% Cover main challenges that data science workers encounter. What they spend their time on. What tools they typically use.
Prior research has investigated how data scientists navigate tensions between the rational and subjective aspects of their work and have documented major challenges that they encounter in their work~\cite{passi_trustInDataScience, muller_HowDataScienceWorkersWorkWithData}. Some major challenges arise around how data scientists collaborate with various stakeholders across disciplines and organizations~\cite{zhang_howDoDataScienceWorkersCollaborate}.

% Hypothesis formalization; why it's bad that the focus is more on the technical
A current problem with the data science workflow is that much of the translational work that ML practitioners perform to bridge between high-level goals and low-level implementations (i.e., via feature extraction and feature engineering) is invisible~\cite{zhang_howDoDataScienceWorkersCollaborate}. Thus, current processes lose important knowledge about the nature and meaning of features and the assumptions and reasoning that underlie modeling decisions, which is especially problematic if ML practitioners need to revisit those decisions to counter harmful model behavior.
Similarly, in the domain of statistical model authoring, recent research has documented that model developers focus their attention on technical, implementation-oriented aspects of the modeling process rather than high-level conceptual hypotheses, and software tools exacerbate the problem~\cite{jun_hypothesisFormalization}. This research has directly called for high-level libraries to ``[express] conceptual hypotheses to bootstrap model implementations'' and bidirectional conceptual modeling to ``[co-author] conceptual models and model implementations''. Our work directly seeks to carry out this vision in the domain of ML model development by allowing ML practitioners to instantiate models using concept-based abstractions and to bridge between that abstraction level to a functional model implementation.

% TODO: cite Software Engineering for ML paper on nine-stage workflow for ML

\subsection{Sketching and machine learning}
% TODO: revised flow
% Relative lack of sketching work in ML
% There is sketching for products/services that use ML, but not for the models themselves
% Discuss existing technologies and why they don't meet our sketch requirements
    % Blackbox models: slow, too detailed
    % Interactive ML: more about speed, not very expressive
    % No-code or low-code ML: fast, and minimal detail, but not expressive
    % LLM prompting: fast, expressive, but too much detail
% Lead from there to our approach to fill that gap


While the value of sketching is broadly acknowledged in HCI and design, sketching is a relatively foreign concept in machine learning. Recent lines of research have called for a greater acknowledgement of ML as a design material and has explored the experiences of UX designers for ML products and services, especially noting the ways in which AI presents unique difficulties for designers~\cite{yang_investigatingHowExperiencedUXDesigners, yang_reexaminingWhetherWhy}. Research in this vein has explored how we might bring sketch-like practices into the design of ML-powered experiences to address these challenges~\cite{yang_sketchingNLP}. 
% Data iteration: Chameleon paper?

However, HCI researchers have not yet explored how we might further expand the reach of sketching practices to the design of machine learning models themselves in terms of their core structure, values, and decision-making logic. \msb{Let's be careful here, I think lots of IML folks might view themselves as creating either metaphorical or literal sketching systems. I suggest being more precise, what's the gap?}
Classic work on interactive machine learning (IML) has explored how we might enable users to author ML models in drastically different manner where the user could coach and refine their model in real time~\cite{fails_olsen_IML}. The focus of work in IML tends to be on speed and iteration of model development in service of rapid error correction, so IML techniques tend to abstract away features and delegate those sensemaking responsibilities to the algorithm~\MSLcite{ other IML work}. Thus, IML approaches are not quite like the sketches that we seek that would aid ML practitioners in thinking about and designing their model's decisionmaking policy.
% Recent work on LLMs and HCI; using prompts to author classifiers and perform other zero-shot tasks
% AI Chains work; comparison with their prototyping approach
Recent work has explored how we might leverage advances in Large Language Models (LLMs) to allow for rapid model authoring via flexible natural language prompts~\cite{wu_AI_chains, jiang_PromptMaker}
We are excited by this line of work because it unlocks a method for users to take a more active, hands-on role in model design while maintaining a lightweight interaction mode. In our work, we seek to take these LLM-based prototyping methods further in the direction of a sketching practice. We further pare down the design language of prompt-based model authoring to center design decisions around the abstraction of concepts, which helps practitioners to focus on the core high-level aspects of their model rather than getting bogged down with implementation tweaks and execution details.

% \subsection{Incorporating human values in machine learning}
% TODO: potentially add this section
% Related thread of work on how to better incorporate values into ML



==> sections/old_versions/2_related_work_v3.tex <==
% v3 (post-MSB comments, revised flow incorporating writing previously in Design Goals section)

We survey research on sketching, prototyping, and the work practices of machine learning practitioners, all of which motivates our model sketching approach.

\subsection{Sketching and prototyping in design and HCI}
% Introduce sketching, benefits; importance for early-stage designs
% Highlight importance as tool for thinking; shifting to high-level
The fields of design and HCI have long upheld the practice of sketching as a valuable tool for thought~\cite{fallman_designOrientedHCI,buxton2010sketching}. A key trait of a successful sketching or prototyping tool is that it refocuses cognitive processes on high-level iteration, empowering the practitioner to engage in ``design thinking rather than implementation tinkering''~\cite{hartmann_dTools}. A sketch is similar to a prototype in that both are instantiations of a design concept, but a sketch serves a different purpose: to explore and raise questions about design approaches rather than to propose answers or solutions~\cite{buxton2010sketching}. Thus, sketches are suitable for the early ideation stages of a design process while prototypes are intended for the later stages. 

% Highlight expressivity, speed, minimal detail
\subsubsection*{What characterizes a sketch?}
\label{section:sketch_characteristics}
Buxton characterizes sketches as quick, plentiful, ambiguous, and minimal in detail~\cite{buxton2010sketching}. We look to these traits to guide the design of model sketching.
% Quick, plentiful
The \textit{quick} and \textit{plentiful} attributes go hand in hand: the speed with which sketches can be authored unlocks increased opportunities for iteration, which produces plentiful artifacts.
Prototyping methods with quick turnaround times enable practitioners to create parallel prototypes that simultaneously explore design paths, an approach that combats harmful design fixation and leads to more diverse, higher-quality designs~\cite{dow_parallelPrototyping, tohidi_buxton_gettingTheRightDesign}. 
Sketches are powerful tools because they allow a practitioner to quickly iterate to test dramatically different high-level ideas.
% While sketches may seem rudimentary, it is because they are so disposable and easy to generate that they allow for designers to more broadly explore a design space and prune unpromising design directions before they become ossified.

% Ambiguous, minimal detail
The \textit{ambiguous} and \textit{minimal detail} attributes are also closely tied: they hold that sketches should remain vague and not veer towards high-fidelity representations. This may seem counterintuitive, but %: it may seem like additional detail could only help to more clearly convey a design vision. However, 
much of the value of the sketch lies in both the cognitive task of distilling an idea into a stylized, minimal representation \cite{lim_anatomyOfPrototypes} and in leaving enough ambiguity to suggest---to oneself and others---multiple interpretations (and thus multiple future directions)~\cite{goel1995sketches}. Early work in user interface design demonstrated that overly-detailed prototyping approaches detract from this valuable cognitive work~\cite{landay_interactiveSketching} and do not substantially improve feedback quality~\cite{walker_hifiOrLofi}; in fact, simpler prototypes have been correlated with better design outcomes~\cite{yang_aStudyOfPrototypes}.

% Expressive
Finally, a sketch is \textit{expressive}. In order for a sketch to hold any value for a practitioner, it must provide enough flexibility and control to allow them to communicate their idea and iterate upon it~\cite{buxton2010sketching,landay_interactiveSketching}. Traditional freehand sketches are highly expressive because designers can draw upon concrete or abstract visual and textual representations to hone their idea, allowing others to perceive both perceptual features and functional relations~\cite{ suwa_tversky_whatArchitectsSeeInTheirSketches}. However, expressivity trades off against the prior attributes of speed and minimal detail and thus requires careful consideration of what abstractions or design vocabularies to provide to a practitioner \msb{I disagree with this---Scott McCloud's Understanding Comics conveys how comics can be very expressive even with minimal detail}.


\subsubsection*{Translating from sketches to implementation}
\msb{I suggest cutting this subsubsection---I don't think it really adds to the RW argument}
% Our intent to bridge between role and implementation prototype
While sketches and prototypes are valuable exercises in their own right to guide designers' thinking, their ultimate aim is to produce a better end-product, and the \textit{purpose} of a prototype defines how it will influence the design of a final product. Houde and Hill highlight three purposes: to clarify the role of a technology, experiment with its implementation, or convey its look and feel~\cite{houde_whatDoPrototypesPrototype}.
In our work, we seek to provide a pathway from sketch-like versions of models to full-scale models, just as prior work enabled seamless transformations from rough interface design sketches to operational look-and-feel interfaces~\cite{landay_interactiveSketching}. Thus, we situate model sketching between a role and implementation prototype, as we aim to emulate the behavior of a full machine learning model in a real-world decision-making setting while roughly capturing its implementation via constituent concepts, which could be turned into fully-built feature extractors and sub-models using more traditional ML methods.


\subsection{The cognitive focus of ML practitioners}
% Who we consider ML practitioners
In our work, we use the terms ML practitioner and model developer interchangeably to refer to users who identify as performing work that primarily deals with authoring, designing, developing, and iterating on machine learning models. ML practitioners often occupy industry roles with the title of Data Scientist, ML Engineer, or AI Developer. 

% The typical work practices of ML practitioners; where their focus lies (more on low-level than on high-level)
A major problem with the current data science workflow is that much of the translational work that ML practitioners perform to bridge between high-level goals and low-level implementations (i.e., via feature extraction and feature engineering) is rendered invisible~\cite{zhang_howDoDataScienceWorkersCollaborate}. ML practitioners frequently must navigate tensions between low-level ``rational'' and high-level ``subjective'' aspects of their work~\cite{passi_trustInDataScience, muller_HowDataScienceWorkersWorkWithData}, but current tools and processes hide this work. As a results, ML teams lose important knowledge about the nature and meaning of features and the assumptions and reasoning that underlie modeling decisions, which is especially problematic if ML practitioners need to revisit those decisions to counter harmful model behavior.
In the related domain of statistical model authoring, recent research has similarly documented that model developers focus their attention on technical, implementation-oriented aspects of the modeling process rather than high-level conceptual hypotheses, and software tools exacerbate the problem~\cite{jun_hypothesisFormalization}. In response to these issues, this research has explicitly called for high-level libraries to ``[express] conceptual hypotheses to bootstrap model implementations'' and bidirectional conceptual modeling to ``[co-author] conceptual models and model implementations''~\cite{jun_hypothesisFormalization}. Our work directly seeks to carry out this vision in the domain of ML model development by allowing ML practitioners to instantiate models using high-level concept-based abstractions and to bridge between this abstraction level to functional model implementations.


\subsection{Sketching and machine learning}
% Relative lack of sketching work in ML
While the value of sketching is broadly acknowledged in HCI and design, sketching is a relatively foreign concept in machine learning. Recent lines of research have called for a greater acknowledgement of ML as a design material and have explored the experiences of UX designers for ML products and services, especially noting the ways in which AI presents unique difficulties for designers~\cite{yang_investigatingHowExperiencedUXDesigners, yang_reexaminingWhetherWhy}. Research in this vein has explored how we might bring sketch-like practices into the design of ML-powered experiences to address these challenges~\cite{yang_sketchingNLP}. 

% There is sketching for products/services that use ML, but not for the models themselves
However, there is still much room to expand the reach of sketching practices to the design of machine learning models themselves---in terms of their core structure, values, and decision-making logic. 
% \msb{Let's be careful here, I think lots of IML folks might view themselves as creating either metaphorical or literal sketching systems. I suggest being more precise, what's the gap?}
Classic work on interactive machine learning (IML) has explored how we might enable users to author ML models in drastically different manner such that a user can coach and refine their model in real time~\cite{fails_olsen_IML}. This work in IML has made great strides on improving the speed and iteration of model development in service of rapid error correction~\msl{cite other IML work}. 
However, IML techniques are designed to act as end-to-end functional systems rather than disposable, minimal-detail prototypes. Additionally, in order to pare down interaction and prevent non-technical users from needing to engage with overly technical details, IML approaches usually abstract away decision-making logic and delegate those sensemaking responsibilities to an algorithm hidden under the hood. Thus, existing IML approaches are not the right fit for the sketches that we seek, which would aid ML practitioners in thinking about and designing their model's decision-making policy.

% Discuss existing technologies and why they don't meet our sketch requirements
    % Blackbox models: slow, too detailed
    % No-code or low-code ML: fast, and minimal detail, but not expressive
    % LLM prompting: fast, expressive, but too much detail
% Lead from there to our approach to fill that gap
\msb{this paragraph is important, but feels wordy}
Turning again to the characteristics of sketches outlined in Section~\ref{section:sketch_characteristics}, we find that existing ML technologies do not yet fully support a sketching practice~(\autoref{fig:design_space}).
% Blackbox models
State-of-the-art technologies tend to involve blackbox models that involve require a great deal of time, cost, and effort to implement. These models are extremely detailed in that they are implemented and tuned down to the last hyperparameter. While they may be theoretically expressive in their modeling capabilities, they are not very expressive from a human point of view: given that these models are not interpretable, ML practitioners cannot easily control or express different intents with these model designs.
% No-code or low-code ML
No-code or low-code ML approaches typically take a supervised learning approach that accepts labeled data examples as the primary control lever~\cite{scikit_learn} ~\msl{cite other tools}. These approaches are quick and minimal in detail since they purely focus the user on the data layer of abstraction, but this same design choice unfortunately limits expressivity since data is an indirect means of communicating intent for a decision-making policy and requires the user to curate intermediary data examples to convey their ideas.
% LLM prompting
Recent work has explored how we might leverage advances in Large Language Models (LLMs) to allow for rapid model authoring via flexible natural language prompts~\cite{wu_AI_chains, jiang_PromptMaker}.
\msb{if you like what I said in the intro about GPT-3, import that here too}
We are excited by this line of work because it unlocks a method for users to take a more active, hands-on role in model design while maintaining a lightweight interaction mode. In our work, we seek to take these LLM-based prototyping methods further in the direction of a sketching practice. We further pare down the design language of prompt-based model authoring to center design decisions around the abstraction of concepts, which helps practitioners to focus on the core high-level aspects of their model rather than getting bogged down with details of individual prompts.

\begin{figure}[!tb]
  \includegraphics[width=0.5\textwidth]{figures/design_space_v1.pdf}
  \caption{A summary of our design space. To accomplish an effective sketching practice, we seek to achieve expressivity, minimal detail, and speed, a combination that current tools lack.}
  \label{fig:design_space}
\end{figure}

% Concepts as a promising direction for model sketching
Concept-based abstractions in particular hold promise for sketch-like approaches to machine learning model authoring.
Prior work on concept evolution in data labeling demonstrated that many decision-making goals are malleable and subjective, but these goals can be clarified through an iterative process of concept elicitation and refinement~\cite{kulesza_conceptEvolution, chang_revolt}. Researchers have even found that for real-life decision-makers such as judges, doctors, and managers, simple, statistically-derived rules based on a small number of human-interpretable features substantially outperform human experts~\cite{jung_goel_simpleRulesExpertClassification}. Concepts map well to the way that humans reason over decision-making tasks, and methods that statistically aggregate concepts work surprisingly well, even beyond prototyping contexts.


==> sections/old_versions/2_related_work_v4.tex <==
% v4 9/15/22

We survey research on sketching and prototyping in design and HCI, the work practices of machine learning practitioners, and current approaches for early-stage model design, all of which motivate our model sketching approach.

\subsection{Sketching and prototyping in design and HCI}
% Introduce sketching, benefits; importance for early-stage designs
% Highlight importance as tool for thinking; shifting to high-level
The fields of design and HCI have long upheld the practice of sketching as a valuable tool for thought~\cite{fallman_designOrientedHCI,buxton2010sketching}. A key trait of a successful sketching or prototyping tool is that it refocuses cognitive processes on high-level iteration, empowering the practitioner to engage in ``design thinking rather than implementation tinkering''~\cite{hartmann_dTools}. A sketch is similar to a prototype in that both are instantiations of a design concept, but a sketch serves a different purpose: to explore and raise questions about design approaches rather than to propose answers or solutions~\cite{buxton2010sketching}. Thus, sketches are suitable for the early ideation stages of a design process while prototypes are intended for the later stages. 

% Highlight expressivity, speed, minimal detail
\subsubsection*{What characterizes a sketch?}
\label{section:sketch_characteristics}
Buxton characterizes sketches as quick, plentiful, ambiguous, and minimal in detail~\cite{buxton2010sketching}. %We look to these traits to guide the design of a novel sketching approach for modeling.
% Quick, plentiful
The \textit{quick} and \textit{plentiful} attributes go hand in hand: % the speed with which sketches can be authored unlocks increased opportunities for iteration, which produces plentiful artifacts.
methods with quick turnaround times enable practitioners to explore parallel design paths, an approach that supports more iterations, combats harmful design fixation and leads to more diverse, higher-quality designs~\cite{dow_parallelPrototyping, tohidi_buxton_gettingTheRightDesign}. 
Sketches are powerful tools because they allow a practitioner to quickly iterate to test dramatically different high-level ideas.
% While sketches may seem rudimentary, it is because they are so disposable and easy to generate that they allow for designers to more broadly explore a design space and prune unpromising design directions before they become ossified.

% Ambiguous, minimal detail
The \textit{ambiguous} and \textit{minimal detail} attributes are also closely tied: %they hold that sketches should remain vague and not veer towards high-fidelity representations. This may seem counterintuitive, but %: it may seem like additional detail could only help to more clearly convey a design vision. However, 
much of the value of the sketch lies in both the cognitive task of distilling an idea into a stylized, minimal representation \cite{lim_anatomyOfPrototypes} and in leaving enough ambiguity to suggest---to oneself and others---multiple interpretations (and thus multiple future directions)~\cite{goel1995sketches}. Early work in user interface design demonstrated that overly-detailed prototyping approaches detract from this valuable cognitive work~\cite{landay_interactiveSketching} and do not substantially improve feedback quality~\cite{walker_hifiOrLofi}; in fact, simpler prototypes have been correlated with better design outcomes~\cite{yang_aStudyOfPrototypes}.

% Expressive
Finally, a sketch is \textit{expressive}: %. In order for a sketch to hold any value for a practitioner, 
it must provide enough flexibility and control to allow a practitioner to communicate their idea and iterate upon it~\cite{buxton2010sketching,landay_interactiveSketching}. Traditional freehand sketches are highly expressive because designers can draw upon concrete or abstract visual and textual representations to hone their idea, allowing others to perceive both perceptual features and functional relations~\cite{ suwa_tversky_whatArchitectsSeeInTheirSketches}.
% However, expressivity trades off against the prior attributes of speed and minimal detail and thus requires careful consideration of what abstractions or design vocabularies to provide to a practitioner \msb{I disagree with this---Scott McCloud's Understanding Comics conveys how comics can be very expressive even with minimal detail}.

% Concepts as a promising direction for model sketching
Concept-based abstractions in particular hold promise for sketch-like approaches to machine learning model authoring.
Prior work on concept evolution in data labeling demonstrated that many decision-making goals are malleable and subjective, but these goals can be clarified through an iterative process of concept elicitation and refinement~\cite{kulesza_conceptEvolution, chang_revolt}. Researchers have even found that for real-life decision-makers such as judges, doctors, and managers, simple, statistically-derived rules based on a small number of human-interpretable features substantially outperform human experts~\cite{jung_goel_simpleRulesExpertClassification}. Concepts map well to the way that humans reason over decision-making tasks, and methods that statistically aggregate concepts work surprisingly well, even beyond prototyping contexts.

% \subsubsection*{Translating from sketches to implementation}
% \msb{I suggest cutting this subsubsection---I don't think it really adds to the RW argument}
% % Our intent to bridge between role and implementation prototype
% While sketches and prototypes are valuable exercises in their own right to guide designers' thinking, their ultimate aim is to produce a better end-product, and the \textit{purpose} of a prototype defines how it will influence the design of a final product. Houde and Hill highlight three purposes: to clarify the role of a technology, experiment with its implementation, or convey its look and feel~\cite{houde_whatDoPrototypesPrototype}.
% In our work, we seek to provide a pathway from sketch-like versions of models to full-scale models, just as prior work enabled seamless transformations from rough interface design sketches to operational look-and-feel interfaces~\cite{landay_interactiveSketching}. Thus, we situate model sketching between a role and implementation prototype, as we aim to emulate the behavior of a full machine learning model in a real-world decision-making setting while roughly capturing its implementation via constituent concepts, which could be turned into fully-built feature extractors and sub-models using more traditional ML methods.
% We argue these characteristics of sketching and prototyping could inspire new practices for early-state ML model design.

\subsection{ML practitioners: work practices and cognitive focus}
% Who we consider ML practitioners
In our work, we use the terms ML practitioner and model developer interchangeably to refer to users who perform work that primarily deals with authoring, designing, developing, and iterating on machine learning models%. 
%ML practitioners often occupy industry roles with the title of Data Scientist, Data Engineer, ML Engineer, or AI Developer
~\cite{muller_HowDataScienceWorkersWorkWithData,zhang_howDoDataScienceWorkersCollaborate}. 
% The typical work practices of ML practitioners; where their focus lies (more on low-level than on high-level)
Recent literature frames the data science and ML project workflow as a multi-stage collaborative lifecycle~\cite{wang2019human,piorkowski_AIDevelopersCommChallenges}.
Along this lifecycle, some business users or domain experts focus on the high-level problem definition and result interpretation, while the ML practitioners place their cognitive focus on the low-level implementation details~\cite{zhang_howDoDataScienceWorkersCollaborate,piorkowski_AIDevelopersCommChallenges}.
However, a major problem with the current workflow is that much of the translational work that ML practitioners perform to bridge between high-level goals and low-level implementations (i.e., via feature extraction and feature engineering) is rendered invisible~\cite{zhang_howDoDataScienceWorkersCollaborate}. 
ML practitioners frequently must navigate tensions between low-level ``rational'' and high-level ``subjective'' aspects of their work~\cite{mao2019data,passi_trustInDataScience, muller_HowDataScienceWorkersWorkWithData}, but current tools and processes often neglect this effort. 
As a result, ML teams lose important knowledge about the nature and meaning of features and the assumptions and reasoning that underlie modeling decisions~\cite{mao2019data,hou2017hacking}, which is especially problematic if ML practitioners need to revisit those decisions to counter harmful model behavior.
%In the related domain of statistical model authoring, recent research has similarly documented that model developers focus their attention on technical, implementation-oriented aspects of the modeling process rather than high-level conceptual hypotheses, and software tools exacerbate the problem
Similar patterns play out in statistical model authoring, which has prompted calls for high-level libraries to ``[express] conceptual hypotheses to bootstrap model implementations'' and bidirectional conceptual modeling to ``[co-author] conceptual models and model implementations''~\cite{jun_hypothesisFormalization}. 
Our work directly seeks to carry out this vision in the domain of ML model development by allowing ML practitioners to instantiate models using high-level concept-based abstractions and to bridge between this abstraction level to functional model implementations.


% \subsection{Sketching and machine learning}
\subsection{Early-stage machine learning model design}
% Relative lack of sketching work in ML
%While the value of sketching is broadly acknowledged in HCI and design, 
Sketching is a relatively foreign concept in machine learning. 
Recent lines of research have called for a greater acknowledgement of ML as a design material and have explored the experiences of UX designers for ML products and services, especially noting the ways in which AI presents unique difficulties for designers~\cite{yang_investigatingHowExperiencedUXDesigners, yang_reexaminingWhetherWhy}.
Research in this vein has explored how we might bring sketch-like practices into the design of ML-powered experiences to address these challenges~\cite{yang_sketchingNLP}. 

% There is sketching for products/services that use ML, but not for the models themselves
%However, there is still much room to expand the reach of sketching practices to the design of machine learning models themselves---in terms of their core structure, values, and decision-making logic. 
Classic work on interactive machine learning (IML) explored how we might enable users to author and refine ML models through demonstration and in real time~\cite{fails_olsen_IML}. This work in IML has made great strides on improving the speed and iteration of model development in service of rapid error correction~\cite{wang2021autods}. 
However, IML techniques are designed to act as end-to-end functional systems %, not disposable, minimal-detail prototypes. Additionally, in order to pare down interaction and prevent non-technical users from needing to engage with overly technical details, IML approaches usually 
and abstract away decision-making logic, delegating those sensemaking responsibilities to an algorithm hidden under the hood. 
Thus, existing IML approaches are not the right fit for the sketches that we seek, which would aid ML practitioners in thinking about and designing their model's decision-making policy.

% Discuss existing technologies and why they don't meet our sketch requirements
    % Blackbox models: slow, too detailed
    % No-code or low-code ML: fast, and minimal detail, but not expressive
    % LLM prompting: fast, expressive, but too much detail
% Lead from there to our approach to fill that gap
% \msb{this paragraph is important, but feels wordy}
Turning again to the characteristics of sketches outlined in Section~\ref{section:sketch_characteristics}, existing ML technologies do not yet fully support a sketching practice~(\autoref{fig:design_space}).
% Blackbox models
State-of-the-art technologies tend to involve blackbox models that require a great deal of time, cost, and effort to implement. 
% These models are extremely detailed in that they are implemented and tuned down to the last hyperparameter. 
While they may be theoretically expressive in their modeling capabilities, they are not very expressive from a human point of view: given that these models are not interpretable, ML practitioners cannot easily control or express different intents with these model designs.
% No-code or low-code ML
No-code or low-code ML approaches typically take a supervised learning approach that accepts labeled data examples as the primary control lever~\cite{scikit_learn,create_ml,teachable_machine}. 
These approaches are quick and minimal in detail since they purely focus the user on the data layer of abstraction, but this same design choice unfortunately limits expressivity since data is an indirect means of communicating intent for a decision-making policy and requires the user to curate intermediary data examples to convey their ideas.
% LLM prompting
Recent work has suggested that advances in Large Language Models (LLMs) may be used to support rapid model authoring via flexible natural language prompts~\cite{wu_AI_chains, jiang_PromptMaker}.
% \msb{if you like what I said in the intro about GPT-3, import that here too}
% We are excited by this line of work because it unlocks a method for users to take a more active, hands-on role in model design while maintaining a lightweight interaction mode. In our work, we seek to take these LLM-based prototyping methods further in the direction of a sketching practice. 
We further pare down the design language of prompt-based model authoring to center design decisions around the abstraction of concepts, which helps practitioners to focus on the core high-level value tradeoffs of their model rather than getting bogged down with details of individual prompts.

\begin{figure}[!tb]
  \includegraphics[width=0.5\textwidth]{figures/design_space_v1.pdf}
  \caption{A summary of our design space. To accomplish an effective sketching practice, we seek to achieve expressivity, minimal detail, and speed, a combination that current tools lack.}
  \label{fig:design_space}
\end{figure}




==> sections/old_versions/2_related_work_v5.tex <==
% v5 11/26/22

We survey research on sketching and prototyping in design and HCI, the work practices of machine learning practitioners, and current approaches for early-stage model design, all of which motivate our model sketching approach.

\subsection{Sketching and prototyping in design and HCI}
% Introduce sketching, benefits; importance for early-stage designs
% Highlight importance as tool for thinking; shifting to high-level
The fields of design and HCI have long upheld the practice of sketching as a valuable tool for thought~\cite{fallman_designOrientedHCI,buxton2010sketching}. A key trait of a successful sketching or prototyping tool is that it refocuses cognitive processes on high-level iteration, empowering the practitioner to engage in ``design thinking rather than implementation tinkering''~\cite{hartmann_dTools}. A sketch is similar to a prototype in that both are instantiations of a design concept, but a sketch serves a different purpose: to explore and raise questions about design approaches rather than to propose answers or solutions~\cite{buxton2010sketching}. Thus, sketches are suitable for the early ideation stages of a design process while prototypes are intended for the later stages. 

% Highlight expressivity, speed, minimal detail
\subsubsection*{What characterizes a sketch?}
\label{section:sketch_characteristics}
Buxton characterizes sketches as quick, plentiful, ambiguous, and minimal in detail~\cite{buxton2010sketching}. %We look to these traits to guide the design of a novel sketching approach for modeling.
% Quick, plentiful
The \textit{quick} and \textit{plentiful} attributes go hand in hand: % the speed with which sketches can be authored unlocks increased opportunities for iteration, which produces plentiful artifacts.
methods with quick turnaround times enable practitioners to explore parallel design paths, an approach that supports more iterations, combats harmful design fixation, and leads to more diverse, higher-quality designs~\cite{dow_parallelPrototyping, tohidi_buxton_gettingTheRightDesign}. 
Sketches are powerful tools because they allow a practitioner to quickly iterate to test dramatically different high-level ideas.
% While sketches may seem rudimentary, it is because they are so disposable and easy to generate that they allow for designers to more broadly explore a design space and prune unpromising design directions before they become ossified.

% Ambiguous, minimal detail
The \textit{ambiguous} and \textit{minimal detail} attributes are also closely tied: %they hold that sketches should remain vague and not veer towards high-fidelity representations. This may seem counterintuitive, but %: it may seem like additional detail could only help to more clearly convey a design vision. However, 
much of the value of a sketch lies in both the cognitive task of distilling an idea into a stylized, minimal representation \cite{lim_anatomyOfPrototypes} and in leaving enough ambiguity to suggest---to oneself and others---multiple interpretations (and thus multiple future directions)~\cite{goel1995sketches}. Early work in user interface design demonstrated that overly-detailed prototyping approaches detract from this valuable cognitive work~\cite{landay_interactiveSketching} and do not substantially improve feedback quality~\cite{walker_hifiOrLofi}; in fact, simpler prototypes have been correlated with better design outcomes~\cite{yang_aStudyOfPrototypes}.

% Expressive
Finally, a sketch is \textit{expressive}: %. In order for a sketch to hold any value for a practitioner, 
it must provide enough flexibility and control to allow a practitioner to communicate their idea and iterate upon it~\cite{buxton2010sketching,landay_interactiveSketching}. Traditional freehand sketches are highly expressive because designers can draw upon concrete or abstract visual and textual representations to hone their idea, allowing others to perceive both perceptual features and functional relations~\cite{ suwa_tversky_whatArchitectsSeeInTheirSketches}.
% However, expressivity trades off against the prior attributes of speed and minimal detail and thus requires careful consideration of what abstractions or design vocabularies to provide to a practitioner \msb{I disagree with this---Scott McCloud's Understanding Comics conveys how comics can be very expressive even with minimal detail}.

% Concepts as a promising direction for model sketching
Concept-based abstractions in particular hold promise for sketch-like approaches to machine learning model authoring.
Prior work on concept evolution in data labeling demonstrated that many decision-making goals are malleable and subjective, but these goals can be clarified through an iterative process of concept elicitation and refinement~\cite{kulesza_conceptEvolution, chang_revolt}. Researchers have even found that for real-life decision-makers such as judges, doctors, and managers, simple, statistically-derived rules based on a small number of human-interpretable features substantially outperform human experts~\cite{jung_goel_simpleRulesExpertClassification}. Concepts map well to the way that humans reason over decision-making tasks, and methods that statistically aggregate concepts work surprisingly well, even beyond prototyping contexts.

% \subsubsection*{Translating from sketches to implementation}
% \msb{I suggest cutting this subsubsection---I don't think it really adds to the RW argument}
% % Our intent to bridge between role and implementation prototype
% While sketches and prototypes are valuable exercises in their own right to guide designers' thinking, their ultimate aim is to produce a better end-product, and the \textit{purpose} of a prototype defines how it will influence the design of a final product. Houde and Hill highlight three purposes: to clarify the role of a technology, experiment with its implementation, or convey its look and feel~\cite{houde_whatDoPrototypesPrototype}.
% In our work, we seek to provide a pathway from sketch-like versions of models to full-scale models, just as prior work enabled seamless transformations from rough interface design sketches to operational look-and-feel interfaces~\cite{landay_interactiveSketching}. Thus, we situate model sketching between a role and implementation prototype, as we aim to emulate the behavior of a full machine learning model in a real-world decision-making setting while roughly capturing its implementation via constituent concepts, which could be turned into fully-built feature extractors and sub-models using more traditional ML methods.
% We argue these characteristics of sketching and prototyping could inspire new practices for early-state ML model design.

\subsection{ML practitioners: work practices and cognitive focus}
% Who we consider ML practitioners
In our work, we use the terms ML practitioner and model developer interchangeably to refer to users who perform work that primarily deals with authoring, designing, developing, and iterating on machine learning models%. 
%ML practitioners often occupy industry roles with the title of Data Scientist, Data Engineer, ML Engineer, or AI Developer
~\cite{muller_HowDataScienceWorkersWorkWithData,zhang_howDoDataScienceWorkersCollaborate}. 
% The typical work practices of ML practitioners; where their focus lies (more on low-level than on high-level)
Recent literature frames the data science and ML project workflow as a multi-stage collaborative lifecycle~\cite{wang2019human,piorkowski_AIDevelopersCommChallenges}.
Along this lifecycle, some business users or domain experts focus on the high-level problem definition and result interpretation, while the ML practitioners place their cognitive focus on the low-level implementation details~\cite{zhang_howDoDataScienceWorkersCollaborate,piorkowski_AIDevelopersCommChallenges}.
However, a major problem with the current workflow is that much of the translational work that ML practitioners perform to bridge between high-level goals and low-level implementations (i.e., via feature extraction and feature engineering) is rendered invisible~\cite{zhang_howDoDataScienceWorkersCollaborate}. 
ML practitioners frequently must navigate tensions between low-level ``rational'' and high-level ``subjective'' aspects of their work~\cite{mao2019data,passi_trustInDataScience, muller_HowDataScienceWorkersWorkWithData}, but current tools and processes often neglect this effort. 
As a result, ML teams lose important knowledge about the nature and meaning of features and the assumptions and reasoning that underlie modeling decisions~\cite{mao2019data,hou2017hacking}, which is especially problematic if ML practitioners need to revisit those decisions to counter harmful model behavior.
%In the related domain of statistical model authoring, recent research has similarly documented that model developers focus their attention on technical, implementation-oriented aspects of the modeling process rather than high-level conceptual hypotheses, and software tools exacerbate the problem
Similar patterns play out in statistical model authoring, which has prompted calls for high-level libraries to ``[express] conceptual hypotheses to bootstrap model implementations'' and bidirectional conceptual modeling to ``[co-author] conceptual models and model implementations''~\cite{jun_hypothesisFormalization}. 
Our work directly seeks to carry out this vision in the domain of ML model development by allowing ML practitioners to instantiate models using high-level concept-based abstractions and to bridge between this abstraction level to functional model implementations.

\rev{\subsection{Early-stage machine learning model design \msl{v4 (in progress)}}}
\rev{Work in interactive machine learning (IML) has long been interested in how we might engage humans in the machine learning development process.  In reaction to the slow and effortful process of building models, classic work in IML demonstrated that by enabling users to interactively train and refine ML models, 
users can more rapidly develop models and keep them aligned with their goals~\cite{fails_olsen_IML,amershi_powerToThePeople}.
In most IML systems, interactions take the form of labeled examples and demonstrations. For example, in CueFlik, users could author rules (nearest-neighbor classifiers for concepts like ``scenic'') by providing sets of positive and negative image examples~\cite{cueflik}, and in Wekinator, users can demonstrate pairs of input gestures and outputs to guide the system to learn a mapping between the two~\cite{wekinator}.

Building on IML, work on interactive machine teaching (IMT) emphasizes the metaphor of \textit{teaching} to focus on the human's role as a teacher rather than just a label-provider~\cite{ramos2020IMT, simard2017IMT}. Through this metaphor, IMT highlights new challenges like the need for richer teaching strategies beyond data labeling.
% and the need to support teachers who are domain experts, but not ML experts.
% Work in this vein has explored how people might express their knowledge to a model
A wizard-of-oz study along this vein explored how users might teach knowledge to a model, and this work found that users decomposed knowledge in terms of concepts, relationships between concepts, and rules that combine and apply these concepts~\cite{ng_IMTknowledgeDecomp}. However, without actually instantiating and evaluating their concepts, users struggled to form a mental model of how the ML model works, which made it especially difficult for them to know how to articulate subtle, abstract forms of knowledge. 
% \msl{May trim down these first two paragraphs a bit.}

\begin{table*}[!tb]
  \centering
  \footnotesize
    \rev{
    \begin{tabular}{p{0.2\textwidth}p{0.07\textwidth} p{0.25\textwidth} p{0.25\textwidth} p{0.1\textwidth}}
    \toprule
    \textbf{Paradigm} & \textbf{Emphasis} & \textbf{Paradigm shift} & \textbf{Strategy to improve ML models} & \textbf{Design reqs}\\
    \midrule
    {Interactive Machine Learning} &
    {\textit{interactive}} &
    {ML models don't need to exist in a vacuum---through human \textit{interaction} and feedback}, we can achieve user alignment and rapid model authoring&
    {Better feedback loops}&
    {Speed}\\
    \midrule
    {Interactive Machine Teaching} &
    {\textit{teaching}} &
    {ML isn't just about learning---we need to focus on \textit{teaching}: \textit{who} is developing ML models and \textit{how} they're sharing their knowledge} &
    {Better teaching}&
    {Expressivity}\\
    \midrule
    {Model Sketching} &
    {\textit{sketching}} &
    {ML models don't need to be high-fidelity---in fact, \textit{low-fidelity}, \textit{transient} models are better at helping us to explore the multiverse of model designs} &
    {Better design space exploration}&
    {Minimal detail, Speed, Expressivity}\\
    \bottomrule
    \end{tabular}
    }
    \caption{
    \rev{A summary of key ideas put forward by Interactive Machine Learning and Interactive Machine Teaching, alongside those of Model Sketching. The three paradigms are complementary, but they each emphasize different perspectives and strategies.}
    }
    \label{table:related_work_comparison}
\end{table*}

Model sketching shares many of the same motivations that underlie IML and IMT; with IML, we share an interest in enabling rapid iteration on ML models through human interaction, and with IMT, we share the goal of enriching users' abilities to share their knowledge with a model. 
However, model sketching has slightly different goals than IML and IMT---to explore a vague, unformulated model design space rather than execute on a crisp modeling vision. 
Given this goal of problem formulation as opposed to task execution, we have additional design constraints in the model sketching domain. 
In addition to the speed and expressivity required by IML and IMT, sketching requires a \textit{minimal representation}. As demonstrated by the practice of sketching in design, sketches must be streamlined, distilled representations in order to facilitate effective design space exploration. 
% What then is the right minimal representation for early-phase model development? 
Model sketching posits that in order to tackle problem formulation, we need \textit{minimal representations of a model's decision-making logic}.
In other words, to support model sketching, we need to provide a mechanism for the user to directly iterate on the decision-making primitives that control how the model ought to act.

% However, IML and IMT would suggest \textit{different} solutions to the problem of early-stage machine learning model design. Interactive machine learning would likely recommend a \textit{faster} mode of model development to enable more feedback loops. Meanwhile, interactive machine teaching would likely suggest a more \textit{expressive} model development method to faithfully capture the ideas in an expert's mind. While these are both reasonable approaches, our work posits that they are necessary but not sufficient to tackle early-phase model development challenges.

% To illustrate where the existing paradigms start to fall short, let us take the example of prompt-based model authoring (or \textit{prompting}), which might seem like an ideal method to achieve both the speed and expressivity that IML and IMT would recommend. There are two key problems with prompting that limit its efficacy for early-stage model development. First, its \textit{internal decisionmaking logic} is not interpretable or iterable. While this internal logic may not matter in settings where the model builder is executing on a clear vision and primarily concerned with instantiating their model, this decisionmaking strategy is the core piece to that a user must iterate on when exploring the model design space. Second, the insights we gather from prompting do not lend themselves to \textit{transferable insights} for a future production-ready model. Unless we want our final model to be implemented with prompt-based models, our early prototyping will not meaningfully inform our full-scale model implementation. 

% These two problems point to a missing piece when we enter the domain of early model development: the need for a \textit{minimal representation} that will allow us to explore the model design space and yield transferable insights that will persist beyond our initial prototypes. Our choice of \textit{sketching} as a metaphor emphasizes that models do not need to be high-fidelity, and that low-fidelity models that distill ideas to a minimal-detail representation can help us to tackle nebulous modeling tasks where we are not executing a vision, but exploring what that vision ought to be~(Table \ref{table:related_work_comparison}). Sketches are especially critical for early phases of model development when these questions are unanswered, and for subjective or ethically-challenging problem spaces where there may be multiple valid approaches to explore.

What should a minimal representation look like? Given that our goal is to represent the model's decision-making logic, we cannot use existing techniques that are black-box and opaque, including prompt-based model authoring. Additionally, since sketches are meant to be transient artifacts, we need the strategies we uncover to be \textit{transferable} to the production models we will eventually build. Thus, concepts are an ideal representation that allows for iteration on decision-making strategy, transferability to production models, and alignment with the ways that humans prefer to decompose and express their knowledge~\cite{ng_IMTknowledgeDecomp}. 

Finally, how should we instantiate this concept-based representation? Past work in IML and IMT has explored concept instantiation with examples, demonstrations, predefined features, and formal knowledge bases \msl{TODO: cite}. Given that sketches are meant to explore a broad design space of models, users must have the flexibility to author arbitrary concepts, so we could not rely on predefined features or static knowledge bases. Furthermore, an added challenge of sketching is that there is a steep cost associated with diverting the user's attention to different tasks (e.g., switching to label examples, develop a feature pipeline, or train a new helper model), which risk pulling the user out of the sketching mindset and into technical tunneling. In order to instantiate concepts, we could not afford to have the user switch over to example-based or demonstration-based approaches if they would pull the user out of their focused state. Thus, we turned to zero-shot modeling approaches to instantiate concepts flexibly and rapidly without diverting attention.
}

\subsection{Early-stage machine learning model design \msl{old version from orig submission}}
% Relative lack of sketching work in ML
%While the value of sketching is broadly acknowledged in HCI and design, 
Sketching is a relatively foreign concept in machine learning. 
Recent lines of research have called for a greater acknowledgement of ML as a design material and have explored the experiences of UX designers for ML products and services, especially noting the ways in which AI presents unique difficulties for designers~\cite{yang_investigatingHowExperiencedUXDesigners, yang_reexaminingWhetherWhy}.
Research in this vein has explored how we might bring sketch-like practices into the design of ML-powered experiences to address these challenges~\cite{yang_sketchingNLP}. 

% There is sketching for products/services that use ML, but not for the models themselves
%However, there is still much room to expand the reach of sketching practices to the design of machine learning models themselves---in terms of their core structure, values, and decision-making logic. 
Classic work on interactive machine learning (IML) explored how we might enable users to author and refine ML models through demonstration and in real time~\cite{fails_olsen_IML}. This work in IML has made great strides on improving the speed and iteration of model development in service of rapid error correction~\cite{wang2021autods}. 
However, IML techniques are designed to act as end-to-end functional systems %, not disposable, minimal-detail prototypes. Additionally, in order to pare down interaction and prevent non-technical users from needing to engage with overly technical details, IML approaches usually 
and abstract away decision-making logic, delegating those sensemaking responsibilities to an algorithm hidden under the hood. 
Thus, existing IML approaches are not the right fit for the sketches that we seek, which would aid ML practitioners in thinking about and designing their model's decision-making policy.

% Discuss existing technologies and why they don't meet our sketch requirements
    % Blackbox models: slow, too detailed
    % No-code or low-code ML: fast, and minimal detail, but not expressive
    % LLM prompting: fast, expressive, but too much detail
% Lead from there to our approach to fill that gap
% \msb{this paragraph is important, but feels wordy}
Turning again to the characteristics of sketches outlined in Section~\ref{section:sketch_characteristics}, existing ML technologies do not yet fully support a sketching practice~(\autoref{fig:design_space}).
% Blackbox models
State-of-the-art technologies tend to involve blackbox models that require a great deal of time, cost, and effort to implement. 
% These models are extremely detailed in that they are implemented and tuned down to the last hyperparameter. 
While they may be theoretically expressive in their modeling capabilities, they are not very expressive from a human point of view: given that these models are not interpretable, ML practitioners cannot easily control or express different intents with these model designs.
% No-code or low-code ML
No-code or low-code ML approaches typically take a supervised learning approach that accepts labeled data examples as the primary control lever~\cite{scikit_learn,create_ml,teachable_machine}. 
These approaches are quick and minimal in detail since they purely focus the user on the data layer of abstraction, but this same design choice unfortunately limits expressivity since data is an indirect means of communicating intent for a decision-making policy and requires the user to curate intermediary data examples to convey their ideas.
% LLM prompting
Recent work has suggested that advances in Large Language Models (LLMs) may be used to support rapid model authoring via flexible natural language prompts~\cite{wu_AI_chains, jiang_PromptMaker}.
% \msb{if you like what I said in the intro about GPT-3, import that here too}
% We are excited by this line of work because it unlocks a method for users to take a more active, hands-on role in model design while maintaining a lightweight interaction mode. In our work, we seek to take these LLM-based prototyping methods further in the direction of a sketching practice. 
We further pare down the design language of prompt-based model authoring to center design decisions around the abstraction of concepts, which helps practitioners to focus on the core high-level value tradeoffs of their model rather than getting bogged down with details of individual prompts.

\begin{figure}[!tb]
  \includegraphics[width=0.5\textwidth]{figures/design_space_v1.pdf}
  \caption{A summary of our design space. To accomplish an effective sketching practice, we seek to achieve expressivity, minimal detail, and speed, a combination that current tools lack.}
  \label{fig:design_space}
\end{figure}




==> sections/old_versions/2_related_work_v6.tex <==
% v5 11/26/22

We survey research on sketching and prototyping in design and HCI, the work practices of machine learning practitioners, and current approaches for early-stage model design, all of which motivate our model sketching approach.

\subsection{Sketching and prototyping in design and HCI}
% Introduce sketching, benefits; importance for early-stage designs
% Highlight importance as tool for thinking; shifting to high-level
The fields of design and HCI have long upheld the practice of sketching as a valuable tool for thought~\cite{fallman_designOrientedHCI,buxton2010sketching}. A key trait of a successful sketching or prototyping tool is that it refocuses cognitive processes on high-level iteration, empowering the practitioner to engage in ``design thinking rather than implementation tinkering''~\cite{hartmann_dTools}. A sketch is similar to a prototype in that both are instantiations of a design concept, but a sketch serves a different purpose: to explore and raise questions about design approaches rather than to propose answers or solutions~\cite{buxton2010sketching}. Thus, sketches are suitable for the early ideation stages of a design process while prototypes are intended for the later stages. 

% Highlight expressivity, speed, minimal detail
\subsubsection*{What characterizes a sketch?}
\label{section:sketch_characteristics}
Buxton characterizes sketches as quick, plentiful, ambiguous, and minimal in detail~\cite{buxton2010sketching}. %We look to these traits to guide the design of a novel sketching approach for modeling.
% Quick, plentiful
The \textit{quick} and \textit{plentiful} attributes go hand in hand: % the speed with which sketches can be authored unlocks increased opportunities for iteration, which produces plentiful artifacts.
methods with quick turnaround times enable practitioners to explore parallel design paths, an approach that supports more iterations, combats harmful design fixation, and leads to more diverse, higher-quality designs~\cite{dow_parallelPrototyping, tohidi_buxton_gettingTheRightDesign}. 
Sketches are powerful tools because they allow a practitioner to quickly iterate to test dramatically different high-level ideas.
% While sketches may seem rudimentary, it is because they are so disposable and easy to generate that they allow for designers to more broadly explore a design space and prune unpromising design directions before they become ossified.

% Ambiguous, minimal detail
The \textit{ambiguous} and \textit{minimal detail} attributes are also closely tied: %they hold that sketches should remain vague and not veer towards high-fidelity representations. This may seem counterintuitive, but %: it may seem like additional detail could only help to more clearly convey a design vision. However, 
much of the value of a sketch lies in both the cognitive task of distilling an idea into a stylized, minimal representation \cite{lim_anatomyOfPrototypes} and in leaving enough ambiguity to suggest---to oneself and others---multiple interpretations (and thus multiple future directions)~\cite{goel1995sketches}. Early work in user interface design demonstrated that overly-detailed prototyping approaches detract from this valuable cognitive work~\cite{landay_interactiveSketching} and do not substantially improve feedback quality~\cite{walker_hifiOrLofi}; in fact, simpler prototypes have been correlated with better design outcomes~\cite{yang_aStudyOfPrototypes}.

% Expressive
Finally, a sketch is \textit{expressive}: %. In order for a sketch to hold any value for a practitioner, 
it must provide enough flexibility and control to allow a practitioner to communicate their idea and iterate upon it~\cite{buxton2010sketching,landay_interactiveSketching}. Traditional freehand sketches are highly expressive because designers can draw upon concrete or abstract visual and textual representations to hone their idea, allowing others to perceive both perceptual features and functional relations~\cite{ suwa_tversky_whatArchitectsSeeInTheirSketches}.
% However, expressivity trades off against the prior attributes of speed and minimal detail and thus requires careful consideration of what abstractions or design vocabularies to provide to a practitioner \msb{I disagree with this---Scott McCloud's Understanding Comics conveys how comics can be very expressive even with minimal detail}.

% Concepts as a promising direction for model sketching
Concept-based abstractions in particular hold promise for sketch-like approaches to machine learning model authoring.
Prior work on concept evolution in data labeling demonstrated that many decision-making goals are malleable and subjective, but these goals can be clarified through an iterative process of concept elicitation and refinement~\cite{kulesza_conceptEvolution, chang_revolt}. Researchers have even found that for real-life decision-makers such as judges, doctors, and managers, simple, statistically-derived rules based on a small number of human-interpretable features substantially outperform human experts~\cite{jung_goel_simpleRulesExpertClassification}. Concepts map well to the way that humans reason over decision-making tasks, and methods that statistically aggregate concepts work surprisingly well, even beyond prototyping contexts.

% \subsubsection*{Translating from sketches to implementation}
% \msb{I suggest cutting this subsubsection---I don't think it really adds to the RW argument}
% % Our intent to bridge between role and implementation prototype
% While sketches and prototypes are valuable exercises in their own right to guide designers' thinking, their ultimate aim is to produce a better end-product, and the \textit{purpose} of a prototype defines how it will influence the design of a final product. Houde and Hill highlight three purposes: to clarify the role of a technology, experiment with its implementation, or convey its look and feel~\cite{houde_whatDoPrototypesPrototype}.
% In our work, we seek to provide a pathway from sketch-like versions of models to full-scale models, just as prior work enabled seamless transformations from rough interface design sketches to operational look-and-feel interfaces~\cite{landay_interactiveSketching}. Thus, we situate model sketching between a role and implementation prototype, as we aim to emulate the behavior of a full machine learning model in a real-world decision-making setting while roughly capturing its implementation via constituent concepts, which could be turned into fully-built feature extractors and sub-models using more traditional ML methods.
% We argue these characteristics of sketching and prototyping could inspire new practices for early-state ML model design.

\subsection{ML practitioners: work practices and cognitive focus}
% Who we consider ML practitioners
In our work, we use the terms ML practitioner and model developer interchangeably to refer to users who perform work that primarily deals with designing, developing, and iterating on machine learning models~\cite{muller_HowDataScienceWorkersWorkWithData,zhang_howDoDataScienceWorkersCollaborate}. 
Recent literature frames the data science and ML project workflow as a multi-stage collaborative lifecycle where business users or domain experts focus on high-level problem definition and results interpretation, while ML practitioners place their cognitive focus on low-level implementation details~\cite{wang2019human, zhang_howDoDataScienceWorkersCollaborate,piorkowski_AIDevelopersCommChallenges}.
However, a major problem with the current workflow is that much of the translational work that ML practitioners perform to bridge between high-level goals and low-level implementation (i.e., via problem formulation, feature extraction, feature engineering) is rendered invisible~\cite{zhang_howDoDataScienceWorkersCollaborate, mao2019data,passi_trustInDataScience, muller_HowDataScienceWorkersWorkWithData}. 
% ML practitioners frequently must navigate tensions between low-level ``rational'' and high-level ``subjective'' aspects of their work~\cite{mao2019data,passi_trustInDataScience, muller_HowDataScienceWorkersWorkWithData}, but current tools and processes often neglect this effort. 
As a result, ML teams lose important knowledge about the nature and meaning of features and the assumptions and reasoning that underlie modeling decisions~\cite{mao2019data,hou2017hacking}, which is especially problematic if ML practitioners need to revisit those decisions to counter harmful model behavior.
%In the related domain of statistical model authoring, recent research has similarly documented that model developers focus their attention on technical, implementation-oriented aspects of the modeling process rather than high-level conceptual hypotheses, and software tools exacerbate the problem
Similar patterns play out in statistical model authoring, which has prompted calls for high-level libraries to ``[express] conceptual hypotheses to bootstrap model implementations'' and bidirectional conceptual modeling to ``[co-author] conceptual models and model implementations''~\cite{jun_hypothesisFormalization}. 
Our work directly seeks to carry out this vision in the domain of ML model development by allowing ML practitioners to instantiate models using high-level concept-based abstractions that bridge to functional model implementations.

\rev{\subsection{Early-stage machine learning model design}}
\rev{Work in interactive machine learning (IML) has long been interested in how we might engage humans in the model development process. In reaction to the slow and effortful process of building models, work in IML demonstrated that by enabling interactive model training and refinement, users can more rapidly develop models and keep them aligned with their goals~\cite{fails_olsen_IML,amershi_powerToThePeople, patel2010gestalt, francoise2021marcelle}.
In most IML systems, interactions take the form of labeled examples and demonstrations, such as positive and negative image examples in CueFlik~\cite{cueflik} and paired input gestures and output actions in Wekinator~\cite{wekinator}. 
% For example, in CueFlik, users could author rules (nearest-neighbor classifiers for concepts like ``scenic'') by providing sets of positive and negative image examples~\cite{cueflik}, and in Wekinator, users can demonstrate pairs of input gestures and outputs to guide the system to learn a mapping between the two~\cite{wekinator}.

Building on IML, work on interactive machine teaching (IMT) emphasizes the metaphor of \textit{teaching} to focus on the human's role as a teacher rather than just a label-provider~\cite{ramos2020IMT, simard2017IMT}. Through this metaphor, IMT highlights new challenges like the need for richer teaching strategies beyond data labeling.
% and the need to support teachers who are domain experts, but not ML experts.
A wizard-of-oz study along this vein explored how users might teach knowledge to a model, and this work found that users decomposed knowledge in terms of concepts, relationships between concepts, and rules that combine and apply these concepts~\cite{ng_IMTknowledgeDecomp}. However, without actually instantiating and evaluating their concepts, users struggled to form a mental model of how the ML model works, which made it especially difficult for them to know how to articulate subtle, abstract forms of knowledge. 

\begin{table*}[!tb]
  \centering
  \footnotesize
    \rev{
    \begin{tabular}{p{0.2\textwidth}p{0.07\textwidth} p{0.25\textwidth} p{0.25\textwidth} p{0.1\textwidth}}
    \toprule
    \textbf{Paradigm} & \textbf{Emphasis} & \textbf{Paradigm shift} & \textbf{Strategy to improve ML models} & \textbf{Design reqs}\\
    \midrule
    {Interactive Machine Learning} &
    {\textit{interactive}} &
    {ML models don't need to exist in a vacuum---through human \textit{interaction} and feedback}, we can achieve user alignment and rapid model authoring&
    {Better feedback loops}&
    {Speed}\\
    \midrule
    {Interactive Machine Teaching} &
    {\textit{teaching}} &
    {ML isn't just about learning---we need to focus on \textit{teaching}: \textit{who} is developing ML models and \textit{how} they're sharing their knowledge} &
    {Better teaching}&
    {Expressivity}\\
    \midrule
    {Model Sketching} &
    {\textit{sketching}} &
    {ML models don't need to be high-fidelity---in fact, \textit{low-fidelity}, \textit{transient} models are better at helping us to explore the multiverse of model designs} &
    {Better design space exploration}&
    {Minimal detail, Speed, Expressivity}\\
    \bottomrule
    \end{tabular}
    }
    \caption{
    \rev{A summary of key ideas put forward by Interactive Machine Learning and Interactive Machine Teaching, alongside those of Model Sketching. The three paradigms are complementary, but they each emphasize different perspectives and strategies.}
    }
    \label{table:related_work_comparison}
\end{table*}

While model sketching shares many of the same motivations that underlie IML and IMT,
% ; with IML, we share an interest in enabling rapid iteration on ML models through human interaction, and with IMT, we share the goal of enriching users' abilities to share their knowledge with a model. 
it has slightly different goals---to explore a vague, unformulated model design space (problem formulation) rather than execute on a crisp modeling vision (model implementation). 
This means that in addition to the speed and expressivity required by IML and IMT, model sketching requires a \textit{minimal representation of a model's decision-making logic} to facilitate effective design space exploration~(Table~\ref{table:related_work_comparison}). 
% Model sketching posits that in order to tackle problem formulation, we need \textit{minimal representations of a model's decision-making logic}.
To support model sketching, we need to provide a mechanism for the user to directly iterate on the decision-making primitives that control a model's actions. Thus, we cannot use black-box methods that opaquely map from inputs to outputs, such as example-based IML approaches and prompt-based model authoring. 
% Additionally, since sketches are meant to be transient artifacts, the strategies we uncover must be \textit{transferable} to production models. 
% \msb{I don't think we've solved the transferability problem in this paper --- cut that sentence?} 
Concepts are an ideal representation that allows for iteration on decision-making strategy and alignment with the ways that humans prefer to decompose and express their knowledge~\cite{ng_IMTknowledgeDecomp}. 
% Concepts are an ideal representation that allows for iteration on decision-making strategy, transferability to production models \msb{again, I don't think we've proven this --- interesting future work for sure}, and alignment with the ways that humans prefer to decompose and express their knowledge~\cite{ng_IMTknowledgeDecomp}. 

% Finally, how should we instantiate this concept-based representation?
The metaphor of sketching also informs how we must instantiate these concept-based representations.
Past work in IML and IMT has explored concept instantiation with examples, demonstrations, predefined features, and formal knowledge bases~\cite{cueflik, wekinator, ramos2020IMT, brooks2015featureInsight}. However, given that sketches are meant to explore a broad model design space that is not known ahead of time, users need to have the flexibility to author arbitrary concepts, so we cannot rely on static features or knowledge bases. An added challenge of sketching is that there is a steep cost associated with diverting the user's attention to different tasks (e.g., switching to label examples, develop a feature pipeline, or train a new helper model), which risk pulling the user out of the sketching mindset and into technical tunneling. 
% In this setting, we cannot use example- or demonstration-based concept instantiation methods that break the user out of their focused state \msb{I think this is a strawman: labeling 2-3 examples wouldn't pull people out of their flow in my opinion}.
Thus, we turn to zero-shot modeling approaches to instantiate concepts flexibly and rapidly without diverting attention.
}

% \begin{figure}[!tb]
%   \includegraphics[width=0.5\textwidth]{figures/design_space_v1.pdf}
%   \caption{A summary of our design space. To accomplish an effective sketching practice, we seek to achieve expressivity, minimal detail, and speed, a combination that current tools lack.}
%   \label{fig:design_space}
% \end{figure}




==> sections/old_versions/3.5_case_studies_v2.tex <==
\section{Demonstration Case studies}
% \msl{NOTE: these case studies are in rough initial form. We would likely represent each case study in a more pared-down form since there are a number of them, and I'd like to synthesize more of the holistic takeaways. We may be replacing this with examples of participants completing a modeling task of their own choosing}\\
To illustrate the breadth of machine learning tasks to which we can apply our model sketching approach, we present example case studies that we authored to demonstrate recommendation, unsupervised clustering, search, and bias audit applications~(Figure~\ref{fig:case_studies}, details in Appendix~\autoref{table:case_studies}).

% Travel
\subsubsection*{Travel planning---personalized recommendation} 
% Model sketching supports a broad range of scoring, ranking, and recommendation tasks. 
In our travel planning example, given a particular user, we aim to recommend travel lodging (an Airbnb listing) that would best match their preferences. We find that our model sketching approach allows for a user to rapidly personalize a recommendation model to their own tastes, for example conveying their preferred aesthetics and desirable attributes of the neighborhood. 
The sketching process also exposed some gaps in the modeling setup such as the potential value of customer reviews to provide an objective assessment of factors like cleanliness and the importance of proximity and specific physical location-related information for the travel use case.
% The sketching process also exposed some gaps in the modeling setup such as the need for additional images to get a better sense of a listing's attributes, the potential value of customer reviews to provide an objective assessment of factors like cleanliness, and the importance of proximity and specific physical location-related information for the travel use case.

% Creative inspiration
\subsubsection*{Creative inspiration---unsupervised embedding and clustering} 
Model sketching can also serve unsupervised learning tasks by allowing users to create customized sketch-like embedding spaces to perform downstream tasks related to item similarity, clustering, and analogical retrieval. In our creative inspiration task that builds on a dataset of museum artwork, sketch models effectively define what concepts we want to capture in our embedding space, such as a elements of visual style or a suite of themes related to social justice. Then, we could apply our visual-style sketch model to any artwork to retrieve its ``embedding'' in terms of its concept scores, allowing us to map out artworks within a rough visual-style embedding space. With these embeddings, we can cluster artworks and identify new themes of visual style. We can also gather creative inspiration by surfacing analogous works of art in disparate genres: if the user selects an artwork in the ``painting'' genre and selects a target genre of ``sculpture'', our system can return analogous artworks from the ``sculpture'' genre that are most similar to the original artwork.
% The model sketching process helped us to uncover that ``thematic'' concepts should be used with caution, as they can pick up both positive and negative handlings of a topic. For example, one ``gender themed'' artwork may handle gender in a sensitive or progressive way, while another may handle it in a harmful way. A user may unintentionally group together artworks like these with thematic concepts.

% Political
\subsubsection*{Political candidate research---personalized search} 
Our approach can also support search-related tasks. For this task, we assist users in researching political candidates before an election; in particular, we seek to help users discover which candidates are most aligned with them on the issues they care about most. Drawing from third-party candidate information sources including platforms, political statements, and speeches, model sketching unlocks a rapid, highly-personalizable tool for political candidate information-gathering. A user can author sketch models with concepts centered around political issues and can iterate on the set of concepts they care about to sift through candidate information and refine their candidate list. This approach is especially beneficial for expressing nuanced candidate stances that aren't explicitly highlighted as core ``issues'' in standard voting guides.
% ; such information is difficult to uncover with manual approaches.

% Reviewer audit
\subsubsection*{Restaurant reviews---reviewer bias auditing}
We can also apply model sketching for auditing tasks by working backwards from decision-making criteria or rubrics to uncover latent weights from human or algorithmic decision-makers. Here, we experimented with a task that assisted a food reviewer in assessing their own potential biases. Based on the reviewer's stated decision-making factors, we created analogous concepts and authored sketch models to aggregate these concepts, trained on the reviewer's overall restaurant review ratings. 
% Model sketching allowed us not only to roughly capture the reviewer’s values, but to infer their implicit weights. 
Our model inferred high positive coefficients for the ``Tasty'' and ``High quality'' concepts, which aligned with the reviewer's top two self-reported decision-making factors. However, the model inferred high negative coefficients for ``Good presentation'' and ``Nice vibes'' concepts, which corresponded to the reviewer's next most important factors. This revealed to the reviewer that these factors had less of a sway on their overall ratings than they intended.
% For example, our sketch model inferred coefficients of 2.22 and 1.26 for ``Tasty'' and ``High quality,'' suggesting that these concepts had the strongest positive correlation with the reviewer's ratings. Indeed, these concepts matched the reviewer’s top two self-reported decision-making factors. However, our model surfaced sizeable negative weights of -2.09 and -1.01 for ``Good presentation'' and ``Nice vibes,'' which were the two next most important factors listed by the reviewer, suggesting that these factors may have less of a sway (and even a counteracting sway) in their overall ratings than they may have intended.

% Model sketching allowed not only captured a reviewer’s values, but also their implicit weights. The ``Naive concepts'' model inferred coefficients of 2.22 and 1.26 for ``Tasty'' and ``High quality,'' suggesting that these concepts had the strongest positive correlation with the reviewer's ratings. Indeed, these concepts matched the reviewer’s self-reported main decision-making factors.


==> sections/old_versions/3.5_case_studies_v3.tex <==
\section{Demonstration Case studies}
% \msl{NOTE: these case studies are in rough initial form. We would likely represent each case study in a more pared-down form since there are a number of them, and I'd like to synthesize more of the holistic takeaways. We may be replacing this with examples of participants completing a modeling task of their own choosing}\\
To illustrate the breadth of machine learning tasks to which we can apply our model sketching approach, we present example case studies that we authored to demonstrate recommendation, unsupervised clustering, search, and bias audit applications~(Figure~\ref{fig:case_studies}; details in Appendix~\autoref{table:case_studies}).

% Travel
\subsubsection*{Travel planning---personalized recommendation} 
% Model sketching supports a broad range of scoring, ranking, and recommendation tasks. 
In our travel planning example, given a particular user, we aimed to recommend an Airbnb listing that would best match their preferences. 
% We created an \textit{aesthetics} sketch (Clean, Bright, Designer), a \textit{fun neighborhood} sketch (Good vibes, Central, Trendy), and a \textit{best overall} sketch (Clean, Bright, Designer, Ugly, Outdated)
% We find that our model sketching approach allows for a user to rapidly personalize a recommendation model to their own tastes, for example conveying their 
Here, our sketches could capture key aspects of a user's taste in Airbnbs: based on images, we expressed preferred aesthetics (Clean, Bright, Designer) and red flags (Outdated, Ugly); based on text descriptions, we conveyed desirable attributes of the neighborhood (Good vibes, Central, Trendy). 
The sketching process helped us to discover gaps in the modeling setup such as the potential value of customer reviews to provide an objective assessment of factors like cleanliness and the importance of proximity and specific physical location-related information for the travel use case.
% The sketching process also exposed some gaps in the modeling setup such as the need for additional images to get a better sense of a listing's attributes, the potential value of customer reviews to provide an objective assessment of factors like cleanliness, and the importance of proximity and specific physical location-related information for the travel use case.

% Creative inspiration
\subsubsection*{Creative inspiration---unsupervised embedding and clustering} 
Model sketching can also serve unsupervised learning tasks by allowing users to create customized sketch-like embedding spaces to perform item similarity, clustering, and analogical retrieval tasks. Building on a dataset of museum artwork, we authored sketch models for text and image fields related to bold visual style (Colorful, Surreal, Fantasy, Abstract), social justice (Social justice themed, Race themed, Feminist, Queer themed), and political movements (Politics themed, Revolution themed, Labor movement themed). Then, we applied our sketch models to new artworks to retrieve their concept score-based ``embeddings.'' We could then cluster artworks and gather creative inspiration by surfacing analogous works of art in disparate genres: by selecting an artwork in the ``painting'' genre and selecting a target genre of ``sculpture'', we could retrieve analogous artworks from the ``sculpture'' genre that were most similar to the original artwork.
% The model sketching process helped us to uncover that ``thematic'' concepts should be used with caution, as they can pick up both positive and negative handlings of a topic. For example, one ``gender themed'' artwork may handle gender in a sensitive or progressive way, while another may handle it in a harmful way. A user may unintentionally group together artworks like these with thematic concepts.

% Political
\subsubsection*{Political candidate research---personalized search}
Our approach can also support search-related tasks. For this example, we assisted a user in researching political candidates before an election to discover which candidates were most aligned with them on the issues they cared about most. Drawing from third-party candidate information sources including platforms, political statements, and speeches, we authored sketches that captured issues related to the environment (Climate change, Environment, Eco-friendly), gun control (Gun control, Anti gun), and other civil rights (Equal rights, Equality, Voting rights, Pro choice). Model sketching was especially beneficial for iteratively exploring nuanced candidate stances that weren't explicitly highlighted as core ``issues'' in standard voting guides.
% model sketching unlocks a rapid, highly-personalizable tool for political candidate information-gathering. A user can author sketch models with concepts centered around political issues and can iterate on the set of concepts they care about to sift through candidate information and refine their candidate list. This approach is especially beneficial for expressing nuanced candidate stances that aren't explicitly highlighted as core ``issues'' in standard voting guides.
% ; such information is difficult to uncover with manual approaches.

% Reviewer audit
\subsubsection*{Restaurant reviews---reviewer bias auditing}
We can also apply model sketching for auditing tasks by working backwards from decision-making criteria to uncover latent weights from human or algorithmic decision-makers. For this example, we assisted a food reviewer in assessing their own potential biases. Based on the reviewer's self-reported decision-making factors (Taste, Quality, Presentation, Vibes, Service Price), we created analogous concepts. Then, we authored sketch models to aggregate these concepts, using the reviewer's overall restaurant review ratings as ground truth. 
% Model sketching allowed us not only to roughly capture the reviewer’s values, but to infer their implicit weights. 
Our model inferred high positive coefficients for the Tasty and Quality concepts, which aligned with the reviewer's top two decision-making factors. However, the model inferred high negative coefficients for the Presentation and Vibes concepts, which corresponded to the reviewer's next most important factors. This revealed to the reviewer that these factors had less of a sway on their overall ratings than they intended.
% For example, our sketch model inferred coefficients of 2.22 and 1.26 for ``Tasty'' and ``High quality,'' suggesting that these concepts had the strongest positive correlation with the reviewer's ratings. Indeed, these concepts matched the reviewer’s top two self-reported decision-making factors. However, our model surfaced sizeable negative weights of -2.09 and -1.01 for ``Good presentation'' and ``Nice vibes,'' which were the two next most important factors listed by the reviewer, suggesting that these factors may have less of a sway (and even a counteracting sway) in their overall ratings than they may have intended.

% Model sketching allowed not only captured a reviewer’s values, but also their implicit weights. The ``Naive concepts'' model inferred coefficients of 2.22 and 1.26 for ``Tasty'' and ``High quality,'' suggesting that these concepts had the strongest positive correlation with the reviewer's ratings. Indeed, these concepts matched the reviewer’s self-reported main decision-making factors.


==> sections/old_versions/3_system_v1.tex <==
In this section, we describe our model sketching approach, which aids ML practitioners in moving beyond technical prototyping to explore the conceptual model design space during early phases of machine learning model development.

% \begin{itemize}
%     \item Concept models: zero-shot modeling
%     \item Sketch models: aggregation models
%     \item Why we selected notebook environment
%     \item ModelSketchBook API
%     \begin{itemize}
%         \item Sketchbook
%         \item Creating concepts
%         \item Creating sketches
%         \item Comparing sketches; evaluating
%     \end{itemize}
% \end{itemize}

\subsection{Design goals}
\msl{TODO: mention that we aim to intervene in the early phases of model development}

% Our design was meant to capture the core elements of sketching that enable a practitioner to shift their thinking from implementation/execution to design/approach
Inspired by the practice of sketching in design, we seek to capture the core elements of sketching that successfully enable a practitioner to shift their thinking from a mode of implementation and execution to one that explores parallel designs and approaches. The key attributes that we seek to emulate are expressivity, minimal detail, and speed~\cite{buxton2010sketching}. 

\textit{Expressivity} captures the level of flexibility and control that a medium affords a practitioner as they attempt to communicate an idea. Traditional pencil-and-paper sketches are highly expressive because designers draw upon any number of concrete or abstract visual and textual elements to hone their idea. For ML model authoring, expressivity would require a similar level of flexibility to express ideas by drawing upon visual and textual ideas of varying concreteness.

\textit{Minimal detail} enforces that, in order to be most effective as tools for thinking, sketches should not veer towards high-fidelity representations. This is a bit counterintuitive: it may seem like additional detail can only help to more clearly communicate a particular design vision. However, much of the value of a sketch lies in the cognitive task of distilling an idea into a stylized, minimal representation. Excessive details tend to distract both a designer and their audience from the most important ideas at stake: for example, overly detailed interface designs tend to distract viewers from the core design ideas and prompt them to comment about granular interface elements rather than high-level interaction modes~\MSLcite{}. Designers counter this tendency by enforcing norms about the level of fidelity they capture (e.g., using wireframes or storyboards that limit details). In ML model development, minimal detail would ideally mean paring down from fully-implemented technical modeling infrastructures to simple representations that convey the core logic, ideas, or values that distinguish one modeling approach from another.

\textit {Speed} is perhaps the most straightforward of these constraints and conveys that sketches should require little time or effort to author. Quick turnaround times in sketching unlock more rounds of iteration, and this iteration is key to discovering design gaps and exploring potential solutions. Simple materials and a loose gestural drawing style make traditional sketching fast. However, for machine learning model development, the status quo turnaround times can range from hours or days to weeks or months, and this work is often split across multiple people or even multiple teams. To reach a sufficient speed comparable to pencil-and-paper, model authoring should happen at interactive speeds, which means that model results should appear within seconds of user input, and it should be possible for a single user to author sketches on their own.

These three factors---expressivity, minimal detail, and speed---together enable an effective sketching practice that focuses a designer's effort on the work that will produce the richest cognitive and communicative benefit. We thus aim to embed these three critical elements in our model sketching method.

\begin{figure}[!tb]
  \includegraphics[width=0.5\textwidth]{figures/design_space_v1.pdf}
  \caption{A summary of our design space. To accomplish an effective sketching practice, we seek to achieve expressivity, minimal detail, and speed, a combination that current tools lack.}
  \label{fig:design_space}
\end{figure}

% \subsection{Motivating scenario}
% TODO: walkthrough of what it would look like to author a sketch model (may not be necessary if we do case studies in the next section)

\subsection{Approach}
% We wanted to fill the gap between high-level modeling goals and low-level implementation --> arrived at intermediate goals/representations in the form of concepts
Currently, ML practitioners commonly capture their modeling work through 1)~high-level descriptions like written documents or presentations stating the goal of a given model or 2)~low-level implementations like computational notebooks or code repositories with data processing, feature extraction, and modeling logic. However, there is a significant amount of translational, interpretational work that goes in between a high-level description and any particular low-level implementation. This work may in fact be the most critical piece of the modeling task to get right given that there is a vast design space of plausible solution strategies for any one high-level modeling goal. Furthermore, these different approaches carry different sets of human values and ethical implications, which is especially important to consider when designing human-facing deployments of machine learning. There is not just one clear solution, and the choice among solutions is not arbitrary, especially in terms of user impact. 

Since current approaches primarily cover only high-level goals or low-level technical instantiations, this important intermediate work remains hidden in the depths of experimental scripts, disorganized notebooks, or even internal reasoning that may never have been documented in any form~\MSLcite{ other DS work}~\cite{zhang_howDoDataScienceWorkersCollaborate}. What we \textit{want} is to foreground the challenging work of bridging between goals and implementations so that ML practitioners can confidently explore numerous solution paths and compare their tradeoffs. What we have is a messy, undocumented process where practitioners themselves may not be able to remember all of the reasons underlying their prior design decisions. This makes it exceedingly difficult to not only revisit those past decisions, but to reverse them or explore alternative implementations after a model has already been built and deployed.

Thus, we specifically seek to address the gap between high-level modeling goals and low-level implementation by introducing \textit{concepts}---human-understandable ideas or factors that are relevant to a decision-making task---as an intermediary representation. By foregrounding this translational step between goals and their implementation, we aim to scaffold ML practitioners' reasoning and help them to more effectively sketch out and explore parallel solutions paths. This concept-based intermediary can also make their work in this vein more visible and organized, both to themselves and to other stakeholders.

% Concepts also allow us to meet our design goals of expressivity, minimal detail, and speed
Concepts as a primary abstraction also allow us to meet our design goals of expressivity, minimal detail, and speed. Given that they can relate to all sorts of modalities (including text and images) and can range from concrete and specific to abstract and ideological, concepts provide an expressive lever for specifying model behavior. Then, centering the model authoring process primarily around concepts naturally enforces a much-simplified representation of a model's decision-making logic, achieving minimal detail while ensuring that the detail that remains is central to the core ideas of a modeling approach. Lastly, thanks to improvements in zero-shot modeling, we can interactively generate models that map from data examples to arbitrary concepts without any training time. This means that users can speedily author functional models by simply specifying concepts and stringing them together. We now describe in greater detail how we break down our model sketching approach into concept models and sketch models.

\subsubsection{Data prerequisites}
Our approach has very few data requirements. We simply require a data table (e.g., spreadsheet, CSV, Pandas DataFrame) where each row represents a single example and each column represents a data field. These data fields can contain text, image, or numeric data. Our approach works best when the data is labeled for the desired modeling task (e.g., if the task is hate speech detection, it is ideal for the data table to include a column with labels indicating the the hate speech label or score for each item). These labels allow us to benchmark our sketch model output against a desired point of reference. However, such labels are not required to author sketch models.

\subsubsection{Concept models: Crafting functional building blocks of decision-making}

\begin{figure}[!tb]
  \includegraphics[width=\textwidth]{figures/sys_concepts_v1.pdf}
  \caption{Concept Models. \msl{TODO: caption}}
  \label{fig:sys_concepts}
\end{figure}

With our method, concepts are the main building blocks that users can use to construct their models.  
Concepts are how we decompose the larger and more ambitious task of a sketch model into more manageable, human-understandable components. A concept is meant to capture a smaller factor or idea that is relevant to the modeling task.

Ordinarily, even if a model developer has certain concepts in mind, they wouldn't necessarily be able to actualize these concepts in their model. They might have the sense that they want a hate speech classifier to account for racism, sexism, or dehumanization, but the main options they have are to either 1)~gather data examples that cover those concepts and hope that the model picks up on them, or 2)~create a feature extraction pipeline (for more concrete attributes) or sub-model (for more abstract ideas) to clue the model into those concepts. Data curation is a significant endeavor that already can take up to 80\% of the time and effort in a data science project~\cite{muller_HowDataScienceWorkersWorkWithData}, and feature extraction pipelines and additional sub-models similarly require a considerable amount of time and engineering effort to build. All of that work must happen before the model developer can even test out whether those technical methods will sufficiently capture their internal understanding of the concept, let alone whether the concept will provide a sufficiently valuable signal for the decision-making task.

In contrast, the concepts that users author using our model sketching approach are actually \textit{models in themselves}, and creating a concept model is as simple as specifying a word or phrase that describes a concept. This means that a model developer can think of a concept and immediately instantiate it in a functional sub-model that they can incorporate into their modeling task. We define a concept model as a mapping from a data example to a score that indicates its relevance to the specified concept, or how well it exemplifies that concept. For example, a concept model for ``colorful'' might produce scores for a set of images indicating roughly how colorful they are; a concept model for ``profanity'' might produce scores for a set of text comments that estimate how profane they are. Thus, concept models bear similarities to feature extractors, but they are not limited to lower-level, objective attributes, and they require much less time and effort to produce. Once created, a concept model can be applied to any arbitrary example, seen or unseen.

We build upon advances in zero-shot modeling to instantiate our vision of concept models. Zero-shot modeling describes any machine learning modeling approach that does not require any training examples to perform a task. Given an input concept term (a brief word or phrase) and a data field (column name) from the dataset, we author a zero-shot model that maps from the provided data to the specified concept idea to produce a concrete score.
The benefit of this approach is that it does not require any labeled examples and does not require any training time to produce its output predictions. Given our design constraints that aim to provide interactive model outputs to users, zero-shot models are an ideal choice. 

For our concept models, we specifically experiment with two different zero-shot modeling approaches: 1)~zero-shot text classification via large language model prompting using GPT-3 and 2)~zero-shot image regression via embedding similarity with a pre-trained image-to-text model using CLIP. 

To achieve zero-shot text classification, we author prompts that list a batch of examples for the model to classify and ask the model to decide on a binary label (``<concept term>'' or ``not <concept term>'') for each provided example. Large language models like GPT-3 are designed to perform text completion on provided input prompts, so plausible completions provided by the model capture a rough sense of binary labels that might be reasonable based on the knowledge available to the model. We include an example prompt below.

\begin{minted}[fontsize=\small,samepage]{markdown}
        Decide whether these comments are "motivational" or "not motivational".
        1. You can do it!!
        2. Ugh, you're the worst.
        3. I'm so tired...
    
        Comment results:
\end{minted}

The GPT-3 model will then return a text completion response similar to this that provides a label for the examples. We parse and post-process this GPT-3 response to retrieve binary labels.
\begin{minted}[fontsize=\small,samepage]{markdown}
        1. motivational
        2. not motivational
        3. not motivational
\end{minted}

To carry out zero-shot image classification, we use CLIP (Contrastive Language-Image Pre-Training)~\cite{CLIP}, a neural network trained on (image, text) pairs that allows images and text to be represented in a shared embedding space. Given a data field containing images and a concept term, we use CLIP to encode both the image and the concept term in that shared image-text embedding space. Then, we calculate and return the cosine similarity between the embedded image and concept term. Thus, the output score approximately captures the extent to which the given image relates to the specified concept term. We also allow users to normalize and re-calibrate these similarity scores to match their internal understanding of the concept, and we also grant users the ability to apply a custom threshold to binarize these continuous concept scores.

While we choose these two zero-shot approaches in our work, we design our model sketching approach to be compatible with any current or future zero-shot modeling method. Our approach works with any method that takes in images or text as input and is capable of producing concept relevance scores or labels at interactive speeds with no additional training data. As these technologies improve and become increasingly accessible, we envision that users will be able to leverage more advanced and specialized pretrained models to serve model sketching. These future models may achieve higher performance or may better capture domain-specific information necessary for targeted applications areas such as medicine, law, and the natural sciences.

\subsubsection{Sketch models: Putting concepts together to envision decision-making outcomes}

\begin{figure}[!tb]
  \includegraphics[width=0.9\textwidth]{figures/sys_sketches_v1.pdf}
  \caption{Sketch Models. \msl{TODO: caption}}
  \label{fig:sys_sketches}
\end{figure}

The second component of our model sketching approach involves aggregating these concepts together to form sketches. 
Without concept models as an intermediary, ML practitioners usually have to map directly from raw data (i.e., resume text) to their modeling outcomes (i.e., a ranked list of promising job applicants). They can tweak model architectures, perform data processing, try out alternate loss functions, and adjust hyperparameters, but these modifications are largely uninterpretable and leave the model as a black box. With the introduction of concept models, ML practitioners can now shift to iterate on their models in terms of human-understandable concepts instantiated in concept models that they themselves brainstormed, authored, and tuned.

A sketch model is simply a lightweight, rapidly-authored version of a full machine learning model that works by aggregating the signals produced by concept models. It is designed to accomplish the same task as the full model that it is meant to emulate, so it expects the same inputs and produces the same kinds of outputs.
Once the user has authored a set of constituent concepts that are relevant to the decision-making task, they can combine the concepts together to produce a sketch model by selecting which concepts they'd like to combine. We provide an initial set of aggregators that can combine concept model scores to produce a single sketch model score: linear regression, logistic regression, decision tree classification, random forest classification, and multi-layer perceptron (MLP) classification. However, we are again not bound to this initial set of aggregators; sketch models are compatible with any aggregation method that can accept multiple concept scores and produce a holistic output score. 
% Sketch model is trained on provided labels, but can be specified more manually if desired
We use the ground-truth labels provided in the training dataset to train these aggregators when a sketch model is created; all subsequent runs of the sketch model will simply evaluate the trained model on new input data. If the dataset does not have labels, then the user can opt to provide manual weights for the concepts using the linear regression aggregator.


Using the specified concepts and aggregation method, our approach produces a sketch model that can generate a score for any arbitrary input example. The concept models operate on the example to generate their individual concept scores, and the sketch model applies the aggregator to these concept scores to produce the overall score.

With the sketch-model layer of abstraction, ML practitioners can focus their attention on experimenting with different combinations of concepts to create sketches that might capture different sets of values in decision-making. For example, when authoring a hate speech detection model, an ML practitioner may experiment with sketches that focus on race-related or gender-related hate speech, or approaches that explicitly account for intersectionality; they may try out sketches that take a lenient stance unless the speech incites violence, or they may experiment with sketches that take a more strict stance on profanity and slurs. By rapidly authoring sketch models and testing them on new data examples, ML practitioners can quickly discover cases where their modeling approach appears to fail. Through inspection of sketch model behavior, they can get inspiration for new concepts that may help them to address gaps in their model, and they can immediately author and incorporate those new concepts. They may also discover gaps in the larger modeling ecosystem---for example, cases where the current data fields do not provide enough information to glean a certain concept, cases where the dataset lacks representation of a certain important phenomenon, or cases where the data labeling scheme is inconsistent or lacks the necessary granularity to separate classes.

% Compatibility with existing features/model outputs
While sketch models in their most stylized form are comprised entirely of concept models, sketch models are also compatible with other, more traditional kinds of features. If a model developer has raw or pre-processed features from an existing feature extractor or data pipeline, they can also incorporate those features and aggregate them into a sketch model. If an engineering team already has an existing version of a model or sub-models that produce scores that may be helpful for the decision-making task, they can also incorporate those scores as inputs to a sketch model.

\subsection{The ModelSketchBook API}
To realize our vision of model sketching, we introduce the \texttt{ModelSketchBook} API, a Python package that allows ML practitioners to create concepts and sketches of their own. Our package will be made open-source and is available in a public Github repository.\footnote{https://github.com/REDACTED (currently a private repository during review)}

\msl{NOTE: this API section is rougher/ a bit dry; just wanted to get the basic info across for now}

\subsubsection{Environment and setup}
% Why we selected a notebook environment; our target demographic
The \texttt{ModelSketchBook} API can be loaded in any Python environment, but it is optimized for use in a computational notebook. We chose to tailor our API design to the notebook environment because this is where many ML practitioners and data scientists already carry out much of their exploratory modeling work~\MSLcite{ work on computational notebooks}. We sought to intervene and provide a sketching tool in the environment where it could provide the most value to our target audience of ML practitioners.

% Setting up the sketchbook and data
After loading in their dataset into a Pandas dataframe and importing the \texttt{ModelSketchBook} package in their notebook, the user can run a brief function to set up their sketchbook with the dataframe(s) and their associated data schema.

% df_train = pd.read_csv("train.csv")
% df_test = pd.read_csv("test.csv")
\begin{minted}[fontsize=\footnotesize,samepage]{python}
    import model_sketch_book as msb

    # Set up the sketchbook
    sb = msb.create_model_sketchbook(
        goal="Detect hateful memes on social media.",
        datasets={  # Pass in datasets to use
            "train": df_train,
            "test": df_test,
        },
        schema = {  # Specify the types of data fields, including the ground-truth column
            "text": InputType.Text,
            "img_url": InputType.Image,
            "overall_rating": InputType.GroundTruth,
        },
    )
\end{minted}

The sketchbook contains all of the datasets, concepts, and sketches that the user will author during their session, and it saves other metadata such as model output scores, performance metrics, and the history of the concepts and sketches in the sketchbook.

\msl{TODO: create system figure demonstrating the notebook API and widgets in practice}

\subsubsection{Creating concepts}
After setting up the sketchbook, users can freely author concepts. While we also provide raw function calls under the hood, for convenience, we use ipywidgets\footnote{\url{ipywidgets.readthedocs.io}}, interactive browser controls for IPython notebooks. These widgets make it much simpler for new users to make sense of the available function parameters and the eligible input options for each parameter. The user can simply make the function call \texttt{create\_concept\_model()}, and a set of widgets will appear that allow the user to specify the input field, a concept term, and other details like the output type of the concept model~(Figure~\msl{TODO: concept input figure}).

Once the user enters in those details, they can execute the cell; after several seconds, the API returns a dataframe visualization that displays a sorted view of the examples in the training dataset along with their concept score~(Figure~\msl{TODO: concept output figure}). The user can browse through the concept score results to determine whether the model's understanding of the concept sufficiently aligns with their own. If not, they can try out other concept terms or experiment with other input fields to work towards better alignment.

The API also includes additional features for users to binarize continuous scores using a custom threshold value, auto-normalize continuous scores to a 0-1 score range, or custom-calibrate continuous scores based on a specified minimum and maximum score value. These features allow the user to bring the raw concept scores in closer alignment with their own personal understanding of a concept.

We also provide functions that assist users as they brainstorm and evaluate the tradeoffs among different concepts. A brainstorming helper function surfaces synonyms or antonyms of a provided word to spur ideas when users seek to verbalize or refine their concept. Meanwhile, a concept comparison helper function allows users to specify two concept terms and see a side-by-side comparison of their respective correlation with the input data and ground-truth ratings.
\msl{TODO: add that participants can write and save scratchnotes with the API}

% AND and OR logical operators for concepts
Finally, to allow for further control and refinement of concepts, we enable users to link existing concepts together with logical \texttt{AND} and \texttt{OR} operators. With a call to \texttt{create\_AND\_concept()}, users can take the logical \texttt{AND} of any number of binary concepts (and can similarly link arbitrary concepts with an \texttt{OR} relation using the \texttt{create\_OR\_concept()} function). This grants users the ability to better link concepts that interact with one another such as a single concept that can manifest in several ways or a multimodal concept that requires semantics from both image and text.

\subsubsection{Creating sketches}
Once a user has authored several concepts, they can proceed to create sketches that aggregate those concepts by calling \texttt{create\_sketch\_model()}. This function will again display a set of widgets that allow the user to select all of the concepts that they would like to use in the sketch model as well as an optional aggregation method (linear regression is the default)~(Figure~\msl{TODO: sketch input figure}).

After executing the cell, the API creates the new sketch model and returns a dataframe visualization that displays all of the input fields of the training examples, all of the relevant concept scores, and the overall prediction produced by the sketch model~(Figure~\msl{TODO: sketch output figure}). This view also includes the ground-truth ratings and the difference between the sketch prediction and these ground-truth ratings. Users can choose to sort by various columns to aid their understanding of the model outputs: sorting by the sketch prediction surfaces an ordering that represents of the sketch model's understanding of the modeling task; sorting by the ground-truth rating foregrounds the ``intended'' understanding of the modeling task; sorting by the difference (or absolute value of difference) between the sketch prediction and ground-truth rating highlights areas where the sketch model most drastically deviated from the intended decision-making behavior. The sketch model output also displays more traditional performance metrics for both regression and classification formulations of the task based on the ground-truth labels and the training examples; we display Mean Absolute Error (MAE), Classification Accuracy, F1 Score, Precision, and Recall.

% Evaluating sketch on unseen data
Finally, the API provides helper functions that help the user to better compare their sketch models. The \texttt{compare\_sketches()} function allows the user to compare the performance metrics for specified sketches, and the \texttt{test\_sketch()} function allows them to test out sketch models on a labeled or unlabeled validation set (if one is provided) to get a sense for how well it generalizes to a broader set of examples.

\msl{TODO: mention somewhere that we recommend a smaller set of examples for use in the sketchbook (on the order of 20-50)}

\subsubsection{Implementation}
% More detailed implementation details/settings; Colab setup
The \texttt{ModelSketchBook} API was authored entirely in Python. We use OpenAI's API for GPT-3 to perform zero-shot prompt-based text classification and use the \texttt{text-davinci-002} model, the current state-of-the-art GPT-3 variant. We use OpenCLIP~\cite{open_clip}, an open-source version of CLIP, to perform zero-shot image regression; we use a Vision Transformer (ViT) model (\texttt{ViT-B-32-quickgelu}) pre-trained on the \texttt{laion400m\_e32} dataset. We use the scikit-learn~\cite{scikit_learn} implementations of linear regression, logistic regression, decision tree classification, random forest classification, and MLP classification for our sketch model aggregators.


==> sections/old_versions/3_system_v2.tex <==
In this section, we describe our model sketching framework, which aids ML practitioners in moving beyond technical prototyping to explore the conceptual model design space during early phases of machine learning model development.

% \begin{itemize}
%     \item Concept models: zero-shot modeling
%     \item Sketch models: aggregation models
%     \item Why we selected notebook environment
%     \item ModelSketchBook API
%     \begin{itemize}
%         \item Sketchbook
%         \item Creating concepts
%         \item Creating sketches
%         \item Comparing sketches; evaluating
%     \end{itemize}
% \end{itemize}

\subsection{Design goals}
\msl{TODO: mention that we aim to intervene in the early phases of model development; NOTE: might move some of this up to Related Work}

% Our design was meant to capture the core elements of sketching that enable a practitioner to shift their thinking from implementation/execution to design/approach
Inspired by the practice of sketching in design, we seek to capture the core elements of sketching that successfully enable a practitioner to shift their thinking from a mode of implementation and execution to one that explores parallel designs and approaches. \msb{If these are key, I'd use them up in the intro as well when explaining why prior work hasn't crossed this chasm yet} The key attributes that we seek to emulate are expressivity, minimal detail, and speed~\cite{buxton2010sketching}. 

\textit{Expressivity} captures the level of flexibility and control that a medium affords a practitioner as they attempt to communicate an idea. Traditional pencil-and-paper sketches are highly expressive because designers draw upon any number of concrete or abstract visual and textual elements to hone their idea. For ML model authoring, expressivity would require a similar level of flexibility to express ideas by drawing upon visual and textual ideas of varying concreteness. \msb{would we say that supervised ML training has no expressivity, or very high expressivity? worth anchoring the reader's understanding here.}

\textit{Minimal detail} enforces that, in order to be most effective as tools for thinking, sketches should not veer towards high-fidelity representations. This is a bit counterintuitive: it may seem like additional detail can only help to more clearly communicate a particular design vision. However, much of the value of a sketch lies in the cognitive task of distilling an idea into a stylized, minimal representation. Excessive details tend to distract both a designer and their audience from the most important ideas at stake: for example, overly detailed interface designs tend to distract viewers from the core design ideas and prompt them to comment about granular interface elements rather than high-level interaction modes~\MSLcite{}. Designers counter this tendency by enforcing norms about the level of fidelity they capture (e.g., using wireframes or storyboards that limit details). In ML model development, minimal detail would ideally mean paring down from fully-implemented technical modeling infrastructures to simple representations that convey the core logic, ideas, or values that distinguish one modeling approach from another.

\textit {Speed} is perhaps the most straightforward of these constraints and conveys that sketches should require little time or effort to author. Quick turnaround times in sketching unlock more rounds of iteration, and this iteration is key to discovering design gaps and exploring potential solutions. Simple materials and a loose gestural drawing style make traditional sketching fast. However, for machine learning model development, the status quo turnaround times can range from hours or days to weeks or months, and this work is often split across multiple people or even multiple teams. To reach a sufficient speed comparable to pencil-and-paper, model authoring should happen at interactive speeds, which means that model results should appear within seconds of user input, and it should be possible for a single user to author sketches on their own.

These three factors---expressivity, minimal detail, and speed---together enable an effective sketching practice that focuses a designer's effort on the work that will produce the richest cognitive and communicative benefit. We thus aim to embed these three critical elements in our model sketching method.

\begin{figure}[!tb]
  \includegraphics[width=0.5\textwidth]{figures/design_space_v1.pdf}
  \caption{A summary of our design space. To accomplish an effective sketching practice, we seek to achieve expressivity, minimal detail, and speed, a combination that current tools lack.}
  \label{fig:design_space}
\end{figure}

% \subsection{Motivating scenario}
% TODO: walkthrough of what it would look like to author a sketch model (may not be necessary if we do case studies in the next section)

\subsection{The Model Sketching Framework}
% We wanted to fill the gap between high-level modeling goals and low-level implementation --> arrived at intermediate goals/representations in the form of concepts
Currently, ML practitioners commonly capture their modeling work through 1)~high-level descriptions like written documents or presentations stating the goal of a given model or 2)~low-level implementations like computational notebooks or code repositories with data processing, feature extraction, and modeling logic. However, there is a significant amount of translational, interpretational work that goes in between a high-level description and any particular low-level implementation. This work may in fact be the most critical piece of the modeling task to get right given that there is a vast design space of plausible solution strategies for any one high-level modeling goal. Furthermore, these different approaches carry different sets of human values and ethical implications, which is especially important to consider when designing human-facing deployments of machine learning. There is not just one clear solution, and the choice among solutions is not arbitrary, especially in terms of user impact. 

Since current approaches primarily cover only high-level goals or low-level technical instantiations, this important intermediate work remains hidden in the depths of experimental scripts, disorganized notebooks, or even internal reasoning that may never have been documented in any form~\MSLcite{ other DS work}~\cite{zhang_howDoDataScienceWorkersCollaborate}. What we \textit{want} is to foreground the challenging work of bridging between goals and implementations so that ML practitioners can confidently explore numerous solution paths and compare their tradeoffs. What we have is a messy, undocumented process where practitioners themselves may not be able to remember all of the reasons underlying their prior design decisions. This makes it exceedingly difficult to not only revisit those past decisions, but to reverse them or explore alternative implementations after a model has already been built and deployed.

Thus, we specifically seek to address the gap between high-level modeling goals and low-level implementation by introducing \textit{concepts}---human-understandable ideas or factors that are relevant to a decision-making task---as an intermediary representation. By foregrounding this translational step between goals and their implementation, we aim to scaffold ML practitioners' reasoning and help them to more effectively sketch out and explore parallel solutions paths. This concept-based intermediary can also make their work in this vein more visible and organized, both to themselves and to other stakeholders.

% Concepts also allow us to meet our design goals of expressivity, minimal detail, and speed
Concepts as a primary abstraction also allow us to meet our design goals of expressivity, minimal detail, and speed. Given that they can relate to all sorts of modalities (including text and images) and can range from concrete and specific to abstract and ideological, concepts provide an expressive lever for specifying model behavior. Then, centering the model authoring process primarily around concepts naturally enforces a much-simplified representation of a model's decision-making logic, achieving minimal detail while ensuring that the detail that remains is central to the core ideas of a modeling approach. Lastly, thanks to improvements in zero-shot modeling, we can interactively generate models that map from data examples to arbitrary concepts without any training time. This means that users can speedily author functional models by simply specifying concepts and stringing them together. We now describe in greater detail how we break down our model sketching framework into concept models and sketch models.

\msb{I think this is where we need to have a paragraph or two explaining how we envision the code or insights from model sketches get applied later in the development process. What are they keeping? What are they tossing? What changes about the full production of the model based on what they learned from the sketch?}

\subsubsection{Data prerequisites}
\msb{Not clear from this paragraph: \textit{how much} data is needed? Enough to train a full DL model, e.g., 10k datapoints?} Our framework has very few data requirements. We simply require a data table (e.g., spreadsheet, CSV, Pandas Dataframe) where each row represents a single example and each column represents a data field. These data fields can contain text, image, or numeric data. Our approach works best when the data is labeled for the desired modeling task (e.g., if the task is hate speech detection, it is ideal for the data table to include a column with labels indicating the the hate speech label or score for each item). These labels allow us to benchmark our sketch model output against a desired point of reference. However, such labels are not required to author sketch models.

\subsubsection{Concept models: Crafting functional building blocks of decision-making}
\msb{This subsubsection and the next are worth looking at from an idea outlining perspective: what idea is each paragraph/sentence really advancing? It felt like there were several areas here, some of which I've highlighted, that have more text than they deserve and it becomes too easy to zone out}

With our method, concepts are the main building blocks that users can use to construct their models. \msb{I would remind the reader of your definition of concepts here}
Concepts are how we decompose the larger and more ambitious task of a sketch model into more manageable, human-understandable components. A concept is meant to capture a smaller factor or idea that is relevant to the modeling task.

\msb{After I got to the end of this paragraph, I wasn't sure what original point it was trying to make that wasn't already discussed elsewhere. Cut?} Ordinarily, even if a model developer has certain concepts in mind, they wouldn't necessarily be able to actualize these concepts in their model. They might have the sense that they want a hate speech classifier to account for racism, sexism, or dehumanization, but the main options they have are to either 1)~gather data examples that cover those concepts and hope that the model picks up on them, or 2)~create a feature extraction pipeline (for more concrete attributes) or sub-model (for more abstract ideas) to clue the model into those concepts \msb{aren't our concepts essentially sub-models? best to emphasize that they'd have to be fully trained models in their own right}. Data curation is a significant endeavor that already can take up to 80\% of the time and effort in a data science project~\cite{muller_HowDataScienceWorkersWorkWithData}, and feature extraction pipelines and additional sub-models similarly require a considerable amount of time and engineering effort to build. All of that work must happen before the model developer can even test out whether those technical methods will sufficiently capture their internal understanding of the concept, let alone whether the concept will provide a sufficiently valuable signal for the decision-making task.

\msb{Cut? Not adding new information} In contrast, the concepts that users author using our model sketching framework are actually \textit{models in themselves}, and creating a concept model is as simple as specifying a word or phrase that describes a concept. This means that a model developer can think of a concept and immediately instantiate it in a functional sub-model that they can incorporate into their modeling task. \msb{This is worth keeping:} We define a concept model as a mapping from a data example to a score that indicates its relevance to the specified concept, or how well it exemplifies that concept~(\autoref{fig:sys_concepts}). For example, a concept model for ``colorful'' might produce scores for a set of images indicating roughly how colorful they are; a concept model for ``profanity'' might produce scores for a set of text comments that estimate how profane they are. Thus, concept models bear similarities to feature extractors, but they are not limited to lower-level, objective attributes, and they require much less time and effort to produce. Once created, a concept model can be applied to any arbitrary example, seen or unseen.

\begin{figure}[!tb]
  \includegraphics[width=\textwidth]{figures/sys_concepts_v1.pdf}
  \caption{
      Concept models enable users to turn human-understandable concepts into functional models. A concept model takes in a concept term and a data field as input. Then, a pretrained zero-shot model produces a score for each example that indicates the extent to which the example relates to the specified concept. We adapt our underlying approach depending on the inferred type of the data field. For text, we leverage GPT-3 prompts for zero-shot classification. For images, we leverage CLIP embeddings for zero-shot regression.
  }
  \label{fig:sys_concepts}
\end{figure}

We build upon advances in zero-shot modeling to instantiate our vision of concept models. Zero-shot modeling describes any machine learning modeling approach that does not require any training examples to perform a task. Given an input concept term (a brief word or phrase) and a data field (column name) from the dataset, we author a zero-shot model that maps from the provided data to the specified concept idea to produce a concrete score.
\msb{cut?: }The benefit of this approach is that it does not require any labeled examples and does not require any training time to produce its output predictions. Given our design constraints that aim to provide interactive model outputs to users, zero-shot models are an ideal choice. 

For our concept models, we implement two zero-shot modeling methods: 1)~zero-shot text classification via large language model prompting using GPT-3 and 2)~zero-shot image regression via embedding similarity with a pre-trained image-to-text model using CLIP. We describe our technical approach in greater depth in Section~\ref{section:concept_technical}. While we choose these two zero-shot method in our work, we design our model sketching framework to be compatible with any current or future zero-shot modeling method. \msb{cut rest of paragraph:} Our approach works with any method that takes in images or text as input and is capable of producing concept relevance scores or labels at interactive speeds with no additional training data. As these technologies improve and become increasingly accessible, we envision that users will be able to leverage more advanced and specialized pretrained models to serve model sketching. These future models may achieve higher performance or may better capture domain-specific information necessary for targeted applications areas such as medicine, law, and the natural sciences.

\subsubsection{Sketch models: Putting concepts together to envision decision-making outcomes}
\msb{stray thought: in the related work, or in the design section here, can we draw on Sharad's paper on adding points as interpretable approximations of ML models? And argue that's what we're doing here with the composite models?}
The second component of our model sketching framework involves aggregating these concepts together to form sketches. 
Without concept models as an intermediary, ML practitioners usually have to map directly from raw data (i.e., resume text) to their modeling outcomes (i.e., a ranked list of promising job applicants). They can tweak model architectures, perform data processing, try out alternate loss functions, and adjust hyperparameters, but these modifications are largely uninterpretable and leave the model as a black box. With the introduction of concept models, ML practitioners can now shift to iterate on their models in terms of human-understandable concepts instantiated in concept models that they themselves brainstormed, authored, and tuned.

A sketch model is a lightweight, rapidly-authored  machine learning model that works by aggregating the signals produced by concept models~(\autoref{fig:sys_sketches}). It is designed to accomplish the same task as the full model that it is meant to emulate, so it expects the same inputs and produces the same class of outputs.
Once the user has authored a set of constituent concepts that are relevant to the decision-making task, they can combine the concepts together to produce a sketch model by selecting which concepts they'd like to combine. We provide an initial set of aggregators that can combine concept model scores to produce a single sketch model score: linear regression, logistic regression, decision tree classification, random forest classification, and multi-layer perceptron (MLP) classification. However, we are again not bound to this initial set of aggregators; sketch models are compatible with any aggregation method that can accept multiple concept scores and produce a holistic output score. 
% Sketch model is trained on provided labels, but can be specified more manually if desired
We use the ground-truth labels provided in the training dataset to train these aggregators when a sketch model is created; all subsequent runs of the sketch model will simply evaluate the trained model on new input data. If the dataset does not have labels, then the user can opt to provide manual weights for the concepts using the linear regression aggregator.

\begin{figure}[!tb]
  \includegraphics[width=0.9\textwidth]{figures/sys_sketches_v1.pdf}
  \caption{
      Sketch models combine concepts together to create an overall model for the decision-making task. Here, we show an example for a hateful post detection task. First, the user chooses from among the concepts they've authored and decides on an aggregation method. We then create a new sketch model by generating the concept scores and training a model using the specified aggregation method and user's provided ground-truth ratings (e.g., ratings of the hatefulness of posts). Once authored, the sketch model can produce predictions (e.g., scores estimating the hatefulness of posts) for any arbitrary example.
  }
  \label{fig:sys_sketches}
\end{figure}

\msb{cut?} Using the specified concepts and aggregation method, our approach produces a sketch model that can generate a score for any arbitrary input example. The concept models operate on the example to generate their individual concept scores, and the sketch model applies the aggregator to these concept scores to produce the overall score.

With the sketch-model layer of abstraction, ML practitioners can focus their attention on experimenting with different combinations of concepts to create sketches that might capture different sets of values in decision-making. For example, when authoring a hate speech detection model, an ML practitioner may experiment with sketches that focus on race-related or gender-related hate speech, or approaches that explicitly account for intersectionality; they may try out sketches that take a lenient stance unless the speech incites violence, or they may experiment with sketches that take a more strict stance on profanity and slurs \msb{I was getting ready to say that this paragraph repeats ideas from before and should be cut. But the idea of experimenting with sketches that take a more strict stance on profanity and slurs caught my eye. It makes me want to know: how do they make the model get more strict or lenient? How do they control the sketch model behavior?}. By rapidly authoring sketch models and testing them on new data examples, ML practitioners can quickly discover cases where their modeling approach appears to fail. Through inspection of sketch model behavior, they can get inspiration for new concepts that may help them to address gaps in their model, and they can immediately author and incorporate those new concepts. They may also discover gaps in the larger modeling ecosystem---for example, cases where the current data fields do not provide enough information to glean a certain concept, cases where the dataset lacks representation of a certain important phenomenon, or cases where the data labeling scheme is inconsistent or lacks the necessary granularity to separate classes.

% Compatibility with existing features/model outputs
While sketch models in their most stylized form are comprised entirely of concept models, sketch models are also compatible with other, more traditional kinds of features. If a model developer has raw or pre-processed features from an existing feature extractor or data pipeline, they can also incorporate those features and aggregate them into a sketch model. If an engineering team already has an existing version of a model or sub-models that produce scores that may be helpful for the decision-making task, they can also incorporate those scores as inputs to a sketch model.

\subsection{The ModelSketchBook tool}
To instantiate our model sketching framework, we introduce the \texttt{ModelSketchBook} API, a Python package that allows ML practitioners to create concepts and sketches of their own. Our package will be made open-source and is available in a public Github repository.\footnote{https://github.com/REDACTED (currently a private repository during review)}
\texttt{ModelSketchBook} is just one example of how we might instantiate our model sketching framework. For example, we envision that one could implement a version with a dedicated graphical user interface to serve the needs of non-technical users, or a version that uses zero-shot video models to target a use-case related to video content.

\subsubsection{Environment and setup}
% Why we selected a notebook environment; our target demographic
The \texttt{ModelSketchBook} API can be loaded in any Python environment, but it is optimized for use in a computational notebook such as Jupyter or CoLab. We chose to tailor our API design to the notebook environment because this is where many ML practitioners and data scientists already carry out much of their exploratory modeling work~\MSLcite{ work on computational notebooks}. \msb{cut, already implied by prior sentences:}We sought to intervene and provide a sketching tool in the environment where it could provide the most value to our target audience of ML practitioners.

% Setting up the sketchbook and data
After loading in their dataset into a Pandas dataframe and importing the \texttt{ModelSketchBook} package in their notebook, the user can run a brief function to set up their sketchbook with the dataframe(s) and their associated data schema. We recommend that users provide a smaller set of examples (on the order of 20-50) for use during model sketching, as this limited dataset size allows the data to better serve as point of reference to facilitate creative iteration, rather than a distractor that might overwhelm them. \msb{I wonder, though, would people over-anchor on the errors in such a small dataset?}

% df_train = pd.read_csv("train.csv")
% df_test = pd.read_csv("test.csv")
\begin{minted}[fontsize=\footnotesize,samepage]{python}
    import model_sketch_book as msb

    # Set up the sketchbook
    sb = msb.create_model_sketchbook(
        goal="Detect hateful memes on social media.",
        datasets={  # Pass in datasets to use
            "train": df_train,
            "test": df_test,
        },
        schema = {  # Specify the types of data fields, including the ground-truth column
            "text": InputType.Text,
            "img_url": InputType.Image,
            "overall_rating": InputType.GroundTruth,
        },
    )
\end{minted}

The sketchbook contains all of the datasets, concepts, and sketches that the user will author during their session, and it saves other metadata such as model output scores, performance metrics, and the history of the concepts and sketches in the sketchbook.

\subsubsection{Creating concepts: under the hood}
\label{section:concept_technical}
As mentioned previously, we specifically support text concepts powered by GPT-3 and image concepts powered by CLIP.
To achieve zero-shot text classification, we author prompts that list a batch of examples for the model to classify and ask the model to decide on a binary label (``<concept term>'' or ``not <concept term>'') for each provided example. Large language models like GPT-3 are designed to perform text completion on provided input prompts, so plausible completions provided by the model capture a rough sense of binary labels that might be reasonable based on the knowledge available to the model. We include an example prompt below.

\begin{minted}[fontsize=\small,samepage]{markdown}
        Decide whether these comments are "motivational" or "not motivational".
        1. You can do it!!
        2. Ugh, you're the worst.
        3. I'm so tired...
    
        Comment results:
\end{minted}

The GPT-3 model will then return a text completion response similar to this that provides a label for the examples. We parse and post-process this GPT-3 response to retrieve binary labels.
\begin{minted}[fontsize=\small,samepage]{markdown}
        1. motivational
        2. not motivational
        3. not motivational
\end{minted}

To carry out zero-shot image classification, we use CLIP (Contrastive Language-Image Pre-Training)~\cite{CLIP}, a neural network trained on (image, text) pairs that allows images and text to be represented in a shared embedding space. Given a data field containing images and a concept term, we use CLIP to encode both the image and the concept term in that shared image-text embedding space. Then, we calculate and return the cosine similarity between the embedded image and concept term. Thus, the output score approximately captures the extent to which the given image relates to the specified concept term. We also allow users to normalize and re-calibrate these similarity scores to match their internal understanding of the concept, and we also grant users the ability to apply a custom threshold to binarize these continuous concept scores.

\subsubsection{Creating concepts with the API}
After setting up the sketchbook, users can freely author concepts. While we also provide raw API functions under the hood, for convenience, we surface simple UI elements via ipywidgets\footnote{\url{http://ipywidgets.readthedocs.io}} that allow for interactive controls in IPython notebooks. These widgets make it much simpler for new users to make sense of the available function parameters and the eligible input options for each parameter. The user can \msb{I've cut a couple ``simply''s in the paper, here's another one. I generally avoid saying things like simply, highly usable, etc., since I think it makes the reader cynical ``well, I don't agree that it's so simple!''. We can just say what it is, and let them decide it's simple.} simply make the function call \texttt{create\_concept\_model()}, and a set of widgets will appear that allow the user to specify the input field, a concept term, and other details like the output type of the concept model~(\autoref{fig:sys_api_concepts}~\circled{A}).

\begin{figure}[!tb]
  \includegraphics[width=\textwidth]{figures/sys_api_concepts_v1.pdf}
  \caption{
      Creating concepts with the \texttt{ModelSketchBook} API. 
      (A)~The \texttt{create\_concept\_model()} function accepts user inputs for the data input field, the concept term, and other settings. 
      (B)~Then, our API returns an output dataframe that displays all training examples sorted by their concept score. 
      (C)~We provide a suite of helper functions that assist users in finetuning and making sense of existing concepts as well as brainstorming new concepts. 
      (D)~We also provide functions that allow users to apply logical \texttt{AND} and \texttt{OR} operators to manually link different concepts together. \msb{I'd make A and B wider, and shrink C and D a little bit. Or, move C and D onto a separate short row below A and B, so that A and B get larger. Currently, A and B are too small to read}
  }
  \label{fig:sys_api_concepts}
\end{figure}

Once the user enters in those details, they can execute the cell; after several seconds, the API returns a dataframe visualization that displays a sorted view of the examples in the training dataset along with their concept score~(\autoref{fig:sys_api_concepts}~\circled{B}). The user can browse through the concept score results to determine whether the model's understanding of the concept sufficiently aligns with their own. If not, they can try out other concept terms or experiment with other input fields to work towards better alignment.

The API also includes additional features for users to binarize continuous scores using a custom threshold value, auto-normalize continuous scores to a 0-1 score range, or custom-calibrate continuous scores based on a specified minimum and maximum score value. These features allow the user to bring the raw concept scores in closer alignment with their own personal understanding of a concept.

We also provide functions that assist users as they brainstorm and evaluate tradeoffs among different concepts. A brainstorming helper function surfaces synonyms or antonyms of a provided word to spur ideas when users seek to verbalize or refine their concept. Meanwhile, a concept comparison helper function allows users to specify two concept terms and see a side-by-side comparison of their respective correlation with the input data and ground-truth ratings. To help scaffold users' sensemaking process, we also provide a note-taking function that allows them to write and save scratch notes on concepts and sketches for future reference.

% AND and OR logical operators for concepts
Finally, to allow for further control and refinement of concepts, we enable users to link existing concepts together with logical \texttt{AND} and \texttt{OR} operators. With a call to \texttt{create\_AND\_concept()}, users can take the logical \texttt{AND} of any number of binary concepts (and can similarly link arbitrary concepts with an \texttt{OR} relation using the \texttt{create\_OR\_concept()} function). This grants users the ability to better link concepts that interact with one another such as a single concept that can manifest in several ways or a multimodal concept that requires semantics from both image and text.

\subsubsection{Creating sketches with the API}
Once a user has authored several concepts, they can proceed to create sketches that aggregate those concepts by calling \texttt{create\_sketch\_model()}. This function will again display a set of widgets that allow the user to select all of the concepts that they would like to use in the sketch model as well as an optional aggregation method (linear regression is the default)~(\autoref{fig:sys_api_sketches}~\circled{A}).

\begin{figure}[!tb]
  \includegraphics[width=\textwidth]{figures/sys_api_sketches_v1.pdf}
  \caption{
      Authoring sketches with the \texttt{ModelSketchBook} API. 
      (A)~The \texttt{create\_sketch\_model()} function accepts user inputs to gather the concepts that the user would like to aggregate as well as optional parameters to set the aggregation method and sort-column.
      (B)~Then, the API returns an output dataframe that displays all training examples sorted by the specified column. This view shows all of the input fields, all of the concept scores, and the sketch model's prediction. It also displays the ground truth rating and the error between the sketch prediction and ground truth rating to help users discover where the sketch model deviated from their ratings.
      \msl{Note: may need to change the image/text examples; just using those as placeholders for now} \msb{I'm on a large display and still can't read the text in this figure. I recommend not letting any text you care about in figures get any smaller than the body text of the paper. Right now, the important stuff looks like it's a at font size one half the body text.}
  }
  \label{fig:sys_api_sketches}
\end{figure}

After executing the cell, the API creates the new sketch model and returns a dataframe visualization that displays all of the input fields of the training examples, all of the relevant concept scores, and the overall prediction produced by the sketch model~(\autoref{fig:sys_api_sketches} \circled{B}). This view also includes the ground-truth ratings and the difference between the sketch prediction and these ground-truth ratings. Users can choose to sort by various columns to aid their understanding of the model outputs: sorting by the sketch prediction surfaces an ordering that represents of the sketch model's understanding of the modeling task; sorting by the ground-truth rating foregrounds the ``intended'' understanding of the modeling task; sorting by the difference (or absolute value of difference) between the sketch prediction and ground-truth rating highlights areas where the sketch model most drastically deviated from the intended decision-making behavior. The sketch model output also displays more traditional performance metrics for both regression and classification formulations of the task based on the ground-truth labels and the training examples; we display Mean Absolute Error (MAE), Classification Accuracy, F1 Score, Precision, and Recall.

% Evaluating sketch on unseen data
Finally, the API provides helper functions that help the user to better compare their sketch models. The \texttt{compare\_sketches()} function allows the user to compare the performance metrics for specified sketches, and the \texttt{test\_sketch()} function allows them to test out sketch models on a labeled or unlabeled validation set (if one is provided) to get a sense for how well it generalizes to a broader set of examples.

\subsubsection{Implementation}
% More detailed implementation details/settings; Colab setup
The \texttt{ModelSketchBook} API was authored entirely in Python. We use OpenAI's API for GPT-3 to perform zero-shot prompt-based text classification and use the \texttt{text-davinci-002} model, the current state-of-the-art GPT-3 variant. We use OpenCLIP~\cite{open_clip}, an open-source version of CLIP, to perform zero-shot image regression; we use a Vision Transformer (ViT) model (\texttt{ViT-B-32-quickgelu}) pre-trained on the \texttt{laion400m\_e32} dataset. We use the scikit-learn~\cite{scikit_learn} implementations of linear regression, logistic regression, decision tree classification, random forest classification, and MLP classification for our sketch model aggregators. \msb{probably worth getting explicit for one sentence about what training and inference is done on the local machine and what is done via API in the cloud}


==> sections/old_versions/3_system_v3.tex <==
% v3 9/10/22, post-MSB comments

In this section, we describe our model sketching framework, which aids ML practitioners in moving beyond technical implementation to explore the conceptual model design space during early phases of ML model development.

\subsection{Design goals}
\msb{I think you should cut this subsection. The three goals were just covered in a fair amount of depth in Related Work. If there are particular sentences you like, you could move them up into RW?}
% \msl{TODO: mention that we aim to intervene in the early phases of model development; NOTE: might move some of this up to Related Work}

Inspired by the practice of sketching in design, we seek for our approach to capture the core elements of sketching outlined in Section~\ref{section:sketch_characteristics}---expressivity, minimal detail, and speed~\cite{buxton2010sketching}. 
% that successfully enable a practitioner to shift their thinking from a mode of implementation and execution to one that explores parallel designs and approaches. 
% \msb{If these are key, I'd use them up in the intro as well when explaining why prior work hasn't crossed this chasm yet} 
% The key attributes that we seek to emulate are expressivity, minimal detail, and speed~\cite{buxton2010sketching}. 
For ML model authoring, \textit{expressivity} would require the flexibility to communicate ideas by drawing upon visual and textual ideas of varying concreteness or abstraction.
% \msb{would we say that supervised ML training has no expressivity, or very high expressivity? worth anchoring the reader's understanding here.}
Meanwhile, \textit{minimal detail} would ideally mean paring down from fully-implemented technical modeling infrastructures to simple representations that convey the core logic, ideas, or values that distinguish one modeling approach from another. 
Finally, typical machine learning model turnaround times can range from hours or days to weeks or months, and this work is often split across multiple people or even multiple teams. To reach a sufficient \textit{speed} comparable to pencil-and-paper sketching, model authoring would need to happen at interactive speeds, which means that model results should appear within seconds of user input.
% and it should be possible for a single user to author sketches on their own.

These three factors together would enable an effective sketching practice that would focus an ML practitioner's efforts on the work that will produce the richest cognitive and communicative benefit. 
% We thus aim to embed these three critical elements in our model sketching method.

% \subsection{Motivating scenario}
% TODO: walkthrough of what it would look like to author a sketch model (may not be necessary if we do case studies in the next section)

\subsection{The Model Sketching Framework}
\msb{The first two paragraphs were wordy and repeating ideas from the intro. So, I tried condensing it here: 
Model sketching facilitates the translational, interpretational work that goes in between a high-level description and any particular low-level implementation~\cite{passi_barocas_problemFormulationFairness,jacobs_wallach_measurementAndFairness}.
This work charts a path through the multitude of plausible strategies for any one high-level modeling goal, and ossifies a set of human values and ethical implications that are encoded into the model.
What we \textit{want} is to foreground this challenging translational work so that ML practitioners can confidently explore numerous solution paths and compare their tradeoffs. What we \textit{have} is a messy, undocumented process where practitioners themselves may not be able to remember all of the reasons underlying their prior design decisions.
}

% We wanted to fill the gap between high-level modeling goals and low-level implementation --> arrived at intermediate goals/representations in the form of concepts
Currently, ML practitioners commonly capture their modeling work through 1)~high-level descriptions like written documents or presentations stating the goal of a given model~\cite{piorkowski_AIDevelopersCommChallenges} or 2)~low-level implementations like computational notebooks or code repositories with data processing, feature extraction, and modeling logic~\cite{rule_explorationExplanationCompNotebooks}. However, there is a significant amount of translational, interpretational work that goes in between a high-level description and any particular low-level implementation~\cite{passi_barocas_problemFormulationFairness,jacobs_wallach_measurementAndFairness}. This work may in fact be the most critical piece of the modeling task to get right given that there is a vast design space of plausible solution strategies for any one high-level modeling goal. Furthermore, these different approaches carry different sets of human values and ethical implications, which is especially important to consider when designing human-facing deployments of machine learning. There is not just one clear solution, and the choice among solutions is not arbitrary, especially in terms of user impact. 

Since current approaches primarily cover only high-level goals or low-level technical instantiations, this important intermediate work remains hidden in the depths of experimental scripts, disorganized notebooks, or even internal reasoning that may never have been documented in any form~\cite{zhang_howDoDataScienceWorkersCollaborate}. What we \textit{want} is to foreground the challenging work of bridging between goals and implementations so that ML practitioners can confidently explore numerous solution paths and compare their tradeoffs. What we have is a messy, undocumented process where practitioners themselves may not be able to remember all of the reasons underlying their prior design decisions. This makes it exceedingly difficult to not only revisit those past decisions, but to reverse them or explore alternative implementations after a model has already been built and deployed.

Thus, we specifically seek to address the gap between high-level modeling goals and low-level implementation by introducing \textit{concepts}---human-understandable ideas or factors that are relevant to a decision-making task---as an intermediary representation. By foregrounding this translational step between goals and their implementation, we aim to scaffold ML practitioners' reasoning and help them to more effectively sketch out and explore parallel solution paths. This concept-based intermediary can also make their work in this vein more visible and organized, both to themselves and to other stakeholders.

% Concepts also allow us to meet our design goals of expressivity, minimal detail, and speed
\msb{shorter version, I got rid of some of the buxton criteria explicitness:
Centering the model authoring process around concepts enforces a simplified representation of a model's decision-making logic, achieving minimal detail while ensuring that the detail that remains is central to the core of a modeling approach. The availability of zero-shot modeling enables interactive mapping from data examples to arbitrary concept scores without any training time, expressively covering several modalities (including text and images) and ranging from concrete and specific to abstract and ideological.
}

Concepts as a primary abstraction also allow us to meet our design goals of expressivity, minimal detail, and speed. Given that they can relate to a variety of modalities (including text and images) and can range from concrete and specific to abstract and ideological, concepts provide an expressive lever for specifying model behavior. Then, centering the model authoring process primarily around concepts naturally enforces a much-simplified representation of a model's decision-making logic, achieving minimal detail while ensuring that the detail that remains is central to the core ideas of a modeling approach. Lastly, thanks to improvements in zero-shot modeling, we can interactively map from data examples to arbitrary concept scores without any training time. This means that users can speedily author functional building blocks by specifying concepts and stringing them together. 
We now describe in greater detail how we break down our model sketching framework into concepts and sketch models.

% \msb{I think this is where we need to have a paragraph or two explaining how we envision the code or insights from model sketches get applied later in the development process. What are they keeping? What are they tossing? What changes about the full production of the model based on what they learned from the sketch?}
% \msl{I think I'll put this after I describe both concepts and sketch models so it'll make a bit more sense!}

\subsubsection{Data prerequisites}
We require a data table (e.g., spreadsheet, CSV, Pandas Dataframe) where each row represents a single example and each column represents a data field. These data fields can contain text, image, or numeric data. 
We require a dataset with at least 40-50 rows to aid sensemaking during model development, but allow for a split between training and test data.
If the user provides test labels, our system can help with sensemaking around model accuracy; however, such labels are not required.%Our approach works best when the data is labeled for the desired modeling task (e.g., if the task is hate speech detection, it is ideal for the data table to include a column with labels indicating the the hate speech label or score for each item). These labels allow us to benchmark our sketch model output against a desired point of reference. However, such labels are not required to author sketch models.

\subsubsection{Concepts: Crafting functional building blocks of decision-making}
%With our method, concepts---human-understandable ideas related to a decision-making task---are the main building blocks that users can use to construct their models. 
Concepts---human-understandable ideas related to a decision-making task---are how we decompose the larger and more ambitious task of a sketch model into more manageable, human-understandable components.
We turn concepts into functional components by mapping from a data example to a score that indicates its relevance to the specified concept, or how well it exemplifies that concept~(\autoref{fig:sys_concepts}). For example, a concept for ``colorful'' might produce scores for a set of images indicating roughly how colorful they are; a concept for ``profanity'' might produce scores for a set of text comments that estimate how profane they are. Thus, concepts bear similarities to feature extractors, but they are not limited to lower-level, objective attributes, and they require much less time and effort to produce. Once created, a concept can be applied to any arbitrary example, seen or unseen.

\begin{figure}[!tb]
  \includegraphics[width=\textwidth]{figures/sys_concepts_v1.pdf}
  \caption{
      Concepts enable users to turn human-understandable concepts into functional building blocks. A concept takes in a concept term and a data field as input. Then, a pretrained zero-shot model produces a score for each example that indicates the extent to which the example relates to the specified concept. We adapt our underlying approach depending on the inferred type of the data field. For text, we leverage GPT-3 prompts for zero-shot classification. For images, we leverage CLIP embeddings for zero-shot regression.
  }
  \label{fig:sys_concepts}
\end{figure}

We build upon advances in zero-shot modeling to instantiate concepts. Zero-shot modeling describes any machine learning modeling approach that does not require any training examples to perform a task. To create a concept, the user provides an input concept term (a brief word or phrase) and a data field (column name) from their dataset. Our framework then authors authors a zero-shot model that maps from the provided data and can output a numeric score for that concept for every item in the dataset.

% \msb{cut?: }The benefit of this approach is that it does not require any labeled examples and does not require any training time to produce its output predictions. Given our design constraints that aim to provide interactive model outputs to users, zero-shot models are an ideal choice. 
For our concepts, we implement two zero-shot modeling methods: 1)~zero-shot text classification via large language model prompting using GPT-3 and 2)~zero-shot image regression via embedding similarity with a pre-trained image-to-text model using CLIP. We describe our technical approach in greater depth in Section~\ref{section:concept_technical}. While we choose these two zero-shot methods in our work, we design our model sketching framework to be compatible with any current or future zero-shot modeling method. 

\subsubsection{Sketch models: Putting concepts together to envision decision-making outcomes}
The second component of our model sketching framework involves aggregating these concepts together to form sketches. 
%Without concepts as an intermediary, ML practitioners usually have to map directly from raw data (i.e., resume text) to their modeling outcomes (i.e., a ranked list of promising job applicants). They can tweak model architectures, perform data processing, try out alternate loss functions, and adjust hyperparameters, but these modifications are largely uninterpretable and leave the model as a black box. With the introduction of concepts, ML practitioners can now shift to iterate on their models in terms of human-understandable concept building blocks that they themselves brainstormed, authored, and tuned.
A sketch model is a lightweight, rapidly-authored  machine learning model that works by aggregating the signals produced by concepts~(\autoref{fig:sys_sketches}). It is designed to accomplish the same task as the full model that it is meant to emulate, so it expects the same inputs and produces the same class of outputs.

Once the user has authored a set of constituent concepts that are relevant to the decision-making task, they select which concepts they'd like to combine into a sketch model. We provide an initial set of aggregators that can combine concept scores to produce a single sketch model score: linear regression, logistic regression, decision tree classification, random forest classification, and multi-layer perceptron (MLP) classification. 
We build on prior research that demonstrated how simple linear models built on small sets of human-interpretable features can achieve impressive performance---exceeding that of human decision-makers and rivaling that of complex prediction models~\cite{jung_goel_simpleRulesExpertClassification}.
However, we are not bound to this initial set of aggregators; sketch models are compatible with any aggregation method that can accept multiple concept scores and produce a holistic output score. 
% Sketch model is trained on provided labels, but can be specified more manually if desired
We use the ground-truth labels provided in the training dataset to train these aggregators when a sketch model is created; all subsequent runs of the sketch model will evaluate the trained model on new input data. If the dataset does not have labels, then the user can opt to provide manual weights for the concepts using the linear regression aggregator.

\begin{figure}[!tb]
  \includegraphics[width=0.9\textwidth]{figures/sys_sketches_v1.pdf}
  \caption{
      Sketch models combine concepts together to create an overall model for the decision-making task. Here, we show an example for a hateful post detection task. First, the user chooses from among the concepts they've authored and decides on an aggregation method. We then create a new sketch model by generating the concept scores and training a model using the specified aggregation method and user's provided ground-truth ratings (e.g., ratings of the hatefulness of posts). Once authored, the sketch model can produce predictions (e.g., scores estimating the hatefulness of posts) for any arbitrary example.
  }
  \label{fig:sys_sketches}
\end{figure}

% \msb{cut?} Using the specified concepts and aggregation method, our approach produces a sketch model that can generate a score for any arbitrary input example. The concept models operate on the example to generate their individual concept scores, and the sketch model applies the aggregator to these concept scores to produce the overall score.

With the sketch-model layer of abstraction, ML practitioners can focus their attention on experimenting with different combinations of concepts to create sketches that might capture different sets of values in decision-making. For example, when authoring a hate speech detection model, an ML practitioner may experiment with sketches that focus on race-related or gender-related hate speech, or approaches that explicitly account for intersectionality. They may try out sketches that take a relatively lenient stance by only adding a concept related to speech that incites violence, or they may experiment with sketches that take a more strict stance on profanity by adding concepts for swearing and slurs. 
By rapidly authoring sketch models and testing them on new data examples, ML practitioners can quickly discover cases where their modeling approach appears to fail. Through inspection of sketch model behavior, they can get inspiration for new concepts that may help them to address gaps in their model, and they can immediately author and incorporate those new concepts. They may also discover gaps in the larger modeling ecosystem---for example, cases where the current data fields do not provide enough information to glean a certain concept, cases where the dataset lacks representation of a certain important phenomenon, or cases where the data labeling scheme is inconsistent or lacks the necessary granularity to separate classes.

% Compatibility with existing features/model outputs
While sketch models in their most stylized form are comprised entirely of concepts, sketch models are also compatible with other, more traditional kinds of features. If a model developer has raw or pre-processed features from an existing feature extractor or data pipeline, they can also incorporate those features and aggregate them into a sketch model. If an engineering team already has an existing version of a model or sub-models that produce scores that may be helpful for the decision-making task, they can also incorporate those scores as inputs to a sketch model.

% From sketches to production models
\subsubsection{From sketch models to production models}
\label{section:sketch_to_production}
\msb{I cut some stuff here to condense}
% how sketches apply to later development process
% What they keep, what they toss
% What changes about full production model based on sketch
While sketch models initially serve as tools for thinking during early model development phases, we envision that they will directly inform the design of full production models. 

% Decomposition
First, a key part of full-scale model design involves deciding how to \textit{decompose the model} into smaller parts. An important characteristic of successful production ML systems---consistent across use cases like feed ranking and content moderation and across platforms like Facebook, LinkedIn, and Reddit---is that they are composed of smaller, more targeted ML models whose outputs are synthesized into a single score, often via weighted linear combination~\cite{eckles_2022, reddit_moderator_tools, linkedin_dwell_time}. While aggregating various signals seems simplistic, it is highly performant in real-world decision-making contexts~\cite{jung_goel_simpleRulesExpertClassification}, and for systems as large and complex as the production ML systems we see in industry, it is important that the signals remain interpretable and tuneable as models and users constantly evolve. %Thus, even as ML teams implement complex black box models that act on raw, uninterpretable features, these are models generally still produce human-understandable scores that may, for example, predict the likelihood that a comment has profanity or the likelihood that a photo contains violence. 
In other words, the sub-models that ML practitioners produce in industry are more complex versions of our concepts, but they typically still boil down to a human-understandable decision-making factor that will be synthesized into a single overall prediction via an aggregation process. Thus, a sketch model lays a direct blueprint for how to decompose a modeling problem into sub-models that will be aggregated together.

% Data requirements
Second, a substantial part of model development (up to 80\% by some estimates) is actually consumed by data cleaning and wrangling, and ML practitioners play an active role in shaping, curating, and designing data~\cite{muller_HowDataScienceWorkersWorkWithData}. Model sketching helps to refine \textit{data requirements} by drawing out what kind of data is necessary for the task based on the concepts that the model must reason over. By testing out concepts on different data fields (e.g., different text or image fields), ML practitioners gain develop a quick understanding of what forms of data are most valuable or informative to serve different concepts and, ultimately, what data fields should be required for the modeling task. 
%For example, they may find that the concepts they care most about for the modeling task tend to be most easily gleaned from the image of a social media post rather than the text, so they may realize that they need to focus more of their data-wrangling efforts on extracting a high-quality image representation.
Testing out concepts on preliminary data versions also surfaces gaps in the representativity of the data. For example, if an ML practitioner tests out a ``weapon'' concept for a hateful post detection task and finds few matches, they may realize that their current dataset has too few examples of military- or violence-related content and can set out to augment the dataset accordingly. %By the end of the model sketching process, the ML practitioner should have a much clearer sense of the specific data fields and the kinds of data representativity that they will need for their full-scale model.

% Labeling and Scoring
\msb{I agree with this, but it's not as central to scaling up to a full model, so could cut entirely}
Finally, model sketching helps to clarify the \textit{labeling or scoring procedure} for a machine learning task. Since decision-making goals are typically underspecified, labeling schemes must evolve over time to capture unanticipated, ambiguous categories~\cite{kulesza_conceptEvolution}. %If not accounting for this concept evolution, labeling policies become inconsistent and illogical, which greatly undermines the performance of any model that builds on top of the resulting labels. 
Model sketching directly engages ML practitioners in this process of concept iteration and has them constantly review both constituent concept scores and aggregate sketch model predictions against provided ground truth ratings. Thus, practitioners can rapidly identify and correct cases where any of these scores, predictions, or ratings are misaligned with their understanding of a concept or of the higher-level decision-making task. 
%Through this process, they may discover that the provided ground-truth ratings are internally inconsistent and require re-labeling, or they may discover that the choice to binarize scores at a $0.5$ threshold results in too little granularity since most scores fall below $0.5$, so a different threshold should be chosen. The insights that ML practitioners gain from iterating on the labeling and scoring schemes in sketch models directly inform the standards that should be used for the full-scale modeling task.


\subsection{The ModelSketchBook tool}
To instantiate our model sketching framework, we introduce the {ModelSketchBook} API, a Python package that allows ML practitioners to create concepts and sketches of their own. Our package will be made open-source and is available in a public Github repository.\footnote{https://github.com/REDACTED (currently a private repository during review)}
\msb{cut the rest of the paragraph}
%{ModelSketchBook} is just one example of how we might instantiate our model sketching framework. For example, we envision that one could implement a version with a dedicated graphical user interface to serve the needs of non-technical users, or a version that uses zero-shot video models to target a use-case related to video content.

\subsubsection{Environment and setup}
% Why we selected a notebook environment; our target demographic
The {ModelSketchBook} API can be loaded in any Python environment, but it is optimized for use in a computational notebook such as Jupyter or Colab. We chose to tailor our API design to the notebook environment because this is where many ML practitioners and data scientists already carry out much of their exploratory modeling work~\cite{rule_explorationExplanationCompNotebooks,zhang_howDoDataScienceWorkersCollaborate}. 
% \msb{cut, already implied by prior sentences:}We sought to intervene and provide a sketching tool in the environment where it could provide the most value to our target audience of ML practitioners.

% Setting up the sketchbook and data
\msb{I cut this paragraph, the dataset requirements were described above and I don't think this is critical, I smoothed it in with some content in the next paragraph:} %After loading in their dataset into a Pandas dataframe and importing the {ModelSketchBook} package in their notebook, the user can run a brief function to set up their sketchbook with the dataframe(s) and their associated data schema. We recommend that users provide a smaller set of examples (on the order of 20-50) for use during model sketching, as this limited dataset size allows the data to better serve as point of reference to facilitate creative iteration, rather than a distractor that might overwhelm them. 

% df_train = pd.read_csv("train.csv")
% df_test = pd.read_csv("test.csv")
\begin{minted}[fontsize=\footnotesize,samepage]{python}
    import model_sketch_book as msb

    # Set up the sketchbook
    sb = msb.create_model_sketchbook(
        goal="Detect hateful memes on social media.",
        datasets={  # Pass in datasets to use
            "train": df_train,
            "test": df_test,
        },
        schema = {  # Specify the types of data fields, including the ground-truth column
            "text": InputType.Text,
            "img_url": InputType.Image,
            "overall_rating": InputType.GroundTruth,
        },
    )
\end{minted}

After loading in their dataset into a Pandas dataframe and importing the {ModelSketchBook} package in their notebook, the user sets up a ModelSketchBook sketchbook in their notebook. The sketchbook contains all of the datasets, concepts, and sketches that the user will author during their session, and it saves other metadata such as model output scores, performance metrics, and the history of the concepts and sketches in the sketchbook.

\subsubsection{Creating concepts: under the hood}
\label{section:concept_technical}
As mentioned previously, we specifically support text concepts powered by GPT-3 and image concepts powered by CLIP.
To achieve zero-shot text classification, we author prompts that list a batch of examples for the model to classify and ask the model to decide on a binary label (``<concept term>'' or ``not <concept term>'') for each provided example. Large language models like GPT-3 are designed to perform text completion on provided input prompts, so plausible completions provided by the model capture a rough sense of binary labels that might be reasonable based on the knowledge available in the model. We include an example prompt below.

\begin{minted}[fontsize=\small,samepage]{markdown}
        Decide whether these comments are "motivational" or "not motivational".
        1. You can do it!!
        2. Ugh, you're the worst.
        3. I'm so tired...
    
        Comment results:
\end{minted}

The GPT-3 model will then return a text completion response similar to this that provides a label for the examples. We parse and post-process this GPT-3 response to retrieve binary labels.
\begin{minted}[fontsize=\small,samepage]{markdown}
        1. motivational
        2. not motivational
        3. not motivational
\end{minted}

To carry out zero-shot image classification, we use CLIP (Contrastive Language-Image Pre-Training)~\cite{CLIP}, a neural network trained on (image, text) pairs that allows images and text to be represented in a shared embedding space. Given a data field containing images and a concept term, we use CLIP to encode both the image and the concept term in that shared image-text embedding space. Then, we calculate and return the cosine similarity between the embedded image and concept term. Thus, the output score approximately captures the extent to which the given image relates to the specified concept term. We also allow users to normalize and re-calibrate these similarity scores to match their internal understanding of the concept, and we also grant users the ability to apply a custom threshold to binarize these continuous concept scores.

\subsubsection{Creating concepts with the API}
After setting up the sketchbook, users can freely author concepts. While we also provide raw API functions under the hood, for convenience, we surface UI elements via ipywidgets\footnote{\url{http://ipywidgets.readthedocs.io}} that allow for interactive controls in IPython notebooks. These widgets clarify the available function parameters and the eligible input options for each parameter. The user can make the function call \texttt{create\_concept\_model()}, and a set of widgets will appear for them to specify the input field, a concept term, and other details like the output type of the concept score~(\autoref{fig:sys_api_concepts}~\circled{A}).

\begin{figure}[!tb]
  \includegraphics[width=\textwidth]{figures/sys_api_concepts_v2.pdf}
  \caption{
      Creating concepts with the {ModelSketchBook} API. 
      (A)~The \texttt{create\_concept\_model()} function accepts user inputs for the data input field, the concept term, and other settings. 
      (B)~Then, our API returns an output dataframe that displays all training examples sorted by their concept score. 
      (C)~We provide a suite of helper functions that assist users in finetuning and making sense of existing concepts as well as brainstorming new concepts. 
      (D)~We also provide functions that allow users to apply logical \texttt{AND} and \texttt{OR} operators to manually link different concepts together. 
      % \msb{I'd make A and B wider, and shrink C and D a little bit. Or, move C and D onto a separate short row below A and B, so that A and B get larger. Currently, A and B are too small to read}
  }
  \label{fig:sys_api_concepts}
\end{figure}

Once the user enters in those details, they can execute the cell; after several seconds, the API returns a dataframe visualization that displays a sorted view of the examples in the training dataset along with their concept score~(\autoref{fig:sys_api_concepts}~\circled{B}). The user can browse through the concept score results to determine whether the model's understanding of the concept sufficiently aligns with their own. If not, they can try out other concept terms or experiment with other input fields to work towards better alignment.

The API also includes additional features for users to binarize continuous scores using a custom threshold value, auto-normalize continuous scores to a 0-1 score range, or custom-calibrate continuous scores based on a specified minimum and maximum score value. These features allow the user to bring the raw concept scores in closer alignment with their own personal understanding of a concept.

We also provide functions that assist users as they brainstorm and evaluate tradeoffs among different concepts. A brainstorming helper function surfaces synonyms or antonyms of a provided word to spur ideas when users seek to verbalize or refine their concept. Meanwhile, a concept comparison helper function allows users to specify two concept terms and see a side-by-side comparison of their respective correlation with the input data and ground-truth ratings. To help scaffold users' sensemaking process, we also provide a note-taking function that allows them to write and save scratch notes on concepts and sketches for future reference.

% AND and OR logical operators for concepts
Finally, to allow for further control and refinement of concepts, we enable users to link existing concepts together with logical \texttt{AND} and \texttt{OR} operators. With a call to \texttt{create\_AND\_concept()}, users can take the logical \texttt{AND} of any number of binary concepts (and can similarly link arbitrary concepts with an \texttt{OR} relation using the \texttt{create\_OR\_concept()} function). This grants users the ability to better link concepts that interact with one another such as a single concept that can manifest in several ways or a multimodal concept that requires semantics from both image and text.

\subsubsection{Creating sketches with the API}
Once a user has authored several concepts, they can proceed to create the full sketch model that aggregates those concepts by calling \texttt{create\_sketch\_model()}. This function will again display a set of widgets for the user to select all of the concepts that they would like to use in the sketch model as well as an optional aggregation method (linear regression is the default)~(\autoref{fig:sys_api_sketches}~\circled{A}).

\begin{figure}[!tb]
  \includegraphics[width=\textwidth]{figures/sys_api_sketches_v2.pdf}
  \caption{
      Authoring sketches with the {ModelSketchBook} API. 
      (A)~The \texttt{create\_sketch\_model()} function accepts user inputs to gather the concepts that the user would like to aggregate as well as optional parameters to set the aggregation method and sort-column.
      (B)~Then, the API returns an output dataframe that displays all training examples sorted by the specified column. This view shows all of the input fields, all of the concept scores, and the sketch model's prediction. It also displays the ground truth rating and the error between the sketch prediction and ground truth rating to help users discover where the sketch model deviated from their ratings.
      \msl{Note: may need to change the image/text examples; just using those as placeholders for now}
      % \msb{I'm on a large display and still can't read the text in this figure. I recommend not letting any text you care about in figures get any smaller than the body text of the paper. Right now, the important stuff looks like it's a at font size one half the body text.}
  }
  \label{fig:sys_api_sketches}
\end{figure}

After executing the cell, the API creates the new sketch model and returns a dataframe visualization that displays all of the input fields of the training examples, all of the relevant concept scores, and the overall prediction produced by the sketch model~(\autoref{fig:sys_api_sketches} \circled{B}). This view also includes the ground-truth ratings and the difference between the sketch prediction and these ground-truth ratings. Users can choose to sort by various columns to aid their understanding of the model outputs: sorting by the sketch prediction surfaces an ordering that represents of the sketch model's understanding of the modeling task; sorting by the ground-truth rating foregrounds the ``intended'' understanding of the modeling task; sorting by the difference (or absolute value of difference) between the sketch prediction and ground-truth rating highlights areas where the sketch model most drastically deviated from the intended decision-making behavior. The sketch model output also displays more traditional performance metrics for both regression and classification formulations of the task based on the ground-truth labels for the training examples; we display Mean Absolute Error (MAE), Classification Accuracy, F1 Score, Precision, and Recall.

% Evaluating sketch on unseen data
Finally, the API provides helper functions that help the user to assess their sketch models. The \texttt{compare\_sketches()} function allows the user to compare the performance metrics for specified sketches, and the \texttt{test\_sketch()} function allows them to test out sketch models on a labeled or unlabeled validation set (if one is provided) to get a sense for how well it generalizes to a broader set of examples.

\subsubsection{Implementation}
% More detailed implementation details/settings; Colab setup
The {ModelSketchBook} API was authored entirely in Python. We use OpenAI's API for GPT-3 to perform zero-shot prompt-based text classification and use the \texttt{text-davinci-002} model, the current state-of-the-art GPT-3 variant. We use OpenCLIP~\cite{open_clip}, an open-source version of CLIP, to perform zero-shot image regression; we use a Vision Transformer (ViT) model (\texttt{ViT-B-32-quickgelu}) pre-trained on the \texttt{laion400m\_e32} dataset. We use the scikit-learn~\cite{scikit_learn} implementations of linear regression, logistic regression, decision tree classification, random forest classification, and MLP classification for our sketch model aggregators. 
% \msb{probably worth getting explicit for one sentence about what training and inference is done on the local machine and what is done via API in the cloud}
All training and inference takes place on the local machine on which the notebook is running (i.e., a user's own machine if they are running a local Juypter notebook, or a Google cloud server if they are running a Colab notebook).


==> sections/old_versions/3_system_v4.tex <==
% v4 9/15/22

In this section, we describe our model sketching framework, which aids ML practitioners in moving beyond technical implementation to explore the conceptual model design space during early phases of ML model development.


\subsection{The Model Sketching Framework}
% \msb{The first two paragraphs were wordy and repeating ideas from the intro. So, I tried condensing it here:} 
Model sketching aims to facilitate the translational, interpretational work that goes in between a high-level description and any particular low-level implementation~\cite{passi_barocas_problemFormulationFairness,jacobs_wallach_measurementAndFairness}.
This work charts a path through the multitude of plausible strategies for any one high-level modeling goal, each of which ossifies a set of human values and ethical implications that are encoded into the model.
%What we \textit{want} is to foreground this challenging translational work so that ML practitioners can confidently explore numerous solution paths and compare their tradeoffs. What we \textit{have} now is a messy, undocumented process where practitioners themselves may not be able to remember all of the reasons underlying prior design decisions.

% % We wanted to fill the gap between high-level modeling goals and low-level implementation --> arrived at intermediate goals/representations in the form of concepts
% Currently, ML practitioners commonly capture their modeling work through 1)~high-level descriptions like written documents or presentations stating the goal of a given model~\cite{piorkowski_AIDevelopersCommChallenges} or 2)~low-level implementations like computational notebooks or code repositories with data processing, feature extraction, and modeling logic~\cite{rule_explorationExplanationCompNotebooks}. However, there is a significant amount of translational, interpretational work that goes in between a high-level description and any particular low-level implementation~\cite{passi_barocas_problemFormulationFairness,jacobs_wallach_measurementAndFairness}. This work may in fact be the most critical piece of the modeling task to get right given that there is a vast design space of plausible solution strategies for any one high-level modeling goal. Furthermore, these different approaches carry different sets of human values and ethical implications, which is especially important to consider when designing human-facing deployments of machine learning. There is not just one clear solution, and the choice among solutions is not arbitrary, especially in terms of user impact. 

% Since current approaches primarily cover only high-level goals or low-level technical instantiations, this important intermediate work remains hidden in the depths of experimental scripts, disorganized notebooks, or even internal reasoning that may never have been documented in any form~\cite{zhang_howDoDataScienceWorkersCollaborate}. What we \textit{want} is to foreground the challenging work of bridging between goals and implementations so that ML practitioners can confidently explore numerous solution paths and compare their tradeoffs. What we have is a messy, undocumented process where practitioners themselves may not be able to remember all of the reasons underlying their prior design decisions. This makes it exceedingly difficult to not only revisit those past decisions, but to reverse them or explore alternative implementations after a model has already been built and deployed.

We seek to address the gap %between high-level modeling goals and low-level implementation 
by introducing \textit{concepts}---human-understandable ideas or factors that are relevant to a decision-making task---as an intermediary representation. By foregrounding this translational step between goals and their implementation, we aim to scaffold ML practitioners' reasoning and help them to more effectively sketch out and explore parallel solution paths. This concept-based intermediary can also make their work in this vein more visible and organized, both to themselves and to other stakeholders.
% Concepts also allow us to meet our design goals of expressivity, minimal detail, and speed
% \msb{shorter version, I got rid of some of the buxton criteria explicitness:}
Centering the model authoring process around concepts enforces a simplified representation of a model's decision-making logic, achieving minimal detail while ensuring that the detail that remains is central to the core of a modeling approach. 
%The availability of zero-shot modeling enables interactive mapping from data examples to arbitrary concept scores without any training time, expressively covering several modalities (including text and images) and ranging from concrete and specific to abstract and ideological.

% Concepts as a primary abstraction also allow us to meet our design goals of expressivity, minimal detail, and speed. Given that they can relate to a variety of modalities (including text and images) and can range from concrete and specific to abstract and ideological, concepts provide an expressive lever for specifying model behavior. Then, centering the model authoring process primarily around concepts naturally enforces a much-simplified representation of a model's decision-making logic, achieving minimal detail while ensuring that the detail that remains is central to the core ideas of a modeling approach. Lastly, thanks to improvements in zero-shot modeling, we can interactively map from data examples to arbitrary concept scores without any training time. This means that users can speedily author functional building blocks by specifying concepts and stringing them together. 
% We now describe in greater detail how we break down our model sketching framework into concepts and sketch models.

% \msb{I think this is where we need to have a paragraph or two explaining how we envision the code or insights from model sketches get applied later in the development process. What are they keeping? What are they tossing? What changes about the full production of the model based on what they learned from the sketch?}
% \msl{I think I'll put this after I describe both concepts and sketch models so it'll make a bit more sense!}

\subsubsection{Data prerequisites}
We require data in table form (e.g., spreadsheet, CSV, Pandas Dataframe) where each row represents a single example and each column represents a data field. These data fields can contain text, image, or numeric data. 
We recommend that the dataset has at least 40-50 rows to aid sensemaking during model development, while also allowing for a split between training and test data.
If the user provides ground-truth labels, our system can help with sensemaking around model accuracy; however, such labels are not required.%Our approach works best when the data is labeled for the desired modeling task (e.g., if the task is hate speech detection, it is ideal for the data table to include a column with labels indicating the the hate speech label or score for each item). These labels allow us to benchmark our sketch model output against a desired point of reference. However, such labels are not required to author sketch models.

\subsubsection{Concepts: Crafting functional building blocks of decision-making}
%With our method, concepts---human-understandable ideas related to a decision-making task---are the main building blocks that users can use to construct their models. 
Concepts are how we decompose the larger and more ambitious task of a sketch model into more manageable, human-understandable components.
We turn concepts into functional components by mapping from a data example to a score that indicates its relevance to the specified concept, or how well it exemplifies that concept~(\autoref{fig:sys_concepts}). For example, a concept for ``colorful'' might produce scores for a set of images indicating roughly how colorful they are; a concept for ``profanity'' might produce scores for a set of text comments that estimate how profane they are. Thus, concepts bear similarities to feature extractors, but they are not limited to lower-level, objective attributes, and they require much less time and effort to produce. Once created, a concept can be applied to any arbitrary example, seen or unseen.

\begin{figure}[!tb]
  \includegraphics[width=\textwidth]{figures/sys_concepts_v1.pdf}
  \caption{
      Users can turn human-understandable concepts into functional building blocks. A concept takes in a concept term and a data field as input. Then, a pretrained zero-shot model produces a score for each example that indicates the extent to which the example relates to the specified concept. We adapt our underlying approach depending on the inferred type of the data field. For text, we leverage GPT-3 prompts for zero-shot classification. For images, we leverage CLIP embeddings for zero-shot regression.
  }
  \label{fig:sys_concepts}
\end{figure}

We build upon advances in zero-shot modeling to instantiate concepts. Zero-shot modeling describes any machine learning modeling approach that does not require any training examples to perform a task. To create a concept, the user provides an input concept term (a brief word or phrase) and a data field (column name) from their dataset. Our framework then authors a zero-shot model that maps from the provided data and can output a numeric score for that concept for every item in the dataset.
For our concepts, we implement two zero-shot modeling methods: 1)~zero-shot text classification via large language model prompting using GPT-3 and 2)~zero-shot image regression via embedding similarity with a pre-trained image-to-text model using CLIP. We describe our technical approach in greater depth in Section~\ref{section:concept_technical}. While we choose these two zero-shot methods in our work, we design our model sketching framework to be compatible with any current or future zero-shot modeling method. 

\subsubsection{Sketch models: Putting concepts together to envision decision-making outcomes}
The second component of our model sketching framework involves aggregating these concepts to form sketches. 
%Without concepts as an intermediary, ML practitioners usually have to map directly from raw data (i.e., resume text) to their modeling outcomes (i.e., a ranked list of promising job applicants). They can tweak model architectures, perform data processing, try out alternate loss functions, and adjust hyperparameters, but these modifications are largely uninterpretable and leave the model as a black box. With the introduction of concepts, ML practitioners can now shift to iterate on their models in terms of human-understandable concept building blocks that they themselves brainstormed, authored, and tuned.
A sketch model is a lightweight ML model that works by aggregating the signals produced by concepts~(\autoref{fig:sys_sketches}). It is designed to accomplish the same task as the full model that it is meant to emulate, so it expects the same inputs and produces the same class of outputs.

Once the user has authored a set of constituent concepts that are relevant to the decision-making task, they select which concepts they would like to combine into a sketch model. We provide an initial set of aggregators that can combine concept scores to produce a single sketch model score: linear regression, logistic regression, decision tree classification, random forest classification, and multi-layer perceptron (MLP) classification. 
Rather than require a complex deep learning model to integrate concepts, we build on prior research that demonstrated how simple linear models with small sets of human-interpretable features can achieve performance exceeding that of human decision-makers and rivaling that of complex prediction models~\cite{jung_goel_simpleRulesExpertClassification}.
However, we are not bound to this initial set of aggregators. %; sketch models are compatible with any aggregation method that can accept multiple concept scores and produce a holistic output score. 
% Sketch model is trained on provided labels, but can be specified more manually if desired
We use the ground-truth labels provided in the training dataset to train these aggregators when a sketch model is created; all subsequent runs of the sketch model will evaluate the trained model on new input data. If the dataset does not have labels, then the user can opt to provide manual weights for the concepts using the linear regression aggregator.

\begin{figure}[!tb]
  \includegraphics[width=0.85\textwidth]{figures/sys_sketches_v1.pdf}
  \caption{
      Sketch models combine concepts together to create an overall model for the decision-making task. Here, we show an example for a hateful post detection task. First, the user chooses from among the concepts they have authored and decides on an aggregation method. We then create a new sketch model by generating the concept scores and training a model using the specified aggregation method and user's provided ground-truth ratings (e.g., ratings of the hatefulness of posts). Once authored, the sketch model can produce predictions (e.g., scores estimating the hatefulness of posts) for any arbitrary example.
  }
  \label{fig:sys_sketches}
\end{figure}

% \msb{cut?} Using the specified concepts and aggregation method, our approach produces a sketch model that can generate a score for any arbitrary input example. The concept models operate on the example to generate their individual concept scores, and the sketch model applies the aggregator to these concept scores to produce the overall score.

With the sketch-model layer of abstraction, ML practitioners can focus their attention on experimenting with different combinations of concepts to create sketches that might capture different sets of values in decision-making. For example, when authoring a hate speech detection model, an ML practitioner may experiment with sketches that focus on race-related or gender-related hate speech, or approaches that explicitly account for intersectionality. They may try out sketches that take a relatively lenient stance by only adding a concept related to speech that incites violence, or they may experiment with sketches that take a more strict stance on profanity by adding concepts for swearing and slurs. 
By rapidly authoring sketch models and testing them on new data examples, ML practitioners can quickly discover cases where their modeling approach appears to fail, get inspiration for new concepts that may help them to address these gaps, and immediately author and incorporate those new concepts. They may also discover gaps in the larger modeling ecosystem---for example, cases where the current data fields do not provide enough information to glean a certain concept, cases where the dataset lacks representation of a certain important phenomenon, or cases where the data labeling scheme lacks the necessary granularity to separate classes.

% Compatibility with existing features/model outputs
While sketch models in their most stylized form are comprised entirely of concepts, sketch models are also compatible with other, more traditional kinds of features. If a model developer has raw or pre-processed features from an existing feature extractor or data pipeline, they can also incorporate those features and aggregate them into a sketch model. If an engineering team already has an existing version of a model or sub-models that produce scores that may be helpful for the decision-making task, they can also incorporate those scores as inputs to a sketch model.

% From sketches to production models
\subsubsection{From sketch models to production models}
\label{section:sketch_to_production}
% \msb{I cut some stuff here to condense}
% how sketches apply to later development process
% What they keep, what they toss
% What changes about full production model based on sketch
While sketch models initially serve as tools for thinking and iterating during early model development phases, we envision that they will directly inform the design of full production models. 

% Decomposition
First, a key part of full-scale model design involves deciding how to \textit{decompose the model} into smaller parts. An important characteristic of successful production ML systems---consistent across use cases like feed ranking and content moderation and across platforms like Facebook, LinkedIn, and Reddit---is that they are composed of smaller, more targeted ML models whose outputs are synthesized into a single score, often via weighted linear combination~\cite{eckles_2022, reddit_moderator_tools, linkedin_dwell_time}. %While aggregating various signals seems simplistic, it is highly performant in real-world decision-making contexts~\cite{jung_goel_simpleRulesExpertClassification}, and for ML systems as large and complex as those we see in industry, it is important that signals remain interpretable and tuneable as models and users constantly evolve. %Thus, even as ML teams implement complex black box models that act on raw, uninterpretable features, these are models generally still produce human-understandable scores that may, for example, predict the likelihood that a comment has profanity or the likelihood that a photo contains violence. 
In other words, the sub-models that ML practitioners produce in industry are more complex versions of our concepts, but they typically still boil down to a human-understandable decision-making factor that will be synthesized into a single prediction via an aggregation process. %Thus, a sketch model lays a direct blueprint for how to decompose a modeling problem into sub-models that will be aggregated together.

% Data requirements
Second, a substantial part of model development (up to 80\% by some estimates) is actually consumed by data cleaning and wrangling, and ML practitioners play an active role in shaping, curating, and designing data~\cite{muller_HowDataScienceWorkersWorkWithData}. Model sketching helps to refine \textit{data requirements} by drawing out what kind of data is necessary for the task based on the concepts that the model must reason over. By testing out concepts on different data fields (e.g., different text or image fields), ML practitioners gain a quick understanding of what forms of data are most valuable or informative to serve different concepts and, ultimately, what data fields should be required for the modeling task. 
%For example, they may find that the concepts they care most about for the modeling task tend to be most easily gleaned from the image of a social media post rather than the text, so they may realize that they need to focus more of their data-wrangling efforts on extracting a high-quality image representation.
Testing out concepts on preliminary data versions also surfaces gaps in the representativity of the data. For example, if an ML practitioner tests out a ``weapon'' concept for a hateful post detection task and finds few matches, they may realize that their current dataset has too few examples of military- or violence-related content and can set out to augment the dataset accordingly. %By the end of the model sketching process, the ML practitioner should have a much clearer sense of the specific data fields and the kinds of data representativity that they will need for their full-scale model.

% Labeling and Scoring
% \msb{I agree with this, but it's not as central to scaling up to a full model, so could cut entirely}
% Finally, model sketching helps to clarify the \textit{labeling or scoring procedure} for a machine learning task. Since decision-making goals are typically underspecified, labeling schemes must evolve over time to capture unanticipated, ambiguous categories~\cite{kulesza_conceptEvolution}. %If not accounting for this concept evolution, labeling policies become inconsistent and illogical, which greatly undermines the performance of any model that builds on top of the resulting labels. 
% Model sketching directly engages ML practitioners in this process of concept iteration and has them constantly review both constituent concept scores and aggregate sketch model predictions against provided ground truth ratings. Thus, practitioners can rapidly identify and correct cases where any of these scores, predictions, or ratings are misaligned with their understanding of a concept or of the higher-level decision-making task. 
% %Through this process, they may discover that the provided ground-truth ratings are internally inconsistent and require re-labeling, or they may discover that the choice to binarize scores at a $0.5$ threshold results in too little granularity since most scores fall below $0.5$, so a different threshold should be chosen. The insights that ML practitioners gain from iterating on the labeling and scoring schemes in sketch models directly inform the standards that should be used for the full-scale modeling task.


\subsection{The ModelSketchBook tool}
To instantiate our model sketching framework, we introduce the {ModelSketchBook} API, a Python package that allows ML practitioners to create concepts and sketches of their own. Our package will be made open-source on Github.\footnote{https://github.com/REDACTED (currently a private repository during review)}
% \msb{cut the rest of the paragraph}
%{ModelSketchBook} is just one example of how we might instantiate our model sketching framework. For example, we envision that one could implement a version with a dedicated graphical user interface to serve the needs of non-technical users, or a version that uses zero-shot video models to target a use-case related to video content.

\subsubsection{Environment and setup}
% Why we selected a notebook environment; our target demographic
Our API can be loaded in any Python environment, but it is optimized for use in a computational notebook such as Jupyter or Colab. We chose to tailor our API design to the notebook environment because this is where many ML practitioners already carry out much of their exploratory modeling work~\cite{rule_explorationExplanationCompNotebooks,zhang_howDoDataScienceWorkersCollaborate}. 

% Setting up the sketchbook and data
% \msb{I cut this paragraph, the dataset requirements were described above and I don't think this is critical, I smoothed it in with some content in the next paragraph:} %After loading in their dataset into a Pandas dataframe and importing the {ModelSketchBook} package in their notebook, the user can run a brief function to set up their sketchbook with the dataframe(s) and their associated data schema. We recommend that users provide a smaller set of examples (on the order of 20-50) for use during model sketching, as this limited dataset size allows the data to better serve as point of reference to facilitate creative iteration, rather than a distractor that might overwhelm them. 

% df_train = pd.read_csv("train.csv")
% df_test = pd.read_csv("test.csv")
\begin{minted}[fontsize=\footnotesize,samepage]{python}
    import model_sketch_book as msb

    # Set up the sketchbook
    sb = msb.create_model_sketchbook(
        goal="Detect hateful memes on social media.",
        datasets={  # Pass in datasets to use
            "train": df_train,
            "test": df_test,
        },
        schema = {  # Specify the types of data fields, including the ground-truth column
            "text": InputType.Text,
            "img_url": InputType.Image,
            "overall_rating": InputType.GroundTruth,
        },
    )
\end{minted}

After loading in their dataset into a Pandas dataframe and importing the {ModelSketchBook} package in their notebook, the user sets up a sketchbook object. The sketchbook contains all of the datasets, concepts, and sketches that the user will author during their session, and it saves other metadata such as model predictions, performance metrics, and a history of concepts and sketches.

\subsubsection{Creating concepts: under the hood}
\label{section:concept_technical}
As mentioned previously, we specifically support text concepts powered by GPT-3 and image concepts powered by CLIP.
To achieve zero-shot text classification, we author prompts that list a batch of examples for the model to classify and ask the model to decide on a binary label (``<concept term>'' or ``not <concept term>'') for each provided example. Large language models like GPT-3 are designed to perform text completion on provided input prompts, so plausible completions provided by the model capture a rough sense of binary labels that might be reasonable based on the knowledge available in the model. We include an example prompt below.

\begin{minted}[fontsize=\footnotesize,samepage]{markdown}
        Decide whether these comments are "motivational" or "not motivational".
        1. You can do it!!
        2. Ugh, you're the worst.
        3. I'm so tired...
    
        Comment results:
\end{minted}

The GPT-3 model will then return a text completion response similar to this that provides a label for the examples. We parse and post-process this GPT-3 response to retrieve binary labels.
\begin{minted}[fontsize=\footnotesize,samepage]{markdown}
        1. motivational
        2. not motivational
        3. not motivational
\end{minted}

To carry out zero-shot image classification, we use CLIP (Contrastive Language-Image Pre-Training)~\cite{CLIP}, a neural network trained on (image, text) pairs that allows images and text to be represented in a shared embedding space. Given a data field containing images and a concept term, we use CLIP to encode both the image and the concept term in that shared image-text embedding space. Then, we calculate and return the cosine similarity between the embedded image and concept term. Thus, the output score approximately captures the extent to which the given image relates to the specified concept term. We also allow users to normalize and re-calibrate these similarity scores to match their internal understanding of the concept, and we also allow users to apply custom thresholds to binarize continuous concept scores.

\subsubsection{Creating concepts with the API}
After setting up the sketchbook, users can freely author concepts. While we also provide raw API functions under the hood, for convenience, we surface UI elements via ipywidgets.\footnote{\url{http://ipywidgets.readthedocs.io}} These widgets clarify the available function parameters and the eligible input options for each parameter. When the user makes a call to \texttt{create\_concept\_model()}, a set of widgets will appear for them to specify the input field, a concept term, and other details like the output type of the concept score~(\autoref{fig:sys_api_concepts}~\circled{A}).

\begin{figure}[!tb]
  \includegraphics[width=\textwidth]{figures/sys_api_concepts_v2.pdf}
  \caption{
      Creating concepts with the {ModelSketchBook} API. 
      (A)~The \texttt{create\_concept\_model()} function accepts user inputs for the data input field, the concept term, and other settings. 
      (B)~Then, our API returns an output dataframe that displays all training examples sorted by their concept score. 
      (C)~We provide a suite of helper functions that assist users in finetuning and making sense of existing concepts as well as brainstorming new concepts. 
      (D)~We also provide functions that allow users to apply logical \texttt{AND} and \texttt{OR} operators to manually link different concepts together. 
      % \msb{I'd make A and B wider, and shrink C and D a little bit. Or, move C and D onto a separate short row below A and B, so that A and B get larger. Currently, A and B are too small to read}
  }
  \label{fig:sys_api_concepts}
\end{figure}

Once the user enters in those details, they can execute the cell; after several seconds, the API returns a dataframe visualization that displays a sorted view of the examples in the training dataset along with their concept score~(\autoref{fig:sys_api_concepts}~\circled{B}). The user can browse through the concept score results to determine whether the model's understanding of the concept sufficiently aligns with their own. If not, they can try out other concept terms or experiment with other input fields to work towards better alignment. The API also includes additional features for users to binarize continuous scores using a custom threshold value, auto-normalize continuous scores to a 0-1 score range, or custom-calibrate continuous scores based on a specified minimum and maximum score value. These features allow the user to bring the raw concept scores in closer alignment with their own personal understanding of a concept.

We provide functions that assist users as they brainstorm and evaluate tradeoffs among different concepts. A brainstorming helper function surfaces synonyms or antonyms of a provided word to spur ideas when users seek to refine their concept. Meanwhile, a concept comparison helper function allows users to specify concept terms and compare their respective correlation with the input data and ground-truth ratings. To scaffold users' sensemaking process, we also provide a note-taking function that allows them to save scratch notes on concepts and sketches for future reference.

% AND and OR logical operators for concepts
Finally, to allow for further control and refinement of concepts, we enable users to link existing concepts together with logical \texttt{AND} and \texttt{OR} operators. With a call to \texttt{create\_AND\_concept()}, users can take the logical \texttt{AND} of any number of binary concepts (and can similarly link arbitrary concepts with an \texttt{OR} relation using the \texttt{create\_OR\_concept()} function). This grants users the ability to better link concepts that interact with one another such as a single concept that can manifest in several ways or a multimodal concept that requires semantics from both image and text.

\subsubsection{Creating sketches with the API}
Once a user has authored several concepts, they can proceed to create the full sketch model that aggregates those concepts by calling \texttt{create\_sketch\_model()}. This function will again display a set of widgets for the user to select all of the concepts that they would like to use in the sketch model as well as an optional aggregation method (linear regression is the default)~(\autoref{fig:sys_api_sketches}~\circled{A}).

\begin{figure}[!tb]
  \includegraphics[width=\textwidth]{figures/sys_api_sketches_v2.pdf}
  \caption{
      Authoring sketches with the {ModelSketchBook} API. 
      (A)~The \texttt{create\_sketch\_model()} function accepts user inputs to gather the concepts that the user would like to aggregate as well as optional parameters to set the aggregation method and sort-column.
      (B)~Then, the API returns an output dataframe that displays all training examples sorted by the specified column. This view shows all of the input fields, all of the concept scores, and the sketch model's prediction. It also displays the ground truth rating and the error between the sketch prediction and ground truth rating to help users discover where the sketch model deviated from their ratings.
      % \msl{Note: may need to change the image/text examples; just using those as placeholders for now}
  }
  \label{fig:sys_api_sketches}
\end{figure}

After executing the cell, the API creates the new sketch model and returns a dataframe visualization that displays all of the input fields of the training examples, all of the relevant concept scores, and the overall prediction produced by the sketch model~(\autoref{fig:sys_api_sketches} \circled{B}). This view also includes the ground-truth ratings and the difference between the sketch prediction and these ground-truth ratings. Users can choose to sort by various columns to aid their understanding of the model outputs: sorting by the sketch prediction surfaces an ordering that represents the sketch model's understanding of the modeling task; sorting by the ground-truth rating foregrounds the ``intended'' understanding of the modeling task; sorting by the difference (or absolute value of difference) between the sketch prediction and ground-truth rating highlights areas where the sketch model most drastically deviated from the intended decision-making behavior. The sketch model output also displays traditional performance metrics for both regression and classification formulations of the task based on the ground-truth labels for the training examples; we display Mean Absolute Error (MAE), Classification Accuracy, F1 Score, Precision, and Recall.

% Evaluating sketch on unseen data
Finally, the API provides functions that help the user to assess their sketch models. The \texttt{compare\_sketches()} function allows the user to compare performance metrics for specified sketches, and the \texttt{test\_sketch()} function allows them to test out sketch models on a labeled or unlabeled validation set (if one is provided) to get a sense for how well it generalizes to a broader set of examples.

\subsubsection{Implementation}
% More detailed implementation details/settings; Colab setup
The {ModelSketchBook} API was authored in Python. We use OpenAI's API for GPT-3 to perform zero-shot prompt-based text classification and use the \texttt{text-davinci-002} model, the current state-of-the-art GPT-3 variant. We use OpenCLIP~\cite{open_clip}, an open-source version of CLIP, to perform zero-shot image regression; we use a Vision Transformer (ViT) model (\texttt{ViT-B-32-quickgelu}) pre-trained on the \texttt{laion400m\_e32} dataset. We use the scikit-learn~\cite{scikit_learn} implementations of linear regression, logistic regression, decision tree classification, random forest classification, and MLP classification for our sketch model aggregators. 
% \msb{probably worth getting explicit for one sentence about what training and inference is done on the local machine and what is done via API in the cloud}
All training and inference takes place on the local machine on which the notebook is running (i.e., a user's own machine if they are running a local Juypter notebook, or a Google cloud server if they are running a Colab notebook).


==> sections/old_versions/3_system_v5.tex <==
% v5 12/10/22

In this section, we describe our model sketching framework, which aids ML practitioners in moving beyond technical implementation to explore the conceptual model design space during early phases of ML model development.


\subsection{The Model Sketching Framework}
% \msb{The first two paragraphs were wordy and repeating ideas from the intro. So, I tried condensing it here:} 
Model sketching aims to facilitate the translational, interpretational work that goes in between a high-level description and any particular low-level implementation~\cite{passi_barocas_problemFormulationFairness,jacobs_wallach_measurementAndFairness}.
This work charts a path through the multitude of plausible strategies for any one high-level modeling goal, each of which ossifies a set of human values and ethical implications that are encoded into the model.
%What we \textit{want} is to foreground this challenging translational work so that ML practitioners can confidently explore numerous solution paths and compare their tradeoffs. What we \textit{have} now is a messy, undocumented process where practitioners themselves may not be able to remember all of the reasons underlying prior design decisions.
%
% % We wanted to fill the gap between high-level modeling goals and low-level implementation --> arrived at intermediate goals/representations in the form of concepts
% Currently, ML practitioners commonly capture their modeling work through 1)~high-level descriptions like written documents or presentations stating the goal of a given model~\cite{piorkowski_AIDevelopersCommChallenges} or 2)~low-level implementations like computational notebooks or code repositories with data processing, feature extraction, and modeling logic~\cite{rule_explorationExplanationCompNotebooks}. However, there is a significant amount of translational, interpretational work that goes in between a high-level description and any particular low-level implementation~\cite{passi_barocas_problemFormulationFairness,jacobs_wallach_measurementAndFairness}. This work may in fact be the most critical piece of the modeling task to get right given that there is a vast design space of plausible solution strategies for any one high-level modeling goal. Furthermore, these different approaches carry different sets of human values and ethical implications, which is especially important to consider when designing human-facing deployments of machine learning. There is not just one clear solution, and the choice among solutions is not arbitrary, especially in terms of user impact. 
%
% Since current approaches primarily cover only high-level goals or low-level technical instantiations, this important intermediate work remains hidden in the depths of experimental scripts, disorganized notebooks, or even internal reasoning that may never have been documented in any form~\cite{zhang_howDoDataScienceWorkersCollaborate}. What we \textit{want} is to foreground the challenging work of bridging between goals and implementations so that ML practitioners can confidently explore numerous solution paths and compare their tradeoffs. What we have is a messy, undocumented process where practitioners themselves may not be able to remember all of the reasons underlying their prior design decisions. This makes it exceedingly difficult to not only revisit those past decisions, but to reverse them or explore alternative implementations after a model has already been built and deployed.
%
\rev{We address the gap between high-level modeling goals and low-level implementation with the intermediary representation of \textit{concepts}---human-understandable ideas or factors that are relevant to a decision-making task.} By foregrounding this translational step between goals and their implementation, we aim to scaffold ML practitioners' reasoning and help them to more effectively sketch out and explore parallel solution paths. 
\cut{This concept-based intermediary can also make their work in this vein more visible and organized, both to themselves and to other stakeholders.
Centering the model authoring process around concepts enforces a simplified representation of a model's decision-making logic, achieving minimal detail while ensuring that the detail that remains is central to the core of a modeling approach.}

% Concepts as a primary abstraction also allow us to meet our design goals of expressivity, minimal detail, and speed. Given that they can relate to a variety of modalities (including text and images) and can range from concrete and specific to abstract and ideological, concepts provide an expressive lever for specifying model behavior. Then, centering the model authoring process primarily around concepts naturally enforces a much-simplified representation of a model's decision-making logic, achieving minimal detail while ensuring that the detail that remains is central to the core ideas of a modeling approach. Lastly, thanks to improvements in zero-shot modeling, we can interactively map from data examples to arbitrary concept scores without any training time. This means that users can speedily author functional building blocks by specifying concepts and stringing them together. 
% We now describe in greater detail how we break down our model sketching framework into concepts and sketch models.

% \msb{I think this is where we need to have a paragraph or two explaining how we envision the code or insights from model sketches get applied later in the development process. What are they keeping? What are they tossing? What changes about the full production of the model based on what they learned from the sketch?}
% \msl{I think I'll put this after I describe both concepts and sketch models so it'll make a bit more sense!}

\subsubsection{Data prerequisites}
We require only a small amount of data in table form (e.g., spreadsheet, CSV, Pandas Dataframe) where each row represents a single example and each column represents a data field. These data fields can contain text, image, or numeric data. 
We recommend that the dataset has at least 40-50 rows to aid sensemaking during model development, while also allowing for a split between training and test data.
If the user provides ground-truth labels, our system can help with sensemaking around model accuracy; however, such labels are not required.%Our approach works best when the data is labeled for the desired modeling task (e.g., if the task is hate speech detection, it is ideal for the data table to include a column with labels indicating the the hate speech label or score for each item). These labels allow us to benchmark our sketch model output against a desired point of reference. However, such labels are not required to author sketch models.

\subsubsection{Concepts: Crafting functional building blocks of decision-making}
Concepts are how we decompose the larger and more ambitious task of a sketch model into more manageable, human-understandable components.
We turn concepts into functional components by mapping from a data example to a score that indicates its relevance to the specified concept, or how well it exemplifies that concept~(\autoref{fig:sys_concepts}). For example, a concept for ``colorful'' might produce scores for a set of images indicating roughly how colorful they are; a concept for ``profanity'' might produce scores for a set of text comments that estimate how profane they are. Thus, concepts bear similarities to feature extractors, but they are not limited to lower-level, objective attributes, and they require much less time and effort to produce\rev{, as a new concept can be created in several seconds}. Once created, a concept can be applied to any arbitrary example, seen or unseen.

\begin{figure*}[!tb]
  \includegraphics[width=\textwidth]{figures/sys_concepts_v1.pdf}
  \caption{
      Users can turn human-understandable concepts into functional building blocks. A concept takes in a concept term and a data field as input. Then, a pretrained zero-shot model produces a score for each example indicating the extent to which the example relates to the specified concept. We adapt our underlying approach depending on the type of the data field. For text, we leverage GPT-3 prompts for zero-shot classification. For images, we leverage CLIP embeddings for zero-shot regression.
  }
  \label{fig:sys_concepts}
\end{figure*}

We build upon advances in zero-shot modeling to instantiate concepts. Zero-shot modeling describes any machine learning modeling approach that does not require any training examples to perform a task. To create a concept, the user provides an input concept term (a brief word or phrase) and a data field (column name) from their dataset. Our framework then authors a zero-shot model that outputs a numeric score for that concept for every item in the dataset.
For our concepts, we implement two methods: 1)~zero-shot text classification via large language model (LLM) prompting using GPT-3 and 2)~zero-shot image regression via embedding similarity with a pre-trained image-to-text model using CLIP. We describe our technical approach in greater depth in Section~\ref{section:concept_technical}. While we use these two zero-shot methods in our work, our model sketching framework is compatible with any current or future zero-shot modeling method. 

\subsubsection{Sketch models: Putting concepts together to envision decision-making outcomes}
The second component of our framework involves authoring sketch models, lightweight ML models that aggregate the signals produced by concepts~(\autoref{fig:sys_sketches}). A sketch model is designed to accomplish the same task as the full model that it is meant to emulate, so it expects the same inputs and produces the same class of outputs.

Once the user has authored a set of constituent concepts that are relevant to the decision-making task, they select which concepts they would like to combine into a sketch model. We provide an initial set of aggregators that can combine concept scores to produce a single sketch model score: linear regression, logistic regression, decision tree classification, random forest classification, and multi-layer perceptron (MLP) classification. 
Rather than require a complex deep learning model to integrate concepts, we build on prior research that demonstrated how simple linear models with small sets of human-interpretable features can achieve performance exceeding that of human decision-makers and rivaling that of complex prediction models~\cite{jung_goel_simpleRulesExpertClassification}.
However, we are not bound to this initial set of aggregators.
We use the ground-truth labels provided in the training dataset to train these aggregators when a sketch model is created; all subsequent runs of the sketch model will evaluate the trained model on new input data. If the dataset does not have labels, then the user can opt to provide manual weights for the concepts using the linear regression aggregator.

\begin{figure*}[!tb]
  \includegraphics[width=0.85\textwidth]{figures/sys_sketches_v1.1.pdf}
  \caption{
      Sketch models combine concepts together to create an overall model for the decision-making task. First, the user chooses from among their authored concepts and decides on an aggregation method. We train a sketch model using the concept scores, the specified aggregator, and the user's ground-truth ratings (e.g., ratings of the hatefulness of posts). Then, the sketch model can produce predictions (e.g., scores estimating the hatefulness of posts) for any arbitrary example.
  }
  \label{fig:sys_sketches}
\end{figure*}

With the sketch-model layer of abstraction, ML practitioners can focus their attention on experimenting with different combinations of concepts to create sketches that might capture different sets of values in decision-making. For example, when authoring a hate speech detection model, an ML practitioner may experiment with sketches that focus on race-related or gender-related hate speech, or approaches that explicitly account for intersectionality. They may try out sketches that take a relatively lenient stance by only adding a concept related to speech that incites violence, or they may experiment with sketches that take a more strict stance on profanity by adding concepts for swearing and slurs.
\cut{By rapidly authoring sketch models and testing them on new data examples, ML practitioners can quickly discover cases where their modeling approach appears to fail, get inspiration for new concepts that may help them to address these gaps, and immediately author and incorporate those new concepts. They may also discover gaps in the larger modeling ecosystem---for example, cases where the current data fields do not provide enough information to glean a certain concept, cases where the dataset lacks representation of a certain important phenomenon, or cases where the data labeling scheme lacks the necessary granularity to separate classes.}
%
% Compatibility with existing features/model outputs
While sketch models in their most stylized form are comprised entirely of concepts, sketch models are also compatible with \rev{more traditional features produced through custom feature extractors or existing ML models}. 
\cut{If a model developer has raw or pre-processed features from an existing feature extractor or data pipeline, they can also incorporate those features and aggregate them into a sketch model. If an engineering team already has an existing version of a model or sub-models that produce scores that may be helpful for the decision-making task, they can also incorporate those scores as inputs to a sketch model.}

% From sketches to production models
\subsubsection{From sketch models to production models}
\label{section:sketch_to_production}
While sketch models initially serve as tools for thinking and iterating during early model development phases, we envision that they could inform the design of full production models. 

% Decomposition
First, a key part of full-scale model design involves deciding how to \textit{decompose the model} into smaller parts. A notable characteristic of successful production ML systems---consistent across use cases like feed ranking and content moderation and across platforms like Facebook, LinkedIn, and Reddit---is that they are composed of smaller, more targeted ML models whose outputs are synthesized into a single score, often via weighted linear combination~\cite{eckles_2022, reddit_moderator_tools, linkedin_dwell_time}. %While aggregating various signals seems simplistic, it is highly performant in real-world decision-making contexts~\cite{jung_goel_simpleRulesExpertClassification}, and for ML systems as large and complex as those we see in industry, it is important that signals remain interpretable and tuneable as models and users constantly evolve. %Thus, even as ML teams implement complex black box models that act on raw, uninterpretable features, these are models generally still produce human-understandable scores that may, for example, predict the likelihood that a comment has profanity or the likelihood that a photo contains violence. 
In other words, the sub-models that ML practitioners produce in industry are more complex versions of our concepts, but they typically still boil down to human-understandable decision-making factors that will be synthesized into a single prediction via an aggregation process. %Thus, a sketch model lays a direct blueprint for how to decompose a modeling problem into sub-models that will be aggregated together.

% Data requirements
Second, a substantial part of model development (up to 80\% by some estimates) is actually consumed by data cleaning and wrangling, and ML practitioners play an active role in shaping, curating, and designing data~\cite{muller_HowDataScienceWorkersWorkWithData}. Model sketching could assist in refining \textit{data requirements} by drawing out what kind of data is necessary for the task based on the concepts that the model must reason over. By testing out concepts on different data fields (e.g., different text or image fields), ML practitioners might gain a quick understanding of what forms of data are most informative to serve different concepts and, ultimately, what data fields and what kinds of data examples should be required for the modeling task. 
%For example, they may find that the concepts they care most about for the modeling task tend to be most easily gleaned from the image of a social media post rather than the text, so they may realize that they need to focus more of their data-wrangling efforts on extracting a high-quality image representation.
% \cut{Testing out concepts on preliminary data versions also surfaces gaps in the representativity of the data. For example, if an ML practitioner tests out a ``weapon'' concept for a hateful post detection task and finds few matches, they may realize that their current dataset has too few examples of military- or violence-related content and can set out to augment the dataset accordingly. 
% By the end of the model sketching process, the ML practitioner should have a much clearer sense of the specific data fields and the kinds of data representativity that they will need for their full-scale model.}

% Labeling and Scoring
% \msb{I agree with this, but it's not as central to scaling up to a full model, so could cut entirely}
% Finally, model sketching helps to clarify the \textit{labeling or scoring procedure} for a machine learning task. Since decision-making goals are typically underspecified, labeling schemes must evolve over time to capture unanticipated, ambiguous categories~\cite{kulesza_conceptEvolution}. %If not accounting for this concept evolution, labeling policies become inconsistent and illogical, which greatly undermines the performance of any model that builds on top of the resulting labels. 
% Model sketching directly engages ML practitioners in this process of concept iteration and has them constantly review both constituent concept scores and aggregate sketch model predictions against provided ground truth ratings. Thus, practitioners can rapidly identify and correct cases where any of these scores, predictions, or ratings are misaligned with their understanding of a concept or of the higher-level decision-making task. 
% %Through this process, they may discover that the provided ground-truth ratings are internally inconsistent and require re-labeling, or they may discover that the choice to binarize scores at a $0.5$ threshold results in too little granularity since most scores fall below $0.5$, so a different threshold should be chosen. The insights that ML practitioners gain from iterating on the labeling and scoring schemes in sketch models directly inform the standards that should be used for the full-scale modeling task.


\subsection{The ModelSketchBook tool}
To instantiate our model sketching framework, we introduce the {ModelSketchBook} API,\footnote{\url{https://github.com/StanfordHCI/ModelSketchBook}} a Python package that allows ML practitioners to create concepts and sketches of their own. 
% Our package will be made open-source on Github.

\subsubsection{Environment and setup}
\label{section:sys-sketchbook-setup}
% Why we selected a notebook environment; our target demographic
Our API can be loaded in any Python environment, but it is optimized for use in a computational notebook such as Jupyter or Colab. 
We chose to tailor our API design to the notebook environment because this is where many ML practitioners already carry out much of their exploratory modeling work~\cite{rule_explorationExplanationCompNotebooks,zhang_howDoDataScienceWorkersCollaborate}. 

% Setting up the sketchbook and data
% \msb{I cut this paragraph, the dataset requirements were described above and I don't think this is critical, I smoothed it in with some content in the next paragraph:} %After loading in their dataset into a Pandas dataframe and importing the {ModelSketchBook} package in their notebook, the user can run a brief function to set up their sketchbook with the dataframe(s) and their associated data schema. We recommend that users provide a smaller set of examples (on the order of 20-50) for use during model sketching, as this limited dataset size allows the data to better serve as point of reference to facilitate creative iteration, rather than a distractor that might overwhelm them. 

% df_train = pd.read_csv("train.csv")
% df_test = pd.read_csv("test.csv")
\begin{minted}[fontsize=\footnotesize,samepage]{python}
    import model_sketch_book as msb

    # Set up the sketchbook
    sb = msb.create_model_sketchbook(
        goal="Detect hateful memes on social media.",
        datasets={  # Pass in datasets to use
            "train": df_train,
            "test": df_test,
        },
        schema = {  # Specify the types of data fields
            "text": InputType.Text,
            "img_url": InputType.Image,
            "overall_rating": InputType.GroundTruth,
        },
    )
\end{minted}

After loading their dataset as a Pandas dataframe and importing the {ModelSketchBook} package in their notebook, the user sets up a sketchbook object. The sketchbook contains all of the datasets, concepts, and sketches that the user will author during their session, and it saves other metadata such as model predictions, performance metrics, and a history of concepts and sketches.

\subsubsection{Creating concepts: under the hood}
\label{section:concept_technical}
As mentioned previously, we specifically support text concepts powered by GPT-3 and image concepts powered by CLIP.
To achieve zero-shot text classification, we author prompts that list a batch of examples for the model to classify and ask the model to decide on a binary label (``<concept term>'' or ``not <concept term>'') for each provided example. Large language models like GPT-3 are designed to perform text completion on provided input prompts, so plausible completions provided by the model capture a rough sense of binary labels that might be reasonable based on the knowledge available in the model. We include an example prompt below.

\begin{minted}[fontsize=\footnotesize,samepage]{markdown}
        Decide whether these comments are "motivational" or "not
        motivational".
        1. You can do it!!
        2. Ugh, you're the worst.
        3. I'm so tired...
    
        Comment results:
\end{minted}

The GPT-3 model will then return a text completion response similar to this that provides a label for the examples. We parse and post-process this GPT-3 response to retrieve binary labels.
\begin{minted}[fontsize=\footnotesize,samepage]{markdown}
        1. motivational
        2. not motivational
        3. not motivational
\end{minted}

To carry out zero-shot image classification, we use CLIP (Contrastive Language-Image Pre-Training)~\cite{CLIP}, a neural network trained on (image, text) pairs that allows images and text to be represented in a shared embedding space. Given a data field containing images and a concept term, we use CLIP to encode both the image and the concept term in that shared image-text embedding space. Then, we calculate and return the cosine similarity between the embedded image and concept term. Thus, the output score approximately captures the extent to which the given image relates to the specified concept term. We also allow users to normalize and re-calibrate these similarity scores to match their internal understanding of the concept, and we also allow users to apply custom thresholds to binarize continuous concept scores.

\subsubsection{Creating concepts with the API}
After setting up the sketchbook, users can freely author concepts. While we also provide raw API functions under the hood, for convenience, we surface UI elements via ipywidgets.\footnote{\url{http://ipywidgets.readthedocs.io}} 
\cut{These widgets clarify the available function parameters and the eligible input options for each parameter.}
When the user makes a call to \texttt{create \_concept\_model()}, a set of widgets will appear for them to specify the input field, a concept term, and other details like the output type of the concept score~(\autoref{fig:sys_api_concepts}~\circled{A}).

\begin{figure*}[!tb]
  \includegraphics[width=\textwidth]{figures/sys_api_concepts_v3.pdf}
  \caption{
      Creating concepts with {ModelSketchBook} \rev{in a computational notebook}. 
      (A)~The \texttt{create\_concept\_model()} function accepts user inputs for the data input field, concept term, and other settings. 
      (B)~Then, the API outputs a dataframe displaying all training examples sorted by their concept score. 
      (C)~We provide helper functions for finetuning, making sense of existing concepts, and brainstorming new concepts. 
      (D)~We also support logical \texttt{AND} and \texttt{OR} operators to create compound concepts. 
  }
  \label{fig:sys_api_concepts}
\end{figure*}

Once the user enters in those details, they can execute the cell; after several seconds, the API returns a dataframe visualization that displays a sorted view of the examples in the training dataset along with their concept score~(\autoref{fig:sys_api_concepts}~\circled{B}). The user can browse through the concept score results to determine whether the model's understanding of the concept sufficiently aligns with their own. If not, they can try out other concept terms or experiment with other input fields to work towards better alignment. The API also includes additional features for users to binarize continuous scores using a custom threshold value, auto-normalize continuous scores to a 0-1 score range, or custom-calibrate continuous scores based on a specified minimum and maximum score value. 
\cut{These features allow the user to bring the raw concept scores in closer alignment with their own personal understanding of a concept.}

We provide functions that assist users as they brainstorm and evaluate tradeoffs among different concepts. A brainstorming helper function surfaces synonyms or antonyms of a provided word to spur ideas when users seek to refine their concept. Meanwhile, a concept comparison helper function allows users to specify concept terms and compare their correlation with the input data and ground-truth ratings. To scaffold users' sensemaking process, we also provide a note-taking function that allows them to save scratch notes on concepts and sketches for future reference.

% AND and OR logical operators for concepts
Finally, to allow for further control and refinement of concepts, we enable users to link existing concepts together with logical \texttt{AND} and \texttt{OR} operators to create compound concepts. With a call to \texttt{create\_AND\_concept()}, users can take the logical \texttt{AND} of any number of binary concepts (and can similarly link arbitrary concepts with an \texttt{OR} relation using the \texttt{create\_OR\_concept()} function). This grants users the ability to \rev{express more complex concepts, such as a single concept that can manifest in several ways or a multimodal concept that requires both image and text signals.}

\subsubsection{Creating sketches with the API}
Once a user has authored several concepts, they can proceed to create the full sketch model that aggregates those concepts by calling \texttt{create\_sketch\_model()}. This function \rev{displays widgets for the user to select the concepts and aggregation method (default: linear regression) for their sketch model}~(\autoref{fig:sys_api_sketches}~\circled{A}).

\begin{figure*}[!tb]
  \includegraphics[width=\textwidth]{figures/sys_api_sketches_v3.pdf}
  \caption{
      Authoring sketches with {ModelSketchBook} \rev{in a computational notebook}. 
      (A)~The \texttt{create\_sketch\_model()} function accepts user inputs on the concepts to aggregate, with optional parameters to set the aggregation method and sort-column.
      (B)~Then, the API outputs a dataframe displaying all training examples sorted by the specified column. This view shows all input fields, all concept scores, and the sketch model's prediction. It also displays the ground truth rating and the error between the sketch prediction and ground truth rating to aid error analysis.
  }
  \label{fig:sys_api_sketches}
\end{figure*}

After executing the cell, the API creates the new sketch model and returns a dataframe visualization that displays all of the input fields of the training examples, all of the relevant concept scores, and the overall prediction produced by the sketch model~(\autoref{fig:sys_api_sketches} \circled{B}). This view also includes the ground-truth ratings and the difference between the sketch prediction and these ground-truth ratings. Users can choose to sort by various columns to aid their understanding of the model outputs.
\cut{: sorting by the sketch prediction surfaces an ordering that represents the sketch model's understanding of the modeling task; sorting by the ground-truth rating foregrounds the ``intended'' understanding of the modeling task; sorting by the difference (or absolute value of difference) between the sketch prediction and ground-truth rating highlights areas where the sketch model most drastically deviated from the intended decision-making behavior.}
The sketch model output also displays traditional performance metrics for both regression and classification formulations of the task based on the ground-truth labels for the training examples; we display Mean Absolute Error (MAE), Classification Accuracy, F1 Score, Precision, and Recall.

% Evaluating sketch on unseen data
Finally, the API provides functions that help the user to assess their sketch models. The \texttt{compare\_sketches()} function allows the user to compare performance metrics for specified sketches \rev{by displaying the performance metrics side by side in a plot similar to Figure~\ref{fig:mean_metric_plot}}. The \texttt{test\_sketch()} function allows users to test out sketch models on a labeled or unlabeled validation set (if one is provided) to get a sense for how well it generalizes to a broader set of examples. \rev{After the user selects a sketch model and a dataset, this function produces a dataframe similar to \autoref{fig:sys_api_sketches} \circled{B}, only including the ground truth rating and error if present.}
\revFinal{Please see Appendix~\ref{appendix:msb-process-overview} for an overview of the three function calls required to instantiate a sketchbook, concept, and sketch model}.

\subsubsection{Implementation}
% More detailed implementation details/settings; Colab setup
The {ModelSketchBook} API was authored in Python. We use OpenAI's API for GPT-3 to perform zero-shot prompt-based text classification and use the \texttt{text-davinci-002} model, the current state-of-the-art GPT-3 variant. We use OpenCLIP~\cite{open_clip}, an open-source version of CLIP, to perform zero-shot image regression; we use a Vision Transformer (ViT) model (\texttt{ViT-B-32 -quickgelu}) pre-trained on the \texttt{laion400m\_e32} dataset. We use scikit-learn~\cite{scikit_learn} model implementations for our sketch model aggregators. 
All training and inference takes place on the local machine on which the notebook is running (i.e., a user's own machine if they are running a local Juypter notebook, or a Google cloud server if they are running a Colab notebook). 
\rev{
When loaded in a computational notebook environment, the input interface elements are rendered using the ipywidgets package. The output visualizations are rendered using Pandas dataframes with custom CSS styling.
}


==> sections/old_versions/4_eval_v1.tex <==
\msb{I tend to just call these sections ``Evaluation'' instead of ``User evaluation'' or ``user study'' because those terms imply usability studies in industry, whereas what we're trying to do is typically more of a summative evaluation and hypothesis testing}

Our study aims to evaluate the impact of applying a model sketching approach to a realistic model authoring task with experienced machine learning practitioners. Since our overall goal with model sketching is to shift the cognitive frame with which ML practitioners approach the task of authoring models, our evaluation centers on these main research questions:

% Summary of our research questions 
% \begin{itemize}
%     \item RQ1---\textit{Does model sketching prompt a change in ML practitioners' cognitive processes?} Using this approach, do they successfully shift away from technical and implementation-oriented thinking and towards higher-level, design-oriented thinking?
%     \item RQ2---\textit{Does such a shift in their cognitive process reap benefits for model development?} When ML practitioners shift to higher-level thinking, do they produce better models, especially in terms of anticipating modeling gaps and considering value tradeoffs in model design? What effect does this mode of thinking have on ML practitioners' sense of comfort and expressivity?
% \end{itemize}

\begin{itemize}
    \item RQ1---\textit{How does engaging in model sketching impact the cognitive focus of ML practitioners during model development?} Using this approach, do they successfully shift away from technical and implementation-oriented thinking and towards higher-level, design-oriented thinking? \msb{I'd be careful with claiming that what they're doing is design-oriented thinking, since that could mean lots of things. (Iteration? Product design? UI design?) I'd suggest just cutting and focusing it on higher level or concept-oriented}
    \item RQ2---\textit{What are the outcomes of a model sketching workflow for ML models and ML practitioners?}
    When ML practitioners shift to higher-level thinking, do they produce better models, especially in terms of anticipating modeling gaps and considering value tradeoffs in model design? What effect does this mode of thinking have on ML practitioners' model authoring experience? \msb{When we say ``do they produce better models'', we're setting the reader up to expect a comparison evaluation. We can show that they do anticipate modeling capts and value tradeoffs, but we don't have the counterfactual that they wouldn't do so if they were using traditional tools, right? The closest we have is the before/after comparison.}
\end{itemize}

A successful outcome would mean that ML practitioners orient their modeling plans around conceptual modeling approaches rather than particular implementation methods after engaging in a model sketching workflow. Furthermore, success would require that participants begin to grapple with ethical value tradeoffs and identify gaps in the modeling task while maintaining a reasonable level of comfort \msb{minor, but as a reader, this makes me go, ``hmmm, how do would they measure what is a `reasonable' level of comfort?''} and expressivity in the modeling process.
To address these research questions, we designed a user evaluation for participants with significant machine learning experience to use our \texttt{ModelSketchBook} API to author models that would detect hateful memes posted on a social platform.

\subsection{Study design}

\subsubsection{Study format}
% Description of the task we posed to users
Our evaluation consisted of an hour-long study session. Participants were sent a brief 10-minute labeling task to complete before the study session so that we could use their personal ground-truth ratings for the model-authoring task. We asked them to provide labels for 40 examples; 20 examples were used as a training set during the study session, and 20 were reserved as a test set. During the hour-long study session, the first 15-20 minutes were allocated to consent, Colab notebook setup, and a tutorial and video demo of the \texttt{ModelSketchBook} API. Then, the participant was given about 30 minutes to work on the model authoring task using the \texttt{ModelSketchBook} API in a Colab notebook. Finally, the last 10-15 minutes were split between a brief interview on their experience and a post-study survey questionnaire.

\subsubsection{The Hateful Memes dataset}
% Background on the Hateful Memes dataset
\msb{can be shortened to 1-2 sentences:} The Hateful Memes dataset originated from the Hateful Memes Challenge~\cite{kiela_hatefulMemes} launched in 2020 by Facebook AI. The dataset holds over 10,000 multimodal meme examples (combining both text and images) that were created by the company, but were directly based on existing real-world memes. The goal of this challenge was to bring awareness and interest to the challenge of identifying multimodal hate speech. This task is challenging for AI systems because it requires deep integration of text and images, as the meaning of a meme is highly dependent on interactions between the semantics of both modalities. Further, memes are also very dependent on references and external world knowledge that cannot be extracted from the meme content itself. 

\msb{shorten to around 2 sentences} We selected this task for our user evaluation because we sought to evaluate model sketching in a difficult, realistic setting. As an example of an open challenge in AI that model developers are actively working on, the Hateful Memes Challenge is a good fit here and will pose similar challenges for our model sketching approach. 
In addition, we wanted our task to be relatively subjective and not have a clear right-or-wrong answer so that there would be a sufficiently broad model design space for participants to work with. This task was again a good fit not only because humor is subjective, but also because there is also broad disagreement among the population on what constitutes hate speech and toxicity~\MSLcite{ disagreement work}.
Finally, since we are interested in having ML practitioners consider the ethical tradeoffs of different modeling approaches, the Hateful Memes task was very suitable since decisions around multimodal hate speech and content moderation commonly involve tough value tradeoffs.

\subsubsection{Hateful Memes detection task}
We described the modeling task to each participant as follows: ``Your task today will be to create a model that will determine whether meme posts should be allowed to remain on a social media platform or should be flagged for removal. You will create sketch models to generate removal-likelihood scores for the posts in the dataset, where a 0 indicates a benign post and a 1 indicates very problematic post. Here's a reminder of the scoring scheme (the same one that you used for the labeling task)''. The scoring scheme that we provided for their labeling task was: $0.00$ = Benign (keep); $0.25$ = Slightly problematic (may be questionable, but keep); $0.50$ = Threshold (problematic enough to be removed from platform); $0.75$ = Problematic (remove); $1.00$ = Very problematic (remove).

\subsubsection{Pre- and Post-task written responses}
Before receiving an introduction to the model sketching approach or the \texttt{ModelSketchBook} API, we asked participants to write out their modeling approach for the Hateful Memes task based on their current knowledge along with an estimate of the time it would take to implement that plan. After participants viewed the tutorial and demo, but before they started using the \texttt{ModelSketchBook} API, we asked them to brainstorm an initial set of at least three concepts that they might want to use in the task. At the end of the task period, we asked participants to once again describe their planned modeling approach for the Hateful Memes task, where they could assume that they had access to a tool like the \texttt{ModelSketchBook} API, but they did not have to use such a tool. We also asked participants to write down any learnings or takeaways they had after engaging in this task, and we asked them to specify which sketch model they viewed as the ``best sketch'' among the sketch models they authored.

\subsubsection{Post-task interview and survey}
% Overview of the starter and concluding tasks, survey questions, and interview questions as well as our planned analysis method (esp for qualitative results)
In post-task interview, we asked participants to walk through their notebook and explain their thought process as they iterated on concepts and sketches. Then, we asked them to compare and contrast this model sketching experience with their prior experience authoring machine learning models. Lastly, we asked them what they learned from the model sketching process and whether they had any takeaways.
Then, our final post-task survey asked participants about their satisfaction with their concept models and sketch models, their perception of the extent of changes and improvements in their modeling approach, their perception of the comfort and expressivity of prior modeling tools and of \texttt{ModelSketchBook}, and other aspects that they liked and disliked about the model sketching experience. 
The full text of our interview script and survey is included in Appendix section \msl{TODO}.

\subsection{Study measurements and data}
\msb{might be able to cut this} Based on this study design, we collected several forms of data, which we summarize here.
\begin{itemize}
    \item \textbf{Sketchbook data}. We export the participant's sketchbook, which includes all concepts and sketches that they authored as well as performance metrics and scratch-notes they entered.
    \item \textbf{Free-text written responses}. Participants provide open-ended text responses in the pre- and post-task within the Colab notebook and in the post-task survey.
    \item \textbf{Likert scale survey responses}. Participants answered several Likert scale questions in the post-task survey.
    \item \textbf{Interview responses}. Participants provided verbal responses during the interview. We extracted transcripts from the recording of the study session.
\end{itemize}

\subsection{Participant recruitment}
% Details on participant pool, recruitment methods, demographics
We sought participants who had significant experience with machine learning and who had prior experience using IPython notebooks. We recruited participants by sending emails to university mailing lists for Computer Science and AI-related groups, and we sent recruitment materials to personal contacts working in the AI industry to share and forward with their networks. Participants were sent a signup survey to provide demographic information and background information on their technical experience. 

We selected from among participants who answered either ``rather much'' or ``very much'' (the two highest options on a 5-point Likert scale) to indicate their amount of experience with IPython notebooks and their experience with machine learning. In total, \MSLtempValue{20} users participated in our study. We had \MSLtempValue{5} women, \MSLtempValue{13} men, \MSLtempValue{1} non-binary participant, and \MSLtempValue{1} participant who preferred not to share their gender; we had \MSLtempValue{16} Asian, \MSLtempValue{2} White, \MSLtempValue{1} participant who identified as White and Hispanic, and \MSLtempValue{1} participant who identified as White and Middle-Eastern. We had \MSLtempValue{10} participants aged 18-24 and \MSLtempValue{10} aged 25-34. For highest educational attainment, \MSLtempValue{10} participants had earned a doctorate, master’s or other professional degree, \MSLtempValue{6} had earned a four-year degree, \MSLtempValue{3} had completed some college education, and \MSLtempValue{1} had graduated from high school. There were \MSLtempValue{10} participants who identified as ML engineers or data scientists working in industry, and there were \MSLtempValue{10} participants who identified as students who use ML in their work or research.
\msl{TODO: potentially add stats on size of companies where industry ML practitioners worked. TODO: update demographic numbers after our final participant pool.}
We compensated participants with a \$60 Amazon gift card for completing the hour-long study session. All studies were conducted remotely over video conferencing.

==> sections/old_versions/4_eval_v2.tex <==
Our study aims to evaluate the impact of applying a model sketching approach to a realistic model authoring task with experienced machine learning practitioners. Since our overall goal with model sketching is to shift the cognitive frame with which ML practitioners approach the task of authoring models, our evaluation centers on these main research questions:

\begin{itemize}
    \item RQ1---\textit{How does engaging in model sketching impact the cognitive focus of ML practitioners during model development?} Using this approach, do they successfully shift away from technical and implementation-oriented thinking and towards higher-level, concept-oriented thinking? 
    % \msb{I'd be careful with claiming that what they're doing is design-oriented thinking, since that could mean lots of things. (Iteration? Product design? UI design?) I'd suggest just cutting and focusing it on higher level or concept-oriented}
    \item RQ2---\textit{What are the outcomes of a model sketching workflow for ML models and ML practitioners?}
    When ML practitioners shift to higher-level thinking, what kind of models do they produce? How do they anticipate modeling gaps and consider value tradeoffs in model design? What effect does this mode of thinking have on ML practitioners' model authoring experience? 
    % \msb{When we say ``do they produce better models'', we're setting the reader up to expect a comparison evaluation. We can show that they do anticipate modeling capts and value tradeoffs, but we don't have the counterfactual that they wouldn't do so if they were using traditional tools, right? The closest we have is the before/after comparison.}
\end{itemize}

\msb{I cut a bit of this, a little redundant:} %A successful outcome would mean that ML practitioners orient their modeling plans around conceptual modeling approaches rather than particular implementation methods after engaging in a model sketching workflow. Furthermore, success would require that participants begin to grapple with ethical value tradeoffs and identify gaps in the modeling task while maintaining comfort and expressivity in the modeling process.
To address these research questions, we designed a user evaluation for participants with significant machine learning experience to use our {ModelSketchBook} API to author models that would detect hateful memes posted on a social platform.

\subsection{Study design}

\subsubsection{Study format}
% Description of the task we posed to users
Our evaluation consisted of an hour-long study session. Participants were sent a brief 10-minute labeling task to complete before the study session so that we could use their personal ground-truth ratings for the model-authoring task. We asked them to provide labels for 40 examples; 20 examples were used as a training set during the study session, and 20 were reserved as a test set. During the hour-long study session, the first 15-20 minutes were allocated to consent, Colab notebook setup, and a tutorial and video demo of the {ModelSketchBook} API. Then, the participant was given about 30 minutes to work on the model authoring task using the {ModelSketchBook} API in a Colab notebook. Finally, the last 10-15 minutes were split between a brief interview on their experience and a post-study survey questionnaire.

\subsubsection{The Hateful Memes detection task}
\msb{I retitled the section and merged it with the next one}
% Background on the Hateful Memes dataset
% \msb{can be shortened to 1-2 sentences:} 
The Hateful Memes dataset originated from the Hateful Memes Challenge~\cite{kiela_hatefulMemes} launched in 2020 by Facebook AI to bring attention to the complex task of identifying multimodal hate speech. The dataset holds over 10,000 multimodal meme examples (combining text and images) based on real-world memes.
The scoring scheme that we provided for their labeling task was: $0.00$ = Benign (keep); $0.25$ = Slightly problematic (may be questionable, but keep); $0.50$ = Threshold (problematic enough to be removed from platform); $0.75$ = Problematic (remove); $1.00$ = Very problematic (remove).
% This task is challenging for AI systems because it requires deep integration of text and images, as the meaning of a meme is highly dependent on interactions between the semantics of both modalities. Further, memes are also very dependent on references and external world knowledge that cannot be extracted from the meme content itself. 

% \msb{shorten to around 2 sentences} 
We selected this task for our user evaluation because we sought to evaluate model sketching in a difficult, realistic setting, and this task represented an open challenge that ML practitioners were actively working on.
In addition, we wanted our task to be relatively subjective and not have clear right-or-wrong answers to provide participants a sufficiently broad model design space. This task was again a good fit not only because humor \msb{maybe memes instead of humor? the thing that's the subject here isn't the humor, it's the hatred} is subjective, but also because there is also broad disagreement among the population on what constitutes hate speech and toxicity~\cite{gordon_dd, kumar2021designing}.
Finally, since we are interested in having ML practitioners consider the ethical tradeoffs of different modeling approaches, the Hateful Memes task was very suitable since decisions around multimodal hate speech and content moderation commonly involve tough value tradeoffs.

%\subsubsection{Hateful Memes detection task}
\msb{I cut the quoted task, and moved up the scores}%We described the modeling task to each participant as follows: ``Your task today will be to create a model that will determine whether meme posts should be allowed to remain on a social media platform or should be flagged for removal. You will create sketch models to generate removal-likelihood scores for the posts in the dataset, where a 0 indicates a benign post and a 1 indicates very problematic post. Here's a reminder of the scoring scheme (the same one that you used for the labeling task)''. 


\subsubsection{Pre- and Post-task written responses}
Before receiving an introduction to the model sketching approach or the {ModelSketchBook} API, we asked participants to write out their modeling approach for the Hateful Memes task based on their current knowledge along with an estimate of the time it would take to implement that plan. After participants viewed the tutorial and demo, but before they started using the {ModelSketchBook} API, we asked them to brainstorm an initial set of at least three concepts that they might want to use in the task. At the end of the task period, we asked participants to once again describe their planned modeling approach for the Hateful Memes task, where they could assume that they had access to a tool like the {ModelSketchBook} API, but they did not have to use such a tool. We also asked participants to write down any learnings or takeaways they had after engaging in this task, and we asked them to specify which sketch model they viewed as the ``best sketch'' among the sketch models they authored.

\subsubsection{Post-task interview and survey}
% Overview of the starter and concluding tasks, survey questions, and interview questions as well as our planned analysis method (esp for qualitative results)
In a post-task interview, we asked participants to walk through their notebook and explain their thought process as they iterated on concepts and sketches. Then, we asked them to compare and contrast this model sketching experience with their prior experience authoring machine learning models. Lastly, we asked them what they learned from the model sketching process and whether they had any takeaways.
Our final post-task survey asked participants about their satisfaction with their concept models and sketch models, their perception of the extent of changes and improvements in their modeling approach, their perception of the comfort and expressivity of prior modeling tools and of {ModelSketchBook}, and other aspects that they liked and disliked about the model sketching experience. 
The full text of our interview script and survey is included in the Appendix.
% ~\ref{section:appendix_interview_questions, section:appendix_survey_questions}.


%\subsection{Study measurements and data}
\msb{I cut this section}
% Based on this study design, we collected several forms of data, which we summarize here.
% \begin{itemize}
%     \item \textbf{Sketchbook data}. We export the participant's sketchbook, which includes all concepts and sketches that they authored as well as performance metrics and scratch notes they entered.
%     \item \textbf{Free-text written responses}. Participants provided open-ended text responses in the pre- and post-task within the Colab notebook and in the post-task survey.
%     \item \textbf{Likert scale survey responses}. Participants answered several Likert scale questions in the post-task survey.
%     \item \textbf{Interview responses}. Participants provided verbal responses during the interview. We extracted transcripts from the recordings of the study sessions.
% \end{itemize}

\subsection{Qualitative analysis}
For the free-text written responses, we sought to summarize the high-level themes that emerged from our participants, so the codes were not the product, but our process~\cite{mcDonald2019IRRQualitativeResearch}. The first author conducted an inductive analysis to summarize participants' model authoring experiences. The first step of this process was to read through all written responses multiple times. Then, the qualitative open coding~\cite{charmaz2006constructing} process was iterative and took place in two phases: the first phase involved line-by-line response coding to closely reflect the original data (e.g., ``noticed minimal representation of violence in the dataset,'' ``plans to use a transformer model,'' or ``there was inconsistency among the labels''). Then, the second phase synthesized codes from the first phase into higher level themes (e.g., ``data representativity'' or ``labeling methodology''). After this theme generation, written responses were coded based on the themes to characterize participants' planned modeling approaches and their learnings and takeaways from the task.

\subsection{Participant recruitment}
% Details on participant pool, recruitment methods, demographics
We sought participants who had significant experience with machine learning and who had prior experience using IPython notebooks. We recruited participants by sending emails to university mailing lists for Computer Science and AI-related groups, and we sent recruitment materials to personal contacts working in the AI industry to share and forward with their networks. Participants were sent a signup survey to provide demographic information and background information on their technical experience. 

We selected from among participants who answered either ``rather much'' or ``very much'' (the two highest options on a 5-point Likert scale) to indicate their amount of experience with IPython notebooks and their experience with machine learning. In total, 17 users participated in our study. We had 3 women, 12 men, 1 non-binary participant, and 1 participant who preferred not to share their gender; we had 14 Asian participants, 2 White participants, and 1 participant who identified as White and Hispanic. We had 9 participants aged 18-24 and 8 aged 25-34. For highest educational attainment, 9 participants had earned a doctorate, master’s or other professional degree, 4 had earned a four-year degree, 3 had completed some college education, and 1 had graduated from high school. There were 9 participants who identified as ML engineers or data scientists working in industry, and there were 8 participants who identified as students who use ML in their work or research. Of the industry practitioners, 3 were employees of startup companies, and 6 were employees of large companies (with 1000+ employees). Participants reported an average of 3.6 years of experience working with machine learning.
We compensated participants with a \$60 Amazon gift card for completing the hour-long study session. All studies were conducted remotely over video conferencing.

==> sections/old_versions/5_results_v1.tex <==
% Potential tasks
% - (*) Controlled study (hateful memes)
% - (*) Exploration of modeling tasks (case studies)
% - Open-ended study (participant choice of task)

% Potential axes
% - Extent of design exploration
% - Characterizing user behavior qualitatively
% - Time spent
% - Problems/limitations

% Main takeaways
% - Change in cognitive process (thinking by doing)
%   - Shift in focus
%       --> from technical to conceptual
%       --> from implementation to design/values
%   - Concept evolution
% 
% - Outcomes of this change in cognitive process
%   - Noticing gaps in other parts of the modeling pipeline (ex: data, problem formulation, labeling, how scores are translated to user interface)
%   - Considering approaches beyond those in their toolkit
%   - Considering more drastic or more ambitious redesigns (rather than minor tweaks)
% - 

\msb{Inserting a reminder note here that the results and discussion should both cover failure models and boundaries of the system --- in what ways did it not achieve our goals, and under what conditions would it not work well?}
\msl{Not sure if you already read through the section; does the ``Failure modes'' section not cover what you're describing above? I also have a limitations section in the Discussion. Can add more to both though!}
\msb{hadn't read, was just making sure to mention it before I forgot!}

\msb{example of tighter sentence structure:} ML practitioners successfully engaged in model sketching, shifting their attention more towards higher-level, model design questions rather than technical model implementation details. This cognitive shift helped ML practitioners to better explore the model design space and identify gaps in the modeling approach while achieving performance that exceeds existing baselines and requiring a small fraction of the time that would ordinarily be required to author a functional model. 

Using our \texttt{ModelSketchBook} API, participants were able to successfully author sketch models for the Hateful Memes task. Participants on average authored about \MSLtempValue{14.9} (SD=\MSLtempValue{4.8}) concept models and produced \MSLtempValue{4.4} (SD=\MSLtempValue{2.8}) different sketch models that built on those concepts~(Figure~\ref{fig:concept_sketch_boxplot}). While we allocated approximately 30 minutes to the main model authoring task, participants in practice worked on the task for a slightly shorter time period---\MSLtempValue{27.1} minutes (SD=\MSLtempValue{4.8}) on average---due to time constraints. \msb{a question I might have as a reader, given that you're using an existing dataset that presumably has ground truth results --- how was the performance of these folks' sketch models vs current SOTA for the task?}

\begin{figure}[!tb]
  \includegraphics[width=0.6\textwidth]{figures/results/concept_and_sketch_num_boxplot.pdf}
  \caption{There was considerable variation in the number of concept and sketch models that participants authored, but all participants authored 8+ concepts and 2+ sketches within our approximately 30-minute task period. \msl{(N=8)}.
  }
  \label{fig:concept_sketch_boxplot}
\end{figure}

\subsection{Changes in the cognitive process of model authoring}
% How we observed a shift from technical+implementation-oriented to conceptual+design/value-oriented thinking
Addressing RQ1, model sketching aided ML practitioners in shifting their thinking from technical, implementation-oriented factors toward higher-level, conceptual, design-oriented factors of model development. 

\subsubsection{Changes in planned modeling approach}
\msb{this repeats information from just a few paragraphs ago, cut?:} To capture how our participants commonly think about and approach machine learning modeling, we asked them to describe their modeling plan for the Hateful Memes task before we introduced our model sketching approach. We then asked them to describe their modeling plan again after the model sketching task, assuming that they would have access to the \texttt{ModelSketchBook} API, but would not be required to use it.

In their pre-task modeling plans, participants tended to focus on implementation details such as specific modeling methods or architectures (e.g., transformer models, convolutional neural networks, supervised model, linear classifier), ML conventions like dataset splits and performance metrics, and general ML ``hygiene'' like ensuring that the examples span a range of scores and adjusting for skewed or imbalanced labels~(Table~\ref{table:modeling_plan}). Then, in their post-task modeling plans, nearly all participants described an approach that would use the \texttt{ModelSketchBook} API \msb{given the novelty bias, I think this sentence should be taken with a grain of salt --- cut and move on to the next sentence?}. Many participants described that they would spend time on brainstorming a broad range of concepts relevant to the decision-making task and that they would iterate on their concepts by inspecting sketch model outputs. Participants also branched out to mention that they would like to consider different subclasses of harm and that they would benefit data labels and model testing from external, diverse users \msb{this one seems more persuasive than the other results, which could just be because of the novelty}.

\msb{I think one or two quotes of before examples and after examples could go a long way here}

\begin{table*}[!tb]
  \centering
  \footnotesize
    \begin{tabular}{p{0.45\textwidth}c|p{0.45\textwidth}c}
    \toprule
    \textbf{Pre-task modeling plan} &  \textbf{\#} &
    \textbf{Post-task modeling plan} &  \textbf{\#}\\
    \midrule
    {Evaluating on training and validation set} & 5 
    & {Planned to use ModelSketchBook} & 9 \\

    {Building low-level features stemming from data} & 5 
    & {Spending time brainstorming a broad range of related concepts} & 6 \\

    {Training on examples with a range of hate/toxicity levels} & 5 
    & {Consider how to aggregate concepts} & 4 \\

    {Specific model architectures or techniques (e.g., transformer model, convolutional neural network)} & 3 
    & {Iterate on concepts by inspecting sketch model outputs} & 4 \\

    {Adjusting for skew or imbalance in labels} & 3 
    & {Consider different categories of harm} & 2 \\

    {Referring to performance metrics (e.g., Accuracy, F1, AUC)} & 2 
    & {Engage the broader population in labeling and testing the model} & 2 \\
    \bottomrule
    \end{tabular}
    \caption{A summary of themes identified from participants' modeling plans before and after the study. Participants willingly chose to adopt the model sketching approach in their future modeling plans and shifted from more technical, implementation-related plans to more procedural, value-oriented plans. \msl{(N=11)} \msb{as a reader, I start wondering --- how was this coded? was there IRR? I didn't notice it in the method.}
    }
    \label{table:modeling_plan}
\end{table*}
% \item Source: Written response in NB
% \item Qualitative coding of themes (grouping into technical vs conceptual)

\subsubsection{Concept evolution}
One window into participants' mindset and approach is the way that their concepts evolve over time while using \texttt{ModelSketchBook}. We identify three main types of intent underlying concept authorship: 1)~\textit{concept innovation}, cases where participants come up with ideas for entirely distinct concepts that they hadn't brainstormed before, 2)~\textit{concept execution}, cases where participants are still continuing an existing concept idea that remains consistent in their mind, but are experimenting with different ways to actualize that concept via concept term inputs, and 3)~\textit{concept abandonment}, cases where participants decided not to continue with a concept and did not include the concept in their future sketch models. \msb{I don't buy these next two sentences: sometimes the point of sketches is to be able to confidently discard them as not promising directions}We hope that our model sketching approach will enable participants to engage in more concept innovation and less concept execution and concept abandonment. The latter two phenomena are still important steps that may need to happen for the user to effectively instantiate their vision of a concept with a zero-shot model, but this incremental, execution-oriented behavior should not dominate the workflow.

\msb{the abstract number of concepts is useful, but it's hard for a reader to wrap their head around --- is this impressive? not impressive? I think a wide variety of examples of the kinds of concepts people created would help substantially}
Analyzing these phenomena among concept evolution histories for all participants, we observe that on average, participants engage in \MSLtempValue{7.4} instances of concept innovation, which we define as the number of distinct concept ideas that were \textit{not} in the participant's original brainstormed list. Participants on average display \MSLtempValue{4.6} instances of concept execution, which we define as the number of concepts authored that were continuations of the same concept idea (for example, switching from an image-based racism concept to a text-based racism concept or changing from a concept term of ``racism'' to one of ``race''). Then, participants underwent concept abandonment for an average of \MSLtempValue{5.6} concept ideas; we define this phenomenon as the number of concept ideas that were not ultimately used in the user's self-designated ``best'' sketch model. Thus, it appears that while participants run into concept execution work and face concept abandonment, they tend to engage in a greater amount of concept innovation overall \msb{again, not sure concept abandonment is bad}.
\msl{(N=9)}
% \item Source: Sketchbook from NB
% \item Direct analysis of progression of concepts and sketches in sketchbook (concept terms, grouping, progression over time)
% \item Qualitative analysis of notes attached to concepts and sketches

\subsubsection{Participants' thought process}
% \msl{TODO: summarize themes from interview responses}
Finally, participants themselves perceived a change in their mode of thinking when they engaged in model sketching. First, participants noted \msb{this phrase, or something like it, has recurred several times in this section and the intro, cut it and go straight to the quotes?} that they were able to shift away from more technically-minded details toward larger conceptual, design-oriented questions; P10 described model sketching as ``a different way of thinking about [modeling]'' compared to their day-to-day modeling work, which was ``a lot more manual and technical and a lot more work and a lot more complex''. Some participants felt that this approach allowed them to take a more \textit{long-range, bird's-eye view} of the modeling process: P1 expressed that ``this process helps put into perspective the long term goals and the structure of the ML lifecycle''. Others described the model sketching process as refreshingly \msb{are these quotes? if so, quote them --- they're great} \textit{creative} and \textit{artistic}, especially in comparison to their typical model authoring experiences that had felt more formulaic or uninspired. As P12 put it, ``[model sketching] forced me to think creatively in a way I don't normally have to. Normally, my work is pretty boilerplate-y and repetitive. In this case, the model's performance was much more limited by my own creativity and ability, so it felt more like I had artistic direction in how the model did.'' Lastly, participants expressed that they enjoyed this new mode of thinking. P1 shared that they ``really enjoyed the experience of thinking about models in this manner'' while P21 said that they ``liked the idea to approach things from how a human will think about things by defining these concepts.''
% \item Source: Interview, Survey
% \item Qualitative analysis of interview responses
% \item Quantitative analysis to survey Q on extent of change/improvement in modeling approach

\subsection{Modeling outcomes}
% TODO: how this produces better or more societally-beneficial models
\msb{throughout, these subsections are not that long, so I would aim for single sentence overview paragraphs rather than full paragraphs like these}
Regarding RQ2, we observed that an apparent high-level cognitive shift in focus during model development brought about many concrete benefits for the models themselves. Participants were able to explore a broad range of high-quality concepts \msb{that's a judgment we are making, but we're biased, so I don't think we can judge whether they are ``high quality concepts''} in the decision-making space, and they were able to rapidly identify gaps in the modeling setup before diving into implementation work. In addition, participants were able to iteratively author sketch models that were more performant than their initial sketch models and that were also more performant than models trained using more traditional methods based on uninterpretable raw image and text features \msb{this is again where I wonder how these models do compared to other SOTA models for the hateful memes dataset}. Finally, ML practitioners in our study were able to achieve all of these benefits in a sliver of the time that they'd estimated would be required to implement a full-scale machine learning model for this task. 

\subsubsection{Identifying modeling gaps}
One of the aims of model sketching is that, in focusing ML practitioners' attention on higher-level design decisions, it will allow them to scope out to identify flaws in not only their model, but in the problem formulation, dataset, and deployment context that surround it. After the model authoring task, we asked participants to describe their learnings and takeaways from the task as well as any gaps they noticed in the modeling approach~(Table~\ref{table:modeling_gaps}) \msb{In general, you shouldn't need to repeat the method in the results section---you should be able to just start with the results}. We found that participants learned a great deal from their brief model sketching task and gained insights beyond just the model itself \msb{how did we evaluate whether they learned a great deal? how do we evaluate whether they gained insights beyond the model? these seems difficult to prove}. Participants uncovered major categories of harm that were not sufficiently represented in the provided sample of the dataset, and they noted that models built on this data may fail in practice due to distribution shift since the memes in the dataset appeared unrealistic compared to current online memes. Participants also identified limitations of the labeling approach such as class imbalance and inconsistent ratings. They also gained intuitions or hunches about the task itself: participants discovered that for these memes, text was often more meaningful since the images were usually quite benign, and they started to form a sense of cases where multimodal approaches may reap more benefits. 

\begin{table*}[!tb]
  \centering
  \footnotesize
    \begin{tabular}{p{0.2\textwidth} p{0.5\textwidth} p{0.05\textwidth}}
    \toprule
    \textbf{Theme} & \textbf{Learning or Takeaway} & \textbf{\#}\\
    \midrule
    {Data representativity} & 
    {There is a need for greater representation in the data. Participants noted that there were currently not enough examples of homophoboa, transphobia, and nudity} & 
    {2}\\[0.4cm]
    
    {} & 
    {The dataset is currently unrealistic and contrived. It needs to better match the distribution of what is actually posted online.} & 
    {1}\\
    \midrule
    {Nuances of the task} & 
    {The textual modality seems more important than the image modality for this task} & 
    {2}\\[0.4cm]

    {} & 
    {Memes are tricky to understand and label. Their meanings can be vague and dependent on inside knowledge.} & 
    {2}\\[0.4cm]
    
    {} & 
    {It may be useful to span the modalities and consider the kinds of cases where images are more helpful or where text is more helpful} & 
    {2}\\
    \midrule
    {Labeling methodology} & 
    {Class imbalance has a large impact on modeling and makes it difficult to calibrate a model. 
    % Since their labels were skewed towards non-removal, it was hard for their model to capture the cases that do necessitate removal
    } & 
    {2}\\[0.4cm]
    
    {} & 
    {Their own labels appeared to be internally inconsistent, so they need to gather a larger set of labels from a diverse population} & 
    {1}\\[0.4cm]
    
    {} & 
    {It would be valuable to increase the removal-score granularity beyond binarization for the classification variant} & 
    {1}\\
    \bottomrule
    \end{tabular}
    \caption{After performing a model sketching task, participants noted gaps in the modeling approach in terms of data representativity and labeling methodology and gained a better understanding of the nuances of the task. \msb{After looking at this table several times, I'm still not entirely sure what it's reporting. Are these themes in the insights that participants derived from having engaged in model sketching? I'm not sure what question about our research this is answering.}}
    \label{table:modeling_gaps}
\end{table*}

% \item Source: Written response in NB, Interview
% \item Summary of gaps identified with counts across participants (ex: data fields, data representativity/balance, problem formulation, labeling method, how scores are translated to user interface)
% \item Deep-dive into particularly compelling examples of identified issues (potentially with quotes)

\subsubsection{Concept diversity}
Participants experimented with a broad variety of concept terms for the Hateful Memes task, ranging from concepts related to race, ethnicity, and culture to concepts related to politics, sentiment, and violence~(Summarized in Table~\ref{table:concept_summary}). Notably, many participants authored concepts that they had not considered in their initial brainstorm (the participants who authored concept models for a topic (see last three columns) often had not written any ideas along that vein in their initial brainstorm (see second column). The process of authoring concept models and sketches helped them to discover important and relevant concepts to incorporate. We are encouraged by these findings since a major goal of the model sketching approach is to have the freedom and flexibility to broadly explore the model design space and experiment with various concepts that may capture differing decision-making approaches.

\begin{table*}[!tb]
  \centering
  \footnotesize % \scriptsize
    \begin{tabular}{p{0.2\textwidth} p{0.15\textwidth} p{0.2\textwidth} p{0.2\textwidth} p{0.2\textwidth}}
    \toprule
    \textbf{Concept Theme} & \textbf{Initial Brainstorm} & \textbf{Concepts (image-based)} & \textbf{Concepts (text-based)} & \textbf{Concepts (logical combinations)}\\
    \midrule
    \textbf{Race, Ethnicity, Culture} & 
    {racist (P3, P5), racism (P7, P9), race (P10), color (P6)} &
    {race (P5), racism (P7, P8), dark skinned (P10)} &
    {racism (P1, P4, P7), racist (P3, P5), white (P5), color (P6), racial (P8), race (P10), ethnicity (P10), culture (P10), muslim (P3, P4, P6)} &
    {racism (text) AND violence (text) (P1)}\\[0.2cm]
    \midrule
    \textbf{Sentiment} & 
    {mean (P5), encouraging (P7), offensive (P8), funny (P8), mean (P8), humor (P7), 
joke (P3)} &
    {anger (P1), scary (P4), positive (P4), humor (P7), offensive (P8), funny (P8), happy (P8), smiling (P8), grotesque (P10)} &
    {happy (P5), unhappy (P5), humor (P7), complain (P7), offensive (P8), funny (P8), hatred (P10), supportive (P10), toxic (P10)} &
    {}\\[0.2cm]
    \midrule
    \textbf{Politics} & 
    {politics (P10)} &
    {political (P3)} &
    {political (P3, P6, P8, P10), politics (P10)} &
    {political (image) OR political (text) (P3),
gun (text) AND political (text) (P6)}\\[0.2cm]
    \midrule
    \textbf{Sexual Content, Nudity} & 
    {sexual (P3), nudity (P4)} &
    {nudity (P4, P5, P10)} &
    {sex (P7), sexual (P10)} &
    {}\\[0.2cm]
    \midrule
    \textbf{Misogyny} & 
    {gender (P6), sexism (P9)} &
    {} &
    {sexist (P1, P5), gender (P6)} &
    {sexist (text) AND violence (text) (P1)}\\[0.2cm]
    \midrule
    \textbf{Bigotry, Discrimination} & 
    {hate speech (P9), hatred (P10), hate (P7)} &
    {} &
    {bigotry (P1), hate speech (P8), 
discrimination (P5)} &
    {bigotry (text) AND racism (text) (P1), 
bigotry (text) AND harm (text) (P1), 
bigotry (text) AND sexist (text) (P1),
discrimination (text) OR happy (text) (P5)}\\[0.2cm]
    \midrule
    \textbf{Violence} & 
    {} &
    {violence (P1, P10), war (P1), fire (P6), klan (P3)} &
    {violence (P1, P7, P8), harm (P1), violent (P5), murder (P5), gun (P6), harassment (P8), terrorism (P8), no terrorism (P8), harmless (P10)} &
    {trolling (text) AND violence (text) (P1),
harassment (text) OR hate speech (text) OR offensive (text) OR terrorism (text) OR violence (text) (P8)}\\[0.2cm]
    \midrule
    \textbf{Religion} & 
    {religion (P6)} &
    {} &
    {religion (P3, P6, P8), religious (P6, P8)} &
    {}\\[0.2cm]
    \midrule
    \textbf{Intersectionality} & 
    {} &
    {} &
    {} &
    {racist (text) AND sexist (text) (P5), 
muslim (text) OR profanity (text) OR racism (text) (P4), 
racist (text) OR sexist (text) (P5),
racism (text) OR sex (text) (P7),
racial (text) OR religion (text) OR religious (text) (P8),
color (text) AND gender (text) (P6)}\\[0.2cm]
    \midrule
    \textbf{Concrete Attributes} & 
    {documentary (P7)} &
    {festival (P4), old photo (P6), animal (P6), police (P6), couple (P6), men and women (P6), married couple (P6)} &
    {taco bell (P8)} &
    {}\\
    \bottomrule
    \end{tabular}
    \caption{Summary of participants' concept models. Here, we include only themes for which 3+ participants authored concepts. We separate concepts that were listed in participants' initial brainstorming notes from concepts that were instantiated in concept models in the three rightmost columns. Among those instantiated concepts, we differentiate concepts based on their input field (image or text) and whether they were logical AND or OR concepts. \msl{N=9} \msb{This table has a lot of high resolution information that makes it hard to pull out the big ideas. For example, are the differences between the brainstorm, image based, text based, and logical combination columns important? What if this were a table that simple reported a bunch of interesting example concepts that participants created? And some of those examples could be text, some could be image, some could be logical. And it could show example inputs and outputs from each of those concept models. ...Actually, it makes me think that the teaser figure could possibly be more gripping by showing some concrete examples like that. Consider something that effectively merges your existing teaser with the example-driven teaser for the stable diffusion concept learning, the image I put in \#rollingtopics?}}
    \label{table:concept_summary}
\end{table*}
% \item Source: Sketchbook from NB
% \item Characterize difference between initial brainstormed concepts vs. concepts in best sketches
% \item Summary of the trends in concepts used for the task across participants; the values taken into account.

\subsubsection{Performance metrics}
To gain a better understanding of the practical functionality of sketch models and the tradeoff that sketch models make compared to full-scale models, we also investigated their performance in terms of standard ML performance metrics~(Figure~\ref{fig:mean_metric_plot}). We compared all participants' self-determined ``best sketch model'' against two kinds of baselines: 1)~\textit{first sketch}, the very first sketch that a participant authored with the \texttt{ModelSketchBook} API and 2)~a set of \textit{raw features} baselines that used only uninterpretable raw image and/or text features to train a model that would capture each participant's ratings \msb{I would need more information to understand this. Is this a bag of words? Raw pixel values? BERT embedding? CLIP embedding? I don't think we could feasibly expect a raw regression to make a useful model with 128-dim embeddings and 20 examples}. The first-sketch baseline allows us to understand whether users are successfully able to improve upon their sketches to achieve higher performance: better alignment between the sketch model and their own ground-truth ratings. The raw-features baseline provides a reference point on how well a more traditional, low-level feature-based modeling approach works for this task. \msb{I think that comparison makes sense more if it's trained on the larger dataset, though?}

We find that overall, participants' ``best sketch'' appeared to outperform both types of baselines, achieving lower Mean Absolute Error (MAE) on the regression version of the task and higher accuracy, F1 score, precision, and recall for the classification version of the task. These results suggest that participants are indeed able to iteratively improve their sketch models to achieve higher alignment with their modeling goals, and that sketch models are just as performant as (and perhaps in this case, even more performant than) standard raw feature-based modeling approaches, all while providing greater expressivity and maintaining human interpretability.

% \item Source: Sketchbook from NB
% \item Comparison of performance of first sketch vs. best sketch
% \item Comparison of performance of raw-features sketch vs. best sketch
% \item (lower-priority) Comparison of performance of SoTA model vs. best sketch

\begin{figure}[!tb]
  \includegraphics[width=0.9\textwidth]{figures/results/mean_metric_plot.pdf}
  \caption{Overall, we observed higher performance---lower error and higher accuracy, F1 score, precision, and recall-- among participants' self-designated ``best'' sketches (the leftmost bar in each plot) compared to a baseline of both their first sketch (second bar from the left) and models that were trained on uninterpretable raw image and text features and participant labels (the three rightmost bars). \msl{(N=8)}.
  }
  \label{fig:mean_metric_plot}
\end{figure}

\subsubsection{Time required}
% \item Source: raw measurement and written response in NB
% \item Compare time estimate provided by participant vs. time spent in tool vs. time to produce SoTA model (ex: for Hateful Memes challenge)
Finally, we note that participants were able to achieve these positive modeling outcomes in a fraction of the time that would be required to author a full machine learning model for this task. Participants' time estimates for executing on their pre-task modeling plans for the Hateful Memes task varied drastically from estimates of half a day to estimates on the order of of several months. However, even considering the most optimistic estimates of several hours, our model sketching approach was able to deliver functional model prototypes in less than 30 minutes. \msb{I try to avoid these kinds of judgments in Results, and defer them to Discussion. So Results is mostly ``what happened'', and Discussion is where we say ``unlocks a drastically different pace''}This shift in the timescale of ML model authoring from a drawn-out, weeks-long project to an exercise carried out at interactive speeds unlocks a drastically different pace of creative iteration and experimentation during model development.

\subsection{Participant experience outcomes}
% TODO: how participants feel about the tool and about their model development process with this different way of thinking
Addressing RQ2 in terms of benefits from the ML practitioner vantage point, we found that participants found the model sketching approach to be comfortable and expressive, and they expressed a great deal of excitement and enthusiasm for this method of model development. \msb{add quotes} Compared to prior experiences authoring machine learning models, participants shared that model sketching was much more interpretable, allowed for fast feedback loops between exploration and modeling, and granted them a greater feeling of agency and creativity.

% \begin{itemize}
%     \item Source: Interview, Survey
%     \item Survey Qs on comfort, expressivity, satisfaction with models, likes/dislikes
%     \item Qualitative analysis of themes on experience/sentiment from interview
% \end{itemize}

\subsubsection{Comparison with existing authoring tools}
In our post-task survey, we asked participants to answer questions related to their experience with more common model authoring tools like Scikit-learn, PyTorch, and TensorFlow as well as their experience with \texttt{ModelSketchBook}~(Figure~\ref{fig:survey_comfort_expressivity}). We found that participants felt similar levels of comfort between the more common model authoring tools and the \texttt{ModelSketchBook} API even though this 30-minute task was their first exposure to our API, and all of our participants has significant experience with model authoring using these more traditional tools. At the same time, we saw that participants reported higher levels of expressivity when using the \texttt{ModelSketchBook} API than when using the common model authoring tools. These results present promising support that our model sketching approach can be successfully adopted by ML practitioners as a lightweight, expressive entrypoint to model authoring.

\begin{figure}[!tb]
  \includegraphics[width=1.0\textwidth]{figures/survey/11_comfort_expressivity.pdf}
  % \setlength{\abovecaptionskip}{0pt}
  % \setlength{\belowcaptionskip}{-10pt}
  % }
  \caption{Upon their first-time use of the \texttt{ModelSketchBook} API, participants indicated similar levels of comfort as they feel with traditional model authoring tools (left), but they indicated higher levels of expressivity using \texttt{ModelSketchBook} (right) \msl{(N=11)}.
  }
  \label{fig:survey_comfort_expressivity}
\end{figure}

\subsubsection{Reflections on the model sketching experience}
In our survey, we also probed users' levels of satisfaction with their concept and sketch models and asked them about the extent to which they felt their own modeling approach changed or improved over time (Figure~\ref{fig:survey_satisfaction_approach}). We observed that participants were highly satisfied with both their concept models and sketch models. \MSLtempValue{All but one} participant rated their satisfaction with both models as ``somewhat satisfied,'' ``satisfied,'' or ``very satisfied.'' \MSLtempValue{All participants} responded that their modeling approach changed as they iterated on concepts and sketches, and \MSLtempValue{the majority} of participants described a ``slight improvement,'' ``noticeable improvement,'' or ``significant improvement'' in their modeling approach.

\begin{figure}[!tb]
  \includegraphics[width=1.0\textwidth]{figures/survey/11_satisfaction_approach.pdf}
  \caption{Participants were largely satisfied with both their concept models and sketch models (left), and most indicated both substantial changes and improvements in their modeling approach throughout the task (right) \msl{(N=11)}. 
  }
  \label{fig:survey_satisfaction_approach}
\end{figure}

In their interview feedback and survey free-responses, participants shared a great deal of excitement about the model sketching approach~(Table~\ref{table:summary_participant_experience}). The most frequently-cited benefits of model sketching were that it was highly interpretable and explainable, easy to use (especially because it required no code), provided fast feedback loops, and prompted them to take on a different, high-level mode of thought. Meanwhile, the main limitations that participants noted were that the notebook environment often became disorganized, that our example-centric (rather than metric-centric) visualizations required more time to interpret, and that they would appreciate more assistance on brainstorming concepts. Multiple participants were excited about the opportunity to allow non-technical users and domain experts who lack ML knowledge to use ModelSketchBook and leverage their domain-specific expertise. They also suggested that we go beyond our notebook prototype to set up a dedicated user interface, and they suggested helper tools that would address potential issues with bias and overfitting in concepts.

\begin{table*}[!tb]
  \centering
  \footnotesize
    \begin{tabular}{p{0.08\textwidth} p{0.25\textwidth} p{0.02\textwidth} p{0.6\textwidth}}
    \toprule
    \textbf{Category} & \textbf{Theme} &  \textbf{\#} & \textbf{Quotes}\\
    \midrule
    % Likes
    {Likes} & 
    {Easy to use and get started} &
    {4} &
    {``...the thing I liked the most was how quickly I was able to get started, like I ran a few lines of code and immediately I was getting some results. So I think ModelSketchBook really makes machine learning more accessible which is really important'' (P9),
    ``I like that I didn't have to write any code for the task.'' (P5),
    ``It's easy to get started and less prone to error'' (P7),
    ``This provides a really solid baseline without writing a single line of code.'' (P3)
    }\\[0.1cm]
    
    {} & 
    {Interpretable, explainable} &
    {4} &
    {
        ``Very interactive and also very interpretable which is something with ML models I usually work with is not the case. So this is super super helpful. It's like a different way of thinking about it.'' (P10),
        ``In terms of interpretability of the decision and explainability, which is also important in this kind of task, it [ModelSketchBook] is very helpful'' (P4)
    }\\[0.1cm]

    {} & 
    {Fast feedback loops} &
    {3} &
    {
        ``This modeling process had a lot more quick feedback loops and iteration of feature exploration and then turning that into models pretty fast, which is a good thing for sure.'' (P5),
        ``In my previous models at work, we do ad targeting, so it's very hard to get this kind of real-time feedback'' (P6)
    }\\[0.1cm]

    {} & 
    {Different, high-level way of thinking} &
    {3} &
    {
        ``I liked the idea to approach things from how a human will think about things by defining these concepts.'' (P21),
        ``...focused around ideas and thinking about the task rather than hyperparameters or technical ML details.'' (P10),
        ``This process helps put into perspective the long term goals and the structure of the ML lifecycle and the pipeline that you need to create: what kind of data you need, which we prioritize, where textual data can provide more insight than image data and vice versa'' (P1)
    }\\
    \midrule
    % Dislikes
    {Dislikes} & 
    {Notebook interface felt messy at times} &
    {3} &
    {``a bit annoying to copy paste some of the cells'' (P5)}\\[0.1cm]
    
    {} & 
    {Takes time to sift through examples to gauge performance} &
    {2} &
    {``hard to go through each example because it's long'' (P6)}\\[0.1cm]

    {} & 
    {Needed more guidance to brainstorm concepts} &
    {2} &
    {
        ``it is hard to make accurate concepts [...] that is more of an issue with choosing relevant features by hand.'' (P9),
        ``Not much experience/guidance on how to come up with concepts creatively.'' (P10)
    }\\
    \midrule
    % Suggestions
    {Suggestions} & 
    {Building a dedicated UI} &
    {2} &
    {
        ``I think taking this out of IPython and having a more native UI would be better'' (P3),
        ``I think having a GUI interface would be nice'' (P21)
    }\\[0.1cm]
    
    {} & 
    {A version tailored for non-technical users and domain experts} &
    {2} &
    {
        ``I think the API is great for model developers who do not have a formal background with ML or deep learning. This API is a super useful tool for folks for product engineers and product managers.'' (P3).
        ``I feel like where this could be really relevant and useful is for folks that don't know much about ML, but know a lot about the task at hand, and for them to get something working in their hands'' (P12)
    }\\[0.1cm]

    {} & 
    {Providing tools to address overfitting and bias} &
    {2} &
    {
        ``It's easy to fall into the trap of just trying to optimize your performance on the examples you're seeing and then ... forget what the rest of the data looks like'' (P8),
        ``Human intervention in designing concepts can be biased.'' (P4),
        ``Perhaps I would miss edge cases.'' (P12)
    }\\
    \bottomrule
    \end{tabular}
    \caption{In written and interview responses, participants shared that they liked the process and cognitive mode that model sketching unlocked. They felt that the tool could be improved with a dedicated UI and additional scaffolding to assist concept brainstorming. \msl{(N=12)}}
    \label{table:summary_participant_experience}
\end{table*}


\subsection{Failure modes}
While our model sketching approach achieved its aims of shifting model developers' cognitive frame and presented a number of benefits for the models they developed and their model authoring experience, we observed several failure modes of the approach. 
% Concept models failing, only can provide another concept term; users often gave up too soon
First, though participants had some promising concept ideas, they were not always able to actualize them with our zero-shot concept model approach. When a participant's concept model failed to give them results that substantially overlapped with their own judgement, there was little recourse other than to attempt another related concept term and see if that achieves better alignment. However, participants often relied heavily on the results of the first concept term that they provided; if that failed to return satisfactory results, they often abandoned the concept idea in general even if it had merit since they perceived that the model probably wasn't sophisticated enough to understand that concept. Participants would benefit from scaffolding to help them to differentiate cases where the model understands the concept but expresses it with different terms versus cases where the model lacks an understanding of the concept at all.

% Tending to cater to the LLM rather than thinking more broadly/creatively
Second, we found that since participants were given an explanation of the underlying zero-shot modeling approaches used to surface concept scores, we found that participants overly tailored their concept terms based on what they thought that these zero-shot models would or would not be able to understand. This meant that some participants stuck with highly specific, concrete concept terms since they anticipated that models would perform better with these kinds of inputs. We observed that several participants who thought in this way eventually branched out and found that broader, more general terms worked well (sometimes, even better than highly specific concept terms). However, the downside still remains that since our concept models rely on pretrained models to surface scores, these models can be limiting factors that may cause users to constrain their thinking to the areas where the pretrained model already excels rather than thinking more broadly and creatively about what decisionmaking factors may be valuable.

% Bad modeling practices (ex: overfitting approaches, ignoring certain kinds of errors)
Finally, we noticed that because our approach emphasized a ``small data'' approach with a curated set of examples to help users stay focused, some participants lost sight of the overall goal to build a sketch of a more robust, general model. In those cases, participants sometimes fell into overfitting approaches by scrutinizing the cases where their sketch model made errors and authoring very specific concepts that were not relevant to the larger decision-making task, but that would allow the model to separate out those examples. Participants would benefit from additional tools that would help them to assess the generalizability of their sketch models while keeping them focused on the high-level sketching task. We still believe that a curated dataset is worth this tradeoff because it encourages ML practitioners to avoid their typical mode of detailed data analysis and to instead focus on broad-strokes concepts. P9 conveyed this well, noting that they ``had a lot of trouble finding the right concepts, but if you are working with a limited dataset, it may be more advantageous to spend time thinking about concepts rather than making your model more complex.''

% Limitations of our approach even if it were to work perfectly
% \begin{itemize}
%     \item Types of concepts that performed poorly; where the LLM or CLIP fails
%     \item Limited kinds of thinking (ex: framing the problem purely in terms of what a pretrained model can currently do)
%     \item Bad modeling practices (ex: overfitting approaches, ignoring certain kinds of errors)
% \end{itemize}
% Other maladaptive strategies that come up using this approach that would impair later model development
% “even if the tool worked perfectly, what are the downsides of this approach”




% To cover
% - Concept innovation vs concept execution vs concept abandonment (the _intent_ behind changes in concept models and sketches)




==> sections/old_versions/5_results_v2.tex <==
% V2 (post MSB comments + adding full results)

% \msb{cut:} %ML practitioners successfully engaged in model sketching, shifting their attention more towards higher-level, model design questions rather than technical model implementation details. This cognitive shift helped them to better explore the model design space and identify gaps in the modeling approach while requiring a fraction of the time that would ordinarily be required to author a functional model. 

Using our {ModelSketchBook} API, participants successfully authored an average of 12.2 (SD=4.7) concepts and 4.1 (SD=2.0) different sketch models that built on those concepts~(Figure~\ref{fig:concept_sketch_boxplot}) for the Hateful Memes task. 
%\msb{cut:} %While we allocated 30 minutes to this model authoring task, participants in practice worked on the task for a slightly shorter time period---28.2 minutes (SD=4.0) on average---due to time constraints. 

\begin{figure}[!tb]
  \includegraphics[width=0.6\textwidth]{figures/results/concept_sketch_num_plot.pdf}
  \caption{There was considerable variation in the number of concept and sketch models that participants authored, but all participants authored 5 or more concepts and 2 or more sketches within our approximately 30-minute task period.
  }
  \label{fig:concept_sketch_boxplot}
\end{figure}

\subsection{Changes in the cognitive process of model authoring}
% How we observed a shift from technical+implementation-oriented to conceptual+design/value-oriented thinking
Addressing RQ1, model sketching aided ML practitioners in shifting their thinking from technical, implementation-oriented factors toward higher-level, conceptual, design-oriented factors of model development. 

\subsubsection{Changes in planned modeling approach}
In their pre-task modeling plans, participants tended to focus on implementation details such as specific modeling methods or architectures (e.g., transformer models, convolutional neural networks, supervised models, linear classifiers), ML conventions like train-test splits and performance metrics, and data-oriented plans for feature extraction (summarized in Table~\ref{table:modeling_plan}). 
% general ML ``hygiene'' like ensuring that the examples span a range of scores and adjusting for skewed or imbalanced labels
For example, P13 described their approach as ``two types of models: [one] sentiment based and another that is a simple CNN, and then combine the two models with a simple fully connected layer,'' and P8 planned to ``create test/val/train sets with equal distributions of data'' and then ``train some model and inspect how it performs on a held out test set.''

However, in their post-task modeling plans, participants described that they would spend time on brainstorming and curating concepts relevant to the decision-making task and that they would iterate on their concepts by inspecting sketch model outputs. P15 described that ``Spending a few days tinkering with concepts could produce a fairly effective model that would be easier to debug.'' Participants also branched out to mention that they would like to consider different subclasses of harm and described how they might combine a concept-based approach with more traditional modeling approaches. For example, while P8 still preferred to use a more complex, non-linear model, they wished to use concepts from ModelSketchBook to augment their datapoints.
% \msb{this one seems more persuasive than the other results, which could just be because of the novelty}.
% \msb{I think one or two quotes of before examples and after examples could go a long way here}

\begin{table*}[!tb]
  \centering
  \footnotesize
    \begin{tabular}{p{0.08\textwidth} p{0.17\textwidth} p{0.65\textwidth}}
    \toprule
    \textbf{Study Phase} &
    \textbf{Modeling Plan Theme} &
    \textbf{Quotes}\\
    \midrule
    \textbf{Pre-task} & 
    {Specific model architectures or techniques} &
    {
        ``I would use a convolutional neural network model [...] probably use transformers in conjunction with CNNs to track long-term dependencies and help contextualize the text data.'' (P1),
        ``Two types of models: sentiment based and another that is a simple CNN, and then combine the two models with a simple fully connected layer'' (P13),
        ``I would use a binary classifier. Read the image and text, then build features using word2vec or some similar method. Depending on the size of the data would use either a tree based classifer or a deep learning model'' (P17)
    } \\[0.2cm]
    
    {} & 
    {Evaluating on training and validation sets} &
    {
        ``Ensure that the dataset is divided into train, test and validation slices. Experiment with several modeling techniques while evaluating on the validation set'' (P3),
        ``Create test/val/train sets with equal distributions of data. Train some model and inspect how it performs on a held out test set'' (P8)
    } \\[0.2cm]

    {} & 
    {Training on a range of toxicity levels} &
    {
        ``Train it on a lot of problematic and unproblematic (benign, slightly problematic, very problematic etc.) images'' (P1),
        ``Collect a bunch of posts of all levels of questionableness (a priori)'' (P5)
    } \\[0.2cm]

    {} & 
    {Standard performance metrics} &
    {
        ``Measure various metrics (accuracy, bias, variance etc.)'' (P1),
        ``Figure out the right set of metrics for evaluating any model that is trained. Choices could be accuracy, F1 scores and other metrics such as AUC or AuPR depending on relative label weights.'' (P3)
    } \\[0.2cm]

    {} & 
    {Building low-level features stemming from data} &
    {
        ``Can use features from the posts and user interactions. Can use general user information along with the post information'' (P4),
        ``Build features representing intuitions for things relevant to removal; like topic metadata, language choice, likes/dislikes/controversiality'' (P5),
        ``Think through what features to construct through data summary, correlation analysis, etc.'' (P7)
    } \\
    
    \midrule
    
    \textbf{Post-task} & 
    {Spending time brainstorming and curating concepts} &
    {
        ``[I would] think about all the concepts related to the underlying tasks'' (P4),
        ``I would focus more on concepts, deep-dive into data to see what it’s actually like, see how the other models are performing.'' (P13),
        ``I would likely lean into feature engineering carefully to have an interpretable model. Spending a few days tinkering with concepts could produce a fairly effective model that would be easier to debug.'' (P15)
    } \\[0.2cm]
    
    {} & 
    {Iterating on concepts by inspecting sketch model outputs} &
    {
        ``[I would] see mislabelled (and correctly labeled) examples from the aggregator and brainstorm more specific features that might account for that'' (P5),
        ``Think of concepts that relate to the task; try the concept; observe performance and then try other concepts; put them together for sketch; observe sketch performance and iterate on concepts'' (P16)
    } \\[0.2cm]

    {} & 
    {Authoring concepts informed by different categories of harm} &
    {
        ``A model to remove problematic social media posts would be a classification model placing different posts in different buckets (based on the degree of harm, violence etc. it may promote).'' (P1),
        ``I think filtering on hate (race/gender/religion) speech and political speech would be good first steps. There are some examples of graphic/violent posts that might not be captured by those categories, so I would add more filters for those specifically.'' (P2)
    } \\[0.2cm]

    {} & 
    {Combining a concept-based approach with traditional approaches} &
    {
        ``Also can use these labels as annotations to the datapoints for a more complex model (nonlinear). Seems like having the original data is still good so wouldn't rely on the CLIP/GPT annotations alone.'' (P8),
        ``I will probably still collect data manually and then instead of using a pretrained model and build the pipeline from scratch, I will use the ModelSketchBook API.'' (P11)
    } \\[0.2cm]

    {} & 
    {Engaging in ethical and user-facing considerations} &
    {
        ``It is very important to avoid suppressing speech especially speech/expression that is not violent or blatantly harmful.'' (P1),
        ``As a baseline, I would compare to the effectiveness of using some Transformer model to judge the end result directly, I wouldn't want to use it because its uninterpretable, hence dangerous.'' (P15)
    } \\
    \bottomrule
    \end{tabular}
    \caption{\msb{Cut some of the rows on the table, I suggest. It's eating up a bunch of words. Maybe move the pre-task part of the table into Appendix? Or, pick only 2-3 categories pre and post. If you keep pre and post, name them more descriptively for someone who's just skimming the paper, e.g., before model sketching, after model sketching} A summary of participants' modeling plans before and after the study. Participants chose to adopt model sketching in their future modeling plans and shifted from more technical, implementation-related plans to more procedural, value-oriented plans.
    }
    \label{table:modeling_plan}
\end{table*}

\subsubsection{Concept evolution}
\msb{cut this paragraph? not sure we need the definitional throat clearing, the next paragraph may be clear from context} One window into participants' mindset and approach is the way that their concepts evolve over time while using {ModelSketchBook}. We identify three main types of intent underlying concept authorship: 1)~\textit{concept innovation}, cases where participants come up with ideas for distinct concepts that they hadn't brainstormed before, 2)~\textit{concept execution}, cases where participants are continuing an existing concept idea, but are experimenting with different ways to actualize that concept via concept term inputs, and 3)~\textit{concept abandonment}, cases where participants decided not to continue with a concept and did not include it in their sketch models. 
% \msb{I don't buy these next two sentences: sometimes the point of sketches is to be able to confidently discard them as not promising directions}
% We hope that our model sketching approach will enable participants to engage in more concept innovation and less concept execution and concept abandonment. The latter two phenomena are still important steps that may need to happen for the user to effectively instantiate their vision of a concept with a zero-shot model, but this incremental, execution-oriented behavior should not dominate the workflow.

% \msb{the abstract number of concepts is useful, but it's hard for a reader to wrap their head around --- is this impressive? not impressive? I think a wide variety of examples of the kinds of concepts people created would help substantially}
% Concept innovation
Analyzing these phenomena among concept evolution histories, we observed that on average, participants engaged in 8.5 (SD=2.7) instances of concept innovation, which we define as the number of distinct concept ideas; on average 5.0 (SD=2.8) of those concept innovations were \textit{not} in the participant's original brainstormed list. Concept evolution often stemmed from participants discovering errors in their sketch models: P7 noted that a sketch model combining racism and sex concepts ran into false positives with humorous posts, which inspired an exploration of humor-related concepts. These progressions often built on each other: P4 initially started with a profanity concept that worked well, so they then brainstormed other dimensions of hate and decided to explore racism-related concepts; they then discovered that race and ethnicity-related hate in this dataset was often targeted at Muslims, so they got the idea to explore concepts related to Islamophobia.
% Concept execution
Participants on average displayed 3.2 (SD=2.3) instances of concept execution, which we define as the number of concepts authored that were continuations of the same concept idea (for example, switching from an image-based racism concept to a text-based racism concept when images don't appear to give a strong signal, or changing from a concept term of ``racism'' to one of ``race'' if the former did not work well). Participants more frequently changed modalities, but rarely modified concept terms.
% Concept abandonment
Then, participants underwent concept abandonment for an average of 4.2 (SD=2.6) concept ideas; we define this phenomenon as the number of concept ideas that were not ultimately used in the user's self-designated ``best'' sketch model. This abandonment is also a valuable part of sketching---to identify and discard paths that appear to be dead-ends. For example, P14 tried a ``harmful'' image-based concept, but found that this surfaced noisy results; they concluded that this was because the concept was too vague and didn't closely relate to the images in the dataset, and they decided to explore more grounded, specific concepts for images.
Thus, participants appear to engage in a variety of different generative, iterative, and reflective modes as they author concepts.
% Thus, it appears that while participants run into concept execution work and face concept abandonment, they tend to engage in a greater amount of concept innovation overall \msb{again, not sure concept abandonment is bad}.

\subsubsection{Participants' thought process}
Participants themselves perceived a change in their mode of thinking when they engaged in model sketching. 
% Removing tedious tasks
Many participants felt that the approach freed them from the tedious tasks that they typically had to work on. P10 described model sketching as ``a different way of thinking about [modeling]'' compared to their day-to-day modeling work, which was ``a lot more manual and technical and a lot more work and a lot more complex'' so they liked how model sketching ``just does it for you''. Similarly, P5 expressed that model sketching ``outsourced a lot of the most annoying parts of ML, like creating pipelines to generate features.''

% Bird's eye view
Some participants felt that this approach allowed them to take a more \textit{long-range, bird's-eye view} of the modeling process: P1 stated that ``this process helps put into perspective the long term goals and the structure of the ML lifecycle''. 
% Creative
Others described the model sketching process as refreshingly \textit{creative} and \textit{artistic}, especially in comparison to their typical model authoring experiences that had felt more formulaic or uninspired. As P12 put it, ``[model sketching] forced me to think creatively in a way I don't normally have to. Normally, my work is pretty boilerplate-y and repetitive. In this case, the model's performance was much more limited by my own creativity and ability, so it felt more like I had artistic direction in how the model did.'' 

% Interpretability; thinking from first principles
Participants also enjoyed the interpretability of model sketching, which afforded them a greater understanding of model behavior compared to past model authoring experiences. P14 shared that ``usually a lot of what I do is just a black box [...] and it's frustrating when it doesn't work,'' but that ``having this other option of trying to build from the bottom up is a pretty good alternative.'' 
% P10 similarly shared: ``I really like this interpretable approach where you can break down each concept and see which ones are doing well and where they fall short.'' 
This modeling approach also allowed participants to think about decision-making from first principles. P16 described that ``in terms of reasoning at a human level, I really like this idea of breaking it down into smaller concepts. It seems like an intuitive way you’d teach a kid... to me that just seems to be building a model that’s more explainable.''
% Enjoyment
% Lastly, participants expressed that they enjoyed this new mode of thinking. P1 shared that they ``really enjoyed the experience of thinking about models in this manner'' while P16 said that they ``liked the idea to approach things from how a human will think about things by defining these concepts.''

\subsection{Modeling outcomes}
% TODO: how this produces better or more societally-beneficial models
Regarding RQ2, we observed that the high-level cognitive shift in focus during model development brought about concrete benefits for the models themselves---from the breadth of concepts that sketch models explored to the gaps that participants uncovered in the modeling setup.

\subsubsection{Identifying modeling gaps}
\msb{cut:} %One of the aims of model sketching is that, in redirecting ML practitioners' attention to higher-level design decisions, it will allow them to identify flaws in not only their model, but in the problem formulation, dataset, and deployment context that surround it. 
% After the model authoring task, we asked participants to describe their learnings and takeaways from the task as well as any gaps they noticed in the modeling approach~(Table~\ref{table:modeling_gaps}) 
% \msb{In general, you shouldn't need to repeat the method in the results section---you should be able to just start with the results}. 
We summarize themes of participants' learnings and takeways in Table~\ref{table:modeling_gaps}, which demonstrates that the brief model sketching task helped participants to gain insights beyond just the model itself.
Participants uncovered major categories of harm that were not sufficiently represented in the provided sample of the dataset, and they noted that models built on this data may fail in practice due to distribution shift since the memes in the dataset appeared unrealistic compared to current online memes. Participants also identified limitations of the labeling approach such as class imbalance and inconsistent ratings. They gained intuitions about the task itself: participants discovered that for these memes, text was often more meaningful since the images were usually quite benign, and they started to form a sense of cases where multimodal approaches may reap more benefits. 

\begin{table*}[!tb]
  \centering
  \footnotesize
    \begin{tabular}{p{0.075\textwidth}p{0.35\textwidth} p{0.5\textwidth}}
    \toprule
    \textbf{Category} & \textbf{Learning or Takeaway} & \textbf{Quotes}\\
    \midrule
    {Task} &
    {Text overall seems more important than images for this task} &
    {
        ``The image could be detached from the text and the text seemed a bit more useful in this exercise'' (P7)
    }\\[0.2cm]

    {} &
    {Depending on the case, it may be important to combine the modalities or focus on text or image} &
    {
        ``How text and images interact together is a super important takeaway. You can’t just think about the images alone; you can’t just think about the text alone, it’s together the effect that they create'' (P16),
        ``One counter to [the greater importance of text] might be images of gore, where text is not necessarily needed for the post to be problematic.'' (P2)
    }\\[0.2cm]

    {} &
    {Memes are tricky to understand and label. 
    % Their meanings can be vague and dependent on inside knowledge.
    } &
    {
        ``Memes are tricky in that the images may be benign but the text may be harmful.'' (P1),
        ``Memes are very vague and tricky to label. The subtext is hard to capture with simple concepts.'' (P6)
    }\\
    \midrule
    {Dataset} &
    {There is a need for greater representativity of kinds of harm in the data} &
    {
        ``Need more data [to capture] problematic posts of all kinds (not just a racism or sexism) [...] Not enough data for homophobia, transphobia etc.'' (P1),
        ``[...] in this case nudity wasn't an issue, but might be for test time'' (P16)
    }\\[0.2cm]

    {} &
    {The dataset is may be too unrealistic and contrived to match the online distribution of posts
    % It needs to better match the distribution of what is actually posted online
    } &
    {
        ``The data seems to be far off from what is normally posted online, so the data definitely seems not good for general use.'' (P8)
    }\\[0.2cm]

    \midrule
    {Labels} &
    {Class imbalance has a large impact on modeling and makes it difficult to calibrate a model} &
    {
        ``I learned that class imbalance plays a large impact on modeling---it seemed for example that my own labeled dataset was relatively weighted towards not removing posts, so it paid dividends to [try] more specific targeted terms towards things that I found truly offensive like advocating for violence'' (P5)
    }\\[0.2cm]

    {} &
    {Their own labels appeared to be internally inconsistent} &
    {
        ``My labels are obviously not very internally consistent either and collecting from larger samples may help to even out the noise'' (P7)
    }\\[0.2cm]

    {} &
    {It would be valuable to increase the removal-score granularity beyond binarization} &
    {
        ``One area of improvement could be to increase the task fidelity to acually use the 5 labels instead of binarizing them.'' (P3)
    }\\
    \bottomrule
    \end{tabular}
    \caption{After performing a model sketching task, participants noted takeaways for their modeling approach and identified gaps in the dataset and labeling methodology. 
    }
    \label{table:modeling_gaps}
\end{table*}

% \item Source: Written response in NB, Interview
% \item Summary of gaps identified with counts across participants (ex: data fields, data representativity/balance, problem formulation, labeling method, how scores are translated to user interface)
% \item Deep-dive into particularly compelling examples of identified issues (potentially with quotes)

\subsubsection{Concept diversity}
Participants experimented with a broad variety of concept terms---ranging from concepts related to race and ethnicity to concepts related to politics, religion, and violence~(summarized in Table~\ref{table:concept_summary}). 
Notably, many participants authored concepts that they had not considered in their initial brainstorm; the process of authoring concepts and sketches helped them to discover important and relevant concepts to incorporate. 
\msl{Potentially add some examples of interesting concepts to call out.}
We are encouraged by these findings since a major goal of the model sketching approach is to have the freedom and flexibility to broadly explore the model design space and experiment with various concepts that may capture differing decision-making approaches.

\begin{table*}[!tb]
  \centering
  \footnotesize % \scriptsize
    \begin{tabular}{p{0.15\textwidth} p{0.25\textwidth} p{0.05\textwidth}}
    \toprule
    \textbf{Theme} & \textbf{Sample Participant Concepts} & \textbf{Count}\\
    \midrule
    \textbf{Ethnicity, Race} & 
    {racism, racist, race} &
    {34}\\[0.1cm]
    
    \textbf{Danger, Violence} & 
    {violence, terrorism, harm} &
    {28}\\[0.1cm]

    \textbf{Emotion} & 
    {rant, scary, anger} &
    {27}\\[0.1cm]
    
    \textbf{Discrimination} & 
    {hate, hate speech, discrimination} &
    {22}\\[0.1cm]
    
    \textbf{Politics} & 
    {political, politics, fake news} &
    {16}\\[0.1cm]
    
    \textbf{Offensive} & 
    {offensive, vulgar, obscene} &
    {15}\\[0.1cm]
    
    \textbf{Religion} & 
    {religion, religious, muslim} &
    {14}\\[0.1cm]
    
    \textbf{Misogyny} & 
    {sexist, sexism, gender} &
    {10}\\[0.1cm]
    
    \textbf{Sexual Content} & 
    {nudity, sexual, sex} &
    {9}\\[0.1cm]
    
    \textbf{Humor} & 
    {funny, humor, joke} &
    {8}\\[0.1cm]
    
    \textbf{Trolling} & 
    {trolling, meme, bad meme} &
    {7}\\[0.1cm]
    
    \textbf{Intersectionality} & 
    {color \& gender, islamophobia | sexism} &
    {7}\\
    \bottomrule
    \end{tabular}
    \caption{Summary of participant concepts. Here, we include only themes for which 3 or more participants authored concepts, and we display the most common concept terms for each theme as well as the total number of participant concepts that fell within the theme.
    }
    \label{table:concept_summary}
\end{table*}
% \item Source: Sketchbook from NB
% \item Characterize difference between initial brainstormed concepts vs. concepts in best sketches
% \item Summary of the trends in concepts used for the task across participants; the values taken into account.

\subsubsection{Performance metrics}
To gain a better understanding of the practical functionality of sketch models and the tradeoff that sketch models make compared to full-scale models, we also investigated their performance in terms of standard ML performance metrics~(Figure~\ref{fig:mean_metric_plot}). We compared all participants' self-determined ``best sketch model'' against two kinds of baselines: 1)~\textit{first sketch}, the very first sketch that a participant authored with the {ModelSketchBook} API and 2)~a set of \textit{raw-features} baselines that used only uninterpretable raw image and/or text features (512-dim CLIP embeddings) to train a model that would capture each participant's ratings.
% \msb{I would need more information to understand this. Is this a bag of words? Raw pixel values? BERT embedding? CLIP embedding? I don't think we could feasibly expect a raw regression to make a useful model with 128-dim embeddings and 20 examples}. 
The first-sketch baseline allows us to understand whether users can improve upon their sketches to achieve higher performance: better alignment between the sketch model and their own ground-truth ratings. The raw-features baseline provides a reference point on how well a more traditional, low-level feature-based modeling approach works for this task, albeit for a much smaller dataset.
% \msb{I think that comparison makes sense more if it's trained on the larger dataset, though?}

\begin{figure}[!tb]
  \includegraphics[width=0.9\textwidth]{figures/results/all_perf_metrics_test_v2.pdf}
  \caption{We observed higher classification performance---higher F1 score, precision, and recall---among participants' self-designated ``best'' sketches (the leftmost bar in each plot) compared to a baseline of both their first sketch (second bar from the left) and models that were trained on uninterpretable raw image and text features and participant labels (the three rightmost bars).
  }
  \label{fig:mean_metric_plot}
\end{figure}

We find that on the participant-labeled test sets, participants' ``best sketch'' appeared to outperform both baselines on classification metrics (F1, precision, recall), but the best sketch appeared to achieve comparable performance to the baselines on the regression version of the task, as measured by Mean Absolute Error (MAE).
These results suggest that participants are able to iteratively improve their sketch models to achieve higher alignment with their modeling goals, but that they may not achieve high enough performance to serve fine-grained regression tasks.
% and that sketch models are just as performant as (and perhaps in this case, even more performant than) standard raw feature-based modeling approaches, all while providing greater expressivity and maintaining human interpretability.

\subsubsection{Time required}
Finally, we note that participants were able to achieve these positive modeling outcomes in a fraction of the time that would be required to author a full model for this task. Participants' time estimates for executing on their pre-task modeling plans for the Hateful Memes task varied drastically from half a day to several weeks or months. However, even considering the most optimistic estimate of several hours (provided by 3 of 17 participants), our model sketching approach was able to deliver functional model prototypes in less than 30 minutes. 
% \msb{I try to avoid these kinds of judgments in Results, and defer them to Discussion. So Results is mostly ``what happened'', and Discussion is where we say ``unlocks a drastically different pace''}This shift in the timescale of ML model authoring from a drawn-out, weeks-long project to an exercise carried out at interactive speeds unlocks a drastically different pace of creative iteration and experimentation during model development.

\subsection{Participant experience outcomes}
\msb{I like it, but ultimately vote to cut this subsection}
Addressing RQ2 in terms of benefits to ML practitioners, we observed that participants found the model sketching approach to be comfortable and expressive. Participants shared a great deal of excitement about this method of model development, expressing that they ``enjoyed the experience of thinking about models in this manner'' (P1) and that the tool ``could be really helpful in the future for similar tasks'' (P11) or for ``showing that something was possible and expanding imaginations'' (P12).

\subsubsection{Comparison with existing authoring tools}
Comparing to their experiences with more common model authoring tools like Scikit-learn, PyTorch, and TensorFlow, participants felt similar levels of comfort with the {ModelSketchBook} API~(Figure~\ref{fig:survey_comfort_expressivity}) even though this 30-minute task was their first exposure to our tool, and all participants had significant experience with model authoring using these more traditional tools. At the same time, we saw that participants reported higher levels of expressivity when using the {ModelSketchBook} API than when using those same common model authoring tools. These results present promising support that our model sketching approach can be successfully adopted by ML practitioners as a lightweight, expressive entrypoint to model authoring.

\begin{figure}[!tb]
  \includegraphics[width=1.0\textwidth]{figures/survey/17 comfort_expressivity.pdf}
  \caption{Upon their first-time use of the {ModelSketchBook} API, participants indicated similar levels of comfort as they feel with traditional model authoring tools (left), but they indicated higher levels of expressivity using {ModelSketchBook} (right).
  }
  \label{fig:survey_comfort_expressivity}
\end{figure}

\subsubsection{Reflections on the model sketching experience}
\msb{This paragraph and the following image are also candidates for cutting---I know it came up in the intro, but I think it's not super convincing to read that people think they're happy with a new system. These self reports bias positive due to novelty and demand characteristics.}
In our survey, we also probed users' levels of satisfaction with their concepts and sketch models and asked them about the extent to which they felt their modeling approach changed or improved over time. We observed that participants were highly satisfied with both their concepts and sketch models. All but two participants rated their satisfaction with both models as ``somewhat satisfied,'' ``satisfied,'' or ``very satisfied.'' All but one participant responded that their modeling approach changed as they iterated on concepts and sketches, and the vast majority of participants (14 of 17) described a ``slight improvement,'' ``noticeable improvement,'' or ``significant improvement'' in their modeling approach.

% \begin{figure}[!tb]
%   \includegraphics[width=1.0\textwidth]{figures/survey/17 satisfaction_approach.pdf}
%   \caption{Participants were largely satisfied with both their concepts and sketch models (left), and most indicated both substantial changes and improvements in their modeling approach throughout the task (right). 
%   }
%   \label{fig:survey_satisfaction_approach}
% \end{figure}

In their interview feedback and survey free-responses, participants expressed enthusiasm about the model sketching approach~(Table~\ref{table:summary_participant_experience}). 
The most frequently-cited benefits of model sketching were that it was highly interpretable and explainable, easy to use (especially because it required no code), provided fast feedback loops, and prompted them to take on a different, high-level mode of thought. Meanwhile, the main limitations that participants noted were that the notebook environment often became disorganized, that our example-centric (rather than metric-centric) visualizations required more time to interpret, and that they would appreciate more assistance on brainstorming concepts. Multiple participants were excited about the opportunity to allow non-technical users and domain experts who lack ML knowledge to use ModelSketchBook and leverage their domain-specific expertise. They also suggested that we go beyond our notebook prototype to set up a dedicated user interface, and they suggested helper tools that would address potential issues with bias and overfitting in concepts.

\subsection{Benchmarking sketch model performance}
While the goal of model sketching is not to produce final, production-ready models, we do want to ensure that our sketch models provide a trustworthy signal on how a fully-implemented model might behave. We compared models authored using ModelSketchBook with state-of-the-art (SOTA) models for three different tasks: a comment toxicity task~\cite{kumar2021designing}, the Hateful Memes task (using the original annotator labels and the original hate-based task formulation)~\cite{kiela_hatefulMemes}, and an IMDB movie review sentiment analysis task. For each task, we used the same headline performance metric and the same train/test datasets as were used by the SOTA model. For the training set, we sampled only up to 500 examples to train our sketch models (in comparison, the SOTA models for these tasks were trained on 100k, 8.5k, and 25k examples, respectively). For evaluation, we calculated performance using a sample of 100 examples from the training set (preserving the same label distribution). 
On the comment toxicity task, a SOTA model reported 0.90 MAE~\cite{gordon_juryLearning}, and our sketch model achieved a slightly higher MAE of 0.93. 
On the IMDB review sentiment task, a SOTA model reported 0.93 accuracy~\cite{imdb_sota}, and our sketch model achieved a slightly lower accuracy of 0.91.
On the Hateful Memes task, a SOTA model reported 0.845 AUROC, and 0.714 AUROC was the SOTA result when the challenge was first released~\cite{kiela_hatefulMemes}; our sketch model achieved 0.584 AUROC. Thus, model sketching demonstrates strong results on two of the tasks, but displays weaker performance results for the third, significantly harder task.


\subsection{Failure modes}
While our model sketching approach achieved its aims of shifting model developers' cognitive frame and presented a number of benefits for the models they developed and their model authoring experience, we observed several failure modes of the approach. 
% Concept models failing, only can provide another concept term; users often gave up too soon
First, though participants had some promising concept ideas, they were not always able to actualize them with our zero-shot model-based approach. When a participant's concept failed to give them results that substantially overlapped with their own judgement, there was little recourse other than to attempt another related concept term and see if that achieves better alignment. However, participants often relied heavily on the results of the first concept term that they provided; if that failed to return satisfactory results, they often abandoned the concept idea in general even if it had merit since they perceived that the model probably wasn't sophisticated enough to understand that concept. Participants would benefit from scaffolding to help them to differentiate cases where the model understands the concept but expresses it with different terms versus cases where the model lacks an understanding of the concept at all.

% Tending to cater to the LLM rather than thinking more broadly/creatively
Second, we found that since participants were given an explanation of the underlying zero-shot modeling approaches used to surface concept scores, participants overly tailored their concept terms based on what they thought that these zero-shot models would be able to understand. This meant that some participants stuck with highly specific, concrete concept terms since they anticipated that models would perform better with these kinds of inputs. We observed that several participants who thought in this way eventually branched out and found that broader, more general terms worked well (sometimes, even better than highly specific concept terms). However, the downside still remains that since our concepts rely on pretrained models to surface scores, these models can be limiting factors that may cause users to constrain their thinking to the areas where the pretrained model already excels rather than thinking more broadly and creatively about what decisionmaking factors may be valuable.

% Bad modeling practices (ex: overfitting approaches, ignoring certain kinds of errors)
Finally, we noticed that because our approach intentionally emphasized a ``small data'' approach to help users stay focused, some participants lost sight of the overall goal to build a robust, general model. In those cases, participants sometimes fell into overfitting approaches by scrutinizing cases where their sketch model made errors and authoring very specific concepts that were not relevant to the larger decision-making task, but that would allow the model to separate out those examples. Participants would benefit from tools that would help them to assess the generalizability of their sketch models while keeping them focused on the high-level sketching task. We still believe that a curated dataset is worth this tradeoff because it encourages ML practitioners to avoid their typical mode of detailed data analysis and to instead focus on broad-strokes concepts. P9 conveyed this well, noting that ``if you are working with a limited dataset, it may be more advantageous to spend time thinking about concepts rather than making your model more complex.''

% Limitations of our approach even if it were to work perfectly
% \begin{itemize}
%     \item Types of concepts that performed poorly; where the LLM or CLIP fails
%     \item Limited kinds of thinking (ex: framing the problem purely in terms of what a pretrained model can currently do)
%     \item Bad modeling practices (ex: overfitting approaches, ignoring certain kinds of errors)
% \end{itemize}
% Other maladaptive strategies that come up using this approach that would impair later model development
% “even if the tool worked perfectly, what are the downsides of this approach”




% To cover
% - Concept innovation vs concept execution vs concept abandonment (the _intent_ behind changes in concept models and sketches)




==> sections/old_versions/5_results_v3.tex <==
% 9/15/22 V3

% \msb{cut:} %ML practitioners successfully engaged in model sketching, shifting their attention more towards higher-level, model design questions rather than technical model implementation details. This cognitive shift helped them to better explore the model design space and identify gaps in the modeling approach while requiring a fraction of the time that would ordinarily be required to author a functional model. 
Using our {ModelSketchBook} API, participants successfully authored an average of 12.2 (SD=4.7) concepts and 4.1 (SD=2.0) different sketch models that built on those concepts~(Figure~\ref{fig:concept_sketch_boxplot}) for the Hateful Memes task. Figure~\ref{fig:eval_sketches} displays sample concepts and sketch models authored by participants.
%\msb{cut:} %While we allocated 30 minutes to this model authoring task, participants in practice worked on the task for a slightly shorter time period---28.2 minutes (SD=4.0) on average---due to time constraints. 

\begin{figure}[!tb]
  \includegraphics[width=0.6\textwidth]{figures/results/concept_sketch_num_plot.pdf}
  \caption{There was considerable variation in the number of concept and sketch models that participants authored, but all participants authored 5 or more concepts and 2 or more sketches within our approximately 30-minute task period.
  }
  \label{fig:concept_sketch_boxplot}
\end{figure}

\begin{figure}[!tb]
  \includegraphics[width=0.85\textwidth]{figures/eval_sketches_v1.pdf}
  \caption{
    Examples of participant sketches. For illustrative purposes, we display the first sketch, best sketch, and other concepts for three study participants. Participants explored a broad range of concepts and expanded from their initial sketch models.
  }
  \label{fig:eval_sketches}
\end{figure}

\subsection{Changes in the cognitive process of model authoring}
% How we observed a shift from technical+implementation-oriented to conceptual+design/value-oriented thinking
Addressing RQ1, model sketching aided ML practitioners in shifting their thinking from technical, implementation-oriented factors toward higher-level, conceptual, design-oriented factors of model development. 

\subsubsection{Changes in planned modeling approach}
In their pre-task modeling plans, participants tended to focus on implementation details such as specific modeling methods or architectures (e.g., transformer models, convolutional neural networks, supervised models, linear classifiers), ML conventions like train-test splits and performance metrics, and data-oriented plans for feature extraction (summarized in Table~\ref{table:modeling_plan}). 
% general ML ``hygiene'' like ensuring that the examples span a range of scores and adjusting for skewed or imbalanced labels
For example, P13 described their approach as ``two types of models: [one] sentiment based and another that is a simple CNN, and then combine the two models with a simple fully connected layer,'' and P8 planned to ``create test/val/train sets with equal distributions of data'' and then ``train some model and inspect how it performs on a held out test set.''

However, after exposure to model sketching, participants described that they would spend time on brainstorming and curating concepts relevant to the decision-making task and that they would iterate on their concepts by inspecting sketch model outputs. P15 described that ``Spending a few days tinkering with concepts could produce a fairly effective model that would be easier to debug.'' Participants also branched out to mention that they would like to consider different subclasses of harm and described how they might combine a concept-based approach with more traditional modeling approaches. For example, while P8 still preferred to use a more complex, non-linear model, they wished to use concepts from ModelSketchBook to augment their datapoints.

\begin{table*}[!tb]
  \centering
  \footnotesize
    \begin{tabular}{p{0.08\textwidth} p{0.22\textwidth} p{0.6\textwidth}}
    \toprule
    \textbf{Study Phase} &
    \textbf{Modeling Plan Theme} &
    \textbf{Quotes}\\
    \midrule
    \textbf{Before model sketching} & 
    {Specific model architectures or techniques} &
    {
        ``I would use a convolutional neural network model [...] probably use transformers in conjunction with CNNs to track long-term dependencies and help contextualize the text data.'' (P1),
        ``Two types of models: sentiment based and another that is a simple CNN, and then combine the two models with a simple fully connected layer'' (P13),
        % ``I would use a binary classifier. Read the image and text, then build features using word2vec or some similar method. Depending on the size of the data would use either a tree based classifer or a deep learning model'' (P17)
    } \\[0.2cm]
    
    {} & 
    {Evaluating on training and validation sets} &
    {
        ``Ensure that the dataset is divided into train, test and validation slices. Experiment with several modeling techniques while evaluating on the validation set'' (P3),
        % ``Create test/val/train sets with equal distributions of data. Train some model and inspect how it performs on a held out test set'' (P8)
    } \\[0.2cm]

    % {} & 
    % {Training on a range of toxicity levels} &
    % {
    %     ``Train it on a lot of problematic and unproblematic (benign, slightly problematic, very problematic etc.) images'' (P1),
    %     ``Collect a bunch of posts of all levels of questionableness (a priori)'' (P5)
    % } \\[0.2cm]

    {} & 
    {Standard performance metrics} &
    {
        ``Measure various metrics (accuracy, bias, variance etc.)'' (P1),
        ``Figure out the right set of metrics for evaluating any model that is trained. Choices could be accuracy, F1 scores and other metrics such as AUC or AuPR depending on relative label weights.'' (P3)
    } \\[0.2cm]

    {} & 
    {Building low-level features stemming from data} &
    {
        ``Can use features from the posts and user interactions. Can use general user information along with the post information'' (P4),
        ``Build features representing intuitions for things relevant to removal; like topic metadata, language choice, likes/dislikes/controversiality'' (P5),
        % ``Think through what features to construct through data summary, correlation analysis, etc.'' (P7)
    } \\
    
    \midrule
    
    \textbf{After model sketching} & 
    {Spending time brainstorming and curating concepts} &
    {
        % ``[I would] think about all the concepts related to the underlying tasks'' (P4),
        % ``I would focus more on concepts, deep-dive into data to see what it’s actually like, see how the other models are performing.'' (P13),
        ``I would likely lean into feature engineering carefully to have an interpretable model. Spending a few days tinkering with concepts could produce a fairly effective model that would be easier to debug.'' (P15)
    } \\[0.2cm]
    
    {} & 
    {Iterating on concepts by inspecting sketch model outputs} &
    {
        ``[I would] see mislabelled (and correctly labeled) examples from the aggregator and brainstorm more specific features that might account for that'' (P5),
        % ``Think of concepts that relate to the task; try the concept; observe performance and then try other concepts; put them together for sketch; observe sketch performance and iterate on concepts'' (P16)
    } \\[0.2cm]

    {} & 
    {Authoring concepts informed by different categories of harm} &
    {
        % ``A model to remove problematic social media posts would be a classification model placing different posts in different buckets (based on the degree of harm, violence etc. it may promote).'' (P1),
        ``I think filtering on hate (race/gender/religion) speech and political speech would be good first steps. There are some examples of graphic/violent posts that might not be captured by those categories, so I would add more filters for those specifically.'' (P2)
    } \\[0.2cm]

    {} & 
    {Combining a concept-based approach with traditional approaches} &
    {
        ``Also can use these labels as annotations to the datapoints for a more complex model (nonlinear). Seems like having the original data is still good so wouldn't rely on the CLIP/GPT annotations alone.'' (P8),
        ``I will probably still collect data manually and then instead of using a pretrained model and build the pipeline from scratch, I will use the ModelSketchBook API.'' (P11)
    } \\%[0.2cm]

    % {} & 
    % {Engaging in ethical and user-facing considerations} &
    % {
    %     ``It is very important to avoid suppressing speech especially speech/expression that is not violent or blatantly harmful.'' (P1),
    %     ``As a baseline, I would compare to the effectiveness of using some Transformer model to judge the end result directly, I wouldn't want to use it because its uninterpretable, hence dangerous.'' (P15)
    % } \\
    \bottomrule
    \end{tabular}
    \caption{
    % \msb{Cut some of the rows on the table, I suggest. It's eating up a bunch of words. Maybe move the pre-task part of the table into Appendix? Or, pick only 2-3 categories pre and post. If you keep pre and post, name them more descriptively for someone who's just skimming the paper, e.g., before model sketching, after model sketching} 
    A summary of participants' modeling plans before and after the study. Participants chose to adopt model sketching in their future modeling plans and shifted from more technical, implementation-related plans to more procedural, value-oriented plans.
    }
    \label{table:modeling_plan}
\end{table*}

\subsubsection{Concept evolution}
% \msb{cut this paragraph? not sure we need the definitional throat clearing, the next paragraph may be clear from context} 
% One window into participants' mindset and approach is the way that their concepts evolve over time while using {ModelSketchBook}. We identify three main types of intent underlying concept authorship: 1)~\textit{concept innovation}, cases where participants come up with ideas for distinct concepts that they hadn't brainstormed before, 2)~\textit{concept execution}, cases where participants are continuing an existing concept idea, but are experimenting with different ways to actualize that concept via concept term inputs, and 3)~\textit{concept abandonment}, cases where participants decided not to continue with a concept and did not include it in their sketch models. 
% Concept innovation
One window into participants' mindset is the way that their concepts evolve over time while using ModelSketchBook.
We observed that on average, participants engaged in 8.5 (SD=2.7) instances of \textit{concept innovation}, which we define as the number of distinct concept ideas; on average 5.0 (SD=2.8) of those concept innovations were \textit{not} in the participant's original brainstormed list. Concept evolution often stemmed from participants discovering errors in their sketch models: P7 noted that a sketch model combining racism and sex concepts ran into false positives with humorous posts, which inspired an exploration of humor-related concepts. These progressions often built on each other: P4 initially started with a profanity concept that worked well, so they then brainstormed other dimensions of hate and decided to explore racism-related concepts; they then discovered that race and ethnicity-related hate in this dataset was often targeted at Muslims, so they got the idea to explore concepts related to Islamophobia.
% Concept execution
Participants on average displayed 3.2 (SD=2.3) instances of \textit{concept execution}, which we define as the number of concepts authored that were continuations of the same concept idea (for example, switching from an image-based racism concept to a text-based racism concept when images don't appear to give a strong signal, or changing from a concept term of ``racism'' to one of ``race'' if the former did not work well). Participants more frequently changed modalities, but rarely modified concept terms.
% Concept abandonment
Then, participants underwent \textit{concept abandonment} for an average of 4.2 (SD=2.6) concept ideas; we define this phenomenon as the number of concept ideas that were not ultimately used in the user's self-designated ``best'' sketch model. This abandonment is also a valuable part of sketching---to identify and discard paths that appear to be dead-ends. For example, P14 tried a ``harmful'' image-based concept, but found that this surfaced noisy results; they concluded that this was because the concept was too vague and didn't closely relate to the images in the dataset, and they decided to explore more grounded, specific concepts for images.
Thus, participants appear to engage in a variety of different generative, iterative, and reflective modes as they author concepts.


\subsubsection{Participants' thought process}
Participants perceived a change in their mode of thinking when they engaged in model sketching. 
% Removing tedious tasks
Many participants felt that the approach freed them from the tedious tasks that they typically had to work on. P10 described model sketching as ``a different way of thinking about [modeling]'' compared to their day-to-day modeling work, which was ``a lot more manual and technical and a lot more work and a lot more complex'' so they liked how model sketching ``just does it for you.'' Similarly, P5 expressed that model sketching ``outsourced a lot of the most annoying parts of ML, like creating pipelines to generate features.''

% Bird's eye view
Some participants felt that this approach allowed them to take a more \textit{long-range view} of the modeling process: P1 stated that ``this process helps put into perspective the long term goals and the structure of the ML lifecycle.'' 
% Creative
Others described the model sketching process as refreshingly \textit{creative} and \textit{artistic}, while their typical model authoring experiences had felt more formulaic. As P12 put it, ``[model sketching] forced me to think creatively in a way I don't normally have to. Normally, my work is pretty boilerplate-y and repetitive. In this case, the model's performance was much more limited by my own creativity and ability, so it felt more like I had artistic direction in how the model did.'' 

% Interpretability; thinking from first principles
Participants also enjoyed the interpretability of model sketching, which afforded them a greater understanding of model behavior compared to past model authoring experiences. P14 shared that ``usually a lot of what I do is just a black box [...] and it's frustrating when it doesn't work,'' but that ``having this other option of trying to build from the bottom up is a pretty good alternative.'' 
% P10 similarly shared: ``I really like this interpretable approach where you can break down each concept and see which ones are doing well and where they fall short.'' 
This modeling approach also allowed participants to think about decision-making from first principles. P16 described that ``in terms of reasoning at a human level, I really like this idea of breaking it down into smaller concepts. It seems like an intuitive way you’d teach a kid... to me that just seems to be building a model that’s more explainable.''
% Enjoyment
% Lastly, participants expressed that they enjoyed this new mode of thinking. P1 shared that they ``really enjoyed the experience of thinking about models in this manner'' while P16 said that they ``liked the idea to approach things from how a human will think about things by defining these concepts.''

\subsection{Modeling outcomes}
% TODO: how this produces better or more societally-beneficial models
Regarding RQ2, we observed that the high-level cognitive shift in focus during model development brought about concrete benefits for the models themselves---from the breadth of concepts that sketch models explored to the gaps that participants uncovered in the modeling setup.

\subsubsection{Identifying modeling gaps}
% \msb{cut:} %One of the aims of model sketching is that, in redirecting ML practitioners' attention to higher-level design decisions, it will allow them to identify flaws in not only their model, but in the problem formulation, dataset, and deployment context that surround it. 
%We summarize themes of participants' learnings and takeways in , which demonstrates that the brief 
Model sketching helped participants to gain insights beyond just the model itself (Table~\ref{table:modeling_gaps}).
Participants uncovered major categories of harm that were not sufficiently represented in the provided sample of the dataset, and they noted that models built on this data may fail in practice due to distribution shift since the memes in the dataset appeared unrealistic compared to current online memes. Participants also identified limitations of the labeling approach such as class imbalance and inconsistent ratings. They gained intuitions about the task itself: participants discovered that for these memes, text was often more meaningful since the images were usually quite benign, and they started to form a sense of cases where multimodal approaches may reap more benefits. 

\begin{table*}[!tb]
  \centering
  \footnotesize
    \begin{tabular}{p{0.075\textwidth}p{0.35\textwidth} p{0.5\textwidth}}
    \toprule
    \textbf{Category} & \textbf{Learning or Takeaway} & \textbf{Quotes}\\
    \midrule
    {Task} &
    {Text overall seems more important than images for this task} &
    {
        ``The image could be detached from the text and the text seemed a bit more useful in this exercise'' (P7)
    }\\[0.2cm]

    {} &
    {Depending on the case, it may be important to combine the modalities or focus on text or image} &
    {
        ``How text and images interact together is a super important takeaway. You can’t just think about the images alone; you can’t just think about the text alone, it’s together the effect that they create'' (P16),
        ``One counter to [the greater importance of text] might be images of gore, where text is not necessarily needed for the post to be problematic.'' (P2)
    }\\[0.2cm]

    {} &
    {Memes are tricky to understand and label. 
    % Their meanings can be vague and dependent on inside knowledge.
    } &
    {
        ``Memes are tricky in that the images may be benign but the text may be harmful.'' (P1),
        ``Memes are very vague and tricky to label. The subtext is hard to capture with simple concepts.'' (P6)
    }\\
    \midrule
    {Dataset} &
    {There is a need for greater representativity of kinds of harm in the data} &
    {
        ``Need more data [to capture] problematic posts of all kinds (not just a racism or sexism) [...] Not enough data for homophobia, transphobia etc.'' (P1),
        ``[...] in this case nudity wasn't an issue, but might be for test time'' (P16)
    }\\[0.2cm]

    {} &
    {The dataset is may be too unrealistic and contrived to match the online distribution of posts
    % It needs to better match the distribution of what is actually posted online
    } &
    {
        ``The data seems to be far off from what is normally posted online, so the data definitely seems not good for general use.'' (P8)
    }\\[0.2cm]

    \midrule
    {Labels} &
    {Class imbalance has a large impact on modeling and makes it difficult to calibrate a model} &
    {
        ``I learned that class imbalance plays a large impact on modeling---it seemed for example that my own labeled dataset was relatively weighted towards not removing posts, so it paid dividends to [try] more specific targeted terms towards things that I found truly offensive like advocating for violence'' (P5)
    }\\[0.2cm]

    {} &
    {Their own labels appeared to be internally inconsistent} &
    {
        ``My labels are obviously not very internally consistent either and collecting from larger samples may help to even out the noise'' (P7)
    }\\[0.2cm]

    {} &
    {It would be valuable to increase the removal-score granularity beyond binarization} &
    {
        ``One area of improvement could be to increase the task fidelity to actually use the 5 labels instead of binarizing them.'' (P3)
    }\\
    \bottomrule
    \end{tabular}
    \caption{After performing a model sketching task, participants noted takeaways for their modeling approach and identified gaps in the dataset and labeling methodology. 
    }
    \label{table:modeling_gaps}
\end{table*}


\subsubsection{Concept diversity}
Participants experimented with a broad variety of concept terms---ranging from concepts related to race and ethnicity to concepts related to politics, religion, and violence~(summarized in Table~\ref{table:concept_summary}). 
Notably, all participants authored concepts that they had not considered in their initial brainstorm; the process of authoring concepts and sketches helped them to discover important and relevant concepts to incorporate. 
% \msl{Potentially add some examples of interesting concepts to call out.}
%We are encouraged by these findings since a major goal of model sketching is to broadly explore the model design space and experiment with concepts that may capture differing decision-making approaches.

\begin{table*}[!tb]
  \centering
  \footnotesize % \scriptsize
    \begin{tabular}{p{0.15\textwidth} p{0.25\textwidth} p{0.05\textwidth}}
    \toprule
    \textbf{Theme} & \textbf{Sample Participant Concepts} & \textbf{Count}\\
    \midrule
    \textbf{Ethnicity, Race} & 
    {racism, racist, race} &
    {34}\\[0.1cm]
    
    \textbf{Danger, Violence} & 
    {violence, terrorism, harm} &
    {28}\\[0.1cm]

    \textbf{Emotion} & 
    {rant, scary, anger} &
    {27}\\[0.1cm]
    
    \textbf{Discrimination} & 
    {hate, hate speech, discrimination} &
    {22}\\[0.1cm]
    
    \textbf{Politics} & 
    {political, politics, fake news} &
    {16}\\[0.1cm]
    
    \textbf{Offensive} & 
    {offensive, vulgar, obscene} &
    {15}\\[0.1cm]
    
    \textbf{Religion} & 
    {religion, religious, muslim} &
    {14}\\[0.1cm]
    
    \textbf{Gender} & 
    {sexist, sexism, gender} &
    {10}\\[0.1cm]
    
    \textbf{Sexual Content} & 
    {nudity, sexual, sex} &
    {9}\\[0.1cm]
    
    \textbf{Humor} & 
    {funny, humor, joke} &
    {8}\\[0.1cm]
    
    \textbf{Trolling} & 
    {trolling, meme, bad meme} &
    {7}\\[0.1cm]
    
    \textbf{Intersectionality} & 
    {color \& gender, islamophobia | sexism} &
    {7}\\
    \bottomrule
    \end{tabular}
    \caption{Summary of participant concepts. Here, we include only themes for which 3 or more participants authored concepts, and we display the most common concept terms for each theme as well as the total number of participant concepts that fell within the theme.
    }
    \label{table:concept_summary}
\end{table*}

\subsubsection{Time required}
Finally, we note that participants were able to achieve these positive modeling outcomes in a fraction of the time that would be required to author a full model for this task. Participants' time estimates for executing on their pre-task modeling plans for the Hateful Memes task varied drastically from half a day to several weeks or months. However, even considering the most optimistic estimate of several hours (provided by 3 of 17 participants), our model sketching approach was able to deliver functional model prototypes in less than 30 minutes. 

\subsection{Participant experience outcomes}
% \msb{I like it, but ultimately vote to cut this subsection}
Addressing RQ2 in terms of benefits to ML practitioners, we observed that participants found the model sketching approach to be comfortable and expressive. Participants shared a great deal of excitement about this method of model development, expressing that they ``enjoyed the experience of thinking about models in this manner'' (P1) and that the tool ``could be really helpful in the future for similar tasks'' (P11) or for ``showing that something was possible and expanding imaginations'' (P12). We summarize these results in Appendix Section~\ref{section:participant_experience}.

% \subsubsection{Comparison with existing authoring tools}
% Comparing to their experiences with more common model authoring tools like Scikit-learn, PyTorch, and TensorFlow, participants felt similar levels of comfort with the {ModelSketchBook} API~(Figure~\ref{fig:survey_comfort_expressivity}) even though this 30-minute task was their first exposure to our tool, and all participants had significant experience with model authoring using these more traditional tools. At the same time, we saw that participants reported higher levels of expressivity when using the {ModelSketchBook} API than when using those same common model authoring tools. These results present promising support that our model sketching approach can be successfully adopted by ML practitioners as a lightweight, expressive entrypoint to model authoring.

% \begin{figure}[!tb]
%   \includegraphics[width=1.0\textwidth]{figures/survey/17 comfort_expressivity.pdf}
%   \caption{Upon their first-time use of the {ModelSketchBook} API, participants indicated similar levels of comfort as they feel with traditional model authoring tools (left), but they indicated higher levels of expressivity using {ModelSketchBook} (right).
%   }
%   \label{fig:survey_comfort_expressivity}
% \end{figure}

% \subsubsection{Reflections on the model sketching experience}
% % \msb{This paragraph and the following image are also candidates for cutting---I know it came up in the intro, but I think it's not super convincing to read that people think they're happy with a new system. These self reports bias positive due to novelty and demand characteristics.}
% In our survey, we also probed users' levels of satisfaction with their concepts and sketch models and asked them about the extent to which they felt their modeling approach changed or improved over time. We observed that participants were highly satisfied with both their concepts and sketch models. All but two participants rated their satisfaction with both models as ``somewhat satisfied,'' ``satisfied,'' or ``very satisfied.'' All but one participant responded that their modeling approach changed as they iterated on concepts and sketches, and the vast majority of participants (14 of 17) described a ``slight improvement,'' ``noticeable improvement,'' or ``significant improvement'' in their modeling approach.

% % \begin{figure}[!tb]
% %   \includegraphics[width=1.0\textwidth]{figures/survey/17 satisfaction_approach.pdf}
% %   \caption{Participants were largely satisfied with both their concepts and sketch models (left), and most indicated both substantial changes and improvements in their modeling approach throughout the task (right). 
% %   }
% %   \label{fig:survey_satisfaction_approach}
% % \end{figure}

% In their interview feedback and survey free-responses, participants expressed enthusiasm about the model sketching approach~(Appendix Table~\ref{table:summary_participant_experience}). 
% The most frequently-cited benefits of model sketching were that it was highly interpretable and explainable, easy to use (especially because it required no code), provided fast feedback loops, and prompted them to take on a different, high-level mode of thought. Meanwhile, the main limitations that participants noted were that the notebook environment often became disorganized, that our example-centric (rather than metric-centric) visualizations required more time to interpret, and that they would appreciate more assistance on brainstorming concepts. Multiple participants were excited about the opportunity to allow non-technical users and domain experts who lack ML knowledge to use ModelSketchBook and leverage their domain-specific expertise. They also suggested that we go beyond our notebook prototype to set up a dedicated user interface, and they suggested helper tools that would address potential issues with bias and overfitting in concepts.

\subsection{Benchmarking sketch model performance}
While the goal of model sketching is not to produce full-scale models, we seek to understand whether sketch models achieve reasonable functionality relative to full-scale models.

\subsubsection{Study participants' sketch models}
First, we investigated the sketch models authored by our study participants. 
We compared all participants' self-determined ``best sketch model'' against two kinds of baselines: 1)~\textit{first sketch}, the very first sketch that a participant authored with the {ModelSketchBook} API and 2)~a set of \textit{raw-features} baselines that used only uninterpretable raw image and/or text features to train a model that would capture each participant's ratings\footnote{For the raw-features baseline, we used 512-dimensional CLIP embeddings and randomly sampled 4 dimensions to use as features to approximately mirror the average number of concepts per sketch among participants (4.0, SD=1.96).}.
% The first-sketch baseline allows us to understand whether users can improve upon their sketches to achieve higher performance: better alignment between the sketch model and their own ground-truth ratings. The raw-features baseline provides a reference point on how well a low-level feature-based modeling approach works for this task, albeit for a much smaller dataset.
We find that on the participant-labeled test sets with 20 examples, participants' best sketches outperformed both baselines on classification metrics (F1, precision, recall), but the best sketches achieved comparable performance to the baselines on the regression version of the task, as measured by Mean Absolute Error (MAE)~(Figure~\ref{fig:mean_metric_plot}). 
These results suggest that participants are able to iteratively improve their sketch models to achieve higher alignment with their modeling goals and that sketch models may work better for classification tasks than for fine-grained regression tasks.
We note that for this task, the classification metrics were relatively low overall due to class imbalance. Many participants had substantial skew in labels toward the negative class (``non-hateful'') and thus ended up producing models that always predicted the negative class (behavior which results in scores of 0.0 for recall, precision, and F1).

\begin{figure}[!tb]
  \includegraphics[width=0.7\textwidth]{figures/results/all_perf_metrics_test_v2.pdf}
  \caption{We observed higher classification performance---higher F1 score, precision, and recall---among participants' self-designated ``best'' sketches (the leftmost bar in each plot) compared to a baseline of both their first sketch (second bar from the left) and models that were trained on uninterpretable raw image and text features and participant labels (the three rightmost bars).
  }
  \label{fig:mean_metric_plot}
\end{figure}

\subsubsection{Investigating the impact of task difficulty on sketch model performance}
Thus, we sought to further investigate the performance of sketch models in cases without such strong class imbalance and with many more than 20 training examples. We prepared three additional tasks: an IMDB movie review sentiment analysis task (easiest: per-example ratings and balanced classes)~\cite{imdb_sota}; a comment toxicity task (harder: per-annotator ratings and class skew)~\cite{kumar2021designing}; and the original Hateful Memes task (hardest: balanced classes, but nuanced and multimodal task)~\cite{kiela_hatefulMemes}. For each of these, we compared sketch models against published state-of-the-art (SOTA) models, using the same headline performance metric and train/test datasets as were used by the SOTA model. 
We sampled up to 500 examples to train our sketch models (in comparison, the SOTA models for these tasks were trained on 25k, 100k, and 8.5k examples, respectively). For evaluation, we calculated performance using a sample of 100 examples from the training set (preserving the same label distribution). 
For the IMDB task, the SOTA model reported 0.93 accuracy and our sketch model achieved 0.91 accuracy, only slightly lower.
On the comment toxicity task (which used a 0-4 score range), the SOTA model reported 0.90 MAE while our sketch model achieved an MAE of 1.39.
On the Hateful Memes task, the SOTA model reported 0.845 AUROC, and 0.714 AUROC was the SOTA result when the challenge was first released; our sketch model achieved 0.584 AUROC.
Thus, model sketching demonstrates strong or reasonable performance on the easy and medium difficulty tasks, but displays weaker performance results for the third, significantly harder task.


\subsection{Failure modes}
While our model sketching approach achieved its aims of shifting model developers' cognitive frame and presented a number of benefits for the models they developed and their model authoring experience, we observed several failure modes.
% Concept models failing, only can provide another concept term; users often gave up too soon
First, though participants had some promising concept ideas, they were not always able to actualize them with our zero-shot model-based approach. 
% When a participant's concept failed to give them results that substantially overlapped with their own judgement, there was little recourse other than to attempt another related concept term and see if that achieves better alignment. 
Participants often relied heavily on the results of the first concept term that they attempted. If that failed to return satisfactory results, they often abandoned the concept idea since they assumed that the model probably was not sophisticated enough to understand that concept. Participants would benefit from scaffolding to understand whether the model lacks an understanding of a given concept or just requires different terminology.
% differentiate cases where the model understands the concept but expresses it with different terms versus cases where the model lacks an understanding of the concept at all.

% Tending to cater to the LLM rather than thinking more broadly/creatively
% Second, we found that since participants were given an explanation of the underlying zero-shot modeling approaches used to surface concept scores, participants overly tailored their concept terms based on what they thought that these zero-shot models would be able to understand. 
Second, we found that some participants heavily tailored their concept terms based on what they thought zero-shot models would be able to understand, especially using concrete, specific concept terms.
% since they anticipated that models would perform better with these kinds of inputs. 
We observed that several of these participants eventually branched out and found that broader terms could work well. However, the downside still remains that since our concepts rely on pretrained models, these models can be limiting factors. Users might constrain their thinking to areas where the pretrained model already excels rather than thinking more creatively about what decisionmaking factors may be valuable.

% Bad modeling practices (ex: overfitting approaches, ignoring certain kinds of errors)
Finally, we noticed that because our approach emphasized a ``small data'' approach to help users stay focused, some participants lost sight of the overall goal to build a robust, general model. Participants sometimes fell into overfitting approaches by scrutinizing cases where their sketch model made errors and patching errors with very specific concepts that were not relevant to the larger decision-making task. Participants would benefit from tools that would help them to assess the generalizability of their sketch models. We believe that a curated dataset is worth this tradeoff because it encourages ML practitioners to avoid detailed data analysis and instead focus on broad-strokes concepts. 
% P9 conveyed this well, noting that ``if you are working with a limited dataset, it may be more advantageous to spend time thinking about concepts rather than making your model more complex.''

% Limitations of our approach even if it were to work perfectly
% \begin{itemize}
%     \item Types of concepts that performed poorly; where the LLM or CLIP fails
%     \item Limited kinds of thinking (ex: framing the problem purely in terms of what a pretrained model can currently do)
%     \item Bad modeling practices (ex: overfitting approaches, ignoring certain kinds of errors)
% \end{itemize}
% Other maladaptive strategies that come up using this approach that would impair later model development
% “even if the tool worked perfectly, what are the downsides of this approach”




% To cover
% - Concept innovation vs concept execution vs concept abandonment (the _intent_ behind changes in concept models and sketches)




==> sections/old_versions/5_results_v4.tex <==
% 11/29/22 V4

% \msb{cut:} %ML practitioners successfully engaged in model sketching, shifting their attention more towards higher-level, model design questions rather than technical model implementation details. This cognitive shift helped them to better explore the model design space and identify gaps in the modeling approach while requiring a fraction of the time that would ordinarily be required to author a functional model. 
Using our {ModelSketchBook} API, participants successfully authored an average of 12.2 (SD=4.7) concepts and 4.1 (SD=2.0) different sketch models that built on those concepts~(Figure~\ref{fig:concept_sketch_boxplot}) for the Hateful Memes task. Figure~\ref{fig:eval_sketches} displays sample concepts and sketch models authored by participants.
%\msb{cut:} %While we allocated 30 minutes to this model authoring task, participants in practice worked on the task for a slightly shorter time period---28.2 minutes (SD=4.0) on average---due to time constraints. 

\rev{
% Label variance
% \msl{Decide where to place this blurb:} 
In our task design, we aimed for our modeling task to involve a high amount of subjectivity to provide a sufficiently broad model design space among participants. We indeed found this to be the case: there were substantial differences in how our participants chose to label the memes dataset provided for the study session. Across participants and data examples, the mean standard deviation in labels (on a 0-1 scale) was $0.23$. For the binarized versions of those same scores, this meant that $75\%$ of the examples had at least one participant who disagreed with the majority label, and $37.5\%$ of the examples had a quarter or more of the participants who disagreed with the majority label.
\msl{Add bridge to next section.}
}

\begin{figure}[!tb]
  \includegraphics[width=0.6\textwidth]{figures/results/concept_sketch_num_plot.pdf}
  \caption{There was considerable variation in the number of concept and sketch models that participants authored, but all participants authored 5 or more concepts and 2 or more sketches within our approximately 30-minute task period.
  }
  \label{fig:concept_sketch_boxplot}
\end{figure}

\begin{figure}[!tb]
  \includegraphics[width=0.85\textwidth]{figures/eval_sketches_v1.pdf}
  \caption{
    Examples of participant sketches. For illustrative purposes, we display the first sketch, best sketch, and other concepts for three study participants. Participants explored a broad range of concepts and expanded from their initial sketch models.
  }
  \label{fig:eval_sketches}
\end{figure}

\subsection{Changes in the cognitive process of model authoring}
% How we observed a shift from technical+implementation-oriented to conceptual+design/value-oriented thinking
Addressing RQ1, model sketching aided ML practitioners in shifting their thinking from technical, implementation-oriented factors toward higher-level, conceptual, design-oriented factors of model development. 

\subsubsection{Changes in planned modeling approach}
In their pre-task modeling plans, participants tended to focus on implementation details such as specific modeling methods or architectures (e.g., transformer models, convolutional neural networks, supervised models, linear classifiers), ML conventions like train-test splits and performance metrics, and data-oriented plans for feature extraction (summarized in Table~\ref{table:modeling_plan}). 
% general ML ``hygiene'' like ensuring that the examples span a range of scores and adjusting for skewed or imbalanced labels
For example, P13 described their approach as ``two types of models: [one] sentiment based and another that is a simple CNN, and then combine the two models with a simple fully connected layer,'' and P8 planned to ``create test/val/train sets with equal distributions of data'' and then ``train some model and inspect how it performs on a held out test set.''

However, after exposure to model sketching, participants described that they would spend time on brainstorming and curating concepts relevant to the decision-making task and that they would iterate on their concepts by inspecting sketch model outputs. P15 described that ``Spending a few days tinkering with concepts could produce a fairly effective model that would be easier to debug.'' Participants also branched out to mention that they would like to consider different subclasses of harm and described how they might combine a concept-based approach with more traditional modeling approaches. For example, while P8 still preferred to use a more complex, non-linear model, they wished to use concepts from ModelSketchBook to augment their datapoints.

\begin{table*}[!tb]
  \centering
  \footnotesize
    \begin{tabular}{p{0.08\textwidth} p{0.22\textwidth} p{0.6\textwidth}}
    \toprule
    \textbf{Study Phase} &
    \textbf{Modeling Plan Theme} &
    \textbf{Quotes}\\
    \midrule
    \textbf{Before model sketching} & 
    {Specific model architectures or techniques} &
    {
        ``I would use a convolutional neural network model [...] probably use transformers in conjunction with CNNs to track long-term dependencies and help contextualize the text data.'' (P1),
        ``Two types of models: sentiment based and another that is a simple CNN, and then combine the two models with a simple fully connected layer'' (P13),
        % ``I would use a binary classifier. Read the image and text, then build features using word2vec or some similar method. Depending on the size of the data would use either a tree based classifer or a deep learning model'' (P17)
    } \\[0.2cm]
    
    {} & 
    {Evaluating on training and validation sets} &
    {
        ``Ensure that the dataset is divided into train, test and validation slices. Experiment with several modeling techniques while evaluating on the validation set'' (P3),
        % ``Create test/val/train sets with equal distributions of data. Train some model and inspect how it performs on a held out test set'' (P8)
    } \\[0.2cm]

    % {} & 
    % {Training on a range of toxicity levels} &
    % {
    %     ``Train it on a lot of problematic and unproblematic (benign, slightly problematic, very problematic etc.) images'' (P1),
    %     ``Collect a bunch of posts of all levels of questionableness (a priori)'' (P5)
    % } \\[0.2cm]

    {} & 
    {Standard performance metrics} &
    {
        ``Measure various metrics (accuracy, bias, variance etc.)'' (P1),
        ``Figure out the right set of metrics for evaluating any model that is trained. Choices could be accuracy, F1 scores and other metrics such as AUC or AuPR depending on relative label weights.'' (P3)
    } \\[0.2cm]

    {} & 
    {Building low-level features stemming from data} &
    {
        ``Can use features from the posts and user interactions. Can use general user information along with the post information'' (P4),
        ``Build features representing intuitions for things relevant to removal; like topic metadata, language choice, likes/dislikes/controversiality'' (P5),
        % ``Think through what features to construct through data summary, correlation analysis, etc.'' (P7)
    } \\
    
    \midrule
    
    \textbf{After model sketching} & 
    {Spending time brainstorming and curating concepts} &
    {
        % ``[I would] think about all the concepts related to the underlying tasks'' (P4),
        % ``I would focus more on concepts, deep-dive into data to see what it’s actually like, see how the other models are performing.'' (P13),
        ``I would likely lean into feature engineering carefully to have an interpretable model. Spending a few days tinkering with concepts could produce a fairly effective model that would be easier to debug.'' (P15)
    } \\[0.2cm]
    
    {} & 
    {Iterating on concepts by inspecting sketch model outputs} &
    {
        ``[I would] see mislabelled (and correctly labeled) examples from the aggregator and brainstorm more specific features that might account for that'' (P5),
        % ``Think of concepts that relate to the task; try the concept; observe performance and then try other concepts; put them together for sketch; observe sketch performance and iterate on concepts'' (P16)
    } \\[0.2cm]

    {} & 
    {Authoring concepts informed by different categories of harm} &
    {
        % ``A model to remove problematic social media posts would be a classification model placing different posts in different buckets (based on the degree of harm, violence etc. it may promote).'' (P1),
        ``I think filtering on hate (race/gender/religion) speech and political speech would be good first steps. There are some examples of graphic/violent posts that might not be captured by those categories, so I would add more filters for those specifically.'' (P2)
    } \\[0.2cm]

    {} & 
    {Combining a concept-based approach with traditional approaches} &
    {
        ``Also can use these labels as annotations to the datapoints for a more complex model (nonlinear). Seems like having the original data is still good so wouldn't rely on the CLIP/GPT annotations alone.'' (P8),
        ``I will probably still collect data manually and then instead of using a pretrained model and build the pipeline from scratch, I will use the ModelSketchBook API.'' (P11)
    } \\%[0.2cm]

    % {} & 
    % {Engaging in ethical and user-facing considerations} &
    % {
    %     ``It is very important to avoid suppressing speech especially speech/expression that is not violent or blatantly harmful.'' (P1),
    %     ``As a baseline, I would compare to the effectiveness of using some Transformer model to judge the end result directly, I wouldn't want to use it because its uninterpretable, hence dangerous.'' (P15)
    % } \\
    \bottomrule
    \end{tabular}
    \caption{
    % \msb{Cut some of the rows on the table, I suggest. It's eating up a bunch of words. Maybe move the pre-task part of the table into Appendix? Or, pick only 2-3 categories pre and post. If you keep pre and post, name them more descriptively for someone who's just skimming the paper, e.g., before model sketching, after model sketching} 
    A summary of participants' modeling plans before and after the study. Participants chose to adopt model sketching in their future modeling plans and shifted from more technical, implementation-related plans to more procedural, value-oriented plans.
    }
    \label{table:modeling_plan}
\end{table*}

\subsubsection{Concept evolution}
% \msb{cut this paragraph? not sure we need the definitional throat clearing, the next paragraph may be clear from context} 
% One window into participants' mindset and approach is the way that their concepts evolve over time while using {ModelSketchBook}. We identify three main types of intent underlying concept authorship: 1)~\textit{concept innovation}, cases where participants come up with ideas for distinct concepts that they hadn't brainstormed before, 2)~\textit{concept execution}, cases where participants are continuing an existing concept idea, but are experimenting with different ways to actualize that concept via concept term inputs, and 3)~\textit{concept abandonment}, cases where participants decided not to continue with a concept and did not include it in their sketch models. 
% Concept innovation
One window into participants' mindset is the way that their concepts evolve over time while using ModelSketchBook.
We observed that on average, participants engaged in 8.5 (SD=2.7) instances of \textit{concept innovation}, which we define as the number of distinct concept ideas; on average 5.0 (SD=2.8) of those concept innovations were \textit{not} in the participant's original brainstormed list. Concept evolution often stemmed from participants discovering errors in their sketch models: P7 noted that a sketch model combining racism and sex concepts ran into false positives with humorous posts, which inspired an exploration of humor-related concepts. These progressions often built on each other: P4 initially started with a profanity concept that worked well, so they then brainstormed other dimensions of hate and decided to explore racism-related concepts; they then discovered that race and ethnicity-related hate in this dataset was often targeted at Muslims, so they got the idea to explore concepts related to Islamophobia.
% Concept execution
Participants on average displayed 3.2 (SD=2.3) instances of \textit{concept execution}, which we define as the number of concepts authored that were continuations of the same concept idea (for example, switching from an image-based racism concept to a text-based racism concept when images don't appear to give a strong signal, or changing from a concept term of ``racism'' to one of ``race'' if the former did not work well). Participants more frequently changed modalities, but rarely modified concept terms.
% Concept abandonment
Then, participants underwent \textit{concept abandonment} for an average of 4.2 (SD=2.6) concept ideas; we define this phenomenon as the number of concept ideas that were not ultimately used in the user's self-designated ``best'' sketch model. This abandonment is also a valuable part of sketching---to identify and discard paths that appear to be dead-ends. For example, P14 tried a ``harmful'' image-based concept, but found that this surfaced noisy results; they concluded that this was because the concept was too vague and didn't closely relate to the images in the dataset, and they decided to explore more grounded, specific concepts for images.
Thus, participants appear to engage in a variety of different generative, iterative, and reflective modes as they author concepts.


\subsubsection{Participants' thought process}
Participants perceived a change in their mode of thinking when they engaged in model sketching. 
% Removing tedious tasks
Many participants felt that the approach freed them from the tedious tasks that they typically had to work on. P10 described model sketching as ``a different way of thinking about [modeling]'' compared to their day-to-day modeling work, which was ``a lot more manual and technical and a lot more work and a lot more complex'' so they liked how model sketching ``just does it for you.'' Similarly, P5 expressed that model sketching ``outsourced a lot of the most annoying parts of ML, like creating pipelines to generate features.''

% Bird's eye view
Some participants felt that this approach allowed them to take a more \textit{long-range view} of the modeling process: P1 stated that ``this process helps put into perspective the long term goals and the structure of the ML lifecycle.'' 
% Creative
Others described the model sketching process as refreshingly \textit{creative} and \textit{artistic}, while their typical model authoring experiences had felt more formulaic. As P12 put it, ``[model sketching] forced me to think creatively in a way I don't normally have to. Normally, my work is pretty boilerplate-y and repetitive. In this case, the model's performance was much more limited by my own creativity and ability, so it felt more like I had artistic direction in how the model did.'' 

% Interpretability; thinking from first principles
Participants also enjoyed the interpretability of model sketching, which afforded them a greater understanding of model behavior compared to past model authoring experiences. P14 shared that ``usually a lot of what I do is just a black box [...] and it's frustrating when it doesn't work,'' but that ``having this other option of trying to build from the bottom up is a pretty good alternative.'' 
% P10 similarly shared: ``I really like this interpretable approach where you can break down each concept and see which ones are doing well and where they fall short.'' 
This modeling approach also allowed participants to think about decision-making from first principles. P16 described that ``in terms of reasoning at a human level, I really like this idea of breaking it down into smaller concepts. It seems like an intuitive way you’d teach a kid... to me that just seems to be building a model that’s more explainable.''
% Enjoyment
% Lastly, participants expressed that they enjoyed this new mode of thinking. P1 shared that they ``really enjoyed the experience of thinking about models in this manner'' while P16 said that they ``liked the idea to approach things from how a human will think about things by defining these concepts.''

\subsection{Modeling outcomes}
% TODO: how this produces better or more societally-beneficial models
Regarding RQ2, we observed that the high-level cognitive shift in focus during model development brought about concrete benefits for the models themselves---from the breadth of concepts that sketch models explored to the gaps that participants uncovered in the modeling setup.

\subsubsection{Identifying modeling gaps}
\label{section:modeling_gaps}
% \msb{cut:} %One of the aims of model sketching is that, in redirecting ML practitioners' attention to higher-level design decisions, it will allow them to identify flaws in not only their model, but in the problem formulation, dataset, and deployment context that surround it. 
%We summarize themes of participants' learnings and takeways in , which demonstrates that the brief 
Model sketching helped participants to gain insights beyond just the model itself (Table~\ref{table:modeling_gaps}).
Participants uncovered major categories of harm that were not sufficiently represented in the provided sample of the dataset, and they noted that models built on this data may fail in practice due to distribution shift since the memes in the dataset appeared unrealistic compared to current online memes. Participants also identified limitations of the labeling approach such as class imbalance and inconsistent ratings. They gained intuitions about the task itself: participants discovered that for these memes, text was often more meaningful since the images were usually quite benign, and they started to form a sense of cases where multimodal approaches may reap more benefits. 

\begin{table*}[!tb]
  \centering
  \footnotesize
    \begin{tabular}{p{0.075\textwidth}p{0.35\textwidth} p{0.5\textwidth}}
    \toprule
    \textbf{Category} & \textbf{Learning or Takeaway} & \textbf{Quotes}\\
    \midrule
    {Task} &
    {Text overall seems more important than images for this task} &
    {
        ``The image could be detached from the text and the text seemed a bit more useful in this exercise'' (P7)
    }\\[0.2cm]

    {} &
    {Depending on the case, it may be important to combine the modalities or focus on text or image} &
    {
        ``How text and images interact together is a super important takeaway. You can’t just think about the images alone; you can’t just think about the text alone, it’s together the effect that they create'' (P16),
        ``One counter to [the greater importance of text] might be images of gore, where text is not necessarily needed for the post to be problematic.'' (P2)
    }\\[0.2cm]

    {} &
    {Memes are tricky to understand and label 
    % Their meanings can be vague and dependent on inside knowledge.
    } &
    {
        ``Memes are tricky in that the images may be benign but the text may be harmful.'' (P1),
        ``Memes are very vague and tricky to label. The subtext is hard to capture with simple concepts.'' (P6)
    }\\
    \midrule
    {Dataset} &
    {There is a need for greater representativity of kinds of harm in the data \rev{(homophobia, transphobia, nudity)}} &
    {
        ``Need more data [to capture] problematic posts of all kinds (not just racism or sexism) [...] Not enough data for homophobia, transphobia etc.'' (P1),
        ``[...] in this case nudity wasn't an issue, but might be for test time'' (P16),
    }\\[0.2cm]

    {} &
    {The dataset is may be too unrealistic and contrived to match the online distribution of posts
    % It needs to better match the distribution of what is actually posted online
    } &
    {
        ``The data seems to be far off from what is normally posted online, so the data definitely seems not good for general use.'' (P8)
    }\\[0.2cm]

    \midrule
    {Labels} &
    {Class imbalance has a large impact on modeling and makes it difficult to calibrate a model} &
    {
        ``I learned that class imbalance plays a large impact on modeling---it seemed for example that my own labeled dataset was relatively weighted towards not removing posts, so it paid dividends to [try] more specific targeted terms towards things that I found truly offensive like advocating for violence'' (P5)
    }\\[0.2cm]

    {} &
    {Their own labels appeared to be internally inconsistent} &
    {
        ``My labels are obviously not very internally consistent either and collecting from larger samples may help to even out the noise'' (P7)
    }\\[0.2cm]

    {} &
    {It would be valuable to increase the removal-score granularity beyond binarization} &
    {
        ``One area of improvement could be to increase the task fidelity to actually use the 5 labels instead of binarizing them.'' (P3)
    }\\
    \bottomrule
    \end{tabular}
    \caption{After performing a model sketching task, participants noted takeaways for their modeling approach and identified gaps in the dataset and labeling methodology. 
    }
    \label{table:modeling_gaps}
\end{table*}

\rev{
After the study concluded, we sought quantitative evidence to support the modeling gaps that participants raised. 
% Dataset representativity
\textit{Dataset representativity}: First, we explored whether the types of hate that participants claimed were insufficiently represented in their 40-example dataset were indeed underrepresented in the full 8.5k-example training dataset. Since the full dataset was not annotated for these categories of hate, a member of our team performed manual labeling for the four categories (homophobia, transphobia, and nudity) for both the 40-example study dataset and a random 2\% sample of the full training set (170 examples). To provide a point of comparison for these underrepresented categories, we additionally performed manual annotation for three participant-authored, higher prevalence concepts---religion, political, and racism---which had 17.5\%, 20.0\%, and 7.5\% prevalence, respectively. We found that indeed homophobia, transphobia, and nudity, which had 0\%, 0\%, and 5\% prevalence in the study dataset, also appear underrepresented in the full training dataset with 1.8\%, 1.2\%, and 10\% prevalence~(Figure~\ref{fig:data_rep_modeling_gap}). 
% Meanwhile, gender bias had a reasonable presence in the study dataset (10\% prevalence) and appears represented in the full training dataset. 
Overall, we see that concept representativity in the small dataset used for model sketching approximates representativity in the full dataset quite well given that it makes use of less than 0.5\% of the examples.

\begin{figure}[!tb]
  \includegraphics[width=0.4\textwidth]{figures/results/data_rep_modeling_gap_v2.pdf}
  \caption{
  \rev{Concepts that participants noted as underrepresented based on their sketching process with the study dataset (left chart) were generally underrepresented in the full training dataset. Already-prevalent concepts (right chart) maintained substantial levels of representation in the full training dataset.}
  }
  \label{fig:data_rep_modeling_gap}
\end{figure}

% Class imbalance
\textit{Class imbalance}: Then, we characterized the extent of class imbalance among participants' labels. During the study, four participants raised the issue of class imbalance; all of these participants indeed had a high level of imbalance, and all were skewed toward negative labels (mean=$79.3\%$ negative). Two of these participants displayed the highest class imbalance among all participants (with $92.5\%$ and $87.5\%$ negative labels). In addition, outside of the participants who noted the issue, three other participants also had more than $75\%$ negative labels. Thus, it appears that indeed class imbalance was a common challenge for this task.

We were encouraged to find that participants were able to rapidly identify potential modeling gaps before gathering a large-scale dataset or implementing a full model. Further, the problems they identified appeared to be valid issues with quantitative backing beyond the sketching context.
}


\subsubsection{Concept diversity}
Participants experimented with a broad variety of concept terms---ranging from concepts related to race and ethnicity to concepts related to politics, religion, and violence~(summarized by theme in Table~\ref{table:concept_summary}). 
Notably, all participants authored concepts that they had not considered in their initial brainstorm; the process of authoring concepts and sketches helped them to discover important and relevant concepts to incorporate. 
\rev{
Mapping from the 12 concept themes that we identified to participants' individual concepts, we found that participants each created concepts that spanned on average $5.65$ of these themes (SD=$1.90$). In the reverse direction, each theme was covered by an average of $8.0$ participants (SD=$3.10$). We thus see that participants individually covered a diverse set of concepts in their sketching sessions, and each concept theme was investigated from a variety of angles by different participants~(Figure~\ref{fig:concept_diversity_sankey}).
}
\begin{figure}[!tb]
  \includegraphics[width=0.65\textwidth]{figures/results/concept_sankey.pdf}
  \caption{
  \rev{We see substantial spread in the mapping between participants and concept themes, indicating that participants each explored diverse sets of concepts. \msl{May see if there's a more pared down representation for this plot?}}
  }
  \label{fig:concept_diversity_sankey}
\end{figure}

\begin{table*}[!tb]
  \centering
  \footnotesize % \scriptsize
    \begin{tabular}{p{0.15\textwidth} p{0.25\textwidth} p{0.05\textwidth}}
    \toprule
    \textbf{Theme} & \textbf{Sample Participant Concepts} & \textbf{Count}\\
    \midrule
    \textbf{Ethnicity, Race} & 
    {racism, racist, race} &
    {34}\\[0.1cm]
    
    \textbf{Danger, Violence} & 
    {violence, terrorism, harm} &
    {28}\\[0.1cm]

    \textbf{Emotion} & 
    {rant, scary, anger} &
    {27}\\[0.1cm]
    
    \textbf{Discrimination} & 
    {hate, hate speech, discrimination} &
    {22}\\[0.1cm]
    
    \textbf{Politics} & 
    {political, politics, fake news} &
    {16}\\[0.1cm]
    
    \textbf{Offensive} & 
    {offensive, vulgar, obscene} &
    {15}\\[0.1cm]
    
    \textbf{Religion} & 
    {religion, religious, muslim} &
    {14}\\[0.1cm]
    
    \textbf{Gender} & 
    {sexist, sexism, gender} &
    {10}\\[0.1cm]
    
    \textbf{Sexual Content} & 
    {nudity, sexual, sex} &
    {9}\\[0.1cm]
    
    \textbf{Humor} & 
    {funny, humor, joke} &
    {8}\\[0.1cm]
    
    \textbf{Trolling} & 
    {trolling, meme, bad meme} &
    {7}\\[0.1cm]
    
    \textbf{Intersectionality} & 
    {color \& gender, islamophobia | sexism} &
    {7}\\
    \bottomrule
    \end{tabular}
    \caption{Summary of participant concepts. Here, we include only themes for which 3 or more participants authored concepts, and we display the most common concept terms for each theme as well as the total number of participant concepts that fell within the theme.
    }
    \label{table:concept_summary}
\end{table*}

\subsubsection{Time required}
Finally, we note that participants were able to achieve these positive modeling outcomes in a fraction of the time that would be required to author a full model for this task. Participants' time estimates for executing on their pre-task modeling plans for the Hateful Memes task varied drastically from half a day to several weeks or months. However, even considering the most optimistic estimate of several hours (provided by 3 of 17 participants), our model sketching approach was able to deliver functional model prototypes in less than 30 minutes. 

\subsection{Participant experience outcomes}
% \msb{I like it, but ultimately vote to cut this subsection}
Addressing RQ2 in terms of benefits to ML practitioners, we observed that participants found the model sketching approach to be comfortable and expressive. Participants shared a great deal of excitement about this method of model development, expressing that they ``enjoyed the experience of thinking about models in this manner'' (P1) and that the tool ``could be really helpful in the future for similar tasks'' (P11) or for ``showing that something was possible and expanding imaginations'' (P12). We summarize these results in Appendix Section~\ref{section:participant_experience}.

% \subsubsection{Comparison with existing authoring tools}
% Comparing to their experiences with more common model authoring tools like Scikit-learn, PyTorch, and TensorFlow, participants felt similar levels of comfort with the {ModelSketchBook} API~(Figure~\ref{fig:survey_comfort_expressivity}) even though this 30-minute task was their first exposure to our tool, and all participants had significant experience with model authoring using these more traditional tools. At the same time, we saw that participants reported higher levels of expressivity when using the {ModelSketchBook} API than when using those same common model authoring tools. These results present promising support that our model sketching approach can be successfully adopted by ML practitioners as a lightweight, expressive entrypoint to model authoring.

% \begin{figure}[!tb]
%   \includegraphics[width=1.0\textwidth]{figures/survey/17 comfort_expressivity.pdf}
%   \caption{Upon their first-time use of the {ModelSketchBook} API, participants indicated similar levels of comfort as they feel with traditional model authoring tools (left), but they indicated higher levels of expressivity using {ModelSketchBook} (right).
%   }
%   \label{fig:survey_comfort_expressivity}
% \end{figure}

% \subsubsection{Reflections on the model sketching experience}
% % \msb{This paragraph and the following image are also candidates for cutting---I know it came up in the intro, but I think it's not super convincing to read that people think they're happy with a new system. These self reports bias positive due to novelty and demand characteristics.}
% In our survey, we also probed users' levels of satisfaction with their concepts and sketch models and asked them about the extent to which they felt their modeling approach changed or improved over time. We observed that participants were highly satisfied with both their concepts and sketch models. All but two participants rated their satisfaction with both models as ``somewhat satisfied,'' ``satisfied,'' or ``very satisfied.'' All but one participant responded that their modeling approach changed as they iterated on concepts and sketches, and the vast majority of participants (14 of 17) described a ``slight improvement,'' ``noticeable improvement,'' or ``significant improvement'' in their modeling approach.

% % \begin{figure}[!tb]
% %   \includegraphics[width=1.0\textwidth]{figures/survey/17 satisfaction_approach.pdf}
% %   \caption{Participants were largely satisfied with both their concepts and sketch models (left), and most indicated both substantial changes and improvements in their modeling approach throughout the task (right). 
% %   }
% %   \label{fig:survey_satisfaction_approach}
% % \end{figure}

% In their interview feedback and survey free-responses, participants expressed enthusiasm about the model sketching approach~(Appendix Table~\ref{table:summary_participant_experience}). 
% The most frequently-cited benefits of model sketching were that it was highly interpretable and explainable, easy to use (especially because it required no code), provided fast feedback loops, and prompted them to take on a different, high-level mode of thought. Meanwhile, the main limitations that participants noted were that the notebook environment often became disorganized, that our example-centric (rather than metric-centric) visualizations required more time to interpret, and that they would appreciate more assistance on brainstorming concepts. Multiple participants were excited about the opportunity to allow non-technical users and domain experts who lack ML knowledge to use ModelSketchBook and leverage their domain-specific expertise. They also suggested that we go beyond our notebook prototype to set up a dedicated user interface, and they suggested helper tools that would address potential issues with bias and overfitting in concepts.

\rev{
\subsection{Benchmarking concept generalization}
While we found in our case study demonstrations and field evaluation that concepts worked sufficiently well to support users' sketch modeling process, we sought to characterize the accuracy of our zero-shot concept scores compared to human annotations. We selected the most frequently-instantiated concepts among our study participants, which had been independently used by 4 or more participants. These included 4 text-based concepts (``religion,'' ``political,'' ``racism,'' and ``violence'') and 3 image-based concepts (``racism,'' ``nudity,'' ``violence''). 

For each of these concepts, we had four members of our team independently provide ratings for these seven concepts on all 40 items shown to participants in our study. To match the valid zero-shot concept score ranges, these labels were true or false for text-based concepts and 0-1 scores for image-based concepts). The inter-rater reliability based on Fleiss' Kappa had a mean of $0.53$ (SD=$0.24$) across the seven concepts, indicating moderate agreement. Based on majority rule using these manual labels, the prevalence for the three image-based concepts was too low to provide a reliable estimate, ranging from $0\%$ to $7.5\%$ (2 examples for racism, 0 for nudity, and 3 for violence) of the participants' datasets. This relates to the same issues that participants raised in Section~\ref{section:modeling_gaps} about the need for greater concept representation in the Hateful Memes dataset. 

However, the prevalence of the text-based concepts was sizeable, ranging from $15.0\%$ to $27.5\%$ of the participants' datasets, and inter-rater agreement was substantial ($\kappa=0.68$). We found that for the text-based concepts, the mean accuracy was $0.78$ (SD=$0.09$), and the mean F1 score was $0.58$ (SD=$0.14$), with a higher recall than precision (Recall=$0.66$, Precision=$0.55$). 

To benchmark image-based concepts, we repeated the same procedure with the next four most frequently-instantiated image-based concepts among our study participants (``muslim,'' ``historical,'' ``political,'' and ``animal''). The prevalence of these concepts ranged from $8.7\%$ to $18.5\%$, and our inter-rater agreement was substantial ($\kappa=0.60$). We found a mean accuracy of $0.90$ (SD=$0.04$) with a mean F1 score of $0.60$ (SD=$0.20$), with higher recall than precision again (Recall=$0.64$, Precision=$0.60$).
Thus, for an approach that requires no data collection, concept labeling, or training time, the zero-shot concept scores provide users with a reasonable starting point for further iteration and refinement.

\msl{Add somewhere about how image concepts didn't work well in this task; image concepts work better with more concrete concepts, and those kinds of concepts aren't particularly helpful for the hateful memes task}
}

\subsection{Benchmarking sketch model performance}
While the goal of model sketching is not to produce full-scale models, we seek to understand whether sketch models achieve reasonable functionality relative to full-scale models.

\subsubsection{Study participants' sketch models}
First, we investigated the sketch models authored by our study participants. 
We compared all participants' self-determined ``best sketch model'' against two kinds of baselines: 
1)~\textit{first sketch}, the very first sketch that a participant authored with the {ModelSketchBook} API and 
2)~\rev{\textit{zero-shot} baseline that used a single GPT-3 prompt to predict whether each example is ``hateful'' or not. For each model variant, performance was measured against the participant's own ground truth labels on their 20-example test set.
We found that participants' best sketches outperformed both baselines on classification metrics (F1, precision, recall), but the best sketches achieved slightly lower performance than the baselines on the regression version of the task, as measured by Mean Absolute Error (MAE)~(Figure~\ref{fig:mean_metric_plot}). Looking back at performance on the 20-example training set upon which users were actively iterating, we observe that participants' best sketches more strongly outperform the first sketch and zero-shot baselines on the classification metrics and MAE.
} 

These results suggest that participants are able to iteratively improve their sketch models to achieve higher alignment with their modeling goals and that sketch models may work better for classification tasks than for fine-grained regression tasks.
\rev{Given that sketch model performance metrics declined from the training set and test set, participants may have overfit to the training dataset during their sketch model development. Meanwhile, the zero-shot baseline displayed a generally worse---but consistent---level of performance between the train and test set as expected, precisely \textit{because} this model was given no opportunity to overfit to the training set. These two extremes fall in line with classic bias-variance tradeoffs in machine learning. 
\msl{Will iterate on this, but working on articulating why overfitting is more valuable than underfitting for our sketching task:}
However, for the task of sketching, overfitting to the data is actually more informative than underfitting with a simplistic, untuned model. Given that our dataset is far too small to learn a generic model, the sketch is intended to lend insights about settings for which this small dataset is a \textit{representative}, realistic sample. The primary purpose of the sketch is to give a reasonable approximation for how a model might behave, so our goal is more to maximize the learnings from this sample rather than generalize to markedly different settings.}
Lastly, we note that for this task, the classification metrics were relatively low overall due to class imbalance \rev{as discussed in Section~\ref{section:modeling_gaps}}. Many participants had substantial skew in labels toward the negative class (``non-hateful'') and thus ended up producing models that always predicted the negative class (behavior which results in scores of 0.0 for recall, precision, and F1).

\begin{figure}[!tb]
  \includegraphics[width=0.6\textwidth]{figures/results/all_perf_metrics_TRAIN_TEST_zeroshot.pdf}
  \caption{
  \rev{
  For the training set (top), we observe consistently better performance (MAE, F1 score, precision, and recall) for participants' self-designated ``best'' sketches compared to baselines of their first sketch and a zero-shot model.
  For the test set (bottom), we observe better classification performance (F1 score, precision, and recall) for the ``best'' sketch, but higher MAE.
  }
  }
  \label{fig:mean_metric_plot}
\end{figure}

\subsubsection{Investigating the impact of task difficulty on sketch model performance}
Thus, we sought to further investigate the performance of sketch models in cases without such strong class imbalance and with many more than 20 training examples. We prepared three additional tasks: an IMDB movie review sentiment analysis task (easiest: per-example ratings and balanced classes)~\cite{imdb_sota}; a comment toxicity task (harder: per-annotator ratings and class skew)~\cite{kumar2021designing}; and the original Hateful Memes task (hardest: balanced classes, but nuanced and multimodal task)~\cite{kiela_hatefulMemes}. For each of these, we compared sketch models against published state-of-the-art (SOTA) models, using the same headline performance metric and train/test datasets as were used by the SOTA model. 
We sampled up to 500 examples to train our sketch models (in comparison, the SOTA models for these tasks were trained on 25k, 100k, and 8.5k examples, respectively). For evaluation, we calculated performance using a sample of 100 examples from the training set (preserving the same label distribution). 
For the IMDB task, the SOTA model reported 0.93 accuracy and our sketch model achieved 0.91 accuracy, only slightly lower.
On the comment toxicity task (which used a 0-4 score range), the SOTA model reported 0.90 MAE while our sketch model achieved an MAE of 1.39.
On the Hateful Memes task, the SOTA model reported 0.845 AUROC, and 0.714 AUROC was the SOTA result when the challenge was first released; our sketch model achieved 0.584 AUROC.
Thus, model sketching demonstrates strong or reasonable performance on the easy and medium difficulty tasks, but displays weaker performance results for the third, significantly harder task.


\subsection{Failure modes}
While our model sketching approach achieved its aims of shifting model developers' cognitive frame and presented a number of benefits for the models they developed and their model authoring experience, we observed several failure modes.
% Concept models failing, only can provide another concept term; users often gave up too soon
First, though participants had some promising concept ideas, they were not always able to actualize them with our zero-shot model-based approach. 
% When a participant's concept failed to give them results that substantially overlapped with their own judgement, there was little recourse other than to attempt another related concept term and see if that achieves better alignment. 
Participants often relied heavily on the results of the first concept term that they attempted. If that failed to return satisfactory results, they often abandoned the concept idea since they assumed that the model probably was not sophisticated enough to understand that concept. Participants would benefit from scaffolding to understand whether the model lacks an understanding of a given concept or just requires different terminology.
% differentiate cases where the model understands the concept but expresses it with different terms versus cases where the model lacks an understanding of the concept at all.

% Tending to cater to the LLM rather than thinking more broadly/creatively
% Second, we found that since participants were given an explanation of the underlying zero-shot modeling approaches used to surface concept scores, participants overly tailored their concept terms based on what they thought that these zero-shot models would be able to understand. 
Second, we found that some participants heavily tailored their concept terms based on what they thought zero-shot models would be able to understand, especially using concrete, specific concept terms.
% since they anticipated that models would perform better with these kinds of inputs. 
We observed that several of these participants eventually branched out and found that broader terms could work well. However, the downside still remains that since our concepts rely on pretrained models, these models can be limiting factors. Users might constrain their thinking to areas where the pretrained model already excels rather than thinking more creatively about what decisionmaking factors may be valuable.

% Bad modeling practices (ex: overfitting approaches, ignoring certain kinds of errors)
Finally, we noticed that because our approach emphasized a ``small data'' approach to help users stay focused, some participants lost sight of the overall goal to build a robust, general model. Participants sometimes fell into overfitting approaches by scrutinizing cases where their sketch model made errors and patching errors with very specific concepts that were not relevant to the larger decision-making task. Participants would benefit from tools that would help them to assess the generalizability of their sketch models. We believe that a curated dataset is worth this tradeoff because it encourages ML practitioners to avoid detailed data analysis and instead focus on broad-strokes concepts. 
% P9 conveyed this well, noting that ``if you are working with a limited dataset, it may be more advantageous to spend time thinking about concepts rather than making your model more complex.''

% Limitations of our approach even if it were to work perfectly
% \begin{itemize}
%     \item Types of concepts that performed poorly; where the LLM or CLIP fails
%     \item Limited kinds of thinking (ex: framing the problem purely in terms of what a pretrained model can currently do)
%     \item Bad modeling practices (ex: overfitting approaches, ignoring certain kinds of errors)
% \end{itemize}
% Other maladaptive strategies that come up using this approach that would impair later model development
% “even if the tool worked perfectly, what are the downsides of this approach”




% To cover
% - Concept innovation vs concept execution vs concept abandonment (the _intent_ behind changes in concept models and sketches)




==> sections/old_versions/5_results_v5.tex <==
% 11/29/22 V4

% \msb{cut:} %ML practitioners successfully engaged in model sketching, shifting their attention more towards higher-level, model design questions rather than technical model implementation details. This cognitive shift helped them to better explore the model design space and identify gaps in the modeling approach while requiring a fraction of the time that would ordinarily be required to author a functional model. 
Using our {ModelSketchBook} API, participants successfully authored an average of 12.2 (SD=4.7) concepts and 4.1 (SD=2.0) different sketch models that built on those concepts for the Hateful Memes task. Figure~\ref{fig:eval_sketches} displays sample concepts and sketch models authored by participants, \rev{and Table~\ref{table:concept_summary} summarizes all participants' concepts.}

\rev{
% Additional stats on concepts
Of the concepts authored in the study, $53.6\%$ were text concepts, and $32.4\%$ were image concepts, and $14.0\%$ were compound concepts involving a logical operator. Participants each authored on average $6.53$ text concepts (SD=$3.00$), $4.19$ image concepts (SD=$2.14$), and $2.07$ compound concepts (SD=$1.53$). Of the compound concepts, $62.1\%$ used an \texttt{AND} operator while $37.9\%$ used an \texttt{OR} operator, and $79.3\%$ combined only text concepts while the remaining $20.7\%$ combined both text and image concepts.
There were 136 distinct concepts authored by the study participants. On an individual level, participants each authored an average of $6.29$ unique concepts (SD=$3.77$) that no other participants had authored.
}

\rev{
% Label variance
We aimed for our modeling task to involve a high amount of subjectivity to provide a sufficiently broad model design space among participants. This was indeed the case: there were substantial differences in how our participants chose to label the provided dataset. Across participants and data examples, the mean standard deviation in labels (on a 0-1 scale) was $0.23$. For the binarized versions of those same scores, this meant that $75\%$ of the examples had at least one participant who disagreed with the majority label, and $37.5\%$ of the examples had a quarter or more of the participants who disagreed with the majority label.
}

% \begin{figure}[!tb]
%   \includegraphics[width=0.6\textwidth]{figures/results/concept_sketch_num_plot.pdf}
%   \caption{There was considerable variation in the number of concept and sketch models that participants authored, but all participants authored 5 or more concepts and 2 or more sketches within our approximately 30-minute task period.
%   }
%   \label{fig:concept_sketch_boxplot}
% \end{figure}

\begin{figure}[!tb]
  \includegraphics[width=\linewidth]{figures/eval_sketches_v1.pdf}
  \caption{
    Examples of participant sketches. For illustrative purposes, we display the first sketch, best sketch, and other concepts for three study participants. Participants explored a broad range of concepts and expanded from their initial sketch models.
  }
  \label{fig:eval_sketches}
\end{figure}

\subsection{Changes in the cognitive process of model authoring}
% How we observed a shift from technical+implementation-oriented to conceptual+design/value-oriented thinking
Addressing RQ1, model sketching aided ML practitioners in shifting their thinking from technical, implementation-oriented factors toward higher-level, conceptual, design-oriented factors of model development. 

\subsubsection{Changes in planned modeling approach}
In their pre-task modeling plans, participants tended to focus on implementation details such as specific modeling methods or architectures (e.g., transformer models, convolutional neural networks, supervised models, linear classifiers), ML conventions like train-test splits and performance metrics, and data-oriented plans for feature extraction (summarized in Table~\ref{table:modeling_plan}). 
% general ML ``hygiene'' like ensuring that the examples span a range of scores and adjusting for skewed or imbalanced labels
For example, P13 described their approach as ``two types of models: [one] sentiment based and another that is a simple CNN, and then combine the two models with a simple fully connected layer,'' and P8 planned to ``create test/val/train sets with equal distributions of data'' and then ``train some model and inspect how it performs on a held out test set.''

However, after exposure to model sketching, participants described that they would spend time on brainstorming and curating concepts relevant to the decision-making task and that they would iterate on their concepts by inspecting sketch model outputs. P15 described that ``Spending a few days tinkering with concepts could produce a fairly effective model that would be easier to debug.'' Participants also branched out to mention that they would like to consider different subclasses of harm and described how they might combine a concept-based approach with more traditional modeling approaches. For example, while P8 still preferred to use a more complex, non-linear model, they wished to use concepts from ModelSketchBook to augment their datapoints. \rev{Participants also described changes to their mode of thinking during model sketching, which we qualitatively summarize in Appendix Section~\ref{section:participant_thought_processes}.}

\begin{table*}[!tb]
  \centering
  \footnotesize
    \begin{tabular}{p{0.08\textwidth} p{0.22\textwidth} p{0.6\textwidth}}
    \toprule
    \textbf{Study Phase} &
    \textbf{Modeling Plan Theme} &
    \textbf{Quotes}\\
    \midrule
    \textbf{Before model sketching} & 
    {Specific model architectures or techniques} &
    {
        ``I would use a convolutional neural network model [...] probably use transformers in conjunction with CNNs to track long-term dependencies and help contextualize the text data.'' (P1),
        ``Two types of models: sentiment based and another that is a simple CNN, and then combine the two models with a simple fully connected layer'' (P13),
        % ``I would use a binary classifier. Read the image and text, then build features using word2vec or some similar method. Depending on the size of the data would use either a tree based classifer or a deep learning model'' (P17)
    } \\[0.2cm]
    
    {} & 
    {Evaluating on training and validation sets} &
    {
        ``Ensure that the dataset is divided into train, test and validation slices. Experiment with several modeling techniques while evaluating on the validation set'' (P3),
        % ``Create test/val/train sets with equal distributions of data. Train some model and inspect how it performs on a held out test set'' (P8)
    } \\[0.2cm]

    % {} & 
    % {Training on a range of toxicity levels} &
    % {
    %     ``Train it on a lot of problematic and unproblematic (benign, slightly problematic, very problematic etc.) images'' (P1),
    %     ``Collect a bunch of posts of all levels of questionableness (a priori)'' (P5)
    % } \\[0.2cm]

    {} & 
    {Standard performance metrics} &
    {
        ``Measure various metrics (accuracy, bias, variance etc.)'' (P1),
        ``Figure out the right set of metrics for evaluating any model that is trained. Choices could be accuracy, F1 scores and other metrics such as AUC or AuPR depending on relative label weights.'' (P3)
    } \\[0.2cm]

    {} & 
    {Building low-level features stemming from data} &
    {
        ``Can use features from the posts and user interactions. Can use general user information along with the post information'' (P4),
        ``Build features representing intuitions for things relevant to removal; like topic metadata, language choice, likes/dislikes/controversiality'' (P5),
        % ``Think through what features to construct through data summary, correlation analysis, etc.'' (P7)
    } \\
    
    \midrule
    
    \textbf{After model sketching} & 
    {Spending time brainstorming and curating concepts} &
    {
        % ``[I would] think about all the concepts related to the underlying tasks'' (P4),
        % ``I would focus more on concepts, deep-dive into data to see what it’s actually like, see how the other models are performing.'' (P13),
        ``I would likely lean into feature engineering carefully to have an interpretable model. Spending a few days tinkering with concepts could produce a fairly effective model that would be easier to debug.'' (P15)
    } \\[0.2cm]
    
    {} & 
    {Iterating on concepts by inspecting sketch model outputs} &
    {
        ``[I would] see mislabelled (and correctly labeled) examples from the aggregator and brainstorm more specific features that might account for that'' (P5),
        % ``Think of concepts that relate to the task; try the concept; observe performance and then try other concepts; put them together for sketch; observe sketch performance and iterate on concepts'' (P16)
    } \\[0.2cm]

    {} & 
    {Authoring concepts informed by different categories of harm} &
    {
        % ``A model to remove problematic social media posts would be a classification model placing different posts in different buckets (based on the degree of harm, violence etc. it may promote).'' (P1),
        ``I think filtering on hate (race/gender/religion) speech and political speech would be good first steps. There are some examples of graphic/violent posts that might not be captured by those categories, so I would add more filters for those specifically.'' (P2)
    } \\[0.2cm]

    {} & 
    {Combining a concept-based approach with traditional approaches} &
    {
        ``Also can use these labels as annotations to the datapoints for a more complex model (nonlinear). Seems like having the original data is still good so wouldn't rely on the CLIP/GPT annotations alone.'' (P8),
        ``I will probably still collect data manually and then instead of using a pretrained model and build the pipeline from scratch, I will use the ModelSketchBook API.'' (P11)
    } \\%[0.2cm]

    % {} & 
    % {Engaging in ethical and user-facing considerations} &
    % {
    %     ``It is very important to avoid suppressing speech especially speech/expression that is not violent or blatantly harmful.'' (P1),
    %     ``As a baseline, I would compare to the effectiveness of using some Transformer model to judge the end result directly, I wouldn't want to use it because its uninterpretable, hence dangerous.'' (P15)
    % } \\
    \bottomrule
    \end{tabular}
    \caption{
    % \msb{Cut some of the rows on the table, I suggest. It's eating up a bunch of words. Maybe move the pre-task part of the table into Appendix? Or, pick only 2-3 categories pre and post. If you keep pre and post, name them more descriptively for someone who's just skimming the paper, e.g., before model sketching, after model sketching} 
    A summary of participants' modeling plans before and after the study. Participants chose to adopt model sketching in their future modeling plans and shifted from more technical, implementation-related plans to more procedural, value-oriented plans.
    }
    \label{table:modeling_plan}
\end{table*}

\subsubsection{Concept evolution}
% \msb{cut this paragraph? not sure we need the definitional throat clearing, the next paragraph may be clear from context} 
% One window into participants' mindset and approach is the way that their concepts evolve over time while using {ModelSketchBook}. We identify three main types of intent underlying concept authorship: 1)~\textit{concept innovation}, cases where participants come up with ideas for distinct concepts that they hadn't brainstormed before, 2)~\textit{concept execution}, cases where participants are continuing an existing concept idea, but are experimenting with different ways to actualize that concept via concept term inputs, and 3)~\textit{concept abandonment}, cases where participants decided not to continue with a concept and did not include it in their sketch models. 
% Concept innovation
One window into participants' mindset is the way that their concepts evolve over time while using ModelSketchBook.
We observed that on average, participants engaged in 8.5 (SD=2.7) instances of \textit{concept innovation}, which we define as the number of distinct concept ideas; on average 5.0 (SD=2.8) of those concept innovations were \textit{not} in the participant's original brainstormed list. Concept evolution often stemmed from participants discovering errors in their sketch models: P7 noted that a sketch model combining racism and sex concepts ran into false positives with humorous posts, which inspired an exploration of humor-related concepts. These progressions often built on each other: P4 initially started with a profanity concept that worked well, so they then brainstormed other dimensions of hate and decided to explore racism-related concepts; they then discovered that race and ethnicity-related hate in this dataset was often targeted at Muslims, so they got the idea to explore concepts related to Islamophobia.
% Concept execution
Participants on average displayed 3.2 (SD=2.3) instances of \textit{concept execution}, which we define as the number of concepts authored that were continuations of the same concept idea (for example, switching from an image-based racism concept to a text-based racism concept, or changing from a concept term of ``racism'' to one of ``race''). Participants more frequently changed modalities, but rarely modified concept terms.
% Concept abandonment
Then, participants underwent \textit{concept abandonment} for an average of 4.2 (SD=2.6) concept ideas; we define this phenomenon as the number of concept ideas that were not ultimately used in the user's self-designated ``best'' sketch model. This abandonment is also a valuable part of sketching---to identify and discard paths that appear to be dead-ends. For example, P14 tried a ``harmful'' image-based concept, but found that this surfaced noisy results; they concluded that this was because the concept was too vague and didn't closely relate to the images in the dataset, and they decided to explore more grounded, specific concepts for images.
Thus, participants appear to engage in a variety of different generative, iterative, and reflective modes as they author concepts.

\subsection{Modeling outcomes}
% TODO: how this produces better or more societally-beneficial models
Regarding RQ2, we observed that the high-level cognitive shift in focus during model development brought about concrete benefits for the models themselves---from the breadth of concepts that sketch models explored to the gaps that participants uncovered in the modeling setup.

\subsubsection{Identifying modeling gaps}
\label{section:modeling_gaps}
% \msb{cut:} %One of the aims of model sketching is that, in redirecting ML practitioners' attention to higher-level design decisions, it will allow them to identify flaws in not only their model, but in the problem formulation, dataset, and deployment context that surround it. 
%We summarize themes of participants' learnings and takeways in , which demonstrates that the brief 
Model sketching helped participants to gain insights beyond just the model itself.
Participants uncovered major categories of harm that were not sufficiently represented in the provided sample of the dataset, \rev{such as homophobia and transphobia, and they noted that memes in the dataset appeared unrealistic compared to current online memes, so models built on this data may fail in practice due to distribution shift}. Participants also identified limitations of the labeling approach such as class imbalance and inconsistent ratings. They gained intuitions about the task itself: participants discovered that for these memes, text was often more meaningful since the images were usually quite benign, and they started to form a sense of cases where multimodal approaches may reap more benefits. 
\rev{See a more detailed summary in Appendix Section~\ref{section:appendix_modeling_gaps}.}

\rev{
After the study concluded, we sought quantitative evidence to support the modeling gaps that participants raised. 
% Dataset representativity
\textit{Dataset representativity}: First, we explored whether the concepts that participants claimed were insufficiently represented in their 40-example dataset were indeed underrepresented in the full 8.5k-example training dataset. Since the full dataset was not annotated for these concepts, a member of our team performed manual labeling for the three participant-identified categories (homophobia, transphobia, and nudity) for both the 40-example study dataset and a random 2\% sample of the full training set (170 examples). As a point of comparison, we additionally performed manual annotation for three participant-authored, higher prevalence concepts---religion, political, and racism---which had 17.5\%, 20.0\%, and 7.5\% prevalence in the study dataset, respectively. We found that indeed homophobia, transphobia, and nudity, which had 0\%, 0\%, and 5\% prevalence in the study dataset, also appear underrepresented in the full training dataset with 1.8\%, 1.2\%, and 10\% prevalence~(Figure~\ref{fig:data_rep_modeling_gap}). 
Overall, we see that concept representativity in the small dataset used for model sketching can provide helpful warning signals on representativity in the full dataset.
% despite using less than 0.5\% of the examples.

\begin{figure}[!tb]
  \includegraphics[width=\linewidth]{figures/results/data_rep_modeling_gap_v3.pdf}
  \caption{
  \rev{Concepts that participants noted as underrepresented based on their sketching process with the study dataset (left) were generally underrepresented in the full dataset. Already-prevalent concepts (right) maintained substantial representation in the full dataset. 
  % \msb{Font size is too small when rendered in the paper. I suggest making the graph less tall (crop at .4?), and more wide.}
  }
  }
  \label{fig:data_rep_modeling_gap}
\end{figure}

% Class imbalance
\textit{Class imbalance}: Then, we characterized the extent of class imbalance among participants' labels. During the study, four participants raised the issue of class imbalance; all of these participants indeed had a high level of imbalance, and all were skewed toward negative labels (mean=$79.3\%$ negative). Two of these participants displayed the highest class imbalance among all participants (with $92.5\%$ and $87.5\%$ negative labels). In addition, outside of the participants who noted the issue, three other participants also had more than $75\%$ negative labels. Thus, it appears that indeed class imbalance was a common challenge for this task.

We were encouraged to find that participants were able to rapidly identify potential modeling gaps before gathering a large-scale dataset or implementing a full model. 
% Further, the problems they identified appeared to be valid issues with quantitative backing beyond the sketching context.
}


\subsubsection{Concept diversity}
Participants experimented with a broad variety of concept terms---ranging from concepts related to race and ethnicity to concepts related to politics, religion, and violence~(summarized by theme in Table~\ref{table:concept_summary}). 
Notably, all participants authored concepts that they had not considered in their initial brainstorm; the process of authoring concepts and sketches helped them to discover important and relevant concepts to incorporate. 
\rev{
Mapping participants' individual concepts to the 12 common themes that we identified, we found that participants created concepts that spanned on average $5.65$ of these themes (SD=$1.90$). In the reverse direction, each theme was covered by an average of $8.0$ participants (SD=$3.10$). We thus see that participants were able to explore a diverse set of concepts in their sketching sessions, and each concept theme was investigated from a variety of angles by different participants~(Figure~\ref{fig:concept_diversity_matrix}).
}

\begin{table}[!tb]
  \centering
  \footnotesize % \scriptsize
    \begin{tabular}{p{0.25\linewidth} p{0.5\linewidth} p{0.1\linewidth}}
    \toprule
    \textbf{Theme} & \textbf{Sample Participant Concepts} & \textbf{Count}\\
    \midrule
    \textbf{Ethnicity, Race} & 
    {racism, racist, race} &
    {34}\\[0.1cm]
    
    \textbf{Danger, Violence} & 
    {violence, terrorism, harm} &
    {28}\\[0.1cm]

    \textbf{Emotion} & 
    {rant, scary, anger} &
    {27}\\[0.1cm]
    
    \textbf{Discrimination} & 
    {hate, hate speech, discrimination} &
    {22}\\[0.1cm]
    
    \textbf{Politics} & 
    {political, politics, fake news} &
    {16}\\[0.1cm]
    
    \textbf{Offensive} & 
    {offensive, vulgar, obscene} &
    {15}\\[0.1cm]
    
    \textbf{Religion} & 
    {religion, religious, muslim} &
    {14}\\[0.1cm]
    
    \textbf{Gender} & 
    {sexist, sexism, gender} &
    {10}\\[0.1cm]
    
    \textbf{Sexual Content} & 
    {nudity, sexual, sex} &
    {9}\\[0.1cm]
    
    \textbf{Humor} & 
    {funny, humor, joke} &
    {8}\\[0.1cm]
    
    \textbf{Trolling} & 
    {trolling, meme, bad meme} &
    {7}\\[0.1cm]
    
    \textbf{Intersectionality} & 
    {color \& gender, islamophobia | sexism} &
    {7}\\
    \bottomrule
    \end{tabular}
    \caption{Summary of participant concepts. Here, we include only themes for which 3 or more participants authored concepts, and we display the most common concept terms for each theme as well as the total number of participant concepts that fell within the theme.
    }
    \label{table:concept_summary}
\end{table}

\begin{figure*}[!tb]
  \includegraphics[width=0.8\linewidth]{figures/results/concept_theme_matrix_v2.pdf}
  \caption{
  \rev{A heatmap matrix mapping from participants (x-axis) to concept themes (y-axis) depicts substantial spread between participants and themes, indicating that participants each explored diverse sets of concepts. The concept themes are sorted from top to bottom by the count of unique participants, and the participants are sorted from left to right by the count of unique concept themes.
  % \msb{sankey diagrams typically show flows over time. This might be more interpretable if you re-encode it as a matrix? \url{https://homes.cs.washington.edu/~jheer//files/zoo/ex/networks/matrix.html} }
  }
  }
  \label{fig:concept_diversity_matrix}
\end{figure*}

\subsubsection{Time required}
Finally, we note that participants were able to achieve these positive modeling outcomes in a fraction of the time that would be required to author a full model for this task. Participants' time estimates for executing on their pre-task modeling plans for the Hateful Memes task varied drastically from half a day to several weeks or months. However, even considering the most optimistic estimate of several hours (provided by 3 of 17 participants), our model sketching approach was able to deliver functional model prototypes in less than 30 minutes. 
\rev{Beyond the speed of model sketching, we document participant experience outcomes in detail in Appendix Section~\ref{section:participant_experience}.}

% \subsection{Participant experience outcomes}
% \msb{I like it, but ultimately vote to cut this subsection}
% Addressing RQ2 in terms of benefits to ML practitioners, we observed that participants found the model sketching approach to be comfortable and expressive. Participants shared a great deal of excitement about this method of model development, expressing that they ``enjoyed the experience of thinking about models in this manner'' (P1) and that the tool ``could be really helpful in the future for similar tasks'' (P11) or for ``showing that something was possible and expanding imaginations'' (P12). We summarize these results in Appendix Section~\ref{section:participant_experience}.

\rev{
\subsection{Benchmarking concept performance}
While we found in our case study demonstrations and field evaluation that concepts worked sufficiently well to support users' sketch modeling process, we sought to characterize the accuracy of our zero-shot concept scores compared to human annotations. We selected the most frequently-instantiated concepts among our study participants, which had been independently used by four or more participants. These included four text-based concepts (``religion,'' ``political,'' ``racism,'' and ``violence'') and three image-based concepts (``racism,'' ``nudity,'' and ``violence''). Four members of our team independently provided ratings for these concepts on all 40 items shown to participants in our study. 
% To match the valid zero-shot concept score ranges, these labels were true or false for text-based concepts and 0-1 scores for image-based concepts. 
Based on these manual labels, the prevalence for the image-based concepts was too low to provide a reliable estimate, with a mean of $4.2\%$ prevalence (including 0 examples for the ``nudity'' concept) in participants' datasets.\footnote{\rev{This relates to the same issues that participants raised in Section~\ref{section:modeling_gaps} about the need for greater concept representation in the Hateful Memes dataset.}}
We thus repeated the same procedure with the next most frequently-instantiated image-based concepts among our study participants (``muslim,'' ``historical,'' ``political,'' and ``animal'').}

% Side-by-side version of concept perf figures
\begin{figure}[!tb]
  \centering
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \small %\footnotesize % \scriptsize
    \rev{  
    \begin{tabular}{r r | c c}
    \toprule
    \textbf{} & \textbf{Concept Type} & \textbf{Text} & \textbf{Image}\\
    \midrule
    \multirow{2}{0.2\textwidth}{\raggedleft\textit{Annotation metrics}}&
    \textbf{Mean Prevalence} & 
    {19.4\%} &
    {13.3\%}\\[0.1cm]
    &\textbf{Fleiss' Kappa} & 
    {0.68} &
    {0.60}\\[0.1cm]
    \midrule
    \multirow{4}{0.2\textwidth}{\raggedleft\textit{Concept performance}}&
    \textbf{Accuracy} & 
    {0.78} &
    {0.90}\\[0.1cm]
    &\textbf{F1 Score} & 
    {0.58} &
    {0.60}\\[0.1cm]
    &\textbf{Recall} & 
    {0.66} &
    {0.64}\\[0.1cm]
    &\textbf{Precision} & 
    {0.55} &
    {0.60}\\
    \bottomrule
    \end{tabular}
    }
    \captionof{table}{\rev{
    Concept performance for text and image concepts created by participants is moderately high based on manual annotations.
    }}
    \label{table:concept_perf}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/results/concept_gen_textAndVis_all.pdf}
    \captionof{figure}{\rev{
    Concept performance for text and image concepts created by participants is moderately high based on manual annotations.
    }}
    \label{fig:concept_perf}
  \end{minipage}  
\end{figure}

\rev{We observe comparable levels of performance for both text and image concepts, as summarized in Table~\ref{table:concept_perf} and Figure~\ref{fig:concept_perf}. Both sets of concepts displayed substantial levels of inter-rater agreement as measured by Fleiss' Kappa and had sufficient prevalence levels based on these manual labels.
% However, the prevalence of the text-based concepts was sizeable, ranging from $15.0\%$ to $27.5\%$ of the participants' datasets, and inter-rater agreement was substantial ($\kappa=0.68$). 
For the text-based concepts, we found a mean accuracy of $0.78$ (SD=$0.09$) and a mean F1 score of $0.58$ (SD=$0.14$), with a higher recall than precision (Recall=$0.66$, Precision=$0.55$). 
% The prevalence of the image-based concepts ranged from $8.7\%$ to $18.5\%$, and our inter-rater agreement was substantial ($\kappa=0.60$). 
We found that for image-based concepts, there was a mean accuracy of $0.90$ (SD=$0.04$) and a mean F1 score of $0.60$ (SD=$0.20$), with higher recall than precision again (Recall=$0.64$, Precision=$0.60$).
Thus, for an approach that requires no data collection, concept labeling, or training time, the zero-shot concept scores provide users with a reasonable starting point for further iteration and refinement.
}

\subsection{Benchmarking sketch model performance}
While the goal of model sketching is not to produce full-scale models, we sought to understand whether sketch models achieve reasonable functionality relative to full-scale models.

\subsubsection{Study participants' sketch models}
First, we investigated the sketch models authored by our study participants. 
We compared all participants' self-determined ``best sketch model'' against two kinds of baselines: 
1)~\textit{first sketch}, the very first sketch that a participant authored with the {ModelSketchBook} API and 
2)~\rev{\textit{zero-shot} baseline that used a single GPT-3 prompt to predict whether each example is ``hateful'' or not. For each model variant, performance was measured against the participant's own ground truth labels on their 20-example test set.
We found that participants' best sketches outperformed both baselines on classification metrics (F1, precision, recall), but the best sketches achieved slightly lower performance than the baselines on the regression version of the task, as measured by Mean Absolute Error (MAE)~(Figure~\ref{fig:mean_metric_plot}). Looking back at performance on the 20-example training set upon which users were actively iterating, participants' best sketches more strongly outperformed the first sketch and zero-shot baselines on all metrics.
} 

These results suggest that participants are able to iteratively improve their sketch models to achieve higher alignment with their modeling goals and that sketch models may generalize better for classification tasks than for fine-grained regression tasks.
\rev{Given that sketch model performance metrics declined between the training set and test set, participants may have overfit to the training dataset during their sketch model development. Meanwhile, the zero-shot baseline displayed a generally worse---but consistent---level of performance between the train and test set as expected, precisely because this model was given no opportunity to overfit to the training set. These two extremes fall in line with classic bias-variance tradeoffs in machine learning. Our sketch model results mirror prior literature on the common challenge of overfitting tendencies in IML~\cite{wu2019localDecisionPitfallsIML, daee2019userModelingAvoidingOverfitting}, especially given that we did not take steps to explicitly steer users away from overfitting behavior.}
% However, for the task of sketching, overfitting to the data is actually more informative than underfitting with a simplistic, untunable model \msb{This is a big and unsubstantiated claim. Why would we want participants to build models that overfit when sketching? Do we need this claim?}. Given that our dataset is far too small to learn a generic model, the sketch is intended to lend insights about settings for which this small dataset is a \textit{representative}, realistic sample \msb{Not sure this is a compelling enough reason; it might be enough to simply note that people can overfit. could instead just say that our results mirror prior literature on human-in-the-loop AI overfitting to the training set? \url{https://dl.acm.org/doi/abs/10.1145/3172944.3172989}}. 
% The primary purpose of the sketch is to give a reasonable approximation for how a model might behave for the purpose of problem formulation, so our goal is more to maximize the learnings from this sample rather than generalize to markedly different settings.}
Lastly, we note that for this task, the classification metrics were relatively low overall due to class imbalance \rev{as discussed in Section~\ref{section:modeling_gaps}}. Many participants had substantial skew in labels toward the negative class (``non-hateful'') and thus ended up producing models that always predicted the negative class (behavior which results in scores of 0.0 for recall, precision, and F1).

\begin{figure*}[!tb]
  \includegraphics[width=\textwidth]{figures/results/all_perf_metrics_TRAIN_TEST_zeroshot_horiz.pdf}
  \caption{
  \rev{
  For the training set (left), we observe consistently better performance (MAE, F1 score, precision, and recall) for participants' self-designated ``best'' sketches compared to baselines of their first sketch and a zero-shot model.
  For the test set (right), we observe better classification performance (F1 score, precision, and recall) for the ``best'' sketch, but higher MAE.
  }
  }
  \label{fig:mean_metric_plot}
\end{figure*}

\subsubsection{Investigating the impact of task difficulty on sketch model performance}
Thus, we sought to further investigate the performance of sketch models in cases without such strong class imbalance and with many more than 20 training examples. We prepared three additional tasks: an IMDB movie review sentiment analysis task (easiest: per-example ratings and balanced classes)~\cite{imdb_sota}; a comment toxicity task (harder: per-annotator ratings and class skew)~\cite{kumar2021designing}; and the original Hateful Memes task (hardest: balanced classes, but nuanced and multimodal task)~\cite{kiela_hatefulMemes}. For each of these, we compared sketch models against published state-of-the-art (SOTA) models, using the same headline performance metric and train/test datasets as were used by the SOTA model. 
Please see Appendix Section~\ref{section:sota_details} for additional details on \revFinal{the benchmarks and our sketch models.}
For the IMDB task, the SOTA model reported 0.93 accuracy and our sketch model achieved 0.91 accuracy, only slightly lower.
On the comment toxicity task (which used a 0-4 score range), the SOTA model reported 0.90 MAE while our sketch model achieved an MAE of 1.39.
On the Hateful Memes task, the SOTA model reported 0.845 AUROC, and 0.714 AUROC was the SOTA result when the challenge was first released; our sketch model achieved 0.584 AUROC.
Thus, model sketching demonstrates strong or reasonable performance on the easy and medium difficulty tasks, but displays weaker performance results for the third, significantly harder task.

\subsection{Failure modes}
While our model sketching approach achieved its aims of shifting model developers' cognitive frame and presented a number of benefits for the models they developed, we observed several failure modes.
% Concept models failing, only can provide another concept term; users often gave up too soon
First, though participants had some promising concept ideas, they were not always able to actualize them with our zero-shot model-based approach. 
% When a participant's concept failed to give them results that substantially overlapped with their own judgement, there was little recourse other than to attempt another related concept term and see if that achieves better alignment. 
Participants often relied heavily on the results of the first concept term that they attempted. If that failed to return satisfactory results, they often abandoned the concept idea since they assumed that the model was not sophisticated enough to understand that concept. Participants would benefit from scaffolding to understand whether the model lacks an understanding of a given concept or just requires different terminology.
% differentiate cases where the model understands the concept but expresses it with different terms versus cases where the model lacks an understanding of the concept at all.

% Tending to cater to the LLM rather than thinking more broadly/creatively
% Second, we found that since participants were given an explanation of the underlying zero-shot modeling approaches used to surface concept scores, participants overly tailored their concept terms based on what they thought that these zero-shot models would be able to understand. 
Second, we found that some participants heavily tailored their concept terms based on what they thought zero-shot models would be able to understand, especially using concrete, specific concept terms.
% since they anticipated that models would perform better with these kinds of inputs. 
We observed that several of these participants eventually branched out and found that broader terms could work well. However, the downside still remains that since our concepts rely on pretrained models, these models can be limiting factors \rev{(further discussed in Section~\ref{section:limits_pretrained_models})}. Users might constrain their thinking to areas where the pretrained model already excels rather than thinking more creatively about what decisionmaking factors may be valuable.

% Bad modeling practices (ex: overfitting approaches, ignoring certain kinds of errors)
Finally, we noticed that because our approach emphasized a ``small data'' approach to help users stay focused, some participants lost sight of the overall goal to build a robust, general model. Participants sometimes fell into overfitting approaches by scrutinizing cases where their sketch model made errors and patching errors with very specific concepts that were not relevant to the larger decision-making task. Participants would benefit from tools that would help them to assess the generalizability of their sketch models. We believe that a curated dataset is worth this tradeoff because it encourages ML practitioners to avoid detailed data analysis and instead focus on broad-strokes concepts. 
% P9 conveyed this well, noting that ``if you are working with a limited dataset, it may be more advantageous to spend time thinking about concepts rather than making your model more complex.''

% Limitations of our approach even if it were to work perfectly
% \begin{itemize}
%     \item Types of concepts that performed poorly; where the LLM or CLIP fails
%     \item Limited kinds of thinking (ex: framing the problem purely in terms of what a pretrained model can currently do)
%     \item Bad modeling practices (ex: overfitting approaches, ignoring certain kinds of errors)
% \end{itemize}
% Other maladaptive strategies that come up using this approach that would impair later model development
% “even if the tool worked perfectly, what are the downsides of this approach”




% To cover
% - Concept innovation vs concept execution vs concept abandonment (the _intent_ behind changes in concept models and sketches)

%  Horizontal version of concept perf table
% \begin{table*}[!tb]
%   \centering
%   \small % \footnotesize % \scriptsize
%     \rev{
%     \begin{tabular}{c | c c | c c c c}
%     \toprule
%     \textbf{Concept type} & \textbf{Mean Prevalence} & \textbf{Fleiss' Kappa} & \textbf{Accuracy} & \textbf{F1 Score} & \textbf{Recall} & \textbf{Precision}\\
%     \midrule
%     \textbf{Text} & 
%     {19.4\%} &
%     {0.68} &
%     {0.78} &
%     {0.58} &
%     {0.66} &
%     {0.55}\\[0.1cm]
    
%     \textbf{Image} & 
%     {13.3\%} &
%     {0.60} &
%     {0.90} &
%     {0.60} &
%     {0.64} &
%     {0.60}\\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{
%         \rev{Concept performance for text and image concepts created by participants is moderately high based on manual annotations. 
%         % \msb{too narrow? Can we widen it and increase the font size?}
%         }
%     }
%     \label{table:concept_perf}
% \end{table*}

% Vertical version of concept perf table
% \begin{table*}[!tb]
%   \centering
%   \small % \footnotesize % \scriptsize
%     \rev{
%     \begin{tabular}{c | c c}
%     \toprule
%     \textbf{Concept Type} & \textbf{Text} & \textbf{Image}\\
%     \midrule
%     \textbf{Mean Prevalence} & 
%     {19.4\%} &
%     {13.3\%}\\[0.1cm]
%     \textbf{Fleiss' Kappa} & 
%     {0.68} &
%     {0.60}\\[0.1cm]
%     \midrule
%     \textbf{Accuracy} & 
%     {0.78} &
%     {0.90}\\[0.1cm]
%     \textbf{F1 Score} & 
%     {0.58} &
%     {0.60}\\[0.1cm]
%     \textbf{Recall} & 
%     {0.66} &
%     {0.64}\\[0.1cm]
%     \textbf{Precision} & 
%     {0.55} &
%     {0.60}\\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{
%         \rev{Concept performance for text and image concepts created by participants is moderately high based on manual annotations. 
%         }
%     }
%     \label{table:concept_perf}
% \end{table*}

==> sections/old_versions/6_discussion_v1.tex <==
\msl{This section is much rougher; just giving a sense of some of the topics I'd like to cover}\\

We have introduced model sketching, instantiated the approach in a tool designed for ML practitioners, and demonstrated that the approach successfully redirects attention to the high-level model design questions that are most critical to get right. Here, we discuss the opportunities afforded by model sketching as well as limitations and areas for future work.

% Potential sections (depends on results as well):
% \begin{itemize}
%     \item TODO: Notable implications of results
%     \item Alternative approaches to model sketching (other than concepts)
%     \item Other target audiences for model sketching (domain experts, designers, end users)
%     \item Bridging from model sketching to full-scale models
%     \item TODO: Other future work / limitations
% \end{itemize}

\subsection{Opportunities for model sketching}
% Opportunities in intervening in the authoring phases of ML; in approaches that bridge between the ideation phase and the implementation phase
\subsubsection{Early-stage cognitive interventions to scaffold and reframe model authoring}
Our work highlights that intervening early in the authoring phases of ML model development is a promising approach to engage ML practitioners in questions around the values embedded in their models. With such approaches, model developers may be able to preemptively catch problematic design directions and anticipate harmful algorithmic biases. While a great deal of work in the algorithmic fairness community has focused on measuring and fixing harmful biases in ML systems, early interventions that deeply alter the way developers \textit{think} about the very act of building a model have received much less attention. However, if successful, these approaches would be preferable to downstream measurements and post-hoc fixes because they could minimize the extent to which harmful model behavior reaches users or deployment contexts. More than simply catching problematic model designs early in the process, we aim for model sketching to serve as a flexible \textit{tool for thought} for ML practitioners that helps them to better reason about the downstream implications of their modeling decisions. We hope that the cognitive toolkit that they build through model sketching can serve them even as the move to other task domains and problem settings.

\msl{To include: something around timing related to prior snippet from Results}
This shift in the timescale of ML model authoring from a drawn-out, weeks-long project to an exercise carried out at interactive speeds unlocks a drastically different pace of creative iteration and experimentation during model development.

% Other target audiences for model sketching (domain experts, designers, end users)
% Using model sketches to facilitate communication
\subsubsection{Empowering non-technical users to participate in ML prototyping}
While our work was initially targeted towards ML practitioners, we believe that our model sketching approach holds promise as a means for non-technical users and domain experts to take an active role in the early phases of machine learning model development. Currently, stakeholders who lack ML experience (whether end users, domain experts, or engineering team members in designer or PM roles) have little ability to take ownership of ML model design decisions. Even if they are included in the design process or asked to provide feedback, they are largely limited by the set of information that ML experts convey to them. Furthermore, if they disagree with an approach, they cannot take action to demonstrate an alternative approach. However, a tool like model sketching could enable non-experts in ML to build their own functional sketch models that incorporate their contextual knowledge or domain expertise, a highly valuable contribution given that ML practitioners typically lack expertise on the deployment domain. Several participants in our user evaluation explicitly brought up that model sketching would be very useful for non-technical users, so we are encouraged that ML practitioners not only find model sketching valuable for their own workflows, but would recommend the practice to non-experts in ML.
% TODO: cite yang_investigatingHowExperiencedUXDesigners
% TODO: cite yang_groundingIMLToolDesign

% Other approaches to model sketching besides using concepts
\subsubsection{Expanding the purview of sketch-inspired approaches to ML model development}
We instantiated model sketching with concept-based intermediary abstractions, but we envision that a sketch-inspired approach to ML model development could take a number of forms. Different abstractions, like different artistic media, are more or less suitable for a given modeling task. While concepts are a sufficiently generic abstraction to cover a broad range of existing ML modeling approaches, other abstractions may be more effective to aid reasoning, depending on the particular prototyping goals one may have. For example, if the ML practitioner's modeling goal is to build a model that captures the opinion of a diverse population, then they may prefer to use individual voices in that population as their core abstraction~\cite{gordon_juryLearning}. If their goal is instead to trade off among multiple competing metrics, then they may prefer a primary abstraction that is based on distinct metrics and that would help them to reason about how the metrics might trade off. We believe that expanding the suite of tools that enable ML practitioners to create the sketch-like models that would best serve their needs is an important next step to bring the benefit of a sketching practice to machine learning.


\subsection{Limitations and future work}
% Basing off of pre-trained models may be limiting
\subsubsection{Expanding beyond the constraints and limitations of pretrained models}
One limitation of our technical approach based on zero-shot modeling using pretrained models is that these models may not be flexible enough to support a broad range of modeling tasks. Given that GPT-3 and CLIP were trained on Internet text and image data, it has a limited view of the world and cannot provide high-quality concept scores for domains that are not well represented in this training data. 
\msl{TODO: will add more on the biases embedded in large language models and how that connects with our approach}

% Bridging to full-scale models
\subsubsection{Bridging from sketches to full-scale models}
Our model sketching approach is meant to produce early, prototype versions of machine learning models. Thus, while sketch models are not intended to exist as a final version of a model, they should still have enough parallels with full-scale models to provide useful signal on the behavior of a full-scale version of the sketch model. We note that many production machine learning systems for large, business-critical purposes such as feed ranking and content moderation are already decomposed into smaller sub-models that are built by individual teams, and those models may themselves consist of a hierarchy of sub-models. It is common for large-scale machine learning tasks to be decomposed in terms of key concepts or decision-making functions, so our sketch models plug in directly to this framework. In simpler model deployments, the concepts that comprise sketch models can be scaled up to small specialized sub-models for each concept. In large-scale deployments, these same concepts can similarly be scaled up to capture the efforts of an engineering team that will build models or a system of models to tackle a certain conceptual decision-making task. An important area of future work will be to further envision the bridging work that happens between a model sketch and its instantiation in a large-scale ML system.



==> sections/old_versions/6_discussion_v2.tex <==
% v2
We have introduced model sketching, instantiated the approach in a tool designed for ML practitioners, and demonstrated that the approach successfully redirects attention to the high-level model design questions that are most critical to get right. Here, we discuss the opportunities afforded by model sketching as well as limitations and areas for future work.

\subsection{Opportunities for model sketching}
We envision several exciting implications for bringing a sketching practice to machine learning.

% \msl{To include: something around timing related to prior snippet from Results}
% This shift in the timescale of ML model authoring from a drawn-out, weeks-long project to an exercise carried out at interactive speeds unlocks a drastically different pace of creative iteration and experimentation during model development.

% Other approaches to model sketching besides using concepts
% Different abstractions, different tasks/goals
\subsubsection{Expanding the purview of sketch-inspired approaches to ML model development}
% We instantiated model sketching with concept-based abstractions, but we envision that a sketch-inspired approach to ML model development could take a number of forms. The choice of abstraction, like that of artistic media, may need to be tailored to the task at hand. 
While concepts are a sufficiently generic abstraction to cover a broad range of existing ML modeling approaches, other abstractions may also enable sketch-like interaction. 
% The choice of abstraction, like that of artistic media, may need to be tailored to the task at hand. 
For example, if the ML practitioner's modeling goal is to build a model that captures the opinion of a diverse population, they may prefer to use individual voices in that population as their core abstraction~\cite{gordon_juryLearning}. If their goal is to reconcile multiple competing metrics or objectives~\cite{yu_keepingDesignersInTheLoop}, then they may prefer a primary abstraction based on distinct metrics to help them to reason about how the metrics might trade off. To reap the benefits of a sketching practice in machine learning, we need to build tools to support different \textit{ways of thinking} about modeling that are suited to varying modeling contexts.
% To reap the benefits of a sketching practice in machine learning, we need to expand the suite of tools that would enable ML practitioners to create sketches for their particular modeling contexts.

\subsubsection{Bringing sketching to model-adjacent tasks}
Participants in our evaluation uncovered gaps not just in their models, but in the larger modeling ecosystem of problem formulation, data, and labeling methods. Data work in particular tends to be neglected and undervalued relative to modeling work~\cite{sambasivan_everyoneWantsToDoModelWork}. %, and sketch-like approaches could assist and foreground this important, but often tedious, work. We envision that our 
The model sketching approach could be extended to assist with some of these tasks. For example, in data annotation tasks, a major challenge lies in iteratively developing a refined labeling policy~\cite{kulesza_conceptEvolution}. Model sketching could iteratively simulate the results of different labeling policies, exposing areas where further concept refinement is needed \textit{before} ML practitioners launch costly human labeling efforts.
% This challenge is further heightened for tasks in specialized domains where only subject matter experts (SMEs) have the expertise to perform annotation

% TO ADAPT:
% In this paper, we proposed a technical framework …  utilizing LLM … and the results shows … It can be generalized to the data annotation tasks in those highly specialized domains, where only SMEs can and need to annotate dataset, in a zero-shot or few-shot settings. … In those scenarios, the Model Sketch approach can assist SMEs to focus on the human-understandable high-level concepts they should have been focused on within their own business context, instead of the AI-desired  low-level  "ground-truth" label... The outcome in this potential scenario is the efficiently labeled dataset with a well-articulated label schema, instead of the models shown in the current paper... But ofcourse in order to achieve this vision, we need to resolve two challenges: 1) a GUI that the non-technical SMEs can interact with our framework, and 2) a better in-context understanding of the SMEs data annotation working routine, so that our instantiated system design can better fit in this context.

% Other target audiences for model sketching (domain experts, designers, end users)
% Using model sketches to facilitate communication
\subsubsection{Empowering non-technical users to participate in ML prototyping}
%While our work was initially targeted towards ML practitioners, model sketching presents a promising route for non-technical users and domain experts to engage in the early phases of model development. 
Currently, stakeholders who lack ML experience (whether end users, domain experts, or engineering team members in designer or PM roles) have little ability to take ownership of ML model design decisions and are largely limited to the information that ML experts convey to them~\cite{piorkowski_AIDevelopersCommChallenges}. Model sketching could enable non-experts in ML to build functional sketch models that incorporate their domain expertise, a highly valuable contribution given that ML practitioners typically lack expertise on the deployment domain. Several participants in our user evaluation explicitly brought up that model sketching would be very useful for non-technical users.%, so we are encouraged that ML practitioners not only find model sketching valuable for their own workflows, but would recommend the practice to non-experts in ML.
% TODO: cite yang_investigatingHowExperiencedUXDesigners
% TODO: cite yang_groundingIMLToolDesign

% \subsubsection{Sketching to facilitate communication about ML models}
% \msl{TODO: section on sketches to aid communication between different team members / stakeholders}

% Opportunities in intervening in the authoring phases of ML; in approaches that bridge between the ideation phase and the implementation phase
% \subsubsection{Early-stage cognitive interventions to scaffold and reframe model authoring}
% Our work highlights that intervening early in the authoring phases of ML model development is a promising approach to engage ML practitioners in questions around the values embedded in their models. With such approaches, model developers may be able to preemptively catch problematic design directions and anticipate harmful algorithmic biases. While a great deal of work in the algorithmic fairness community has focused on measuring and fixing harmful biases in ML systems, early interventions that deeply alter the way developers \textit{think} about the very act of building a model have received much less attention. However, if successful, these approaches would be preferable to downstream measurements and post-hoc fixes because they could minimize the extent to which harmful model behavior reaches users or deployment contexts. More than simply catching problematic model designs early in the process, we aim for model sketching to serve as a flexible \textit{tool for thought} for ML practitioners that helps them to better reason about the downstream implications of their modeling decisions. We hope that the cognitive toolkit that they build through model sketching can serve them even as the move to other task domains and problem settings.

\subsection{Limitations and future work}
% Basing off of pre-trained models may be limiting
\subsubsection{Expanding beyond the constraints and limitations of pretrained models}
% \msl{TODO: will add more on the biases embedded in large language models and how that connects with our approach}
% \msl{TODO: cover dual use; adversarial applications of sketch modeling}
One limitation of our technical approach based on zero-shot modeling using pretrained models is that these models may not be flexible enough to support a broad range of modeling tasks. Given that the GPT-3 and CLIP models were trained on Internet text and image data, these models have a limited view of the world and cannot provide high-quality concept scores for domains that are not well represented in this training data. Future work might explore the efficacy of other specialized pretrained models or alternative zero-shot modeling approaches that could overcome these gaps.

Additionally, as with any technology that builds on top of large language models and other pretrained models, sketch models will be subject to biases embedded in these models~\cite{kurita-etal-2019-measuring, sheng_biasesInLangGeneration}. It is crucial that ML practitioners are aware of these risks, so we encourage others who adopt model sketching to make clear to users that these underlying models can display harmful biases that may manifest in their sketch models. Though these biases in themselves are negative, one positive side effect is that encountering them early in the model development process forces ML practitioners to consider how the same kinds of biases might impact their full-scale models. Early encounters with such failures may prompt model developers to prioritize fairness-related work, and our approach allows them to experiment with different strategies---whether with the modeling approach, upstream data curation, or downstream score processing and bias checks---that might mitigate the harmful biases they encounter.

%Finally, it is possible that model sketching could be leveraged in problematic ways to build models that, for example, amplify hateful posts or surface triggering content. We limit the dataset size in our sketchbooks to 100 examples, so this naturally limits the scale at which such an adversarial actor can operate. However, in our future deployment of the tool, we will require users to register their usecases to gain access, and we will log all sketchbooks and outputs so that we can identify harmful uses of the tool and restrict access for bad actors.

% Bridging to full-scale models
\subsubsection{Bridging from sketches to full-scale models}
While sketch models are early explorations rather than final versions of a model, they still need to provide useful signal on a full-scale model's behavior. As detailed in Section~\ref{section:sketch_to_production}, sketch models can inform the design of production models by guiding decisions on how to decompose large modeling tasks and refine data requirements. Our technical benchmark against state-of-the-art models suggests that model sketching can achieve substantial performance on some tasks, but may struggle to generalize on more challenging tasks.
The model sketching process still provides value in facilitating reflection and iteration on high-level modeling approaches even if performance metrics hit a ceiling. However, an important area of future work will be to provide stronger guarantees on the mapping between sketch and full-scale performance metrics. Future work might directly tackle the bridging work that must happen between a model sketch and its instantiation in a large-scale ML system.

% We note that many production machine learning systems for large, business-critical purposes such as feed ranking and content moderation are already decomposed into smaller sub-models that are built by individual teams, and those models may themselves consist of a hierarchy of sub-models. It is common for large-scale machine learning tasks to be decomposed in terms of key concepts or decision-making functions, so our sketch models plug in directly to this framework. In simpler model deployments, the concepts that comprise sketch models can be scaled up to small specialized sub-models for each concept. In large-scale deployments, these same concepts can similarly be scaled up to capture the efforts of an engineering team that will build models or a system of models to tackle a certain conceptual decision-making task. An important area of future work will be to further envision the bridging work that happens between a model sketch and its instantiation in a large-scale ML system.



==> sections/old_versions/TBD_case_studies_v1.tex <==
\section{Case studies}
\msl{NOTE: these case studies are in rough initial form. We would likely represent each case study in a more pared-down form since there are a number of them, and I'd like to synthesize more of the holistic takeaways. We may be replacing this with examples of participants completing a modeling task of their own choosing}\\
To illustrate the breadth of machine learning tasks to which we can apply our model sketching approach, we present several case studies that demonstrate ranking, research/planning, clustering, and search applications.
% \msl{decide on placement of this section (nested within System or Evaluation, or in a separate section maybe between System and Evaluation?); decide on order of case studies}

\subsection{Travel planning}
% Owner: Michelle
% High-level task
\subsubsection{Task}
For a sample travel planning task, we assist travelers with selecting an Airbnb for a trip to New York City.
% Dataset format
Our dataset includes \MSLtempValue{10k} Airbnb listings in the city and includes the name, image, description, and neighborhood overview for each.
% More-detailed task
Here, we built sketch models that capture a user's level of interest in (or willingness to stay at) a given Airbnb listing. For each listing in a training set of 40 listings, we had the user provide a 0-1 score indicating their interest in the listing, where $0$ indicated ``very uninterested,'' $1$ indicated ``very interested,'' and $0.5$ indicated the threshold at or above which they would consider staying at a listing.
% Concepts used; sketches crated
\subsubsection{Concepts} We explored the following concepts for this task:
\begin{itemize}
    \item {\texttt{description} field}: {Trendy, Central, Clean}
    \item {\texttt{image} field}: {Dingy, Tidy, Designed well, Designer, Bright, Outdated, Sunlight natural, Spacious, Ugly}
    \item {\texttt{neighborhood\_overview} field}: {Things to do, Activities, Good vibes}
\end{itemize}

\subsubsection{Sketches} Then, we experimented with combining these concepts in sketches (and iteratively adding new concepts above) to capture what made listings most appealing.
\begin{itemize}
    \item \textbf{Aesthetic}: {Clean , Bright, Designer}
    \item \textbf{Cool}: {Central, Trendy}
    \item \textbf{Modern and clean}: {Outdated, Ugly, Clean}
    \item \textbf{Fun neighborhood}: {Good vibes, Central, Trendy}
    \item \textbf{Best overall}: {Clean, Bright, Designer, Ugly , Outdated}
\end{itemize}

\subsubsection{Learnings}
% Discoveries/learnings unlocked by taking a model sketching approach
Through our model sketching process, we learned that an important factor was the physical location of the Airbnb and its proximity to specific points of interest, so it would be valuable to augment the data with fields related to this proximity. We also realized that additional images would be helpful to get a better sense of the overall aesthetics of a listing, since a single image often was not enough to convey its appearance. Finally, we discovered that most Airbnb hosts brand their listings with positive attributes like ``clean,'' so it might be more helpful to extract customer reviews to gather more objective impressions.
% Gather images of example data that may be helpful for figures later

\subsection{Creative inspiration}
% Owner: Anne
\subsubsection{Task}
For this task, we assist users with uncovering creative connections across artists and artworks. Our dataset of 20 artworks includes the artist’s name, title, type, style, genre, media, geographic region, image and text description for each artwork. Here, we build sketch models that capture themes and perspectives for the purposes of finding similarities.
\subsubsection{Concepts} We explored the following concepts for this task:
\begin{itemize}
    \item {\texttt{image} and \texttt{text} fields}: {colorful, surreal, fantasy, abstract, realist, politics themed, revolution themed, labor movement themed, social justice themed, race themed, gender themed, feminist, queer themed}
\end{itemize}

\subsubsection{Sketches} Then, we experimented with combining these concepts in sketches (and iteratively adding new concepts above) to capture elements of artworks we were interested in.
\begin{itemize}
    \item \textbf{Social justice}: {social justice themed, race themed, feminist, queer themed}
    \item \textbf{Political movements}: {politics themed, revolution themed, labor movement themed}
    \item \textbf{Bold}: {colorful, surreal, fantasy, abstract}
\end{itemize}

\subsubsection{Learnings}
``Thematic'' concepts should be used with caution: while they can signal representation, they can also encapsulate both positive and negative handlings of a topic. For example, one ``gender themed'' artwork may handle gender in a sensitive or progressive way, while another may handle it in a harmful way. A user may unintentionally group together artworks like these with thematic concepts.

\subsection{Political candidate research}
% Owner: Ulo
\subsubsection{Task}
For a sample political alignment informer task, we assist voters with finding a candidate for the 2022 California gubernatorial election who aligns with concepts (issues) that matter to them. Our dataset includes dozens of responses to prompted questions around various campaign issues and includes the respective candidate, the prompted question, the associated campaign issue, and the candidate’s response or stance (often represented as a quote from a political statement or speech). This information was aggregated from the nonprofit, nonpartisan, third-party group CalMatters.

\subsubsection{Concepts} We explored the following concepts for this task:
\begin{itemize}
    \item {\texttt{campaign\_values\_details} field}: {Environment, Equality, Gun control, Reproductive rights, Voting rights}
\end{itemize}

\subsubsection{Sketches} Then, we experimented with combining these concepts in sketches (and iteratively adding new concepts shown above) to capture more personalized values in order to find the most compatible candidate.
\begin{itemize}
    \item \textbf{Sketch 1}: {Climate change, Gun control}
    \item \textbf{Sketch 2}: {Environment, Anti gun}
    \item \textbf{Sketch 3}: {Eco-friendly, Anti gun, Equal rights}
    \item \textbf{Sketch 4}: {Eco-friendly, Anti gun, Pro choice, Equality, Voting Rights}
\end{itemize}

\subsubsection{Learnings}
Model sketching allowed for a more customized, personal experience in this task by providing an interactive method for a voter to be quickly informed about different candidates’ stances on political issues important to the voter. Interestingly, the model sketching process enables more nuanced concepts that weren’t explicitly outlined in the initial dataset, but are still aligned with the candidate’s general stance and sentiment, to be expressed. For example, the dataset contained seven campaign issue categories (Justice, Housing/Homelessness, Economy, Health care, Environment, K-12 education, and Higher education), however, the model was able to reasonably provide feedback about a candidate’s stance on an issue not explicitly covered in the dataset like “pro choice” or “voting rights”. Finally, through model sketching, we learned when a dataset was poor and negatively impacting the model’s potential. Initially, the dataset formulated for this task was created by scraping the issues outlined on each candidate’s website, however this created a skewed dataset as notably the incumbent’s website only provided sentence-long descriptions of their stances meanwhile their challengers’ websites contained paragraphs about their stances. From the quick feedback through model sketching, it became clear that using third-party sources for the dataset information would create a more balanced dataset.

\subsection{Reviewer bias auditing}
% Owner: Zixian
\subsubsection{Task}
For a sample reviewer bias-checking (or value-surfacing) task, we assist a food reviewer with checking their biases in reviewing cafes and restaurants (mainly in the Bay Area and Seattle). We manually collected 30 recent food reviews from their foodie instagram account. Each example consists of the name of the food place, post date, post text, overall rating as well as the number of likes and comments. We asked this reviewer about their preferences and values and built sketch models based on them. The values they considered most important included taste, quality, presentation, vibes, services, and price, where price influenced how much they cared about the other factors. For each food place, the reviewer gave a rating between 0 and 12, where 0 indicated “extremely disappointing / will not come back again” and 12 indicated “exceeding expectations / will definitely consider coming back”. 

\subsubsection{Concepts} We explored the following concepts for this task:
\begin{itemize}
    \item {\texttt{post\_text} field}: 
    \begin{itemize}
        \item Naive version: {Tasty, Affordable, Creative, Nice vibes, Good service, High quality, Good presentation}
        \item Refined version: {Yummy, Cheap, Original, Decent vibes, Sound service}
    \end{itemize}
\end{itemize}

\subsubsection{Sketches} Then, we experimented with combining these concepts in sketches and iteratively refining existing concepts with concept brainstorming and comparison tools to capture the reviewer’s preferences. 
\begin{itemize}
    \item \textbf{Naive concepts 4}: {Tasty, High quality, Affordable, Creative}
    \item \textbf{Naive concepts 7}: {Tasty, High quality, Affordable, Creative, Nice vibes, Good service, Good presentation}
    \item \textbf{Refined concepts 4}: {Yummy, High quality, Cheap, Original}
    \item \textbf{Refined concepts 7:}: {Yummy, High quality, Cheap, Original, Decent vibes, Sound service, Good presentation}
\end{itemize}

\subsubsection{Learnings}
The approach of model sketching enabled us to not only capture a reviewer’s values with simple concepts but also surface how much they value each concept. For example, the ``Naive concepts 7'' sketch model was trained to assign ``Tasty'' and ``High quality'' the coefficients of 2.22 and 1.26, meaning that this model weighted these two concepts strongly in the positive direction. These concepts matched the reviewer’s top two preferences. Interestingly, while we were able to improve on the sketch models’ performance on the training dataset by 10-20\% through concepts brainstorming and comparison tools, we observed a small drop in the test performance. We hypothesized that this happened because we tuned the concepts based only on the training dataset, which led to overfitting and lower generalizability to the test set. We plan to mitigate this limitation by encouraging users to think more broadly (and looking at more data if available) when brainstorming concepts. 


\subsection{Product ranking and rating}
% Owner: Zixian

\subsubsection{Task}
For a sample product ranking/rating task, we assist buyers with rating Amazon products such as video games. We gathered our dataset from publicly available Amazon reviews. Our dataset includes 31 products rated and reviewed by a randomly selected reviewer. Each data example consists of the buyer’s review text and rating of the product, the product’s images, as well as its metadata, including brand, main category, price and rank. The buyer’s rating ranges from 0 to 5, where 0 means ``unsatisfied'' and 5 means ``satisfied'' with the product. 

\subsubsection{Concepts} We explored the following image and text concepts for this task:
\begin{itemize}
    \item {\texttt{high\_resolution\_image} field}: {Realistic, Violent, Friendly, First person, Colorful, Informative}
    \item {\texttt{review\_text} field}: {Exciting, Enjoyable, Worthy}
\end{itemize}

\subsubsection{Sketches} Then, we experimented with combining image and/or text concepts in sketches to capture the buyer’s ratings.
\begin{itemize}
    \item \textbf{All image 4}: {Realistic, Friendly, First person, Colorful}
    \item \textbf{All image 6}: {Realistic, Friendly, First person, Colorful, Violent, Informative}
    \item \textbf{Image and text 8}: {Realistic, Friendly, First person, Colorful, Violent, Informative, Exciting, Worthy}
\end{itemize}

\subsubsection{Learnings}
We found that the model sketching approach can be easily applied on a multi-modal dataset like Amazon product reviews. We also realized that model sketching is especially useful on subjective scoring/rating/ranking tasks, because it helps uncover reviewers’ subjective values. Through iterating on concepts and sketches, we learned that while more concepts can help sketch models improve, they do not necessarily always lead to better performance. Similarly, adding an input modality could benefit or harm the model depending on the specific concepts. 

% \subsection{Feed ranking}
% TODO: IG/Twitter feed ranking

% \subsubsection{Task}
% TODO

% \subsubsection{Concepts} We explored the following concepts for this task:
% \begin{itemize}
%     \item {\texttt{TODO} field}: {}
% \end{itemize}

% \subsubsection{Sketches} TODO
% \begin{itemize}
%     \item \textbf{Sketch 1}: {}
%     \item \textbf{Sketch 2}: {}
% \end{itemize}

% \subsubsection{Learnings}
% TODO

==> sections/old_versions/title_ideas.tex <==
Title brainstorming

Model Sketching: Empowering Machine Learning Practitioners to Iterate on Concepts, Not Code

"Concepts, not Models"?
Early stage
Drop practitioners

Early-stage design of concepts for 
Model Sketching: Early-stage model design with concepts for machine learning
Sketching for the early phases of model design


Rapidly iterable model design

James:
“Interactive Sketching for the Early Stages of User Interface Design” -> “Sketching for the Early Stages of ML Model Design”

Model Sketching: Bringing concepts into the early phases of ML model design
Model Sketching: Exploring Concepts in the Early Stages of ML Model Design

Constructing ML models with intermediate concepts

Model Sketching for Early Stage ML Model Design
Model Sketching: Exploring Human Interpretable Concepts in the Early Stages of ML Model Design

* Model Sketching: Leveraging concept-based building blocks for early stage ML model design

Model Sketching: Concepts as building blocks for early stage ML model design

Constructing ML models from concept-based building blocks

Model Sketching: Using Human Interpretable Concepts for Early Stage ML Model Design
Model Sketching: Human Interpretable Concepts for Early Stage ML Model Design



Crafting

To consider
something around intermediate goals? that can be predicted and reasoned over

How are concepts enabling a sketch?

% 9/8
**Model Sketching: Centering Concepts in Early-Stage Machine Learning Model Design
Model Sketching: Centering Concepts in Early-Stage Machine Learning Design
Model Sketching: Centering Concepts in Early-Stage Machine Learning Development
    --> a focus on ML practitioners' attention
    Concepts, not [X]
Model Sketching: Centering Concepts Rather Than Models in Early-Stage Machine Learning Development


**Model Sketching: Concept-based Iteration in Early-Stage Machine Learning Model Design
    --> highlighting key aspect/benefit of sketching

Model Sketching: Concept-based Abstractions for Early-Stage Machine Learning Model Design

Model Sketching: Early-Stage Machine Learning Model Design via Concepts
Model Sketching: Early-Stage Machine Learning Model Design via [Adj] Concepts
    --> de-emphasizing concepts

% Front-runners
**Model Sketching: Centering Concepts in Early-Stage Machine Learning Model Design
Model Sketching: Concept-based Iteration in Early-Stage Machine Learning Model Design

